Principles of Lipschitz continuity in neural networks

Deep learning has achieved remarkable success across a wide range of domains, significantly expanding the frontiers of what is achievable in artificial intelligence. Yet, despite these advances, critical challenges remain -- most notably, ensuring robustness to small input perturbations and generalization to out-of-distribution data. These critical challenges underscore the need to understand the underlying fundamental principles that govern robustness and generalization. Among the theoretical tools available, Lipschitz continuity plays a pivotal role in governing the fundamental properties of neural networks related to robustness and generalization. It quantifies the worst-case sensitivity of network's outputs to small input perturbations. While its importance is widely acknowledged, prior research has predominantly focused on empirical regularization approaches based on Lipschitz constraints, leaving the underlying principles less explored. This thesis seeks to advance a principled understanding of the principles of Lipschitz continuity in neural networks within the paradigm of machine learning, examined from two complementary perspectives: an internal perspective -- focusing on the temporal evolution of Lipschitz continuity in neural networks during training (i.e., training dynamics); and an external perspective -- investigating how Lipschitz continuity modulates the behavior of neural networks with respect to features in the input data, particularly its role in governing frequency signal propagation (i.e., modulation of frequency signal propagation).

==> front_matter/acknowledgements.tex <==
\chapter*{Acknowledgements}

First and foremost, I owe myself a debt of gratitude for the perseverance, curiosity, and courage that carried me through my doctoral journey. This journey was never easy, but it was deeply rewarding. I'm proud of the dedication that brought me here.

To my beloved grandparents — thank you for your precious love, unwavering companionship, and tender care through life's hardships. In you, I found a world of kindness, tenderness and resilience, an eternal harbor where my dreams could set sail, even when the days felt most difficult. I cherish those unforgettable moments in summer, when the Milky Way fell down behind our backyard, so poetic and so spectacular. It feels as though I saw you only yesterday — your faces bathed in the rosy evening glow, your voices still echoing softly at our past home. I truly miss our home and those moments dearly --- the serenity, the beauty, the feeling of being loved.

To my supportive and kind supervisors, Dr. Colm O'Riordan and Dr. James McDermott --- I am deeply grateful for their unwavering guidance, insightful feedback, and invaluable encouragement. Their expertise and high standards have shaped this work in countless ways, and their belief in my potential has sustained me through every setback.


To my colleagues and friends --- both near and far --- I hold with heartfelt gratitude to their invaluable advice and your steadfast friendship throughout this journey.



==> front_matter/examiners.tex <==
\clearpage

\thispagestyle{empty}

    
    
\begin{center}

        \setlength{\parindent}{0pt}
        \setlength{\parskip}{0pt}

        %distribution remaining space.
        \vspace*{\stretch{0.5}}  
        
        { %<-- scope
          \adjustbox{max width=\linewidth}{%
          \setstretch{2.0} %<-- local
          \large
          \begin{tabular}{ll}       
            \textbf{Internal Examiner}: 
            & \underline{\makebox[52ex][l]{\textbf{Prof. Niall Madden}}} \\
            & \underline{\makebox[52ex][l]{School of Mathematical and Statistical Sciences}} \\
            & \underline{\makebox[52ex][l]{University of Galway, Ireland}}
         \end{tabular} 
         }%end of adjustbox
        }


        
        \vspace*{\stretch{0.3}} 

        {%<-- scope
          \adjustbox{max width=\linewidth}{%
          \setstretch{2.0} %<-- local
          \large 
          \begin{tabular}{ll}       
            \textbf{External Examiner}: 
            & \underline{\makebox[52ex][l]{\textbf{Dist. Prof. Padhraic Smyth}}} \\
            & \underline{\makebox[52ex][l]{Hasso Plattner Endowed Chair in Artificial Intelligence}} \\
            & \underline{\makebox[52ex][l]{Department of Computer Science (Vice-Chair)}} \\
            & \underline{\makebox[52ex][l]{Department of Statistics}} \\
            & \underline{\makebox[52ex][l]{School of Information and Computer Sciences}} \\
           & \underline{\makebox[52ex][l]{University of California, Irvine}} 
        \end{tabular}
        }%end of adjustbox
        }

        
        \vfill \vfill
        
\end{center}

\clearpage

==> front_matter/thesis_guidelines.tex <==
\clearpage 
\vspace{0pt}

\href{https://www.universityofgalway.ie/media/graduatestudies/files/writingascientificstylethesis/writing_a_scientific_thesis.pdf}{Click here for UoG Thesis writing guidelines}
\\

Front matter of thesis

Anything that appears after the title page and before Chapter 1.

\begin{itemize}
    \item Title page (Required)
    \item Frontispiece (Optional)
    \item Copyright page (Optional)
    \item Dedication (Optional)
    \item Epigraph (Optional)
    \item Acknowledgements (Optional)
    \item Abstract (Required)
    \item Table of Contents (Required)
    \item List of Figures (Required)
    \item List of Tables (Required)
    \item List of Appendices (Optional)
    \item Declaration (Required)
    \item List of publications (Optional - could also be placed in introduction)
\end{itemize}

\vfill
\clearpage


==> main_matter/chapters/Conclusions/text.tex <==


\lettrine[lines=3]{T}{his} thesis advances a principled understanding of the \textbf{principles of Lipschitz continuity in neural networks} from a \textbf{complementary dichotomy of perspectives}: an \textbf{internal} perspective --- focusing on the temporal evolution of Lipschitz continuity in neural networks during training (\ie, \textbf{Training Dynamics}); and an \textbf{external} perspective --- investigating how Lipschitz continuity modulates the behavior of neural networks with respect to features in the input data, particularly its role in governing frequency signal propagation (\ie, \textbf{Modulation of Frequency Signal Propagation}).

The inquiry thus is guided by three primary research questions (RQs) framed within a structured approach: (RQ1) \textbf{State of Knowledge} --- what is the state of knowledge of Lipschitz continuity in deep learning? (RQ2) \textbf{Training Dynamics} --- how does Lipschitz continuity of neural networks evolve over time during training? (RQ3) \textbf{Modulation of Frequency Signal Propagation} --- how does Lipschitz continuity modulate the frequency signal propagation in neural networks, and how does this help us understand the global robustness of image models? Each primary research question gives rise to a set of secondary research questions (SRQs), addressed across one or two dedicated chapters. The research was conducted cumulatively during the Ph.D. training. This thesis compiles and presents a selection of research articles --- either published or under review as of the submission date --- into a \underline{\textbf{self-contained}}, \underline{\textbf{modular}}, \underline{\textbf{coherent}}, \underline{\textbf{monograph-style}} presentation format, all centered on the principles of Lipschitz continuity in neural networks.


In response to these research questions, in Chapter~\ref{chapter:literature_review}, this thesis first consolidates the existing state of knowledge of Lipschitz continuity in deep learning through a comprehensive literature review. In Chapter~\ref{chapter:perturbation_analysis}--\ref{chapter:optimization_induced_dynamics}, it then develops a stochastic dynamic framework for analyzing Lipschitz continuity during training by drawing on tools from operator theory, perturbation analysis, and high-dimensional stochastic differential equations (SDEs). Finally, in Chapter~\ref{chapter:fourier_analysis_of_lipschitz_continuity}, it conducts a Fourier-theoretic analysis to examine how Lipschitz continuity governs the modulation of frequency-domain signals in neural networks. Additionally, in Chapter~\ref{chapter:interpreting_global_robustness}, the thesis introduces an interpretability perspective by linking frequency-domain perturbations to global robustness through the underpinning lens of Lipschitz continuity. In doing so, it establishes a mathematically rigorous and conceptually unified understanding of Lipschitz continuity in deep learning, moving beyond the prevailing static and regularization-focused views in the literature.








\section{Research Summary}

% RQ1
\paragraph{(RQ1) State of Knowledge.} (RQ1) gives rise to two secondary research questions: (SRQ1) \textbf{Theoretical Foundations} --- what are the theoretical foundations of Lipschitz continuity in deep learning? (SRQ2) \textbf{Regularization Mechanism} --- how does Lipschitz continuity serve as a regularization mechanism for improving robustness and generalization capabilities in deep learning? 

\begin{enumerate}[label={}, left=1em]
    \item \textbf{Contributions of Addressing (SRQ1) and (SRQ2).} To address (SRQ1) and (SRQ2), Chapter~\ref{chapter:literature_review} presents a comprehensive literature review that synthesizes theoretical foundations, estimation methods, regularization approaches, and certifiable robustness. This chapter consolidates existing knowledge of Lipschitz continuity in deep learning, and provides a background for the research.
\end{enumerate}



% RQ2
\paragraph{(RQ2) Training Dynamics.} (RQ2) gives rise to two secondary research questions: (SRQ3) \textbf{Parameter Space Perturbation} --- how do the spectral properties (\ie, singular values) of parameter matrices change in training? (SRQ4) \textbf{Stochastic Dynamic Analysis of Lipschitz Continuity} --- how does Lipschitz continuity evolve over time during training in neural networks?

\begin{enumerate}[label={}, left=1em]
    \item \textbf{Contributions of Addressing (SRQ3).} To address (SRQ3), Chapter~\ref{chapter:perturbation_analysis} develops an operator-theoretic framework for analyzing spectral variations in parameter matrices during optimization, enabling stochastic analysis of their spectral properties. As a direct corollary, this framework yields an explicit analytic formulation of the operator-norm Hessian of rectangular matrices. 
    %In Chapter~\ref{chapter:optimization_induced_dynamics}, it serves as a foundation for the stochastic dynamic analysis of the temporal evolution of Lipschitz continuity using stochastic differential equations (SDEs). %To the best of our knowledge, this constitutes the first rigorous and formal analytic framework for deriving arbitrary-order Fr\'echet derivatives of rectangular matrices. It also paves the way for a principled treatment of parameter perturbations during deep learning training.

    \item \textbf{Contributions of Addressing (SRQ4).} To address (SRQ4), building on the foundations laid in Chapter~\ref{chapter:perturbation_analysis}, Chapter~\ref{chapter:optimization_induced_dynamics} establishes a rigorous theoretical framework for analyzing the dynamics of Lipschitz continuity using a system of stochastic differential equations (SDEs), applying It\^o's lemma to derive analytical expressions for the temporal evolution of Lipschitz bounds. These results reveal three fundamental driving factors governing the dynamics of Lipschitz continuity in neural networks:
    \begin{enumerate}[label=(\roman*)]
        \item the projection of gradient
flows, induced by the optimization dynamics, onto the operator-norm Jacobian of parameter matrices;
    
        \item the projection of gradient noise, arising from the randomness in mini-batch sampling, onto the operator-norm Jacobian; 
    
        \item the projection of the gradient noise onto the operator-norm Hessian of parameter matrices.

    \end{enumerate}

    The theoretical framework is validated through numerical experiments with multiple regularization configurations. Furthermore, our theoretical framework sheds light on how noisy supervision, parameter initialization, batch size, and mini-batch sampling trajectories, among other factors, shape the evolution of the Lipschitz continuity of neural networks. To the best of our knowledge, it is the first theoretical framework rigorously analyzing the temporal evolution of Lipschitz continuity of neural networks during training. 
        
\end{enumerate}


% RQ3
\paragraph{(RQ3) Modulation of Frequency Signal Propagation.} (RQ3) gives rise to two secondary research questions: (SRQ5) \textbf{Fourier Analysis of Lipschitz Continuity} --- how does Lipschitz continuity modulate frequency signal propagation in image models? (SRQ6) \textbf{Interpreting Global Robustness} --- how can global robustness be explained through the lens of spectral bias in Lipschitz continuity?


\begin{enumerate}[label={}, left=1em]

    \item \textbf{Contributions of Addressing (SRQ5).} To address (SRQ5), Chapter~\ref{chapter:fourier_analysis_of_lipschitz_continuity} presents a Fourier-theoretic analysis of Lipschitz continuity, drawing on tools from harmonic analysis, information theory, and Shapley value theory, supported by analytical derivations and verification examples. To complement the theoretical findings, we also provide empirical studies investigating the relationship between Lipschitz continuity and frequency-domain features.

    The analysis begins with a spectral decomposition of the Lipschitz continuity bound, revealing a \textbf{spectral bias}: \textbf{high-frequency components contribute disproportionately to the Lipschitz constant}, amplified by the frequency $\ell_2$-norm. This result is consistent with empirical observations, showing that high-frequency signals tend to increase the Lipschitz constants of neural networks during training.

    Furthermore, we derive a frequency-domain perturbation bound, showing that the functional perturbation caused by frequency-domain input perturbation is approximately bounded above by the spectral contribution of the Lipschitz continuity decomposition. As a direct corollary, we demonstrate that the variational mutual information between classifier outputs and labels --- under frequency-domain input perturbations --- is also upper bounded by this spectral contribution. \textbf{These results reveals how Lipschitz continuity modulates feature propagation in the frequency domain}.
    
    %Finally, the theoretical results in this chapter lay the foundation for the interpretability analysis in Chapter~\ref{chapter:interpreting_global_robustness}, where global robustness is examined via frequency perturbations. The methodology in that chapter can be interpreted as measuring a \textbf{proxy of the spectral decomposition of Lipschitz continuity of neural networks} --- an NP-hard quantity to compute directly.
    


    \item \textbf{Contributions of Addressing (SRQ6).} To address (SRQ6), Chapter~\ref{chapter:interpreting_global_robustness}, building on the theoretical framework developed in Chapter~\ref{chapter:fourier_analysis_of_lipschitz_continuity}, proposes a method for quantifying the global robustness of image classifiers. This method leverages Shapley value theory to measure the predictive importance of frequency components in input signals.

    The empirical results reveal that the importance of frequency components --- quantified via Shapley values --- aligns with model sensitivity under a variety of perturbation sources, including corruptions and adversarial attacks. These correlations support the hypothesis that certain frequency bands disproportionately influence predictive robustness. Together, these findings reinforce the theoretical results and demonstrate that frequency-domain analysis offers a principled and interpretable approach for evaluating the global robustness of deep learning models.
    
\end{enumerate}



\section{Closing Remarks}


In conclusion, this thesis establishes both theoretical and empirical foundations for understanding the \textbf{principles of Lipschitz continuity} in neural networks. Guided by three primary research questions, it advances our understanding of how Lipschitz continuity evolves over time during training, how it modulates frequency signal propagation, and how it can be used to interpret the global robustness of deep learning models.



%To the best of our knowledge, Chapter~\ref{chapter:optimization_induced_dynamics} establishes the \underline{\textbf{first theoretical framework}} for modeling the temporal evolution of Lipschitz continuity in neural networks through a system of stochastic differential equations (SDEs), marking a central contribution of this thesis. Building on the analytic operator-norm Hessian formulation developed in Chapter~\ref{chapter:perturbation_analysis} and the theory of matrix-valued SDEs, this framework rigorously characterizes how Lipschitz properties evolve during training, and is supported by numerical validation. In doing so, it not only provides novel theoretical insights but also lays a strong foundation for future research into robust and interpretable deep learning systems.

==> main_matter/chapters/FourierAnalysis/text.tex <==
\section{Introduction}

\lettrine[lines=3]{L}{ipschitz} continuity in neural networks refers to a constraint on the network's function, ensuring that the output changes at a bounded rate with respect to input changes. Mathematically, a function $f: \mathbb{R}^m \mapsto \mathbb{R}^n$ is $K$-Lipschitz continuous if there exists a constant $L$ (the Lipschitz constant) such that 
\begin{align}
\|f(u) - f(v)\| \leq K \|u - v\| 
,   
\end{align}
for all inputs $\forall~u, v$. In neural networks, this property governs multiple fundamental properties such as robustness to small input changes and generalization to unseen data~\citep{cisse2017parseval}. 

Lipschitz continuity also governs frequency feature propagation in neural networks, a phenomenon closely tied to \textbf{spectral bias}~\citep{rahaman2019spectral}. Spectral bias refers to the tendency of neural networks to learn low-frequency components of a target function more quickly and effectively than high-frequency components~\citep{rahaman2019spectral,xu2019frequency,luo2024interpreting}. 

\paragraph{Content Organization.} We present two complementary investigations: one theoretical and one empirical. The content is organized as follows:
\begin{enumerate}

    \item Section~\ref{sec:spectral_bias_lipschitz:theoretical_analysis}~(\nameref{sec:spectral_bias_lipschitz:theoretical_analysis}) provides a theoretical analysis of the role of Lipschitz continuity using Fourier analysis. We show that the variational mutual information gap under frequency perturbations is locally upper-bounded by the contribution of the spectral Lipschitz constant.
    

    \item Section~\ref{sec:spectral_bias_lipschitz:empirical_analysis}~(\nameref{sec:spectral_bias_lipschitz:empirical_analysis}) presents an empirical analysis of the relationship between Lipschitz continuity and the frequency structure of training data. Our experiments demonstrate that networks trained on high-frequency data tend to exhibit larger Lipschitz constants and sharper loss landscapes, which in turn lead to reduced robustness and generalization performance.
\end{enumerate}


\section{Preliminaries}

\paragraph{Lebesgue Measure.}
The \emph{Lebesgue measure} $\mu$ on $\mathbb{R}^d$ is a complete, translation-invariant measure defined on the $\sigma$-algebra of Lebesgue-measurable subsets of $\mathbb{R}^d$. It extends the intuitive notions of length (in $\mathbb{R}$), area (in $\mathbb{R}^2$), and volume (in $\mathbb{R}^3$) to arbitrary dimension and to more general sets than those handled by the Riemann integral. Formally, for any box (\ie, product of intervals) $I = \prod_{i=1}^d [a_i, b_i] \subseteq \mathbb{R}^d$, the Lebesgue measure is defined as:
\begin{align}
    \mu(I) := \prod_{i=1}^d (b_i - a_i).
\end{align}

\paragraph{Key Properties.}
The Lebesgue measure satisfies the following key properties:
\begin{itemize}
    \item \textbf{Non-negativity.} $\mu(E) \geq 0$ for all measurable sets $E \subseteq \mathbb{R}^d$.
    
    \item \textbf{Countable additivity.} If $\{E_n\}_{n=1}^\infty$ is a countable collection of pairwise disjoint measurable sets, then
    \begin{align}
        \mu\left( \bigcup_{n=1}^\infty E_n \right) = \sum_{n=1}^\infty \mu(E_n).
    \end{align}
    
    \item \textbf{Translation invariance.} For any measurable set $E \subseteq \mathbb{R}^d$ and any vector $x \in \mathbb{R}^d$, we have
    \begin{align}
        \mu(E + x) = \mu(E),
    \end{align}
    where $E + x := \{y + x : y \in E\}$.
\end{itemize}


\paragraph{Lebesgue Measurable.} A set $E \subseteq \mathbb{R}^d$ is \emph{Lebesgue measurable} if for every $\varepsilon > 0$, there exists an open set $O \supseteq E$ such that
\begin{align}
\mu(O \setminus E) < \varepsilon.
\end{align}

\paragraph{Lebesgue Integral.} Let $f: \mathbb{R}^d \to \mathbb{R}$ be a Lebesgue-measurable function. The Lebesgue integral of $f$ with respect to the Lebesgue measure $\mu$ is defined by first considering non-negative functions, where
\begin{align}
\int_{\mathbb{R}^d} f \, d\mu := \sup \left\{ \int_{\mathbb{R}^d} s \, d\mu : 0 \leq s \leq f, \ s \text{ simple} \right\},
\end{align}
and each simple function takes the form $s(x) = \sum_{i=1}^n a_i \cdot \mathbf{1}_{E_i}(x)$ for $a_i \geq 0$ and measurable sets $E_i$. For a general function $f$, we write $f = f^+ - f^-$ with $f^+ := \max(f, 0)$ and $f^- := \max(-f, 0)$, and define the integral as
\begin{align}
\int_{\mathbb{R}^d} f \, d\mu := \int_{\mathbb{R}^d} f^+ \, d\mu - \int_{\mathbb{R}^d} f^- \, d\mu
.
\end{align}
%provided at least one term is finite. %Unlike the Riemann integral, this formulation accommodates unbounded domains, discontinuities, and irregular regions, making it fundamental in real analysis and harmonic analysis~\citep{stein2011fourier}.


\paragraph{Inequalities in Function Spaces $L^p$.} Minkowski's inequality states that for $1 \leq p \leq \infty$ and functions $f, g \in L^p(\mathbb{R}^d)$, the norm satisfies
\begin{align}
\|f + g\|_p \leq \|f\|_p + \|g\|_p,
\end{align}
ensuring the triangle inequality in $L^p$. 

H\"older's inequality, for $1 \leq p, q \leq \infty$ with $\frac{1}{p} + \frac{1}{q} = 1$, asserts that for $f \in L^p(\mathbb{R}^d)$ and $g \in L^q(\mathbb{R}^d)$,
\begin{align}
\int |fg| \, d\mu \leq \|f\|_p \|g\|_q.
\end{align}

Cauchy-Schwarz inequality, a special case of H\"older's inequality, of when $p = q = 2$, yields
\begin{align}
\int |fg| \, d\mu \leq \left( \int |f|^2 \, d\mu \right)^{1/2} \left( \int |g|^2 \, d\mu \right)^{1/2}.
\end{align}


\paragraph{Fourier Representation of Function.}
Let $f \in L^1(\mathbb{R}^d)$, the space of Lebesgue integrable functions. The \emph{Fourier transform} of $f$ is defined as
\begin{align}
\hat{f}(\zeta) := \int_{\mathbb{R}^d} f(x) e^{-2\pi i \langle \zeta, x \rangle} \, dx,
\end{align}
where $\zeta \in \mathbb{R}^d$ is the frequency variable. The \emph{inverse Fourier transform} recovers $f$ from its frequency representation when $\hat{f} \in L^1(\mathbb{R}^d)$:
\begin{align}
f(x) = \int_{\mathbb{R}^d} \hat{f}(\zeta) e^{2\pi i \langle \zeta, x \rangle} \, d\zeta.
\end{align}


%This defines a continuous function $\hat{f} \in C_0(\mathbb{R}^d)$ that vanishes at infinity. 
\paragraph{Parseval's Identity.} If additionally $f \in L^1(\mathbb{R}^d) \cap L^2(\mathbb{R}^d)$ (\ie, absolutely integrable and square-integrable with respect to the Lebesgue measure), then $\hat{f} \in L^2(\mathbb{R}^d)$ and Parseval's identity holds:
\begin{align}
\int_{\mathbb{R}^d} |f(x)|^2 \, dx = \int_{\mathbb{R}^d} |\hat{f}(\zeta)|^2 \, d\zeta.
\end{align}




\paragraph{Directional Fourier Representation.} 
The \textbf{Fourier series} of a real-valued, integrable, and periodic function $f: \mathbb{R} \mapsto \mathbb{R}$ with period $T$, its Fourier series spans a set of \textbf{discrete Fourier bases}:
\begin{align}
f(x) = a_0 + \sum_{n=1}^{\infty} \left( a_n \cos\left( \frac{2\pi n}{T} x \right) + b_n \sin\left( \frac{2\pi n}{T} x \right) \right),
\end{align}
where the Fourier coefficients are:
\begin{align}
a_0 &= \frac{1}{T} \int_{0}^{T} f(x)  dx, \\
a_n &= \frac{2}{T} \int_{0}^{T} f(x) \cos\left( \frac{2\pi n}{T} x \right)  dx, \\
b_n &= \frac{2}{T} \int_{0}^{T} f(x) \sin\left( \frac{2\pi n}{T} x \right)  dx.
\end{align}

In contrast, the Fourier representation of a function on $\mathbb{R}^d$ spans an \textbf{infinite continuum of frequency components} across $\mathbb{R}^d$. For visualization and analysis, it is often useful to examine the behavior of the transform along a fixed direction in frequency space, reducing the high-dimensional spectrum to a one-dimensional slice. Let $f \in L^1(\mathbb{R}^d)$ and fix a direction $\zeta_0 \in \mathbb{R}^d$ with $\|\zeta_0\| = 1$. The \emph{directional Fourier transform} of $f$ along $\zeta_0$ is defined for $t \in \mathbb{R}$ as:
\begin{align}
\hat{f}_{\zeta_0}(t) := \int_{\mathbb{R}^d} f(x) e^{-2\pi i \langle t\zeta_0, x \rangle} \, dx,
\end{align}
which equals the restriction of the full Fourier transform $\hat{f}$ to the line $\zeta = t\zeta_0$, \ie, $\hat{f}_{\zeta_0}(t) = \hat{f}(t\zeta_0)$. 

It is notable that the directional Fourier transform $\hat{f}_{\zeta_0}(t)$ captures the frequency content of $f$ along a fixed direction $\zeta_0$, but in general, $f(x)$ cannot be fully recovered from $\hat{f}_{\zeta_0}(t)$ alone. Full reconstruction requires that $f$ be supported on, or constant along, hyperplanes orthogonal to $\zeta_0$, thereby reducing the problem to a one-dimensional setting.


\section{Fourier Analysis}
\label{sec:spectral_bias_lipschitz:theoretical_analysis}


This section develops a Fourier representation of the Lipschitz continuity bound, establishing a theoretical framework that expresses the Lipschitz constant as an integral over local spectral contributions. We further demonstrate that the variational mutual information gap resulting from the removal of a frequency component is directly controlled by these spectral terms. Together, these results provide a principled connection between frequency-domain signal propagation and Lipschitz continuity.



\subsection{Fourier Representation of Lipschitz Continuity Bound}


\begin{theorem}[Spectral Bound of Lipschitz Continuity]
\label{theorem:spectral_bound_of_lipschitz}
Let $f : \mathbb{R}^d \to \mathbb{R}$ be a differentiable function that is $K_f$-Lipschitz continuous, with Fourier transform $\hat{f}(\zeta) \in L^1(\mathbb{R}^d)$:
\begin{align}
\int_{\mathbb{R}^d} |\hat{f}(\zeta)| \, d\zeta < \infty
,
\end{align}
the space of Lebesgue absolutely integrable functions. Then the Lipschitz constant of $f$ satisfies:
\begin{align}
K_f := \sup_{x \in \mathbb{R}^d} \|\nabla f(x)\|_2 \leq \int_{\mathbb{R}^d} 2\pi \|\zeta\|_2 |\hat{f}(\zeta)| \, d\zeta,
\end{align}
where $\zeta \in \mathbb{R}^d$ denotes the frequency variable, and $\|\cdot\|_2$ is the Euclidean norm. Furthermore, define the \textbf{spectral Lipschitz contribution} at frequency $\zeta$ as:
\begin{align}
K_\zeta := 2\pi \|\zeta\|_2 |\hat{f}(\zeta)|.
\end{align}
Then:
\begin{align}
K_f \leq \int_{\mathbb{R}^d} K_\zeta \, d\zeta.
\end{align}
\end{theorem}


\begin{proof}
Since $f$ is differentiable and $\hat{f} \in L^1(\mathbb{R}^d)$, the Fourier transform of $f$ is defined as:
\begin{align}
\hat{f}(\zeta) = \int_{\mathbb{R}^d} f(x) e^{-2\pi i \langle \zeta, x \rangle} \, dx,
\end{align}
where $dx$ denotes the Lebesgue measure on $\mathbb{R}^d$, and $\langle \cdot, \cdot \rangle$ is the standard inner product.

By the Fourier inversion theorem \citep{stein2011fourier}, since $\hat{f} \in L^1(\mathbb{R}^d)$, we have:
\begin{align}
f(x) = \int_{\mathbb{R}^d} \hat{f}(\zeta) e^{2\pi i \langle \zeta, x \rangle} \, d\zeta,
\end{align}
where $d\zeta$ is the Lebesgue measure on $\mathbb{R}^d$.

Since $f$ is differentiable, we compute the gradient by interchanging differentiation and integration, which is justified by the dominated convergence theorem and the integrability of $\hat{f}$ \citep{rudin1987real}:
\begin{align}
\nabla_x f(x) &= \nabla_x \int_{\mathbb{R}^d} \hat{f}(\zeta) e^{2\pi i \langle \zeta, x \rangle} \, d\zeta \notag \\
&= \int_{\mathbb{R}^d} \hat{f}(\zeta) \nabla_x \left( e^{2\pi i \langle \zeta, x \rangle} \right) \, d\zeta \notag \\
&= \int_{\mathbb{R}^d} \hat{f}(\zeta) \cdot 2\pi i \zeta e^{2\pi i \langle \zeta, x \rangle} \, d\zeta.
\end{align}
Thus, the Fourier transform of the gradient is $\widehat{\nabla f}(\zeta) = 2\pi i \zeta \hat{f}(\zeta)$.

To bound the Lipschitz constant, note that since $f$ is differentiable and $K_f$-Lipschitz:
\begin{align}
K_f = \sup_{x \in \mathbb{R}^d} \|\nabla_x f(x)\|_2
,
\end{align}
we estimate:
\begin{align}
\|\nabla_x f(x)\|_2 &= \left\| \int_{\mathbb{R}^d} 2\pi i \zeta \hat{f}(\zeta) e^{2\pi i \langle \zeta, x \rangle} \, d\zeta \right\|_2 \notag \\
&\leq \int_{\mathbb{R}^d} \| 2\pi i \zeta \hat{f}(\zeta) e^{2\pi i \langle \zeta, x \rangle} \|_2 \, d\zeta  \notag \\
&= \int_{\mathbb{R}^d} |2\pi i| \|\zeta\|_2 |\hat{f}(\zeta)| \cdot |e^{2\pi i \langle \zeta, x \rangle}| \, d\zeta \notag \\
&= \int_{\mathbb{R}^d} 2\pi \|\zeta\|_2 |\hat{f}(\zeta)| \, d\zeta,
\end{align}
since $|e^{2\pi i \langle \zeta, x \rangle}| = 1$ and $|i| = 1$. The integral converges because $\hat{f} \in L^1(\mathbb{R}^d)$.

Define the spectral Lipschitz contribution as:
\begin{align}
K_\zeta = 2\pi \|\zeta\|_2 |\hat{f}(\zeta)|
,
\end{align}
then:
\begin{align}
K_f = \sup_{x \in \mathbb{R}^d} \|\nabla_x f(x)\|_2 \leq \int_{\mathbb{R}^d} K_\zeta \, d\zeta
.
\end{align}

\end{proof}


\begin{figure}[t!]
    \centering
 
       \begin{minipage}[t]{0.45\linewidth}
     \centering 
     \subfloat[$\hat{f}(\zeta_t)$]{
     \includegraphics[width=1\linewidth]{plots/mlp_mnist_principal_direction_nuft.pdf} 
     }
   \end{minipage}
   %\hspace*{\fill}%
   \begin{minipage}[t]{0.45\linewidth}
     \centering 
     \subfloat[$K_{\zeta_t}$]{
     \includegraphics[width=1\linewidth]{plots/mlp_mnist_principal_direction_K_zeta.pdf} 
     }
  \end{minipage}

  \caption[Directional Frequency Analysis of Three-Layer MLP]{Directional frequency analysis of a three-layer MLP (Table~\ref{tab:mlp_freq}). The directional frequency vector is chosen as the principal direction of the training set. We visualize $|\hat{f}(\zeta_t)|$ and $K_{\zeta_t}$ along the principal component direction $\zeta_t := \frac{t}{2\pi} \cdot \zeta$, with $t \in [0, 2\pi]$.}
    
  \label{fig:directional_frequency_response}
    
\end{figure}

\subsubsection{Experiment of Directional Frequency Response}
Figure~\ref{fig:directional_frequency_response} presents results from an experiment using a three-layer MLP trained on MNIST. The $f(x):x \to [0,1]$ is defined as the predicted probability for the true label. The $\hat{f}$ is normalized by $\sfrac{1}{N}$ where $N$ is the number of samples. We visualize $|\hat{f}(\zeta_t)|$ and the corresponding spectral Lipschitz contribution $K_{\zeta_t}$ along a chosen frequency direction of the form $\zeta_t := \frac{t}{2\pi}\zeta$, where $\zeta$ is the principal component direction of the training data. Frequency $t$ is normalized over the interval $[0, 2\pi]$, enabling a directional analysis of the learned function’s frequency response and its contribution to the Lipschitz bound. The MLP model, detailed in Table~\ref{tab:mlp_freq}, is trained for 10 epochs using the Adam optimizer with a learning rate of $0.001$.

%The $\hat{f}$ is normalized. 

\begin{table}[H]
    \centering
    \adjustbox{max width=\textwidth}{%
    \begin{tabular}{|c|l|l|}
        \hline
        \textbf{Function Block} & \textbf{Layer \#} & \textbf{Module} \\
        \hline

        \multirow{2}{*}{Input Layer} & \cellcolor{lime!20}1 & \cellcolor{lime!20}\texttt{nn.Linear(768, 200)} \\
        \cline{2-3}
        & 2 & \texttt{nn.ReLU()} \\
        \hline

        \multirow{2}{*}{Hidden Layer \#1} & \cellcolor{lime!20}3 & \cellcolor{lime!20}\texttt{nn.Linear(200, 200)} \\
        \cline{2-3}
        & 4 & \texttt{nn.ReLU()} \\
        \hline

        \multirow{2}{*}{Output Layer} & \cellcolor{lime!20}5 & \cellcolor{lime!20}\texttt{nn.Linear(200, 10)} \\
        \cline{2-3}
        & 6 & \texttt{nn.LogSoftmax(dim=1)} \\
        \hline
    \end{tabular}
    }% adjustbox
    \caption{MLP configuration used in the directional frequency response experiment. }
    \label{tab:mlp_freq}
\end{table}


\begin{remark}
The term $|\hat{f}(\zeta)|$ represents the amplitude of $f$ at frequency $\zeta$ in the frequency domain. This theorem implies that the Lipschitz constant $K_f$ is controlled by the weighted contribution of all frequencies, with higher frequencies (large $\|\zeta\|_2$) amplifying the effect of $|\hat{f}(\zeta)|$. For neural networks modeled by $f$, large $|\hat{f}(\zeta)|$ at high frequencies indicates sensitivity to rapid changes, leading to a larger $K_f$ and potentially less robust behavior.
\end{remark}

\subsubsection{Numerical Validation -- Synthesized Function}
\label{sec:numerical_verification_lipschitz_decomposition:synthesized_function}

\begin{figure}[!t]
 
  \centering


   \begin{minipage}[t]{0.3\linewidth}
     \centering 
     \subfloat[$f(x)$ ($\text{random seed}: 0$)]{
     \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_theorem_function_trial_0.pdf} 
     }
  \end{minipage}
  %\hspace*{\fill}%
  \begin{minipage}[t]{0.3\linewidth}
     \centering 
     \subfloat[$f(x)$ ($\text{random seed}: 1$)]{
     \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_theorem_function_trial_1.pdf} 
     }
  \end{minipage}
  %\hspace*{\fill}%
  \begin{minipage}[t]{0.3\linewidth}
     \centering 
     \subfloat[$f(x)$ ($\text{random seed}: 2$)]{
     \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_theorem_function_trial_2.pdf} 
     }
  \end{minipage}

   \begin{minipage}[t]{0.3\linewidth}
     \centering 
     \subfloat[$|\hat{f}(\zeta)|$ ($\text{random seed}: 0$)]{
     \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_theorem_f_hat_trial_0.pdf} 
     }
  \end{minipage}
  %\hspace*{\fill}%
  \begin{minipage}[t]{0.3\linewidth}
     \centering 
     \subfloat[$|\hat{f}(\zeta)|$ ($\text{random seed}: 1$)]{
     \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_theorem_f_hat_trial_1.pdf} 
     }
  \end{minipage}
  %\hspace*{\fill}%
  \begin{minipage}[t]{0.3\linewidth}
     \centering 
     \subfloat[$|\hat{f}(\zeta)|$ ($\text{random seed}: 2$)]{
     \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_theorem_f_hat_trial_2.pdf} 
     }
  \end{minipage}
  
  
  \begin{minipage}[t]{0.5\linewidth}
     \centering 
     \subfloat[$K_f$ and $\int K_{\zeta} d \zeta$]{
     \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_theorem_trials.pdf} 
     }
  \end{minipage}

  \caption[Spectral Bound of Lipschitz Continuity with Synthesized Multi-Sine Functions]{Spectral bound of Lipschitz continuity with synthesized functions. (a)–(c): Three functions $f(x)$ generated using different random seeds, each as a sum of sinusoidal components with randomly sampled frequencies and amplitudes. (d)-(f): Fourier transforms $\hat{f}(x)$ of $f(x)$. (g): Comparison between the theoretical Lipschitz constant $K_f = \sup_{x} \|\nabla f(x)\|_2$ and the theoretical spectral bound $\int K_\zeta \, d\zeta$ computed using Theorem~\ref{theorem:spectral_bound_of_lipschitz}. The close agreement across trials numerically validates the proposed spectral decomposition of Lipschitz continuity bound.}
  
 
\label{fig:lipschitz_spectral_decomposition_synthesized_function}
\end{figure}


We now demonstrate the validity of Theorem~\ref{theorem:spectral_bound_of_lipschitz} using synthesized functions, as illustrated in Figure~\ref{fig:lipschitz_spectral_decomposition_synthesized_function}. Specifically, we construct a \emph{multi-sine} function defined as:
\begin{align}
    f(x) = \sum_{n=1}^{N} a_n \sin{(2\pi \omega_n x)},
\end{align}
where $N=10$, $x \in [-5, 5]$ is sampled at $50,\!000$ evenly spaced points, and the amplitudes $a_n$ and frequencies $\omega_n$ are independently drawn from uniform distributions: $a_n \sim \mathcal{U}[0.1, 1]$ and $\omega_n \sim \mathcal{U}[0.1, 5]$. The corresponding Fourier transform of this function admits:
\begin{align}
    \hat{f}(\zeta) = \sum_{n=1}^N \frac{a_n}{2i}\Big[\delta(\zeta - \omega_n) - \delta(\zeta + \omega_n)\Big]
    ,
\end{align}
where $\delta(\cdot)$ represents the Dirac delta distribution.
% , defined as:
% \begin{align}
%     \delta(x) = \begin{cases}
%         1, &x=0\\
%         0, &x \ne 0
%     \end{cases}
%     .
% \end{align}

Using Theorem~\ref{theorem:spectral_bound_of_lipschitz}, we compute the theoretical spectral bound of the Lipschitz constant of $f$ across three independent trials with random seeds $1$, $2$, and $3$, respectively. The results consistently confirm that the theorem accurately bounds the Lipschitz continuity of the synthesized function.




\subsubsection{Numerical Validation -- Well-Defined Example}
\label{sec:numerical_verification_lipschitz_decomposition:well_defined_example}

We now show that Theorem~\ref{theorem:spectral_bound_of_lipschitz} holds true with a well-defined example. 

\begin{proposition}
Suppose $f: \mathbb{R}^2 \to \mathbb{R}$ is given by:
\begin{align}
f(x) = e^{-a (x_1^2 + x_2^2)},
\end{align}
where $a > 0$. Then $f$ is smooth and globally defined. The $f(x) = e^{-a (x_1^2 + x_2^2)}$ has a Lipschitz constant:
    \begin{align}
        K_f = \sqrt{\frac{2a}{e}}
        ,
    \end{align}
    spectral Lipschitz contribution:
    \begin{align}
        K_\zeta = \frac{2\pi^2}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a}\|\zeta\|_2^2}
        ,
    \end{align}
    and spectral bound:
    \begin{align}
        \int K_\zeta = \int_{\mathbb{R}^2} K_\zeta d\zeta = \sqrt{a}.
    \end{align}
\end{proposition}

\begin{proof}
\textbf{True Lipschitz constant.} Set $r = \sqrt{x_1^2 + x_2^2}$. The gradient is:
\begin{align}
\nabla f(x) = 
\begin{bmatrix}
    -2a x_1 e^{-a r^2} \\
    -2a x_2 e^{-a r^2}
\end{bmatrix}
\end{align}
and its norm is:
\begin{align}
g(r) := \|\nabla f(x)\|_2 = 2a r e^{-a r^2}.
\end{align}

Maximizing $g(r)$ over $r \geq 0$, we find:
\begin{align}
g'(r) = 2a e^{-a r^2} (1 - 2a r^2) = 0 \quad \Rightarrow \quad r = \frac{1}{\sqrt{2a}}.
\end{align}
Hence,
\begin{align}
K_f := \sup_x \|\nabla f(x)\|_2 = g\left(\frac{1}{\sqrt{2a}}\right) = \sqrt{\frac{2a}{e}}.
\end{align}

\textbf{Derive Fourier transform.} The Fourier transform is:
\begin{align}
\hat{f}(\zeta) = \int_{\mathbb{R}^2} e^{-a (x_1^2 + x_2^2)} e^{-2\pi i (\zeta_1 x_1 + \zeta_2 x_2)} \, dx_1 dx_2 = \left( \int_{-\infty}^\infty e^{-a x_1^2 - 2\pi i \zeta_1 x_1} \, dx_1 \right)^2.
\end{align}

Note the square:
\begin{align}
-a x_1^2 - 2\pi i \zeta_1 x_1 = -a \left( x_1 + \frac{\pi i \zeta_1}{a} \right)^2 + \frac{\pi^2 \zeta_1^2}{a},
\end{align}

\begin{align}
\int_{-\infty}^\infty e^{-a \left( x_1 + \frac{\pi i \zeta_1}{a} \right)^2 + \frac{\pi^2 \zeta_1^2}{a}} \, dx_1 = e^{-\frac{\pi^2 \zeta_1^2}{a}} \sqrt{\frac{\pi}{a}},
\end{align}

\begin{align}
\hat{f}(\zeta) = \frac{\pi}{a} e^{-\frac{\pi^2 (\zeta_1^2 + \zeta_2^2)}{a}}.
\end{align}

Verify that $\hat{f} \in L^1(\mathbb{R}^2)$ is absolute integrable with respect to Lebesgue measure:
\begin{align}
\int_{\mathbb{R}^2} |\hat{f}(\zeta)| d\zeta =
\int_{\mathbb{R}^2} \frac{\pi}{a} e^{-\frac{\pi^2 (\zeta_1^2 + \zeta_2^2)}{a}} \, d\zeta = 1 < \infty.
\end{align}

% The spectral Lipschitz contribution is:

% \begin{align}
% K_\zeta = \frac{2\pi^2}{a} \sqrt{\zeta_1^2 + \zeta_2^2} e^{-\frac{\pi^2 (\zeta_1^2 + \zeta_2^2)}{a}}.
% \end{align}


% We compute the Fourier transform of $f$ under the $2\pi$ convention:
% \begin{align}
% \hat{f}(\zeta) = \int_{\mathbb{R}^2} f(x) e^{-2\pi i \langle \zeta, x \rangle} dx = \frac{\pi}{a} e^{-\frac{\pi^2}{a} (\zeta_1^2 + \zeta_2^2)}.
% \end{align}

\textbf{Spectral bound.}
By Theorem~\ref{theorem:spectral_bound_of_lipschitz}, define the point-wise spectral contribution:
\begin{align}
K_\zeta = 2\pi \|\zeta\|_2 |\hat{f}(\zeta)| = \frac{2\pi^2}{a} \|\zeta\|_2 e^{- \frac{\pi^2}{a} \|\zeta\|_2^2}.
\end{align}

Applying polar coordinates in frequency-domain $\mathbb{R^2}$:
\begin{align}
    \begin{cases}
        \zeta_1 = r \cos\theta \\
        \zeta_2 = r \sin\theta
    \end{cases}
    ,
\end{align}
hence:
\begin{align}
\int_{\mathbb{R}^2} K_\zeta \, d\zeta 
= \int_0^{2\pi} \int_0^\infty \frac{2\pi^2}{a} r \cdot r e^{- \frac{\pi^2}{a} r^2} dr d\theta = \frac{2\pi^2}{a} \cdot 2\pi \int_0^\infty r^2 e^{-\frac{\pi^2}{a} r^2} dr.
\end{align}

Use the standard integral:
\begin{align}
\int_0^\infty r^2 e^{-c r^2} dr = \frac{1}{2} \cdot \frac{\sqrt{\pi}}{2 c^{3/2}} = \frac{\sqrt{\pi}}{4 c^{3/2}}.
\end{align}
Apply with $c = \frac{\pi^2}{a}$:
\begin{align}
\int_0^\infty r^2 e^{-\frac{\pi^2}{a} r^2} dr = \frac{\sqrt{\pi}}{4} \left( \frac{a}{\pi^2} \right)^{3/2}.
\end{align}

Therefore:
\begin{align}
\int_{\mathbb{R}^2} K_\zeta \, d\zeta 
&= \frac{2\pi^2}{a} \cdot 2\pi \cdot \frac{\sqrt{\pi}}{4} \left( \frac{a}{\pi^2} \right)^{3/2}
= \sqrt{\pi\,a}.
\end{align}

\textbf{Results.} We compare $K_f$ with its spectral bound:
\begin{align}
K_f = \sqrt{\frac{2a}{e}} \leq \sqrt{\pi\, a} \quad \Longleftrightarrow \quad \frac{2}{\pi \,e} \leq 1,
\end{align}
which always holds. Hence, the spectral Lipschitz bound
\begin{align}
K_f \leq \int_{\mathbb{R}^2} K_\zeta \, d\zeta
\end{align}
is valid for all $a > 0$.
\end{proof}






\begin{figure}[t!]
    \centering
    \resizebox{0.95\linewidth}{!}{
        \input{tikz/spectral_band_perturbation_bound}
    }
    
    \caption[Spectral Lipschitz Continuity Representation Bounds Frequency-Band Perturbation]{Lemma~\ref{lemma:input_space_frequency_perturbation_bound}: 
\textbf{Spectral-Band Perturbation Bound} states that the output change due to a perturbation at a frequency point $\zeta$, within the ball $B_\delta(\zeta)$ of energy $\varepsilon$ in the frequency domain of the input space, is proportionally bounded above by the supremum $M_\delta$ of the spectral Lipschitz contribution at that frequency ball.}
    \label{fig:spectral_band_perturbation_bound}
\end{figure}






\subsection{Small Frequency Perturbation in Input Spaces}

\begin{lemma}[Spectral-Band Perturbation Bound]
\label{lemma:input_space_frequency_perturbation_bound}
Let $f:\mathbb{R}^d \to \mathbb{R}$ be a continuously differentiable function with Fourier transform $\hat{f} \in L^1(\mathbb{R}^d) \cap L^2(\mathbb{R}^d)$, and assume
\begin{align}
\int_{\mathbb{R}^d} 2\pi \|\omega\| \cdot |\hat{f}(\omega)| \, d\omega < \infty.
\end{align}
Fix $\zeta \in \mathbb{R}^d$ and $\delta > 0$, and define the frequency ball $B_\delta(\zeta) := \{\omega \in \mathbb{R}^d : \|\omega - \zeta\| \leq \delta\}$. Let $x^{(-\zeta)}$ be the signal obtained by removing the frequency ball $B_\delta(\zeta)$ from the Fourier transform of $x$, and define
\begin{align}
\Delta x := x - x^{(-\zeta)}, \qquad \|\Delta x\|_2 = \varepsilon.
\end{align}
Define the local spectral Lipschitz bound
\begin{align}
M_\delta := \sup_{\omega \in B_\delta(\zeta)} 2\pi \|\omega\| \cdot |\hat{f}(\omega)|,
\end{align}
and let $\mu(B_\delta(\zeta))$ denote the Lebesgue measure of the frequency ball.

Then the output perturbation satisfies
\begin{align}
\sup_x |f(x) - f(x^{(-\zeta)})| \lesssim M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))} .
\end{align}

\end{lemma}

\begin{proof}
By the Fourier inversion formula,
\begin{align}
f(x) = \int_{\mathbb{R}^d} \hat{f}(\omega) e^{2\pi i \langle \omega, x \rangle} \, d\omega.
\end{align}
Differentiating under the integral gives
\begin{align}
\nabla f(x) = \int_{\mathbb{R}^d} 2\pi i \omega \hat{f}(\omega) e^{2\pi i \langle \omega, x \rangle} \, d\omega,
\end{align}
so the Fourier transform of $\nabla f$ is
\begin{align}
\widehat{\nabla f}(\omega) = 2\pi i \omega \hat{f}(\omega), \qquad \|\widehat{\nabla f}(\omega)\| = 2\pi \|\omega\| \cdot |\hat{f}(\omega)|.
\end{align}

By a Taylor expansion,
\begin{align}
f(x)  = f(x^{(-\zeta)}) + \langle \nabla f(\tilde{x}), \Delta x \rangle + o(\|\Delta x\|_2^2),
\end{align}
for some $\tilde{x}$ on the line segment between $x$ and $x^{(-\zeta)}$.

By Parseval’s identity \citep{stein2011fourier}, the inner product is preserved in frequency domain:
\begin{align}
\langle \nabla f(\tilde{x}), \Delta x \rangle = \int_{\mathbb{R}^d} \langle \widehat{\nabla f}(\omega)^*, \widehat{\Delta x}(\omega) \rangle \, d\omega.
\end{align}

Since $\widehat{\Delta x}$ is supported on $B_\delta(\zeta)$, applying H\"older's inequality, the integral reduces to
\begin{align}
|\langle \nabla f(\tilde{x}), \Delta x \rangle| 
=
\left| \int_{\mathbb{R}^d} \langle \widehat{\nabla f}(\omega)^*, \widehat{\Delta x}(\omega) \rangle \, d\omega\right|
\leq \int_{B_\delta(\zeta)} \|\widehat{\nabla f}(\omega)\|_2 \cdot \|\widehat{\Delta x}(\omega)\|_2 \, d\omega.
\end{align}

Using Cauchy–Schwarz:
\begin{align}
\int_{B_\delta(\zeta)} |\widehat{\Delta x}(\omega)| \, d\omega \leq \|\widehat{\Delta x}\|_2 \cdot \sqrt{\mu(B_\delta(\zeta))} = \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))}.
\end{align}
Therefore,
\begin{align}
|f(x) - f(x^{(-\zeta)})| \lesssim M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))} ,
\end{align}
uniformly in $x$, as claimed.
\end{proof}



\begin{remark}
An illustration is provided in Figure~\ref{fig:spectral_band_perturbation_bound}. This result establishes a connection between input-space frequency perturbation at frequency $\zeta$ and the Fourier representation of the function $f$ at the same frequency. It highlights how localized spectral properties of $f$ govern its sensitivity to frequency-specific perturbations in the input.
\end{remark}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/gradient_norm_wrt_freq.pdf}
    
    \caption[Low- and High-Frequency Signals Induce Low- and High Gradient Norms]{We train a ConvNet (see Table~\ref{tab:convnet_freq}) on three versions of the CIFAR-10 dataset. The low-frequency dataset is obtained by applying a low-pass filter with cutoff frequency $0.5$, while the high-frequency dataset is obtained using a high-pass filter with the same cutoff. The ConvNet is trained separately on each dataset. We then compute and visualize the $\ell_2$ norms of the input gradients. Theoretically, larger gradient norms correspond to larger Lipschitz constants. The results show that models trained on higher-frequency data tend to exhibit larger Lipschitz constants.}
    \label{fig:lipschitz_spectral_bias_gradient_norm}
\end{figure}

% \begin{figure}[!t]
 
%   \centering
  
%   % \begin{minipage}[t]{0.45\linewidth}
%   %    \centering 
%   %    \subfloat[$|\hat{f}(\zeta)|$]{
%   %    \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_mlp_mnist_f_hat.pdf} 
%   %    }
%   % \end{minipage}
%   % \begin{minipage}[t]{0.45\linewidth}
%   %    \centering 
%   %    \subfloat[$K_\zeta$]{
%   %    \includegraphics[width=1\linewidth]{plots/spectral_lipschitz_mlp_mnist_K_zeta.pdf} 
%   %    }
%   % \end{minipage}

%   \begin{minipage}[t]{0.45\linewidth}
%      \centering 
%      \subfloat[Frequency perturbation at $\zeta=2$ with $\delta=0.01$.]{
%      \includegraphics[width=1\linewidth]{plots/spectral_perturbation_lemma_zeta_2_delta_0.01.pdf} 
%      }
%   \end{minipage}
%   \begin{minipage}[t]{0.45\linewidth}
%      \centering 
%      \subfloat[Frequency perturbation at $\zeta=5$ with $\delta=0.01$.]{
%      \includegraphics[width=1\linewidth]{plots/spectral_perturbation_lemma_zeta_5_delta_0.01.pdf} 
%      }
%   \end{minipage}
  
  
%   \caption{Verification of Lemma~\ref{lemma:input_space_frequency_perturbation_bound}. The measured perturbation $\sup_x |f(x) - f(x^{(-\zeta)})|$ consistently, approximately correlates with the theoretical bound $\epsilon K_\zeta$, confirming the lemma, with a linear trend in both quantities.}
  
 
% \label{fig:lemma_perturbation_verification}
% \end{figure}

\subsubsection{Numerical Validation -- Well-Defined Example}

To verify Lemma~\ref{lemma:input_space_frequency_perturbation_bound}, we use the function $f(x) = e^{-a (x_1^2 + x_2^2)}$, where $a > 0$, defined on $\mathbb{R}^2$. We first compute the direct perturbation supremum $\sup_x |f(x) - f(x^{(-\zeta)})|$, where $x^{(-\zeta)}$ is the signal with frequencies in the ball $B_\delta(\zeta) = \{\omega \in \mathbb{R}^2 : \|\omega - \zeta\|_2 \leq \delta\}$ removed, and $\|\Delta x\|_2 = \|x - x^{(-\zeta)}\|_2 = \varepsilon$. We then compute the theoretical bound $M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))}$, where $M_\delta = \sup_{\omega \in B_\delta(\zeta)} 2\pi \|\omega\|_2 \cdot |\hat{f}(\omega)|$, and compare to confirm the lemma holds.

\paragraph{Function perturbation supremum.} 


Use the Fourier representation of $f(x)$:
\begin{align}
f(x) - f(x^{(-\zeta)}) &= \int_{B_\delta(\zeta)} \hat{f}(\omega) \left( e^{2\pi i \langle \omega, x \rangle} - e^{2\pi i \langle \omega, x^{(-\zeta)} \rangle} \right) d\omega \\
&=\int_{B_\delta(\zeta)} \hat{f}(\omega) \left( e^{2\pi i \langle \omega, x \rangle} - e^{2\pi i \langle \omega, x - \Delta x \rangle} \right) d\omega \\
&=\int_{B_\delta(\zeta)} \hat{f}(\omega) e^{2\pi i \langle \omega, x \rangle} \left( 1 - e^{2\pi i \langle \omega, -\Delta x \rangle} \right) d\omega \\
&=\int_{B_\delta(\zeta)} \hat{f}(\omega) e^{2\pi i \langle \omega, x \rangle} \left( 1 - e^{-2\pi i \langle \omega, \Delta x \rangle} \right) d\omega
.
\end{align}

Suppose $\|\Delta x\|_2$ is a small perturbation:
\begin{align}
    \langle \omega, \Delta x \rangle \to 0,
\end{align}
then:
\begin{align}
\left| 1 - e^{-2\pi i \langle \omega, \Delta x \rangle} \right| 
&= 
\left| 1- \cos{(-2\pi \langle \omega, \Delta x \rangle)} - i \sin{(-2\pi \langle \omega, \Delta x \rangle)} \right| \\
&\approx \left| \sin{(-2\pi \langle \omega, \Delta x \rangle)} \right| \\
&\approx 2\pi \|\omega\|_2 \varepsilon.
\end{align}


Since:
\begin{align}
\hat{f}(\omega) = \frac{\pi}{a} e^{-\frac{\pi^2}{a} \|\omega\|_2^2}
,
\end{align}
hence:
\begin{align}
|f(x) - f(x^{(-\zeta)})| \leq \frac{2\pi^2 \varepsilon}{a} \int_{B_\delta(\zeta)} \|\omega\|_2 e^{-\frac{\pi^2}{a} \|\omega\|_2^2} d\omega.
\end{align}
For small $\delta$, $\|\omega\|_2 \approx \|\zeta\|_2$, so:
\begin{align}
\sup_x |f(x) - f(x^{(-\zeta)})| \approx \frac{2\pi^2 \varepsilon}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a} \|\zeta\|_2^2} \cdot \pi \delta^2 = \frac{2\pi^3 \delta^2 \varepsilon}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a} \|\zeta\|_2^2}.
\end{align}

\paragraph{Theoretical bound.} The bound is:
\begin{align}
M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))},
\end{align}
where:
\begin{align}
M_\delta = \sup_{\omega \in B_\delta(\zeta)} \frac{2\pi^2}{a} \|\omega\|_2 e^{-\frac{\pi^2}{a} \|\omega\|_2^2}, \quad \mu(B_\delta(\zeta)) = \pi \delta^2.
\end{align}
For small $\delta$, $M_\delta \approx \frac{2\pi^2}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a} \|\zeta\|_2^2}$, and $\sqrt{\mu(B_\delta(\zeta))} = \sqrt{\pi} \delta$. Thus:
\begin{align}
M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))} \approx \frac{2\pi^2}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a} \|\zeta\|_2^2} \cdot \varepsilon \cdot \sqrt{\pi} \delta = \frac{2\pi^{5/2} \delta \varepsilon}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a} \|\zeta\|_2^2}.
\end{align}

\paragraph{Comparison.} Compare:
\begin{align}
\frac{\sup_x |f(x) - f(x^{(-\zeta)})|}{M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))}} \approx \frac{\frac{2\pi^3 \delta^2 \varepsilon}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a} \|\zeta\|_2^2}}{\frac{2\pi^{5/2} \delta \varepsilon}{a} \|\zeta\|_2 e^{-\frac{\pi^2}{a} \|\zeta\|_2^2}} = \frac{\pi^3 \delta^2}{\pi^{5/2} \delta} = \sqrt{\pi} \delta \leq 1
,
\end{align}
subject to:
\begin{align}
    \sqrt{\pi}\delta < 1 \Longleftrightarrow \delta < \frac{1}{\sqrt{\pi}} \approx 0.56418\cdots
    .
\end{align}
This shows that the Lemma~\ref{lemma:input_space_frequency_perturbation_bound} holds true if the frequency perturbation band is sufficiently small.




\subsection{Variational Mutual Information Gap in Image Classifiers}

\begin{corollary}[Spectral Lipschitz Contribution Bounds Variational Mutual Information Gap]
\label{corollary:variational_mutual_information_bound}
Let $(X,Y)$ be a classification dataset with a joint distribution $P_{X,Y}$. Let $P(Y)$ be the prior distribution of labels. Let $Q(y|x): x \mapsto [0,1]$ be a probabilistic classifier. Let $Y=\{1,\cdots,k\}$ be the label set. The variational mutual information of the classifier is defined as:
\begin{align}
    I(Q(y|x); Y) = \mathbb{E}_{x,y} \left[ \log \frac{Q(y|x)}{P(y)} \right]
\end{align}
where $(x, y) \sim P_{X,Y}$ sampled the dataset $P_{X,Y}$.

The absolute variational mutual information gap $\Delta I_\zeta$ perturbed by removing frequency $\zeta$ is approximately bounded above by:
\begin{align}
\abs{\Delta I_\zeta} := 
\left| I(Q(y|x); Y) - I(Q(y|x^{(-\zeta)}); Y) \right|
\lesssim 
M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))} %+ o(\varepsilon^2)
,    
\end{align}
where $\varepsilon$ is the perturbed magnitude and $B_\delta(\zeta)$ is a frequency ball.
\end{corollary}

\begin{proof}

By definition:
\begin{align}
\abs{\Delta I_\zeta} &= 
\left|\mathbb{E}_{x,y} \left[ \log \frac{Q(y|x)}{Q(y|x^{(-\zeta)})} + \log \frac{P(y)}{P(y)} \right] 
\right| \\
&\leq
\mathbb{E}_{x,y} \left[ \left|\log \frac{Q(y|x)}{Q(y|x^{(-\zeta)})} + \log \frac{P(y)}{P(y)} \right|\right] \\
&= \mathbb{E}_{x,y} \left[ \left|\log Q(y|x) - \log Q(y|x^{(-\zeta)}) \right|\right].
\end{align}

Set:
\begin{align}
    f(x) = \log Q(y|x)
    \quad \text{and} \quad
    f(x^{(-\zeta)}) = \log Q(y|x^{(-\zeta)})
    ,
\end{align}
then use Lemma~\ref{lemma:input_space_frequency_perturbation_bound}:
\begin{align}
\abs{\Delta I_\zeta}  &=     \mathbb{E}_{x,y} \left[ \left|f(x) - f(x^{(-\zeta)}) \right|\right] \\
&\leq \sup_{x,y} \left|f(x) - f(x^{(-\zeta)}) \right| \\
&\leq 
M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))} + o(\varepsilon^2) \\
&\lesssim M_\delta \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))}.
\end{align}

\end{proof}

\begin{remark}
This result shows that the variational mutual information perturbation due to frequency perturbation is bounded below locally by $2\pi \varepsilon \cdot \|\zeta\| \cdot |\hat{f}(\zeta)|$ and proportional to frequency $2$-norm.
\end{remark}




\section{Empirical Study}
\label{sec:spectral_bias_lipschitz:empirical_analysis}





\paragraph{Experimental Setting.} We use a convolutional neural network (ConvNet), shown in Table~\ref{tab:convnet_freq}, consisting of three convolutional layers, followed by an adaptive average pooling layer and two fully connected layers serving as the classifier. We construct frequency CIFAR10 datasets by applying a low-passing filters, varying the cutoff frequencies from $0.1$ to $1.0$ with step size $0.1$. For reproducibility, we fix random seeds to $42$. We use learning rate $0.001$, batch size $128$ and SGD optimizer.

\begin{table}[H]
    \centering
   \adjustbox{max width=\textwidth}{%
    \begin{tabular}{|c|l|l|}
        \hline
        
        \textbf{Function Block} &\textbf{\# of Layer} &  \textbf{Module} \\
        \hline
        
        \multirow{2}{*}{Block \#1} & \cellcolor{lime!20}$1$ & \cellcolor{lime!20}\texttt{nn.Conv2d(3, 64, kernel\_size=3, stride=2)} \\
        \cline{2-3}
        
        &$2$ & \texttt{nn.ReLU()} \\
        \hline


        \multirow{2}{*}{Block \#2}& \cellcolor{lime!20}$3$ &\cellcolor{lime!20}\texttt{nn.Conv2d(64, 128, kernel\_size=3, stride=2)} \\
        \cline{2-3}

        &$4$ & \texttt{nn.ReLU()} \\
        \hline


        \multirow{3}{*}{Block \#3}& \cellcolor{lime!20}$5$ &\cellcolor{lime!20}\texttt{nn.Conv2d(128, 256, kernel\_size=3, stride=2)} \\
        \cline{2-3}

        &$6$& \texttt{nn.ReLU()} \\
        \hline

        &$7$& \texttt{nn.AdaptiveAvgPool2d(output\_size = 1)} \\
        \hline

        \multirow{3}{*}{Classifier} & \cellcolor{lime!20}$8$ &\cellcolor{lime!20}\texttt{nn.Linear(256, 100)} \\
        \cline{2-3}

        &$9$ & \texttt{nn.ReLU()} \\
        \cline{2-3}


        &\cellcolor{lime!20}$10$ & \cellcolor{lime!20}\texttt{nn.Linear(100, 10)} \\
        \hline
        
    \end{tabular}
    }%adjustbox
    \caption{ConvNet configuration for the experiments exploring the connection between frequency signal propagation and Lipschitz continuity.}
    
    \label{tab:convnet_freq}
\end{table}



\begin{figure}[!t]
 
  \centering


   \begin{minipage}[t]{0.45\linewidth}
     \centering 
     \subfloat[Empirical Lipschitz]{
     \includegraphics[width=1\linewidth]{plots/empirical_lipschitz_wrt_cutoff_cifar10.pdf} 
     }
  \end{minipage}
  \hspace*{\fill}%
  \begin{minipage}[t]{0.45\linewidth}
     \centering 
     \subfloat[Theoretical Lipschitz]{
     \includegraphics[width=1\linewidth]{plots/theoretical_lipschitz_wrt_cutoff_cifar10.pdf} 
     }
  \end{minipage}
  
  \caption[Empirical and Theoretical Lipschitz Constants with respect to Frequency Signals in Training Data]{Empirical and theoretical Lipschitz constants with respect to frequency signals in training data. The results show that models trained on datasets with stronger high-frequency
components associate with larger Lipschitz constants.}
  
 
\label{fig:empirical_and_theoretical_lipschitz_wrt_freq}
\end{figure}

\subsection{Role of High-Frequency Components}

\begin{figure}[!t]

  \centering


   \begin{minipage}[t]{0.45\linewidth}
     \centering 
     \subfloat[Frequency cutoff at $0.1$]{
     \includegraphics[width=1\linewidth]{plots/losslandscape_cutoff_0.1.pdf} 
     }
  \end{minipage}
  %\hspace*{\fill}%
  \begin{minipage}[t]{0.45\linewidth}
     \centering 
     \subfloat[Frequency cutoff at $0.3$]{
     \includegraphics[width=1\linewidth]{plots/losslandscape_cutoff_0.3.pdf} 
     }
  \end{minipage}
  
  %\hspace*{\fill}%
  \begin{minipage}[t]{0.45\linewidth}
     \centering 
     \subfloat[Frequency cutoff at $0.7$]{
     \includegraphics[width=1\linewidth]{plots/losslandscape_cutoff_0.7.pdf} 
     }
  \end{minipage}
  
  % \begin{minipage}[t]{0.46\linewidth}
  %    \centering 
  %    \subfloat[Frequency cutoff at $0.7$]{
  %    \includegraphics[width=1\linewidth]{plots/losslandscape_cutoff_0.7.pdf} 
  %    }
  % \end{minipage}
  
  \caption[Frequency Signals in Training Data Shape Loss Landscape Flatness]{Frequency Signals in Training Data Shape Loss Landscape Flatness of a ConvNet on CIFAR-10 (Table~\ref{tab:convnet_freq}). Training with high-frequency signals not only increases the Lipschitz constant but also sharpens the loss landscape. The cutoff frequencies are normalized into $[0, 1]$.}
  
 
\label{fig:losslandscape_flatness}
\end{figure}

Theorem~\ref{theorem:spectral_bound_of_lipschitz} states that the spectral Lipschitz contribution $K_\zeta$ at frequency $\zeta$ is:
contribution term:
\begin{align}
    K_\zeta = 2\pi \cdot \|\zeta\| \cdot |\hat{f}(\zeta)|.
\end{align}
This implies that if a network $f$ is sensitive to high-frequency components --- \ie, $|\hat{f}(\zeta)|$ is large for large $\|\zeta\|$ --- then these components contribute more strongly to the overall Lipschitz constant $K_f$. The frequency $2$-norm $\|\zeta\|$ further amplifies the contribution term. This impacts neural network training, as shown in Figure~\ref{fig:lipschitz_spectral_bias_gradient_norm}, where a network trained on a low-frequency-only dataset displays lower gradient norms, while one trained on a high-frequency-only dataset exhibits higher gradient norms. 


To comprehensively study the impact of high-frequency components on Lipschitz continuity, we conduct experiments in which a low-pass frequency-domain filter is applied to the CIFAR-10 dataset. We vary the normalized cutoff frequency from $0.1$ to $1.0$ in increments of $0.1$, producing a series of progressively low-pass filtered datasets. For each filtered dataset, we train a ConvNet (see Table~\ref{tab:convnet_freq}).

Figure~\ref{fig:empirical_and_theoretical_lipschitz_wrt_freq} reports both the empirical Lipschitz constants and the corresponding theoretical upper bounds. The empirical Lipschitz constant is estimated as
\begin{align}
\max_{x \in \hat{X}} \|\nabla f(x)\|_2,
\end{align}
using a validation set $\hat{X}$ containing 500 samples. The theoretical upper bound is computed as
\begin{align}
\prod_{\ell=1}^L \sigma_1^{(\ell)},
\end{align}
where $\sigma_1^{(\ell)}$ denotes the largest singular value of the weight matrix in the $\ell$-th layer. The results show a clear correlation: models trained on datasets with stronger high-frequency components associate with larger Lipschitz constants.



\begin{remark}
The actual Lipschitz constant $K$ lies between the empirical Lipschitz constant:
\begin{align}
\max_{x \in \hat{X}} \|\nabla f(x)\|_2,
\end{align}
and the upper bound:
\begin{align}
\prod_{\ell=1}^L \sigma_1^{(\ell)},
\end{align}
such that:
\begin{align}
 \max_{x \in \hat{X}} \|\nabla f(x)\|_2 \leq K \leq    \prod_{\ell=1}^L \sigma_1^{(\ell)}.
\end{align}
Figure~\ref{fig:empirical_and_theoretical_lipschitz_wrt_freq} shows a correlation between the empirical Lipschitz constant and the upper bound.
\end{remark}

\subsection{Flatness of Loss Landscape}

High-frequency components affect not only the Lipschitz constant but also the geometric properties of the loss landscape. As shown in Figure~\ref{fig:losslandscape_flatness}, networks trained on data with stronger high-frequency components tend to exhibit sharper loss landscapes, while those trained on data with weaker high-frequency content result in smoother, flatter landscapes.





\section{Conclusions}

% This work establishes a theoretical and empirical connection between Lipschitz continuity and the frequency structure of data in neural networks. We introduced a spectral decomposition of the Lipschitz constant, showing that it can be expressed as an integral over frequency-local contributions. We further demonstrated that the impact of frequency perturbations on mutual information is bounded by these local spectral Lipschitz coefficients, linking spectral sensitivity to robustness. Empirically, we showed that networks trained on high-frequency data tend to exhibit larger Lipschitz constants and sharper loss landscapes, correlating with reduced robustness and generalization. In contrast, low-frequency training data lead to smoother models with better stability. Together, our results offer a unified spectral perspective on how frequency content shapes learning dynamics and model robustness, providing both theoretical insight and practical guidance for frequency-aware model design.


This work establishes a theoretical and empirical connection between Lipschitz continuity and the frequency structure of data in neural networks. We introduced a spectral decomposition of the Lipschitz constant, showing that it can be expressed as an integral over frequency-local contributions. We further demonstrated that the impact of frequency perturbations on mutual information is bounded by these local spectral Lipschitz coefficients, linking spectral sensitivity to robustness. Empirically, we showed that networks trained on high-frequency data tend to exhibit larger Lipschitz constants and sharper loss landscapes. Lipschitz constants directly quantify how strongly a model amplifies input perturbations; consequently, larger Lipschitz constants are associated with reduced robustness and weaker generalization. In contrast, low-frequency training data lead to smoother models with better stability. Together, our results offer a unified spectral perspective on how frequency content shapes learning dynamics and model robustness, providing both theoretical insight and practical guidance for frequency-aware model design.


==> main_matter/chapters/FourierAnalysis/tikz/spectral_band_perturbation_bound.tex <==
% \documentclass[tikz,border=6pt]{standalone}
% \usetikzlibrary{arrows.meta,decorations.pathmorphing,decorations.pathreplacing,calc,positioning}
% \usetikzlibrary{patterns} 


% \usepackage{amsmath}
% \usepackage{amssymb}



% \begin{document}



\begin{tikzpicture}%[>=Latex,thick]

%--- left box ---------------------------------------------------------------
\coordinate (A) at (0,0);
\coordinate (B) at (4,3);
\draw (A) rectangle (B);


% Ball with dashed outline + pattern fill
\coordinate (ball) at ($(A)!0.35!(B) + (-0.2,0.1)$);
\fill[pattern=north east lines] (ball) circle [radius=0.35];
\draw[dashed] (ball) circle [radius=0.35];


% mu(B) label inside the box
\draw[->] ($(ball)+(1,0.)$) -- ($(ball)+(0.5, 0.)$);
\node[anchor=west] at ($(ball)+(1,0.)$) {$\varepsilon$};

% label \hat{x} under the box
\node[below=4pt] at ($(A)!.5!(B |- A)$) {Frequency domain of input $\hat{x}$};


\draw[<-] ($(ball)+(0,0.55)$) -- ++(0,0.5) -- ++(0.9,0)
      node[above, xshift=-0.4cm] {$B_\delta(\zeta)$};
      
% "B_\delta(\xi)" callout over the small ball
\draw ($(ball)+(0,0.55)$) -- ++(0,0.5) -- ++(0.9,0) node[above, xshift=-0.4cm] {$B_\delta(\zeta)$};

%--- wavy arrow labeled f ---------------------

\draw[decorate,decoration={snake,amplitude=0.9,segment length=6pt},->]
  ($(B)!0.5!(B |- A)+(0.5,0)$) -- node[above]{\large $f$} ++(4,0) coordinate (waveend);

% Vertical line to the right of wavy arrow
\draw[->] (waveend)++(1,-3) coordinate (lineStart) -- ++(0,5) coordinate (lineEnd);

% Hatched interval centered vertically
\fill[pattern=north east lines] ($(lineStart)+( -0.1, 2)$) rectangle ($(lineStart)+(0.1, 4)$);

% Horizontal ticks at ends of hatched interval
\draw ($(lineStart)+(-0.3,2)$) -- ($(lineStart)+(0.3,2)$);
\draw ($(lineStart)+(-0.3,4)$) -- ($(lineStart)+(0.3,4)$);

% Point in the middle of hatched interval
\fill ($(lineStart)+(0,3)$) circle [radius=1.4pt];
\node[left=4pt] at ($(lineStart)+(0,3)$) {}; %{$\tilde y$};

% Brace to the right of hatched interval
% \draw[decorate,decoration={brace,amplitude=4pt,mirror}]
%   ($(lineStart)+(0.6,2)$) -- node[right=6pt] {$M_{\delta} \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))}$}
%   ($(lineStart)+(0.6,4)$);

\draw[decorate,decoration={brace,amplitude=4pt,mirror}]
  ($(lineStart)+(0.6,2)$) -- node[right=6pt] {$\underbrace{\left[\sup_{\omega \in B_\delta(\zeta)} K_\omega\right]}_{M_\delta} \cdot \varepsilon \cdot \sqrt{\mu(B_\delta(\zeta))}$}
  ($(lineStart)+(0.6,4)$);

% Place the \sup as a separate node below the formula
%\node[right=6pt,align=center] at ($(lineStart)+(0.6,2)$) {$M_\delta := \sup_{\omega \in B_\delta(\zeta)} K_\omega$};

% ℝ at the top
\node[above] at (lineEnd) {Output space $\mathbb{R}$};


\end{tikzpicture}

%\end{document}

==> main_matter/chapters/FutureWork/text.tex <==
\section{Introduction}

\lettrine[lines=3]{T}{his} thesis has emphasized a theoretical understanding of the principles of Lipschitz continuity in neural networks. Building upon the foundations laid herein, we outline several promising directions for further exploration, including ongoing research currently in preparation as well as avenues for future investigation.


% \section{Lipschitz drift effect in quantization}

% An interesting direction for future investigation concerns what we term the \emph{Lipschitz drift effect} in quantized neural networks. Preliminary experiments in Figure~\ref{fig:lipschitzdrift:main} suggest that the distribution of the Lipschitz constants of weight matrices in large language models (LLMs) may undergo a substantial shift after quantization. Contrary to the expectation that quantization introduces only minor perturbations, the observed changes in the Lipschitz spectrum appear to be significant and systematic. In particular, two trends emerge consistently across model families such as LLaMA, Qwen, and DeepSeek: (1) the drift effect seems to be present in all examined LLMs, and (2) the magnitude of drift increases as the quantization bit-width decreases, with the Lipschitz constants shifting toward higher values. This phenomenon may help explain the degradation of generalization performance often observed in low-bit quantized models. A deeper theoretical and empirical understanding of this Lipschitz drift effect could offer valuable insight into the stability and generalization properties of quantized large-scale models.


% \begin{figure*}[!t]
%   \centering

%   \begin{minipage}[t]{0.46\textwidth}
%      \centering 
%      \subfloat[TinyLlama/TinyLlama-1.1B-Chat-v1.0]{
%       \includegraphics[width=1\linewidth]{plots/TinyLlama_TinyLlama_1_1B_Chat_v1_0_lipschitz_variation.pdf}  
%       %\label{fig:KL3D:magnitude}
%      }
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[t]{0.46\textwidth}
%      \centering 
%      \subfloat[Qwen/Qwen2.5-1.5B]{
%       \includegraphics[width=1\linewidth]{plots/Qwen_Qwen2_5_1_5B_lipschitz_variation.pdf}  
%       %\label{fig:KL3D:phase}
%      }
%   \end{minipage}

%   % \begin{minipage}[t]{1\textwidth}
%   %    \centering 
%   %    \subfloat[deepseek-coder-1.3b-instruct]{
%   %     \includegraphics[width=1\linewidth]{plots/deepseek_ai_deepseek_coder_1_3b_instruct_lipschitz_variation.pdf}  
%   %     %\label{fig:KL3D:magnitude}
%   %    }
%   % \end{minipage}%
  
  
%   \caption[Lipschitz Drift Effect in Quantization]{\textbf{Lipschitz Drift Effect in Quantization}. Distributions of Lipschitz constants across different quantization bit-widths for LLMs. Lower bit-widths cause the distributions to shift toward higher values, indicating increasing Lipschitz drift.}
  
%   \label{fig:lipschitzdrift:main}

% \end{figure*}


% \section{Dynamics in continual learning}


% \paragraph{Setting.} Let $\pi$ denote a large language model (LLM):
% \begin{align}
%     \pi(y_t \mid \boldsymbol{x}, \boldsymbol{y}_{<t}; \boldsymbol{\theta}): 
%     (\boldsymbol{x}, \boldsymbol{y}_{<t}, y_t, \boldsymbol{\theta}) \mapsto [0,1],
% \end{align}
% where $\boldsymbol{x}$ is the input sequence (\ie, the prompt), 
% $\boldsymbol{y}_{<t}$ denotes the sequence of previously generated tokens up to (but not including) time step $t$, 
% $y_t$ is the next predicted token, and $\boldsymbol{\theta}$ are the model parameters.

% We define $\pi_{\mathrm{ref}}$ as an LLM pre-trained on a reference dataset $\mathcal{D}_{\mathrm{ref}}$ with parameters $\boldsymbol{\theta}_{\mathrm{ref}}$. 
% Similarly, let $\pi_{\mathrm{new}}$ denote the same LLM that is further trained (continued pretraining or fine-tuning) on a new dataset $\mathcal{D}_{\mathrm{new}}$, 
% resulting in updated parameters $\boldsymbol{\theta}_{\mathrm{new}}$.

% \paragraph{Knowledge retention.} 
% At token level, the knowledge retention in the fine-tuned LLM $\pi_{\mathrm{new}}$ can be quantified by the token-level Kullback–Leibler (KL) divergence with respect to the reference model $\pi_{\mathrm{ref}}$:
% \begin{align}
%     \mathrm{KL}\!\left[\pi_{\mathrm{new}} \,\|\, \pi_{\mathrm{ref}}\right]
%     &= \mathbb{E}_{\boldsymbol{x} \sim \mathcal{D}_{\mathrm{ref}}} 
%     \, \mathbb{E}_{\boldsymbol{y}_{<t} \sim \pi_{\mathrm{ref}}} 
%     \left[ \sum_{y_t} 
%     \pi_{\mathrm{new}}(y_t \mid \boldsymbol{x}, \boldsymbol{y}_{<t}) 
%     \log \frac{\pi_{\mathrm{new}}(y_t \mid \boldsymbol{x}, \boldsymbol{y}_{<t}; \boldsymbol{\theta}_{\mathrm{new}})}
%               {\pi_{\mathrm{ref}}(y_t \mid \boldsymbol{x}, \boldsymbol{y}_{<t}; \boldsymbol{\theta}_{\mathrm{ref}})} \right].
% \end{align}

% Note that the dynamics of $\boldsymbol{\theta}_{\mathrm{new}}$ in optimization can be modeled as an It\^o process. Accordingly, the evolution of 
% \begin{align}
%     \mathrm{KL}\!\left[\pi_{\mathrm{new}} \,\|\, \pi_{\mathrm{ref}}\right]
% \end{align}
% represents an optimization-induced dynamics of knowledge retention. Understanding this dynamics may provide useful insights for the design of novel optimization algorithms. By constraining the optimization on a smoother Riemannian parameter submanifold --- \eg, the parameter manifold that preserve the norms, the optimization can lead to higher knowledge retention to reference model. 

% \begin{figure}[t]
%     \centering

%     \resizebox{0.8\linewidth}{!}{
%       \input{tikz/fpt_concept}
%     }

%     \caption[Fourier representation of real weight tensor]{\textbf{Fourier representation of real weight tensor}. The Fourier representation $\hat{\boldsymbol{\theta}}$ of a real weight tensor $\boldsymbol{\theta}$ consists of its \emph{magnitudes} $\rho(\boldsymbol{\theta})$ and \emph{phases} $\phi(\boldsymbol{\theta})$. The \emph{magnitudes} characterize the spectral energy; while the \emph{phases} characterize the correlations. Preserving spectral energy regularizes optimization by retaining pretrained capacity while adapting correlation structure.}
    
%     \label{fig:tensor_fourier_representation}
% \end{figure}

% We treat model parameters $\boldsymbol{\theta}$ as signals, which allows them to be represented in the Fourier domain, as illustrated in Figure~\ref{fig:tensor_fourier_representation}~\citep{luo2025fouriertuning}. Intuitively, since the parameters are modulated by phases through smooth $1$-Lipschitz \emph{sinusoidal} and \emph{cosinusoidal} functions, the resulting Fourier phase manifold is expected to be smooth and flat. Figure~\ref{fig:KL_landscape:main} further illustrates the KL landscape with respect to the Fourier magnitudes and phases of the parameters~\citep{luo2025fouriertuning}.



% \begin{figure*}[!t]
%   \centering

%   \begin{minipage}[t]{0.46\textwidth}
%      \centering 
%      \subfloat[Fourier magnitude]{
%       \includegraphics[width=1\linewidth]{plots/KL_landscape_fourier_magnitude_3D.pdf}  
%       %\label{fig:KL3D:magnitude}
%      }
%   \end{minipage}%
%   \hfill%
%   \begin{minipage}[t]{0.46\textwidth}
%      \centering 
%      \subfloat[Fourier phase]{
%       \includegraphics[width=1\linewidth]{plots/KL_landscape_fourier_phase_3D.pdf}  
%       %\label{fig:KL3D:phase}
%      }
%   \end{minipage}

%   \begin{minipage}[t]{0.46\textwidth}
%      \centering 
%      \subfloat[Fourier magnitude]{
%       \includegraphics[width=1\linewidth]{plots/KL_landscape_fourier_magnitude_contour.pdf}  
%       %\label{fig:KL3D:magnitude}
%      }
%   \end{minipage}%
%   \hfill%
%   \begin{minipage}[t]{0.46\textwidth}
%      \centering 
%      \subfloat[Fourier phase]{
%       \includegraphics[width=1\linewidth]{plots/KL_landscape_fourier_phase_contour.pdf}  
%       %\label{fig:KL3D:phase}
%      }
%   \end{minipage}
  
%   \caption[Fourier Phase Manifold Flatness Hypothesis]{\textbf{Fourier Phase Manifold Flatness Hypothesis}. Landscape of the Kullback--Leibler (KL) divergence of \emph{GPT2} in Fourier space. We first fine-tune the pre-trained \emph{GPT2} as the \textit{reference model} ($\pi_{\text{ref}}$) on the \emph{WikiText-2} dataset using the Adam optimizer with a learning rate of $5\times 10^{-4}$ for $50$ epochs. We then perturb the model parameters as the \textit{perturbed model} ($\pi_{\text{perturbed}}$) along two randomly chosen orthogonal directions (\ie, $\alpha$ and $\beta$) and evaluate the divergence between the perturbed model distribution and the fine-tuned reference model, measured as $\mathrm{KL}\!\left[\pi_{\text{perturbed}} \,\|\, \pi_{\text{ref}}\right]$. The visualizations show that the geometry of the phase landscape exhibits a smoother and flatter basin, in contrast to the sharper curvature observed in the magnitude landscape.}
  
%   \label{fig:KL_landscape:main}

% \end{figure*}


% This is particular useful for continual instruction tuning in LLMs for provably preserving knowledge. A work under manuscript preparation by the thesis author is:
% \begin{enumerate}
%     \item \fullcite{luo2025fouriertuning}.
% \end{enumerate}




% \section{Dynamics of modulated sparsity}
% \paragraph{Setting.} Let $f(x; \boldsymbol{\theta})$ be a neural network parameterized 



\section{Spectral-gap regularization}
A linear unit, parameterized by $\boldsymbol{\theta}$, \ie, a fully connected layer or convolutional operation, represents an input $z$ into $\rank(\boldsymbol{\theta})$ orthogonal subspaces:
\begin{align}
    \boldsymbol{\theta} z 
    = \sum_{i=1}^{\rank(\boldsymbol{\theta})} \sigma_i\, u_i v_i^\top,
\end{align}
where $\sigma_i$, $u_i$, and $v_i$ denote the $i$-th singular value, left-singular vector, and right-singular vector, respectively. The \emph{spectral gap} between $\sigma_i$ and $\sigma_j$ is defined as:
\begin{align}
    \big| \sigma_i - \sigma_j \big|.
\end{align}

One theoretical insight gained from Chapters~\ref{chapter:perturbation_analysis}--\ref{chapter:optimization_induced_dynamics} is that smaller spectral gaps amplify the influence of stochastic noise. This observation motivates the introduction of a regularization term:
\begin{align}
    \big| \sigma_{\mathrm{max}} - \sigma_{\mathrm{min}} \big|,
\end{align}
which has the following effects:
\begin{itemize}
    \item a \textbf{smaller gap} encourages whitening of the subspaces by distributing features more evenly across all subspaces. This helps mitigate overfitting to dominant features and promotes fair feature learning;
    
    \item a \textbf{larger gap} may improve training stability but can also increase the Lipschitz constant, potentially reducing robustness.
\end{itemize}

\section{Spectrum-gradient alignment}

The stochastic dynamics of Lipschitz continuity, as presented in Chapter~\ref{chapter:optimization_induced_dynamics}, reveal that the alignment between the gradient of the loss with respect to parameters and the principal direction of the parameter matrix governs the deterministic component in the evolution of the Lipschitz constant. Specifically, this alignment is captured by:
\begin{align}
    \mu^{(\ell)}(t) = \frac{1}{\sigma_{1}^{(\ell)}(t)} \left\langle \boldsymbol{J}_{op}^{(\ell)}(t), \, -\mathrm{vec}\left[ \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t)) \right] \right\rangle,
\end{align}
where $\sigma_1^{(\ell)}(t)$ is the largest singular value and $\boldsymbol{J}_{op}^{(\ell)}(t)$ denotes the principal direction of the parameter matrix at layer $\ell$ and time $t$.

Motivated by this insight, we propose a regularization term that explicitly controls this alignment through:
\begin{align}
    \left| \left\langle \boldsymbol{J}_{op}^{(\ell)}(t), \, -\mathrm{vec}\left[ \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t)) \right] \right\rangle \right|,
\end{align}
which has the following implications:
\begin{itemize}
    \item a \textbf{higher alignment} promotes an increase in the Lipschitz constant during training, thereby reducing robustness;
    
    \item a \textbf{lower alignment} suppresses the growth of the Lipschitz constant, leading to improved robustness.
\end{itemize}



\section{Conclusions}


This chapter has outlined several promising avenues for future research inspired by the theoretical and empirical findings of this thesis. In continual learning, a deeper understanding of the dynamics of pretraining knowledge retention in LLMs may guide the development of novel optimization methods. In spectral analysis, regularization based on spectral-gaps and spectrum–gradient alignment offers a principled approach for improving both robustness and generalization.

==> main_matter/chapters/FutureWork/tikz/fpt_concept.tex <==
% \documentclass[tikz,border=6pt]{standalone}
% \usepackage{amsmath,mathrsfs}
% \usetikzlibrary{positioning,arrows.meta}


% \begin{document}

\begin{tikzpicture}[>=Stealth, node distance=2cm and 1.5cm]

\newcommand{\phasornode}[7]{%
  \pgfmathsetmacro{\R}{#7} % circle radius
  \pgfmathsetmacro{\A}{#3} % angle in degrees

  % put a coordinate (O) and use it for baseline inside the tikzpicture
  \node[#2, inner sep=0pt, anchor=center] (#1) {%
    \begin{tikzpicture}[scale=1, baseline={(O)}]
      \coordinate (O) at (0,0);

      % proportional axes
      \draw[->,thin] (-1.3*\R,0) -- (1.3*\R,0) node[right,xshift=2mm] {$i$};
      \draw[->,thin] (0,-1.3*\R) -- (0,1.3*\R) node[above,yshift=2mm] {$j$};

      % circle
      \draw[dashed] (O) circle (\R);

      % phasor vector
      \draw[thick,->,blue] (O) -- ({\R*cos(\A)},{\R*sin(\A)})
        node[pos=1.2] {$#4$};

      % angle arc + annotation
      \draw[thick,red] (0.45*\R,0) arc[start angle=0,end angle=\A,radius=0.45*\R];
      \node at ({0.8*\R*cos(\A/2)},{0.8*\R*sin(\A/2)}) {$#5$};
    \end{tikzpicture}%
  };
  % caption under the phasor
  \node[below=1mm of #1] {$#6$};
}

\node (lhs) {$\hat{\boldsymbol{\theta}}=\mathscr{F}[\boldsymbol{\theta}]=
\begin{bmatrix}
\hat{\boldsymbol{\theta}}_1\\
\vdots\\
\hat{\boldsymbol{\theta}}_d
\end{bmatrix}=$};


\node[right=-0.1cm of lhs] (e1) {$
\begin{bmatrix}
1\\
\vdots\\
0
\end{bmatrix}$};

\node[right=2mm of e1] (times1) {$\times$};

\phasornode{p1}{right=1.5cm of times1,yshift=2.2mm}{60}{\rho_1}{\phi_1}{\hat{\boldsymbol{\theta}}_1=\rho_1 e^{j\phi_1}}{0.8}

\node[right=5mm of p1,yshift=-2mm] (plus) {$+ ~\cdots~ + $};

\node[right=0.15cm of plus] (e2) {$\begin{bmatrix}
0\\
\vdots\\
1\end{bmatrix}$};

\node[right=2mm of e2] (times2) {$\times$};

\phasornode{p2}{right=1.5cm of times2,yshift=2.2mm}{130}{\rho_d}{\phi_d}{\hat{\boldsymbol{\theta}}_d=\rho_d e^{j\phi_d}}{1.}

\end{tikzpicture}

% \end{document}

==> main_matter/chapters/GlobalRobustness/text.tex <==
%\vspace{2em}
\section{Introduction}

\lettrine[lines=3]{I}{mage} modeling with deep neural networks has achieved great success \citep{li2021survey}. Yet, deep neural networks are known to be vulnerable to perturbations. For example, the perturbations may arise from corruptions and adversarial attacks \citep{goodfellow2014explaining,hendrycks2019benchmarking,szegedy2014intriguing}, \etc. Perturbation robustness, henceforth referred to as robustness, characterizes a crucial intrinsic property of models \citep{hendrycks2019benchmarking,bai2021recent,goodfellow2014explaining}. 



Robustness mechanisms refer to the mechanisms which lead to robustness in models. The study of robustness mechanisms aims to answer the question `\textbf{why some models are more robust than others}' \citep{bereska2024mechanistic}. The causes within this question can arise from multifarious aspects, including architecture designs \citep{zhou2022understanding}, data annotations, training methods \citep{pang2020bag}, inferences, etc. For example, noisy labels can arise from data annotations \citep{frenay2013classification,natarajan2013learning}; adversarial attacks often take place in inferences. This research provides a unified view regarding the mechanisms of image model robustness on spectra. We only focus on global interpretation of robustness mechanisms of image models by examining the robustness globally on an entire dataset. Our method is primarily motivated by two key aspects, as detailed below.

Despite the substantial advances in previous global interpretability works \citep{covert2020understanding,kolek2022cartoon}, in tandem with the wide adoption of empirical robustness benchmarks \citep{hendrycks2019benchmarking}, these methods are not designed to provide global interpretations regarding model robustness. For example, SAGE \citep{covert2020understanding}, a global interpretability work, can attribute the decisive pixel features in model's decision-makings. Yet, the importance of decisive pixel features fails to interpret the global robustness. Although the robustness of image models can be quantified by mean corruption errors (mCE) \citep{hendrycks2019benchmarking} or the distances in feature spaces between clean and perturbed image pairs \citep{zheng2016improving}, these scalar metrics often fall short in interpreting the underlying `why' question. This gap prompts us to provide global mechanistic interpretations of perturbation robustness.




\begin{figure}[tp!]
 

    \centering
         
    \includegraphics[width=1\textwidth,]{plots/standalone_spectrum_and_robustness_narrow_v2.pdf}
    
    \caption[Power-Law-Like Energy Spectral Density Distribution of Natural Images Over Frequency]{Power-law-like energy spectral density (ESD) distribution of natural images over the frequency. The signal spectrum is divided into $M$ bands (from $\mathcal{I}_0$ to $\mathcal{I}_{M-1}$). Each spectral band is a robustness band.} 

  
    \label{fig:robust_features_vs_non_robust_features}
\end{figure} 

Motivation also arises from the robustness characterization of the spectral signals within natural images. Images can be represented as spectral signals \citep{korner2022fourier}. The signal-to-noise ratios (SNR) of spectral signals can be used to characterize the signal robustness with respect to perturbations. Our later empirical study, as illustrated in Figure~\ref{fig:snr_char}, suggests that the spectral SNRs of perturbed natural images decay over the frequency with a power-law-like distribution. We refer to the \textit{spectral SNR} as the ratio of the point-wise energy spectral density (ESD) \citep{stoica2005spectral} of spectral signal to noise (\ie~perturbation): 
\begin{align}
 SNR(r) := \frac{ESD_r(x)}{ESD_r(\Delta x)}
\end{align}
where $r$ is a radial frequency point, $x$ is an image, $\Delta x$ is the perturbation, $ESD_r(\cdot)$ gives the point-wise energy density at $r$. The $ESD_r(\cdot)$ is defined as:
\begin{align}
    ESD_r(x):= \frac{1}{|L_r|} \cdot \sum\limits_{(u,v) \in L_r} |\mathscr{F}(x)(u,v)|^2
\end{align}
where $L_r$ denotes a circle as illustrated in Figure~\ref{fig:robust_features_vs_non_robust_features}, $|L_r|$ denotes the circumference of $L_r$, and $\mathscr{F}(x)$ denotes the 2D Discrete Fourier Transform (DFT) of $x$. Readers can further refer to more details in Appendix~\ref{app:image_ssnr}. 






Why do the spectral SNRs of some corruptions and adversarial attacks exhibit a power-law-like decay over the frequency?  We surmise that the ESDs of many perturbations are often not power-law-like, while the ESDs of natural images are power-law-like empirically, as shown in Figure~\ref{fig:robust_features_vs_non_robust_features}. For example, the spatial perturbation drawn from $\mathcal{N}(0, \sigma^2)$ (\ie~white noise) has a constant ESD: $ESD_r(\Delta x) = \sigma^2$. In Figure~\ref{fig:snr_char}, we characterize the spectral SNR distributions of perturbed images. We set the energy of perturbations to $10\%$ of the energy of the clean image for a fair comparison. The perturbation sources include corruptions \citep{hendrycks2019benchmarking} and adversarial attacks \citep{szegedy2014intriguing,tsipras2018robustness}. We notice that the SNR distributions are also power-law-like over the frequency. We refer to \textit{spectral signals} as \textit{spectral features} or simply as \textit{features} if without ambiguity. This power-law-like SNR decay suggests an empirical feature robustness prior: \textbf{Low-frequency features are robust features (RFs) while high-frequency features are non-robust features (NRFs)}. The experiments in Figure~\ref{fig:freq_role} demonstrate that models trained with low-frequency signals exhibit higher robustness compared to the models trained with high-frequency signals. This also echoes with our earlier claim ``low-frequency signals are generally more robust than high-frequency signals --- yet high classification accuracy can not be achieved by low-frequency signals alone''.





\textbf{Contributions}. By applying the Shapley value theory framework \citep{roth1988shapley}, we are able to assess the predictive powers of RFs and NRFs. Further leveraging a specifically designed characteristic function of the Shapley value theory framework, the predictive powers are assessed on the basis of their information gains. \textbf{I-ASIDE} uses information theory within the Shapley value theory framework, for interpreting robustness mechanisms, as detailed in Section~\ref{sec:decomp}. We claim our major contributions as:
\begin{itemize}
    \item We propose a model-agnostic, global interpretability method, for interpreting robustness mechanisms of image models, through the lens of the predictive powers of robust features and non-robust features;

     \item We analyze the robustness mechanisms of image models within information theory on spectra;

     \item We showcase a case study that \textbf{I-ASIDE}~has the potential to interpret how supervision noise levels affect model robustness. 
    
\end{itemize}
%We also make our code as open source for the research community to further investigate the topics in robustness. 







\begin{figure}[t!]
 
    %\vspace{-2em} 

    \centering
    
    % \setlength{\abovecaptionskip}{-2em}
    % \setlength{\belowcaptionskip}{-15pt}
  
    %\resizebox{0.9\columnwidth}{!}{
        
        %\includestandalone[width=1\textwidth]{standalone_pdfs/standalone_spectrum_and_robustness_narrow.tex}

        %\includestandalone[width=1\textwidth]{standalone_pdfs/standalone_spectrum_and_robustness_narrow_v2.tex}

         %% Answer: [trim=left bottom right top,clip]

        %\includegraphics[trim=0 0 0 1.1cm, width=0.75\textwidth, clip]{figures/snr_characterization.pdf}
    %}

    \begin{tikzpicture}
    \node[inner sep=0pt, opacity=1] (img) at (0in, 0in){\includegraphics[trim=0 0 0 1.1cm, width=6.in, clip]{plots/snr_characterization.pdf}};

    \draw[->,draw=cyan,line width=0.5mm] (-1.3in, 0.5in) -- (-1.9in,0) node[scale=0.8, midway,xshift=0.4in,yshift=0.38in] {RFs (Higher SNR)}; 

    \draw[->,draw=cyan,line width=0.5mm] (1.5in, -0.4in) -- (1.9in, -0.9in) node[scale=0.8, midway,xshift=-0.2in,yshift=0.38in] {NRFs (Lower SNR)}; 

     \draw[->,draw=red,line width=0.5mm] (-0.8in, -0.2in) -- (-1in, -0.6in) node[scale=0.8, midway,xshift=0.1in,yshift=0.38in] {Perturbations begin to overwhelm NRFs}; 
    
    \end{tikzpicture}

 
    
    \caption[Spectral Signal-to-Noise (SNR) Characterization with respect to Corruptions and Adversarial Attacks]{Spectral SNR characterization with respect to multiple corruptions and adversarial attacks. The corruptions include: white noise, Poisson noise, Salt-and-pepper noise, and Gaussian blur. The adversarial attacks include: FGSM \citep{goodfellow2014explaining}, PGD \citep{madry2018towards}, SparseFool \citep{modas2019sparsefool} and Pixel \citep{pomponi2022pixle}. We set the perturbation energy to $10\%$ of the energy of the reference image. The results are shown in decibels (dB) for better visualization. The dB below zero indicates that the perturbations overwhelm the spectral features.} 


    %\vspace{-1.5em}
  
    \label{fig:snr_char}
\end{figure} 







 

\begin{figure*}[t]
\begin{minipage}{\textwidth}
  \begin{minipage}{0.6\textwidth}
    \centering
\includegraphics[width=1\textwidth]{plots/standalone_freq_role.pdf}
  
    \label{fig:freq_role}
  \end{minipage}\hfill
  \begin{minipage}{0.4\textwidth}
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}[t]{c|c|c|c}
        \hline
        &\multicolumn{3}{c}{training frequency range} \\
        \cline{2-4}
        & \begin{tabular}{@{}c@{}} full-freq \\ $[0,1]$ \end{tabular} & \cellcolor{cyan!30}\begin{tabular}{@{}c@{}} low-freq \\ $[0,0.3]$ \end{tabular} & \begin{tabular}{@{}c@{}} high-freq \\ $[0.3,1]$ \end{tabular} \\ \hline
        train acc. & $98.05\%$ & \cellcolor{cyan!30}$\textbf{97.13}\%$& $96.18\%$ \\
        \hline
        \begin{tabular}{@{}c@{}} val. acc. w/ clean\\ generalization gap \end{tabular}  & \begin{tabular}{@{}c@{}} $96.10\%$\\ \textcolor{black}{$-1.95~\downarrow$} \end{tabular} & \cellcolor{cyan!30}\begin{tabular}{@{}c@{}} $\textbf{98.80}\%$\\ \textcolor{red}{$+1.67~\uparrow$} \end{tabular} & \begin{tabular}{@{}c@{}} $56.70\%$\\ \textcolor{black}{$-39.48~\downarrow$} \end{tabular} \\
        \hline
        \begin{tabular}{@{}c@{}} val. acc. w/ Gaussian\\generalization gap \end{tabular}   & \begin{tabular}{@{}c@{}} $92.60\%$\\ \textcolor{black}{$-5.45~\downarrow$} \end{tabular} & \cellcolor{cyan!30}\begin{tabular}{@{}c@{}} $\textbf{98.00}\%$\\ \textcolor{red}{$+0.87~\uparrow$} \end{tabular} & \begin{tabular}{@{}c@{}} $26.70\%$\\ \textcolor{black}{$-69.48~\downarrow$} \end{tabular} \\
        \hline
      \end{tabular}
      }%resizebox.
      %\captionof{table}{A table beside a figure}
    \end{minipage}
  \end{minipage}



   \caption[Frequency Signals Shape Robustness in Training]{Understanding the role of spectral signals. We train a \textit{resnet18} on three datasets derived from \textit{STL10} \citep{coates2011analysis}: $[0,1]$ contains full-frequency signals; $[0, 0.3]$ only contains low-frequency signals with a cut-off frequency by $0.3$; and $[0.3, 1]$ only contains the high-frequency signal with a cut-off frequency by $0.3$. In the derived datasets, the filtered high or low frequency signals are randomly replaced by the high or low frequency signals sampled from the full-frequency train set. We visualize the embeddings in the left figure with respect to clean samples and perturbed samples with Gaussian noise ($\sigma=0.1$). The samples are from the validation set. The accuracy on both the train and validation sets is provided in the right table. We also provide generalization gaps, measured by the differences between validation accuracy and train accuracy (\ie~$\mathrm{acc}_{val} - \mathrm{acc}_{train}$). We have noted in that: (1) both high-frequency and low-frequency signals contain sufficient discriminative information to achieve high training accuracy; (2) high-frequency signals alone are not robust signals because they fail to generalize well from train to validation; (3) overall, low-frequency signals are more robust signals because models trained alone with them generalize better and exhibit higher robustness. We summarize these empirical observations into Assumption~\ref{assump:robustness_prior}.}

%   %\vspace{-1em} 
 
 \label{fig:freq_role}

\end{figure*}






\section{Notations}
\label{sec:notations}

\textbf{Image classifier}. The primary task of an image classifier is to predict the probability distributions over discrete classes for given images. We use $Q(y|x; \theta): (x, y) \mapsto [0, 1]$ to denote a classifier in the form of conditional probability. The $Q$ predicts the probability that an image $x$ is of class $y$. The $\theta$ are the parameters. For brevity, we ignore the parameter $\theta$. For example, we denote $Q(y|x; \theta)$ as $Q(y|x)$.


\textbf{Dataset and annotation}. We use a tuple $\langle \mathcal{X}, \mathcal{Y} \rangle$ to denote an image classification dataset, where $\mathcal{X}$ is the image set and $\mathcal{Y}$ is the label set. We use $|\mathcal{Y}|$ to denote the number of classes (\ie~the cardinality of set $\mathcal{Y}$). The annotation task of image classification datasets is to assign each image with a discrete class probability distribution. We use $P(y|x)$ to denote the ground-truth probability that an image $x$ is assigned as a class $y$. We use $P(x)$ to denote the probability of $x$ in set $\mathcal{X}$. We use $P(y)$ to denote the probability of $y$ in set $\mathcal{Y}$. In class-balanced datasets, $P(y)=\frac{1}{|\mathcal{Y}|}$. %The annotations are often referred as supervision signals in the literature \citep{sucholutsky2023informativeness,zhang2020distilling}. 




\section{Method}
\label{sec:decomp}



\textbf{High-level overview}. We apply Shapley value theory for axiomatically assigning credits to spectral bands. Within this framework, the specially devised characteristic function measures the information gains of spectral bands. \textbf{I-ASIDE} interprets robustness mechanisms using this axiomatic framework with the information theory.

\textbf{Problem formulation}.
Quantifying the predictive powers of features can be viewed as a \textit{value} decomposition problem. In this research, the \textit{value} is the information quantity that a features contribute to decisions. Specifically, the \textit{value} is in the form of the log-likelihood expectation of predictions (\ie~the negative cross-entropy loss). The \textit{value} decomposition aims to assign each robustness band a predictive power such that: (1) The sums of the predictive powers are equal to the \textit{value}, and (2) the assigned predictive powers should reflect their importance in the decisions. In the coalitional game theory, this decomposition scheme is known as an \textit{axiomatic fairness division problem} \citep{roth1988shapley,klamler2010fair}. The fairness division must satisfy four axioms: \textit{efficiency}, \textit{symmetry}, \textit{linearity} and \textit{dummy player} \citep{roth1988shapley}. We refer to the \textit{axiomatic fairness division} as \textit{axiomatic decomposition}. Of the scheme, the axioms guarantee \textit{uniqueness} and \textit{fairness} \citep{aumann1985game,aumann2015efficiency,roth1988shapley}. The property \textit{fairness} refers to the principle `\textit{equal treatment of equals}' \citep{navarro2019necessary}. Shapley value theory is the unique solution satisfying the above axioms. However, the theory merely provides an abstract framework. To employ, we have to instantiate two abstracts: (1) players and coalitions, and (2) characteristic function. 

\textbf{Abstract (1): players and coalitions}. The spectral bands are dubbed as \textit{spectral players}. A subset of the spectral player set is dubbed as a \textit{spectral coalition}. The details are as shown in Section~\ref{sec:spectral_coalition_game}. The $M$ spectral players can forge $2^M$ spectral coalitions. We represent the presences and absences of the spectral players as the pass-bands and stop-bands in a multi-band-pass digital signal filter \citep{oppenheim1978applications}, as shown in Section~\ref{sec:coalition_filtering}.

\textbf{Abstract (2): characteristic function}. The characteristic function is designed to measure the contributions that the coalitions contribute in decisions. The contributions of the $2^M$ coalitions are then combined to compute their marginal contributions in decisions. We specially design the characteristic function, as shown in Section~\ref{sec:char_func_design} and Appendix~\ref{app:theo_char_func}, to measure the information gains. Figure~\ref{fig:design} shows the framework 
of applying the Shapley value theory. Figure~\ref{fig:dsp} shows the block diagram of the spectral coalition filtering. Figure~\ref{fig:coalitions_example} shows an example of $2^M$ spectral coalitions. 




We organize the implementation details of instantiating the aforementioned two abstracts from three aspects: (1) formulating a spectral coalitional game, (2) the implementation of spectral coalitions and (3) the design of the characteristic function.





\begin{figure}[t!]
 
  %\vspace{-16pt} 

  \centering
  % \setlength{\abovecaptionskip}{5pt}
  % \setlength{\belowcaptionskip}{-15pt}
  
        
    %\includegraphics[width=0.7\textwidth]{figures/design_standalone.pdf} 

    %\includestandalone[width=1\textwidth]{standalone_pdfs/standalone_design_succinct.tex}

    %\includegraphics[width=1\textwidth,]{standalone_pdfs/pdf_outputs/standalone_design_succinct_v8.pdf}

     \includegraphics[width=1\textwidth,]{plots/standalone_design.pdf}
    
    %\includegraphics[width=0.8\textwidth]{figures/evaluation_projection-imagenet.pdf}
        %\caption{This diagram illustrates the overview of \textbf{I-ASIDE} and shows how the spectral importance distributions are derived through the \textbf{ASIDE} equation.} 

    \caption[Framework of Applying Shapley Value Theory]{Framework of applying Shapley value theory. Spectral coalition filtering creates spectral coalitions over $\mathcal{X}$. Each coalition contains a unique combination of spectral signals, in which some spectral bands are present and others are absent. The coalitions are fed into a classifier $Q$. For each coalition, $Q$ outputs the predictions. The characteristic function $v$ then uses the predictions to estimate the contributions of the features present in the coalitions. The results from $v$ are combined to compute the marginal contributions of spectral bands --- \ie~the spectral importance distribution of $Q$.
   } 
   
    %\vspace{-1.5em}
  
    \label{fig:design}

\end{figure}


\subsection{Spectral coalitional game}
\label{sec:spectral_coalition_game}



\textbf{Spectral player}. We use $\mathcal{I}_i$ (where $i \in [M] := \{0,1,\cdots,M-1\}$) to denote the $i$-th spectral player. The $\mathcal{I}_0$ contains the most robust features and the $\mathcal{I}_{M-1}$ contains the most non-robust features. The $M$ spectral players constitute a player set $\mathcal{I} :=\{\mathcal{I}_i\}_{i=0}^{M-1}$. Figure~\ref{fig:linfty_vs_l2_ball} in Appendix~\ref{app:linfty_vs_l2_ball} shows two partition schemes to partition spectral bands ($\ell_{\infty}$ and $\ell_{2}$). We empirically choose $\ell_{\infty}$.



\textbf{Spectral coalition}. A subset $\widetilde{\mathcal{I}} \subseteq \mathcal{I}$ is referred to as the \textit{spectral coalition}. The player set $\mathcal{I}$ is often referred to as the \textit{grand coalition}.

\textbf{Characteristic function}. A characteristic function $v(\widetilde{\mathcal{I}}): \widetilde{\mathcal{I}} \mapsto \mathbb{R}$ measures the contribution for a given coalition and satisfies $v(\emptyset) = 0$. In this research, the contribution of $\widetilde{\mathcal{I}}$ is measured in the form of the log-likelihood expectation of the predictions by the $Q$, in which the input images only contain the signals present in the $\widetilde{\mathcal{I}}$. We show that this design of $v$ theoretically measures how much information the $Q$ uses from the features in the $\widetilde{\mathcal{I}}$ for decisions.




\textbf{Shapley value}. A spectral coalitional game $(\mathcal{I}, v)$ is defined on a spectral player set $\mathcal{I}$ equipped with a characteristic function $v$. The weighted marginal contribution of a spectral player $\mathcal{I}_{i}$ over all possible coalitions is referred to as the Shapley value of the spectral player $\mathcal{I}_{i}$. We use $\psi_{i}(\mathcal{I}, v)$ to represent the Shapley value of the player $\mathcal{I}_i$. The Shapley value $\psi_i(\mathcal{I},v)$ is uniquely given by:
\begin{align}
\label{equ:shapley_value}
    \psi_i(\mathcal{I},v)= \sum\limits_{\Tilde{\mathcal{I}} \subseteq \mathcal{I} \setminus \mathcal{I}_i} \frac{1}{M}\binom{M - 1}{|\Tilde{\mathcal{I}}|}^{-1}
    \left\{ v(\Tilde{\mathcal{I}} \cup \{\mathcal{I}_i\}) -v(\Tilde{\mathcal{I}}) \right\}
\end{align}
where $\frac{1}{M}\binom{M - 1}{|\Tilde{\mathcal{I}}|}^{-1}$ gives the weight of the player $\mathcal{I}_i$ presenting in the coalition $\Tilde{\mathcal{I}}$.



\textbf{Spectral importance distribution (SID)}. We use $\Psi(v) := \left(\psi_i\right)_{i \in [M]} \in \mathbb{R}^M$ to denote the collection of $\psi_i(\mathcal{I}, v)$ over all players. We min-max normalize $\Psi(v)$ by taking $\bar\Psi(v)=\frac{\Psi(v) - \min{\Psi(v)}}{||\Psi(v) - \min{\Psi(v)}||_1}$. The reason for normalizing the SIDs is that we want to scalarize the SIDs for numerical comparisons. The $\bar\Psi(v)$ is referred to as \textit{spectral importance distribution}. Figure~\ref{fig:spectral_importance_distributions} shows examples of the spectral importance distributions of trained and un-trained models. 

\textbf{Spectral robustness score (SRS)}. We can also summarize spectral importance distributions into scalar values. We refer to the summarized scalar values as \textit{spectral robustness scores}. We use $S(v): v \mapsto [0,1]$ to denote the summarizing function.












\subsection{Spectral coalition filtering}
\label{sec:coalition_filtering}

We represent the \textit{presences} and \textit{absences} of the spectral players through the signal \textit{pass-bands} and \textit{stop-bands} using a multi-band-pass digital signal filtering \citep{oppenheim1978applications}, as shown in Figure~\ref{fig:dsp}. For example, the example spectral coalition $\{\mathcal{I}_0, \mathcal{I}_2\}$ signifies the signals present only in $\mathcal{I}_0$ and $\mathcal{I}_2$. With the spectral coalition filtering, we are able to evaluate the contributions of the combinations of various spectral features. Figure~\ref{fig:coalitions_example} shows an example of $2^M$ spectral coalitions.


\begin{figure}[t!]
 
  %\vspace{-16pt} 

  \centering
  % \setlength{\abovecaptionskip}{5pt}
  % \setlength{\belowcaptionskip}{-15pt}
  
        
    %\includegraphics[width=0.7\textwidth]{figures/design_standalone.pdf} 

    %\includestandalone[width=1\textwidth]{standalone_pdfs/standalone_design_succinct.tex}

    \includegraphics[width=1\textwidth,]{plots/standalone_dsp.pdf}

    
    %\includegraphics[width=0.8\textwidth]{figures/evaluation_projection-imagenet.pdf}
        %\caption{This diagram illustrates the overview of \textbf{I-ASIDE} and shows how the spectral importance distributions are derived through the \textbf{ASIDE} equation.} 

    \caption[Implementation Scheme of Spectral Coalition Filtering in Spectral Game]{Spectral coalition filtering. In this example, the mask map $\mathbb{T}(\widetilde{\mathcal{I}})$ (\ie~transfer
function) only allows to pass the signals present in the spectral coalition $\{\mathcal{I}_0, \mathcal{I}_2\}$. The $M$ is $4$ and the absences are assigned to zeros. The images after spectral coalition filtering ($x \bowtie \widetilde{I}$) are then fed into frozen classifiers to assess the contributions of spectral coalitions. The binary operation notation $\bowtie$ denotes coalition filtering given by Definition~\ref{def:spectral_coalition_filtering}. The notation $\odot$ denotes Hadamard product.}
 
    \vspace{-1.em}
  
    \label{fig:dsp}

\end{figure}




To implement the presences and absences of spectral signals, we define a mask map $\mathbb{T}(\widetilde{\mathcal{I}}): \widetilde{\mathcal{I}} \mapsto \{0, 1\}^{M \times N}$ on 2D spectrum, where $\widetilde{\mathcal{I}}$ is a spectral coalition and $M \times N$ denotes 2D image dimensions. The mask map is point-wisely defined as:
\begin{align}
    \label{equ:combfilter_transform_function}
    \mathbb{T}(\widetilde{\mathcal{I}})(m,n) =
    \begin{cases}
       1, & \text{if the frequency point}~$(m,n)$~\text{is present in coalition}~\widetilde{\mathcal{I}}, \\
       0, & \text{otherwise}
     \end{cases}
\end{align}
where $(m,n) \in [M] \times [N]$. In the digital signal processing literature, this mask map is known as a \textit{transfer function} \citep{oppenheim1978applications}. In the 2D mask map, the frequency points are `1' in pass-bands (presences) and `0' in stop-bands (absences). The process of spectral coalition filtering with the mask map for a given spectral coalition $\widetilde{\mathcal{I}}$ is shown as in Figure~\ref{fig:dsp}. 







We apply the transfer function $\mathbb{T}(\widetilde{\mathcal{I}})$ on the spectra of images with element-wise product (\ie~Hadamard product \citep{horn1990hadamard}). Let $\mathscr{F}$ be the Discrete Fourier transform (DFT) operator and $\mathscr{F}^{-1}$ be the inverse DFT (IDFT) operator \citep{oppenheim1978applications}. Readers can further refer to Appendix~\ref{app:image_ssnr}. 


\begin{definition}[Spectral coalition filtering]
We define a binary operator `$\bowtie$' to represent the signal filtering by:
\begin{align}
    %\vspace{1em}
    \label{equ:feature_filtering_operator}
    %\widetilde{x}_{\widetilde{\mathcal{I}}} =
    x \bowtie \widetilde{\mathcal{I}} 
    := %\stackrel{def}{=} 
    \mathscr{F}^{-1}\left[ \underbrace{ \mathscr{F}(x) \odot \mathbb{T}(\widetilde{\mathcal{I}})}_{\mathrm{Spectral~presence}} + \underbrace{\vb*b \odot (\mathbb{1} - \mathbb{T}(\widetilde{\mathcal{I}}))}_{\mathrm{Spectral~absence}} \right ] 
\end{align}
where `$\odot$' denotes Hadamard product (\ie~element-wise product), $\mathbb{1} \in \mathbb{R}^{M \times N}$ denotes an all-ones matrix and $\vb*b \in \mathbb{C}^{M \times N}$ represents the assignments of the absences of spectral players. In the context of attribution analysis, $\vb*b$ is often referred as the baseline. In our implementation, we empirically set $\vb*b = \vb*0$.  
\label{def:spectral_coalition_filtering}
\end{definition}


\begin{remark}[Absence baseline]



Formally, in the context of attribution analysis, the term `baseline' defines the absence assignments of players \citep{sundararajan2017axiomatic,shrikumar2017learning,binder2016layer}. For example, if we use `zeros' to represent the absence of players, the `zeros' are dubbed as the `baseline' in the attribution analysis. We have discussed multiple baselines in Appendix~\ref{app:absence_assignment}. % and the results are shown in Figure~\ref{fig:maskout_examples}.
\end{remark}



\begin{definition}[Spectral coalition filtering over set]
Accordingly, we define the filtering over a set $\mathcal{X}$ as:
\begin{align}
    \mathcal{X} \bowtie \widetilde{\mathcal{I}} := %\stackrel{def}{=} 
    \{x \bowtie \widetilde{\mathcal{I}} | x \in \mathcal{X}\}.
\end{align}    
\end{definition}





\begin{figure}[!t]
 
  %\vspace{-16pt} 

  \centering
  % \setlength{\abovecaptionskip}{5pt}
  % \setlength{\belowcaptionskip}{-15pt}
  
        
    %\includegraphics[width=0.7\textwidth]{figures/design_standalone.pdf} 

    %\includestandalone[width=1\textwidth]{standalone_pdfs/standalone_design_succinct.tex}

    %\includegraphics[width=1\textwidth,]{figures/coalitions_example.pdf}

    \resizebox{\linewidth}{!}{
    \begin{tikzpicture}
    \node[inner sep=0pt, opacity=1] (img) at (0in, 0in){\includegraphics[width=6.5in,]{plots/coalitions_example.pdf}};

    \def\dx{0.81in}
    \def\x{-3.05in}

    \foreach \i/\b in {0/0000, 1/0001,
                  2/0010, 3/0011,
                  4/0100, 5/0101,
                  6/0110, 7/0111}{
        \node [ scale=1, 
            %text width=1.5in, 
            rotate=0, 
            yshift=0in, 
            xshift=0in, 
            white, 
            align=left] at (\x + \i * \dx, 0.7in) (label) {$\b$};
    }

\foreach \i/\b in {0/1000, 1/1001,
                  2/1010, 3/1011,
                  4/1100, 5/1101,
                  6/1110, 7/1111}{
    \node [ scale=1, 
            %text width=1.5in, 
            rotate=0, 
            yshift=0in, 
            xshift=0in, 
            white, 
            align=left] at (\x + \i * \dx, -0.1in) (label) {$\b$};
    }
    
    \end{tikzpicture}
    }%resizebox
    
    %\includegraphics[width=0.8\textwidth]{figures/evaluation_projection-imagenet.pdf}
        %\caption{This diagram illustrates the overview of \textbf{I-ASIDE} and shows how the spectral importance distributions are derived through the \textbf{ASIDE} equation.} 

    \caption[Examples of Spectral Coalitions]{An example of a complete $2^M$ spectral coalitions. This example shows $16$ spectral coalitions with $M=4$. Each coalition provides various information relevant to decisions. Each image is a coalition. Each coalition contains a unique spectral signal combination. We use binary code to index these coalitions. The `1' in the $i$-th position indicates the presence of the $i$-th player. For example, $1001$ indicates the presences of two spectral players ($\mathcal{I}_0$ and $\mathcal{I}_3$) in the coalition.
    }
 
    %\vspace{-1.5em}
  
    \label{fig:coalitions_example}

\end{figure}










\subsection{Characteristic function design}
\label{sec:char_func_design}




The characteristic function is needed in order to measure the contributions of the features in $\widetilde{\mathcal{I}}$. We define the characteristic function as the gains of the negative cross-entropy loss values between feature presences and absences.




\begin{definition}[Characteristic function]
\label{def:char_func}
The characteristic function $v(\widetilde{\mathcal{I}}): \widetilde{\mathcal{I}} \mapsto \mathbb{R}$ is defined as:  
\begin{align}
\label{equ:char_func_v_def}
v(\widetilde{\mathcal{I}}) 
&:=
 \mathop{\mathbb{E}}\limits_{x \thicksim \mathcal{X}} \sum_{y \in \mathcal{Y}} \left\{ 
 \underbrace{P(y|x) \cdot \log Q(y | x \bowtie \widetilde{\mathcal{I}})}_{\mathrm{Feature~presence}} - \underbrace{P(y|x) \cdot \log Q(y | x \bowtie \emptyset)}_{\mathrm{Absence~baseline}}
 \right\} \nonumber \\
 &=
\mathop{\mathbb{E}}\limits_{x \thicksim \mathcal{X}} \sum_{y \in \mathcal{Y}} P(y|x) \cdot \log Q(y | x \bowtie \widetilde{\mathcal{I}}) - C %\quad (nats)
\end{align}
where the constant term $C:=\mathop{\mathbb{E}}\limits_{x \thicksim \mathcal{X}} \sum\limits_{y \in \mathcal{Y}} P(y|x) \cdot \log Q(y | x \bowtie \emptyset)$ is used to fulfil $v(\emptyset) = 0$. We refer to the $C$ as the \textit{Dummy player constant}. 
%In the case of not causing ambiguity, we simplify $v(\widetilde{\mathcal{I}}; Q, \langle \mathcal{X}, \mathcal{Y} \rangle)$ into $v(\widetilde{\mathcal{I}})$.
\end{definition}

\begin{remark}
If the labels are one-hot, then \eqref{equ:char_func_v_def} is simplified into:
    \begin{align}
        v(\widetilde{\mathcal{I}}) :=\mathop{\mathbb{E}}\limits_{x,y \thicksim \langle \mathcal{X}, \mathcal{Y} \rangle} \log Q(y | x \bowtie \widetilde{\mathcal{I}}) - C %\quad (nats)
    \end{align}
   and $C:=\mathop{\mathbb{E}}\limits_{x,y \thicksim \langle \mathcal{X}, \mathcal{Y} \rangle} \log Q(y | x \bowtie \emptyset)$. 
    %Unsurprisingly, $v$ is in the form of the negative of cross-entropy loss. This is because the negative cross-entropy loss is to estimate the mutual information between predictions and labels \citep{qin2021neural,poole2019variational,barber2003information}.
\end{remark}

%The $v$ can be interpreted as the information gains of the features present in the $\widetilde{\mathcal{I}}$ versus their absences, which they are utilized by classifiers. 

\textbf{Linking to information theory}. The relationship between information theory and the characteristic function in the form of negative log-likelihood of Bayes classifiers has been discussed in the literature \citep{covert2020understanding,aas2021explaining,lundberg2017unified}. Following on from their discussions, we show that the $v$ in \eqref{equ:char_func_v_def} profoundly links to information theory in terms of spectral signals. The maximal information of features relevant to labels in $\widetilde{\mathcal{I}}$ is the mutual information $\mathbb{I}(\mathcal{X} \bowtie \widetilde{\mathcal{I}}, \mathcal{Y})$. A classifier $Q$ can merely utilize a proportion of the information. Theorem~\ref{theo:coalition_information_identity} states an information quantity identity regarding the $\mathbb{I}(\mathcal{X} \bowtie \widetilde{\mathcal{I}}, \mathcal{Y})$ and the $v$. The term $D_{KL}[P||Q]$ measures the point-wise (\ie~for an image $x$) KL-divergence between the predictions and ground-truth labels. On the basis of the information quantity identity, the $v$ can be interpreted as the information gains between the presences and absences of the features, which the $Q$ utilizes in decisions from the $\widetilde{\mathcal{I}}$. By enumerating all coalitions, the information gains are then combined to compute the marginal information gains of features in decisions via \eqref{equ:shapley_value}. 

%This equation can be interpreted as the information gain that the coalition $\widetilde{\mathcal{I}}$ over the baseline coalition $\emptyset$ in predictions.

\begin{theorem}[Spectral coalition information identity]
\label{theo:coalition_information_identity}
The information quantity relationship is given as:
\begin{align}
    \mathbb{I}(\mathcal{X} \bowtie \widetilde{\mathcal{I}}, \mathcal{Y}) 
    \equiv \mathop\mathbb{E}\limits_{x\in \mathcal{X} \bowtie \widetilde{\mathcal{I}}} D_{KL}[P(y|x) || Q(y||x)] + H(\mathcal{Y}) + v(\widetilde{\mathcal{I}}) + C
\end{align}
where $v$ is defined in \eqref{equ:char_func_v_def} and $H(\mathcal{Y})$ is the Shannon entropy of the label set $\mathcal{Y}$. The proof is provided in Appendix~\ref{app:theo_char_func}.
\end{theorem}








\begin{figure}[t!]
 
  %\vspace{-16pt} 

  \centering
  % \setlength{\abovecaptionskip}{5pt}
  % \setlength{\belowcaptionskip}{-15pt}
  
        
    %\includegraphics[width=0.7\textwidth]{figures/design_standalone.pdf} 

    %\includestandalone[width=1\textwidth]{standalone_pdfs/standalone_distributions_v8.tex}

    \includegraphics[width=1\textwidth,]{plots/standalone_distributions_v8.pdf}
    
    %\includegraphics[width=0.8\textwidth]{figures/evaluation_projection-imagenet.pdf}
        %\caption{This diagram illustrates the overview of \textbf{I-ASIDE} and shows how the spectral importance distributions are derived through the \textbf{ASIDE} equation.} 

    %There are three findings: (1) The spectral importance of the robustness of feature representations of trained models is \textcolor{blue}{non-uniform}, (2) the spectral importance of the robustness of the feature representations of un-trained models is \textcolor{blue}{uniform}, and (3) the models trained on larger datasets (e.g. the middle row) learn more robust feature representations.
    
    \caption[Spectral Importance Distributions of Trained Models and Un-Trained Models]{Spectral importance distributions (SIDs) of trained models and un-trained models.
    The experimental models are pre-trained on \textit{ImageNet}. We also include the models with random weights as a control marked by the blue box. We have noticed that: (1) The spectral importance distributions of trained models exhibit non-uniformity, and (2) the spectral importance distributions of un-trained models exhibit uniformity. We summarize these empirical observations as Assumption \ref{assump:spectral_uniformity}.}
    
    %\vspace{-1.em}
  
    \label{fig:spectral_importance_distributions}

\end{figure}












\subsection{Spectral robustness score (SRS)}
\label{sec:summarizing_score}

%We want to scalarize the vector SIDs for numerical comparisons, and also correlation studies against previous robustness metrics (e.g. mCE). 

Although we are firstly interested in using the spectral importance distributions (SID) for robustness interpretations, 
they can also be summarized into scalar scores for purposes such as numerical comparisons, and later correlation studies. 

\begin{assumption}[Spectral uniformity assumption of random decisions]
\label{assump:spectral_uniformity}
The second row in Figure~\ref{fig:spectral_importance_distributions} shows the SIDs from various models with randomized weights. We randomize the model weights with \textit{Kaiming} initialization \citep{he2015delving}. The measured SIDs exhibit spectral uniformity. This suggests: \textbf{Un-trained models do not have spectral preferences}. We refer to `the models with randomized parameters' as random decisions. Therefore, we assume that the SIDs of random decisions are uniform: $\frac{\mathbb{1}}{M}$. 
\end{assumption}

\begin{assumption}[Robustness prior]
\label{assump:robustness_prior}
We assume: \textbf{Higher utilization of robust features in decisions implies robust models}. This is further substantiated by the experiments in Figure~\ref{fig:freq_role}. To reflect this robustness prior, we empirically design a series $\vb*\beta := (\beta^0, \beta^1, \cdots, \beta^{M-1})^T$ where $\beta \in (0, 1)$ as the summing weights of SIDs. Empirically, we choose $\beta=0.75$ because this choice achieves the best correlation with model robustness.    
\end{assumption}


%Let $S(v): v \mapsto [0,1]$ be a map, 

\textbf{Summarizing with weighted sum}. Let $\Psi(v)$ be the measured spectral importance distribution (SID). Set $\bar\Psi(v)=\frac{\Psi(v) - \min{\Psi(v)}}{||\Psi(v) - \min{\Psi(v)}||_1}$ with min-max normalization. The weighted sum of the $\Psi(v)$ with the weights $\vb*\beta$ is given by:
\begin{align}
\label{equ:unnorm_SRS_score}
  \abs{
 {\vb*\beta}^T \bar\Psi(v) - {\vb*\beta}^T \frac{\mathbb{1}}{M}
 } 
\end{align}
where ${\vb*\beta}^T \frac{\mathbb{1}}{M}$ is served as a random decision baseline. Let $S(v): v \mapsto [0,1]$ be the normalized result in \eqref{equ:unnorm_SRS_score}. The $S(v)$ is given by:
\begin{align}
\label{equ:formula_s_v}
   S(v) :=  \frac{
\abs{{\vb*\beta}^T \bar\Psi(v) - {\vb*\beta}^T \frac{\mathbb{1}}{M}}   
   }{
   \sup\limits_{\bar\Psi} \abs{{\vb*\beta}^T \bar\Psi(v) - {\vb*\beta}^T \frac{\mathbb{1}}{M}} 
   } 
   = 
   \abs{\frac{{{\vb*{\bar\beta}}}^T \bar\Psi(v) - \eta}{1 - \eta}} 
\end{align}
where $\beta \in (0,1)$, ${\vb*{\bar\beta}} = \frac{\vb*{\beta}}{||\vb*{\beta}||_2}$ and $\eta=\frac{1}{M}\frac{||\vb*\beta||_1}{||\vb*\beta||_2}$. Readers can refer to Appendix~\ref{app:proof_score_formula} for the simplification deduction. 

%The deduction of this formula is provided in Appendix~\ref{app:proof_score_formula}.



\begin{figure}[t!]
 
  %\vspace{-16pt} 
  %\vspace{-2em}
      
 %\begin{figure}[H]
  \centering
  % \setlength{\abovecaptionskip}{5pt}
  % \setlength{\belowcaptionskip}{-15pt}
  
    \includegraphics[width=0.5\columnwidth,]{plots/mCE_correlation.pdf}

 
   


  \caption[Scalarized Spectral Robustness Scores Correlate with Mean Corruption Errors in Literature]{The spectral robustness scores (SRS), measured with I-ASIDE, correlate to the mean corruption errors (mCE) in the literature \citep{hendrycks2019benchmarking}.}
  
  
  %and information bottleneck principle \citep{tishby2015deep,tishby2000information} regarding learning dynamics
  
  %\vspace{-1.5em}
  
\label{fig:mce_correlation}
\end{figure} 






\section{Experiments}
\label{sec:experiments}

We design experiments to show the dual functionality of \textbf{I-ASIDE}, which can not only \textbf{measure} robustness and but also \textbf{interpret} robustness. We organize the experiments in three categories: 
\begin{itemize}
    \item Section~\ref{sec:experiment_correlation}: Correlation to a variety of robustness metrics;
    
    \item Section~\ref{sec:experiment_arch}: Studying architectural robustness;

    \item Section~\ref{sec:experiment_potential}: A case study interpreting how supervision noise levels affect model robustness. 
\end{itemize}

Section~\ref{sec:experiment_correlation} shows that the scores obtained with \textbf{I-ASIDE}~correlate with the model robustness scores measured with other methods. Section~\ref{sec:experiment_arch} and Section~\ref{sec:experiment_potential} show that \textbf{I-ASIDE} is able to interpret robustness by examining SIDs. 

\textbf{Reproducibility}. We choose $M=8$ and $200$ samples to conduct experiments. We choose $200$ samples because the experiments in Appendix~\ref{app:error_bound_analaysis}. The experiment shows that: \textbf{A small amount of examples are sufficiently representative for spectral signals}.



\begin{figure}[!t]
 
  %\vspace{-10pt} 

 %\begin{figure}[H]
  \centering


   \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{FGSM ($eps=0.1$)}]{
     \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_perturbation_fgsm_eps_0.1.pdf} 
     }
  \end{minipage}
  \hspace*{\fill}%
  \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{FGSM ($eps=0.2$)}]{
     \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_perturbation_fgsm_eps_0.2.pdf} 
     }
  \end{minipage}\\
  \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{PGD ($eps=0.1$)}]{
     \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_perturbation_pgd_eps_0.1.pdf} 
     }
  \end{minipage}
  \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{PGD ($eps=0.2$)}]{
     \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_perturbation_pgd_eps_0.2.pdf} 
     }
  \end{minipage}

  
  \caption[Scalarized Spectral Robustness Scores Correlates with Mean Prediction Errors in Adversarial Attacks]{The spectral robustness scores (SRS), measured with I-ASIDE, correlate with the mean prediction errors (mPE) in adversarial attacks. The circle sizes in (b) are proportional to the SRS.}
  
  %\vspace{-1.5em} 
 
\label{fig:adv_mPE}
\end{figure}





\begin{figure}[!t]
 
  %\vspace{-10pt} 

 %\begin{figure}[H]
  \centering

    \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{White noise ($\sigma=0.1$)}]{
      \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_ood_gaussian_std_0.1.pdf} 
     }
  \end{minipage}
  \hspace*{\fill}%
 \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{White noise ($\sigma=0.2$)}]{
      \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_ood_gaussian_std_0.2.pdf} 
     }
  \end{minipage}\\
 \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{Gaussian-blur ($3 \times 3$)}]{
      \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_ood_gaussian-blur_std_3.pdf}
     }
  \end{minipage}
  \hspace*{\fill}%
 \begin{minipage}[t]{0.44\textwidth}
     \centering 
     \subfloat[{Gaussian-blur ($7 \times 7$)}]{
      \includegraphics[width=1\textwidth,height=1\textwidth]{plots/adv_ood_gaussian-blur_std_7.pdf}
     }
  \end{minipage}
  


 
 %} %resize
  
  \caption[Scalarized Spectral Robustness Scores Correlates with Mean Prediction Errors in Corruptions]{The spectral robustness scores (SRS), measured with I-ASIDE, correlate to the mean prediction errors (mPE) in corruptions. The circle sizes in (b) are proportional to the SRS.}
  
  %\vspace{-1.5em} 
 
\label{fig:ood_mPE}
\end{figure}



%We also provide an extra showcase experiment in Appendix~\ref{app:training_dynamics}. The experiment showcases how model spectral robustness distributions evolve with respect to training steps. This help us to understand model training dynamics. 


\subsection{Correlation to robustness metrics}
\label{sec:experiment_correlation}
 
\begin{definition}[\textbf{Mean prediction error}]
    In our experiments, we measure model perturbation robustness with mean prediction errors (mPE) besides the mean corruption errors (mCE). Let $x$ be some clean image and $x^*$ be the perturbed image. For a classifier $Q$, we define the mean prediction error (mPE) as:
    \begin{align}
        \Delta \mathcal{P}:=\mathop\mathbb{E}\limits_{x, y \thicksim \langle \mathcal{X}, \mathcal{Y} \rangle} |Q(y|x) - Q(y|x^*)|.
    \end{align}
\end{definition}


We demonstrate that \textbf{I-ASIDE}~is able to measure model robustness. The experiments are broken down into three aspects: (1) correlation to mCE scores, (2) correlation to adversarial robustness, and (3) correlation to corruption robustness.




\textbf{Correlation to mCE scores}. Figure~\ref{fig:mce_correlation} shows the correlation between spectral robustness scores (SRS) and the mean corruption errors (mCE). The mCE scores are taken from the literature \citep{hendrycks2019benchmarking}. The mCE scores are measured on a corrupted \textit{ImageNet} which is known as \textit{ImageNet-C} in the literature \citep{hendrycks2019benchmarking}. The \textit{ImageNet-C} includes 75 common visual corruptions with five levels of severity in each corruption. This correlation suggests that the results measured with \textbf{I-ASIDE}~correlate with the results measured with robustness metric mCE.

\textbf{Correlation to adversarial robustness}. Figure~\ref{fig:adv_mPE} shows the correlation between the correlation between spectral robustness scores (SRS) and the mean prediction errors (mPE) of the adversarial attacks with FGSM and PGD. We vary the $eps$ from $0.1$ to $0.2$. The results show that our scores correlate with the mean prediction errors in various $eps$ settings. This suggests that the results measured by our method correlate with adversarial robustness.

\textbf{Correlation to corruption robustness}. Figure~\ref{fig:ood_mPE} shows the correlation between the correlation between spectral robustness scores (SRS) and the mean prediction errors (mPE) of the corruptions with white noise and Gaussian blurring. We vary the $\sigma$ of white noise from $0.1$ to $0.2$. We vary the Gaussian blurring kernel sizes from $3 \times 3$ to $7 \times 7$. The results show that our scores correlate with the mean prediction errors in all cases. This suggests that the results measured by our method can reflect the corruption robustness.






\begin{figure}[!t]
 
  %\vspace{-10pt} 

  \centering


  \begin{minipage}[b]{0.45\textwidth}
     \centering 
     \subfloat[{Spectral robustness score (SRS) comparison}]{
      \label{subfig:numerical_comparison}
      \includegraphics[width=1\textwidth,height=1\textwidth]{plots/dist_bidirectional_bar.pdf} 
     }
  \end{minipage}
  \hspace*{\fill}%
  \begin{minipage}[b]{0.45\textwidth}
     \centering 
     \subfloat[{Spectral importance distribution (SID) t-SNE projection}]{
      \label{subfig:numerical_comparison}
       %\begin{minipage}[t]{0.7\textwidth}
            %\includegraphics[trim=left botm right top, width=0.95\textwidth, clip]{...}

    \resizebox{0.9\textwidth}{!}{
	\begin{tikzpicture}
    
    % \node[inner sep=0pt, opacity=1] (img) at (0in, 0in){\includegraphics[trim=0 0 0 0cm, width=3.2in, clip]{figures/dist_proj_tsne_annotated.pdf}};

    \node[inner sep=0pt, opacity=1] (img) at (0in, 0in){\includegraphics[trim=0 0 0 0cm, width=3.2in, clip]{plots/dist_proj_tsne_v3_manual_edit.pdf}};

    \draw[dotted,
          color=black,
          line width=1.pt] (0.8in,1.in) rectangle (1.55in, 1.51in);

    

    \draw[->,draw=black,line width=1.pt] (0.5in, 1.2in) -- (0.75in, 1.2in);
    
    \node [align=center,
            xshift=0in,
            yshift=0in,
            scale=0.6,
            color=black,
            %text width=2.2in,
            rotate=0] at (0.1in, 1.2in) (label) {Transformer-based};

    \draw[->,draw=black,line width=1.pt] (0.5in, 0.9in) -- (0.75in, 0.9in);

    \node [align=center,
            xshift=0in,
            yshift=0in,
            scale=0.6,
            color=black,
            %text width=2.2in,
            rotate=0] at (0.1in, 0.9in) (label) {ConvNet-based};
    
    \draw[dotted,
          color=blue,
          line width=1.pt] (-0.3in,0.8in) rectangle (1.6in, 1.55in);

    \draw[->,draw=black,line width=1.pt] (-0.6in, 1.15in) -- (-0.4in, 1.15in);

    \node [align=center,
            xshift=0in,
            yshift=0in,
            scale=0.6,
            color=black,
            %text width=2.2in,
            rotate=0] at (-0.9in, 1.15in) (label) {Robust models};


    \draw[dotted,
          color=black,
          line width=1.pt] (-1.35in,-1.35in) rectangle (0.2in, -0.5in);


    \draw[->,draw=black,line width=1.pt] (-1.1in, -0.2in) -- (-1.1in, -0.4in);

    \node [align=center,
            xshift=0in,
            yshift=0in,
            scale=0.6,
            color=black,
            %text width=2.2in,
            rotate=0] at (-1.in, -0.1in) (label) {Non-robust models};
    
    \end{tikzpicture}
    }
    }
    \end{minipage}

  
 
  \caption[Effects of Architectural Elements on Robustness]{How do architectural elements affect robustness? The left figure is to answer: ``Does model parameter size play a role on robustness?''. The right figure, a t-SNE projection of SIDs, is to answer: ``Are vision transformers more robust than convolutional neural networks?''. For the two questions, the answers suggested by using \textbf{I-ASIDE} are yes. But the story is more complicated, we have provided a brief discussion regarding this case study within Section~\ref{sec:experiment_arch}. We also have noted that \textit{efficientnet} surprisingly exhibits comparable perturbation robustness as the architectures in Transformer family. All experimental models are pre-trained on \textit{ImageNet}. The circle sizes in (b) are proportional to SRS.}
  
 % \vspace{-1.em} 
 
\label{fig:scores_and_projections}
\end{figure}




\subsection{Studying architectural robustness}
\label{sec:experiment_arch}



\textbf{I-ASIDE}~is able to answer questions such as:
\begin{itemize}
    \item Does model parameter size play a role in robustness?

    \item Are vision transformers more robust than convolutional neural networks (ConvNets)?
\end{itemize}




\textbf{Does model parameter size play a role in robustness}? Figure~\ref{fig:scores_and_projections} (a) shows parameter counts do not correlate with model robustness. Thus, \textbf{the tendency of a model to use robust features is not determined by parameter counts alone}. We would like to carry out further investigation in future work.


\textbf{Are vision transformers more robust than ConvNets}? Figure~\ref{fig:scores_and_projections} (b) shows a t-SNE projection of the spectral importance distributions of a variety of models. The results show that vision transformers form a cluster (\textit{swin\_b}, \textit{maxvit\_t} and \textit{vit\_b\_16}) and outperform ConvNets in terms of robustness. This results correlate with the recent robustness research in the literature \citep{paul2022vision,zhou2022understanding,shao2021adversarial}. The interpretation is that: \textbf{Vision transformers tend to use more robust features than ConvNets}. 


\textbf{Discussion}. Vision transformers generally outperform ConvNets; nevertheless, state-of-the-art ConvNets, \eg~\textit{efficientnet} \citep{tan2019efficientnet}, can achieve comparable robustness performance (\eg~by error rates on benchmark datasets) \citep{li2023trade}. The literature \citep{devaguptapu2021adversarial} affirms that \textit{efficientnet} is more robust than most ConvNets. But, why \textit{efficientnet} is unique? The \textit{efficientnet} introduces an innovative concept in that the network sizes can be controlled by scaling the width, depth, and resolution with a compound coefficient \citep{tan2019efficientnet}. The base architecture is then searched with neural architecture searching (NAS) \citep{Thomas2019NASSurvey} instead of hand-crafted design. The NAS optimization objective is to maximize the network accuracy subject to arbitrary image resolutions. The searching implicitly encourages that the network structure of \textit{efficientnet} uses more robust features. This is because: \textbf{The low-frequency signals in various resolutions are robust signals while high-frequency signals are not.} The second column in Figure~\ref{fig:spectral_importance_distributions} shows the SID of \textit{efficientnet} pre-trained on \textit{ImageNet}. The SID shows that \textit{efficientnet\_v2\_s} uses more robust features than \textit{alexnet} and \textit{resnet18}.








\subsection{Interpreting how supervision noise levels affect model robustness}
\label{sec:experiment_potential}

The previous robustness benchmarks with mean corruption errors (mCE) are not able to answer the long-standing question: ``\textbf{How and why label noise levels affect robustness?}''. We demonstrate that \textbf{I-ASIDE}~is able to answer this question.




\textbf{Learning with noisy labels}. Supervision signals refer to the prior knowledge provided by labels \citep{sucholutsky2023informativeness,zhang2020distilling,xiao2020should}. There is a substantial line of previous research on the question of ``how supervision noise affects robustness'' \citep{gou2021knowledge,frenay2013classification,lukasik2020does}. This question is not completely answered yet. For example, \citeauthor{flatow2017robustness} add uniform label noise into \textit{CIFAR-10} and study its impact on model robustness \citep{flatow2017robustness}. Their results show that classification test accuracy decreases as the training label noise level increases. However, empirical studies like this are not able to answer the underlying `why' question.




\textbf{Noisy-label dataset}. We derive noisy-label datasets from a clean \textit{Caltech101}. We randomly assign a proportion of labels with a uniform distribution over label classes to create a noisy-label dataset. We refer to the randomly assigned proportion as supervision noise level. We vary the noise level from $0.2$ to $1.0$ to derive five training datasets.

\textbf{Experiment}. We train three models (\textit{googlenet}, \textit{resnet18} and \textit{mobilenet\_v2}) over the clean and the five noisy-label datasets for $120$ epochs respectively. We then measure their SIDs. The results are visualized in Figure~\ref{fig:label_noise} with heat maps. The results show that there is a pattern across the above three models in that: \textbf{The SIDs are more uniform with higher supervision noise levels}. The interpretation regarding the learning dynamics with the presence of label noise is that: \textbf{Models tend to use more non-robust features in the presence of higher label noise within training set}.








\begin{figure}[!t]
 
  %\vspace{-0.9em} 

 %\begin{figure}[H]
  \centering
  %\setlength{\abovecaptionskip}{-6pt}
  %\setlength{\belowcaptionskip}{-6pt}


\begin{minipage}[t]{0.32\textwidth}
     \centering 
     \subfloat[\textit{googlenet}]{
      \includegraphics[trim=0in 0in 0in 0in, width=1\textwidth, clip]{plots/googlenet_Caltech101_64_noisy_label_heatmap.pdf}
     }
  \end{minipage}
\hspace*{\fill}%
\begin{minipage}[t]{0.32\textwidth}
     \centering 
     \subfloat[\textit{resnet18}]{
      \includegraphics[trim=0in 0in 0in 0in, width=1\textwidth, clip]{plots/resnet18_Caltech101_64_noisy_label_heatmap.pdf}
     }
  \end{minipage}
\hspace*{\fill}%
\begin{minipage}[t]{0.32\textwidth}
     \centering 
     \subfloat[\textit{mobilenet\_v2}]{
      \includegraphics[trim=0in 0in 0in 0in, width=1\textwidth, clip]{plots/mobilenet_v2_Caltech101_64_noisy_label_heatmap.pdf.pdf}
     }
  \end{minipage}
  


  
  \caption[Effect of Label Noise on Robustness]{How do models respond to label noise? Our results show that models trained with higher label noise levels tend to use spectral signals uniformly, \ie~without a preference for robust (low-frequency) features. 
  }

  
  %\vspace{-1.5em}
  
 
\label{fig:label_noise}
\end{figure} 



\section{Related work}
\label{sec:related_work}



We further conduct a literature investigation from three research lines: (1) global interpretability, (2) model robustness, and (3) frequency-domain research. This literature study shows that \textbf{I-ASIDE} provides unique insights in these research lines.




\textbf{Global interpretability}. Global interpretability summarizes the decision behaviours of models from a holistic view. In contrast, local interpretability merely provides explanations on the basis of instances \citep{sundararajan2017axiomatic,smilkov2017smoothgrad,selvaraju2017grad,zhou2016learning,ribeiro2016should,lundberg2017unified,lakkaraju2019faithful,shrikumar2017learning}. There are four major research lines in image models: (1) feature visualization, (2) network dissection, (3) concept-based method, and (4) feature importance. 

Feature visualization seeks the ideal inputs for specific neurons or classes by maximizing activations \citep{nguyen2019understanding,zeiler2010deconvolutional,nguyen2016synthesizing}. This method provides intuitions regarding the question: ``What inputs maximize the activations of specific neurons or classes?''. Network dissection aims to connect the functions of network units (\eg~\textit{channels} or \textit{layers}) with specific concepts (\eg~\textit{eyes} or \textit{ears}) \citep{bau2017network}. Concept-based methods understand the decisions by answering the question ``how do models use a set of given concepts in decisions?'' \citep{kim2018interpretability,ghorbani2019towards,koh2020concept}. For example, TCAV explains model decisions by evaluating the importance of a given set of concepts (\eg~the textures \textit{dotted}, \textit{striped} and \textit{zigzagged}) for a given class (\eg~the class \textit{zebra}) \citep{kim2018interpretability}. 

Global input feature importance analysis, often by using Shapley value theory framework, attempts to answer the question: ``How do input features contribute to predictions?'' \citep{lundberg2017unified,ribeiro2016should,sundararajan2017axiomatic,covert2020understanding}. However, there are few works falling in the scope of global interpretability with feature importance analysis. A related work, SAGE, applying the Shapley value theory framework, globally assigns spatial input features with importance values for interpreting spatial feature contributions \citep{covert2020understanding}. 



Although the aforementioned global interpretability methods provide insights into understanding decisions inside black-box models, they do not provide interpretations regarding robustness mechanisms. Our work fundamentally differs from them in that: We provide interpretations regarding robustness mechanisms. We attempt to answer the fundamental question: ``Why some models are more robust than others?''.


\textbf{Model robustness}. Model robustness refers to the prediction sensitivity of models to perturbations. The perturbations can perturb in spaces such as the input space and the parameter space \citep{hendrycks2019benchmarking}. In this research, we focus on the perturbations within the input space. The perturbations can stem from sources such as adversarial attacks \citep{szegedy2014intriguing,goodfellow2014explaining}, corruptions \citep{hendrycks2019benchmarking}, outliers \citep{hendrycks2018deep} and supervision signal noise \citep{hendrycks2018using}. 

Model robustness is often assessed using scalar metrics \citep{hendrycks2019benchmarking,krizhevsky2012imagenet,taori2020measuring}. For example, robustness can be measured by the distances between clean and perturbed pairs in feature spaces \citep{zheng2016improving}. \citeauthor{hendrycks2019benchmarking} benchmark the corruption robustness with mean corruption errors (mCE) over a set of corrupted datasets like \textit{ImageNet-C} \citep{hendrycks2019benchmarking}, using AlexNet \citep{hendrycks2019benchmarking} as a normalization baseline. 


Despite their widespread adoption in previous literature, these scalar metrics lack the ability to provide detailed insights into the robustness mechanisms. Our work not only serves as a robustness metric but also offers mechanistic interpretations, answering the ``why'' question behind model robustness. This dual functionality distinguishes our approach, providing a deeper understanding of the mechanisms.


\textbf{Frequency-domain research}. Neural networks are non-linear parameterized signal processing filters. Investigating how neural networks respond to input signals in the frequency-domain can provide a unique insight into understanding its functions. \citeauthor{xu2019frequency} delve into the learning dynamics of neural networks in the frequency-domain \citep{xu2019frequency,xu2019training}. They present their findings as `F-Principle'. Their work suggests that the learning behaviors of neural networks exhibit spectral non-uniformity: Neural networks fit low-frequency components first, then high-frequency components. 

In a related study, \citeauthor{tsuzuku2019structural} show that convolutional neural networks have spectral non-uniformity with respect to Fourier bases \citep{tsuzuku2019structural}. Later, \citeauthor{wang2020high} connect model generalization behaviors and image spectrum \citep{wang2020high}. They argue that: (1) The supervision signals provided by humans use more low-frequency signals in images and (2) models trained on it tend to use more low-frequency signals. Our showcase experiment in Figure~\ref{fig:label_noise} provides the interpretations regarding their empirical findings. 

In the interpretability research line within the frequency-domain, \citeauthor{kolek2022cartoon} propose `CartoonX' based on the rate-distortion explanation (RDE) framework \citep{macdonald2019rate}. The RDE framework identifies decision-critical features by partially obfuscating the features. They refer to `the prediction errors between clean inputs and the partially obfuscated inputs' as distortions. CartoonX pinpoints the decision-critical features within wavelet domain to answer the query: ``What features are crucial for decisions?'' \citep{kolek2022cartoon}. Our work differs from CartoonX in that: (1) Our method aims to interpret model robustness mechanisms while CartoonX does not, (2) our method is a global interpretability method while CartoonX is a local interpretability method, (3) our method analyzes within an information theory framework while CartoonX uses RDE framework, and (4) our method uses Fourier bases while CartoonX uses wavelet bases.





\section{Limitations}
%\commentbox{TODO}
\textbf{I-ASIDE}~provides a unique insight into the perturbation robustness mechanisms. Yet, our method has two major limitations: (1) The spectral perspective can merely reflect one aspect of the holistic view of model robustness, and (2) the SID resolutions are low.


\textbf{Limitation (1)}. For example, carefully crafted malicious adversarial perturbations on low-frequency components can fool neural networks \citep{luo2022frequency}. \citeauthor{luo2022frequency} demonstrate that attacking low-frequency signals can fool neural networks, resulting in attacks which are imperceptible to humans. This further implies the complexity of this research topic. 

\textbf{Limitation (2)}. The computation cost is imposed by $\mathcal{O}(2^M)$. Fortunately, we do not need high SID resolution to analyze the model robustness problem. For example, a choice with $M=8$ is sufficient to interpret robustness mechanisms (as we have shown) while the computational cost remains reasonable.



\section{Conclusions}


On the solid ground provided by information theory and coalitional game theory, we present an axiomatic method to interpret model robustness mechanisms, by leveraging the power-law-like decay of SNRs over the frequency. Our method addresses the limitation that scalar metrics fail to interpret robustness mechanisms. We carry out extensive experiments over a variety of architectures. The SIDs, when scalarized, can largely reproduce the results found with previous methods, but addresses their failures to answer the underlying `why' questions. Our method goes beyond them with the dual functionality in that: \textbf{I-ASIDE}~can not only measure the robustness but also interpret its mechanisms. Our work provides a unique insight into the robustness mechanisms of image classifiers.





==> main_matter/chapters/Introduction/tikz/lipschitz_in_sobolev_space.tex <==
\begin{tikzpicture}
% \pgfplotsset{
%   colormap={custommap}{
%     rgb255(0cm)=(0,255,255)     % cyan
%     rgb255(1cm)=(255,255,128)   % light yellow
%     rgb255(2cm)=(128,100,0)     % brownish
%   }
% }
\begin{axis}[
    view={-50}{25}, 
    %z buffer=sort,     % <--- add this
    xlabel={\scriptsize $x_1$},
    ylabel={\scriptsize $x_2$},
    zlabel={\scriptsize $\|\nabla_{x} f(x)\|_2$},
    % xtick={0,90,...,360},
    % ytick={0,90,...,360},
    zmin=0, %zmax=6,
    %zmin=-3, point meta min=-1,
    domain=-3.5:3.5, y domain=-3.5:3.5,
    %shader=interp,
    ticks=none,
    ticklabel style={font=\scriptsize},
    %colormap/viridis, 
    %colormap name=viridis, 
    grid=none
]
% The surface:
\pgfmathsetmacro{\C}{6.55113333} % from the numeric minimum above
\addplot3[
  surf, 
  %shader=interp, 
  %opacity=1,
  samples=60, 
  samples y=60,
] ({x},{y},{\C
   + 3*(1-x)^2*exp(-(x^2)-(y+1)^2)
   - 10*(x/5 - x^3 - y^5)*exp(-(x^2+y^2))
   - (1/3)*exp(-((x+1)^2 + y^2))});

% --- constants / point of max (x*, y*)
\pgfmathsetmacro{\C}{6.5506884466}   % set 0 if you plotted g(x,y) only
\pgfmathsetmacro{\xK}{-0.006012}
\pgfmathsetmacro{\yK}{ 1.581162}
% compute z* from the SAME expression as the surface
\pgfmathsetmacro{\zK}{
  \C
  + 3*(1-\xK)^2*exp(-(\xK*\xK)-(\yK+1)^2)
  - 10*(\xK/5 - \xK^3 - \yK^5)*exp(-(\xK*\xK+\yK*\yK))
  - (1/3)*exp(-((\xK+1)^2 + \yK*\yK))
}

% mark and label
\addplot3[only marks, mark=*, mark size=2pt]
  coordinates {(\xK,\yK,\zK)};
\node[anchor=south] at (axis cs:\xK,\yK,\zK) {\scriptsize $K_f$};

% guides
\addplot3[dotted, color=darkgray] coordinates {(\xK,\yK,0) (\xK,\yK,\zK)};
\addplot3[dotted, color=darkgray] coordinates {(\xK,-3.5,0) (\xK,\yK,0)};
\addplot3[dotted, color=darkgray] coordinates {(-3.5,\yK,0) (\xK,\yK,0)};

\end{axis}
\end{tikzpicture}

==> main_matter/chapters/Introduction/tikz/thesis_research_questions.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usetikzlibrary{trees, arrows.meta}

% \begin{document}

% \begin{tikzpicture}[
%   grow'=right,
%   edge from parent/.style={draw, -{Stealth[length=4pt, width=6pt]}, thick},
%   % sibling distance=8cm,
%   % level distance=16cm,
%   level 1/.style={level distance=10cm, sibling distance=5cm},
%   level 2/.style={level distance=10cm, sibling distance=2cm},
%   every node/.style={
%     rectangle, draw=black, rounded corners,
%     align=center, font=\small,
%     text width=6.5cm, minimum height=1.5cm,
%     fill=gray!10, inner sep=6pt
%   }
% ]
\begin{tikzpicture}[
  grow'=right,
  edge from parent/.style={
    draw,
    thick,
    -{Stealth[length=4pt, width=6pt]},
    looseness=1.2, % controls how "loose" the curve is
    out=0,         % starting angle from parent
    in=180         % ending angle into child
  },
  level 1/.style={level distance=10cm, sibling distance=5cm},
  level 2/.style={level distance=10cm, sibling distance=2cm},
  every node/.style={
    rectangle, draw=black, rounded corners,
    align=center, font=\small,
    text width=6.5cm, minimum height=1.5cm,
    fill=gray!10, inner sep=6pt
  }
]

% Root node
\node[fill=blue!15, font=\bfseries] {Principles of Lipschitz Continuity}
  child { node[fill=lime!30, font=\bfseries] {RQ1: State of Knowledge}
    child { node[fill=lime!15] {SRQ1: Theoretical Foundations} }
    child { node[fill=lime!15] {SRQ2: Regularization Mechanisms} }
  }
  child { node[fill=purple!30, font=\bfseries] {RQ2: Training Dynamics}
    child { node[fill=purple!15] {SRQ3: Parameter Space Perturbation} }
    child { node[fill=purple!15] {SRQ4: Optimization-Induced Stochastic Dynamics} }
  }
  child { node[fill=orange!30, font=\bfseries] {RQ3: Modulation of Frequency Signal Propagation}
    child { node[fill=orange!15] {SRQ5: Spectral Bias of Lipschitz Continuity} }
    child { node[fill=orange!15] {SRQ6: Interpreting Global Robustness} }
  };

% % Root node
% \node[fill=blue!15, font=\bfseries] {Principles of Lipschitz Continuity}
%   % RQ1
%   child { node[fill=lime!30, font=\bfseries] {RQ1: State of Knowledge}
%     child { node[fill=lime!15] {SRQ1: Theoretical Foundations} }
%     child { node[fill=lime!15] {SRQ2: Regularization Mechanisms} }
%   }
%   % RQ2
%   child { node[fill=purple!30, font=\bfseries] {RQ2: Training Dynamics}
%     child { node[fill=purple!15] {SRQ3: Parameter Space Perturbation} }
%     child { node[fill=purple!15] {SRQ4: Optimization-Induced Stochastic Dynamics} }
%   }
%   % RQ3
%   child { node[fill=orange!30, font=\bfseries] {RQ3: Modulation of Frequency Signal Propagation}
%     child { node[fill=orange!15] {SRQ5: Spectral Bias of Lipschitz Continuity} }
%     child { node[fill=orange!15] {SRQ6: Interpreting Global Robustness} }
%   };

\end{tikzpicture}

% \end{document}

==> main_matter/chapters/LiteratureReview/text.tex <==

\section{Introduction}
\label{sec:intro}


Deep learning has achieved remarkable success across various domains, including computer vision, natural language processing, and graph-based learning. Advances in state-of-the-art architectures, such as convolutional neural networks (CNNs) \citep{krizhevsky2012imagenet}, transformers \citep{vaswani2017attention, brown2020language}, and graph neural networks (GNNs) \citep{kipf2017semi}, as well as their large-scale applications, including large language models (LLMs) \citep{brown2020language, chowdhery2022palm, touvron2023llama,openai2023gpt4,deepseekai2025deepseekr1} and large vision-language models (LVLMs) \citep{radford21aclip,li22nblip,geminiteam2025}, have significantly expanded the frontiers of deep learning, enabling powerful capabilities across a wide range of tasks.

Beyond their remarkable success, ensuring safety \citep{amodei2016concrete}, robustness \citep{madry2018towards} and generalization, remains a critical challenge. These properties are intrinsically linked to the sensitivity of neural networks to input perturbations \citep{madry2018towards,tsipras2018robustness,hendrycks2019benchmarking,amerehi25a}, which can significantly impact their reliability in real-world applications. For instance, adversarial vulnerabilities \citep{goodfellow2014explaining, carlini2017towards}, and out-of-distribution (OOD) generalization \citep{sokolic2017robust,Neyshabur2017nips,bartlett2017spectrally,hendrycks2021many} are major concerns in developing reliable deep learning models. A fundamental mathematical concept that characterizes network sensitivity and governs these properties is \textbf{Lipschitz continuity}, which measures the upper bound of the outputs of neural networks to inputs.

Although numerous studies have explored Lipschitz continuity from both theoretical \citep{bartlett2017spectrally, luo2025lipschitz} and applied \citep{arjovsky2017wasserstein, gulrajani2017improved, miyato2018spectral} perspectives, a unified survey that consolidates these insights is still lacking. Existing works primarily focus on isolated aspects, such as adversarial robustness \citep{szegedy2014intriguing, madry2018towards, weng2018clever}, regularization \citep{arjovsky2017wasserstein, gulrajani2017improved}, or theoretical bounds without practical considerations \citep{bartlett2017spectrally}. The absence of a comprehensive survey integrating these perspectives leaves a critical gap in the literature. To address this, we provide a systematic review of Lipschitz continuity in deep learning, covering its \textbf{theoretical foundations},  \textbf{estimation methods}, \textbf{regularization approaches in optimization and architecture}, and \textbf{certifiable robustness}. By synthesizing key findings across these domains, this survey serves as a valuable resource for researchers and practitioners seeking a deeper understanding of Lipschitz continuity and its role in trustworthy learning systems. Beyond conducting a survey, we also critically distill the existing knowledge, present it in a more accessible manner, and provide the results or proofs \textbf{missing} or \textbf{incorrect} in the literature. The message of this survey is that Lipschitz continuity is not just a niche mathematical property; it is a fundamental principle for building and analyzing trustworthy neural networks.

\subsection{Scope}

This survey aims to consolidate existing knowledge across these domains, providing a comprehensive resource for researchers and practitioners seeking to understand and leverage Lipschitz continuity in deep learning. To ensure a high-quality review, we focus primarily on the literature published in prestigious and other well-regarded sources. The scope of this survey is organized as below:

\begin{enumerate}

    \item Section~\ref{sec:theory}:~\nameref{sec:theory}  
    presents the formal definitions and fundamental properties of Lipschitz continuity, followed by key theoretical developments in deep learning. It covers the mathematical foundations, Lipschitz properties of activation functions and neural networks, Lipschitz analysis of multi-head self-attention, complexity-theoretic generalization bounds, and advances in training dynamics.

    \item Section~\ref{sec:estimating_lipschitz}:~\nameref{sec:estimating_lipschitz}  
    surveys the principal methods for estimating the Lipschitz constants of neural networks, including derivative bound propagation, spectral alignment, convex optimization relaxations, and relaxed integer programming approaches.


    \item Section~\ref{sec:lipschitz_regularizations}:~\nameref{sec:lipschitz_regularizations}  
    reviews approaches for enforcing Lipschitz continuity in neural networks through both optimization-based and architectural approaches, covering weight regularization, gradient regularization, activation regularization, and class-margin regularization.
    

    \item Section~\ref{sec:certifiable_robustness}:~\nameref{sec:certifiable_robustness}  
    examines methods for achieving certifiable robustness through Lipschitz bounds, including the theoretical foundations of Lipschitz-margin robustness radii, certification via global Lipschitz bounds, certification via local Lipschitz bounds and certificated robustness in LLMs.
    
\end{enumerate}





\subsection{Contributions}


Our key contributions are as follows:
\begin{enumerate}

    \item \textbf{A Unified Systematic Review}. We close a critical gap in the literature by conducting a comprehensive survey of Lipschitz continuity in deep learning. Our review unites disparate research threads --- spanning theoretical foundations, estimation methods, regularization approaches, architectural designs, and certified robustness --- into a coherent framework that highlights their interconnections from the lens of Lipschitz continuity.
    

    \item \textbf{Comprehensive Analysis}. We provide in-depth examinations of existing techniques organized into four categories:
    \begin{itemize}
        \item \textbf{Theoretical Foundations}. We review the formal definitions and properties of Lipschitz continuity, analyze Lipschitz behavior of activations and network architectures, and synthesize key results on generalization bounds, optimization convergence, and training-induced Lipschitz dynamics. 
        
        \item \textbf{Estimation Methods}. From power-iteration spectral-norm approximations and extreme-value theory to randomized and interval-analysis approaches, we compare each method's tightness, computational overhead, and scalability to modern architectures.
        
        \item \textbf{Regularization Approaches}. We critically assess gradient-based penalties, spectral normalization, orthogonal and Parseval constraints, and novel Lipschitz-bounded activations, examining their theoretical guarantees, implementation trade-offs, and empirical effects on robustness, generalization, and training dynamics.
        
        \item \textbf{Certifiable Robustness}. We survey Lipschitz-based certification frameworks --- covering global and local Lipschitz bounds, path-based and convex-relaxation certificates, randomized smoothing, and Lipschitz-constrained architectures --- analyzing their provable guarantees, computational requirements, and applicability to real-world deep models.
    \end{itemize}

   
 


    

    
    \item \textbf{Results and Proofs}. We contribute new and complementary results, including corrected Lipschitz constants for common activation functions (validated by our numerical experiments) and a Lipschitz continuity bound for arbitrary neural networks represented as directed acyclic graphs (DAGs). Furthermore, we provide theoretical results \textbf{missing or incorrect} from prior work, such as rigorous proofs of the closed-form expressions for the Lipschitz constants of common activation functions and a general perturbation bound for certifiable robustness based on H\"older's conjugacy relation.
    
\end{enumerate}

 




\section{Theoretical Foundations}
\label{sec:theory}


Lipschitz continuity is a foundational concept in deep learning theory, offering a rigorous framework for quantifying a neural network's sensitivity to input perturbations. It plays a central role in understanding robustness, generalization, and optimization dynamics. Throughout, we use operator $\mathrm{Lip}_p\left[ \bullet \right]$ to denote the $p$-norm Lipschitz constant for $\bullet$, and use operator $\mathrm{Lip}\left[ \bullet \right]$ to denote the $2$-norm Lipschitz constant for $\bullet$.





\subsection{Preliminaries}
\label{sec:preliminaries}

\begin{definition}[$p$-Norm in Finite-Dimensional Vector Spaces]
Let $V \subseteq \mathbb{R}^d$ be a finite-dimensional vector space. The $p$-norm (\ie~$\ell_p$-norm) in $V$ is defined as:
\begin{equation}
    \|z\|_p =
    \begin{cases}
        \left( \sum\limits_{i=1}^d |z_i|^p \right)^{1/p}, & \text{if } 1 \leq p < \infty, \\
        \quad \\
        \max\limits_{i=1,\dots,d} |z_i|, & \text{if } p = \infty,
    \end{cases}
\end{equation}
where $z = (z_1, z_2, \dots, z_d) \in V$ \citep[Definition~3.6, \S~3]{rudin1987real}.
\end{definition}



\begin{definition}[Globally $K$-Lipschitz Continuous]
\label{def:lipschitz_definition}
Let $f: X \mapsto Y$ be a function, where $X \subseteq \mathbb{R}^d$ and $Y \subseteq \mathbb{R}^c$. The function $f$ is said to be \emph{globally $K$-Lipschitz continuous} (with respect to the 2-norm) if there exists a constant scalar $K > 0$ such that:
\begin{equation}
    \|f(u) - f(v)\|_2 \leq K \|u - v\|_2, \quad \forall\, u, v \in X
    ,
\end{equation}
\citep[Theorem 9.19, \S~9]{rudin1976principles}. Throughout, unless specified otherwise, the \emph{Lipschitz norm} is assumed to be the $2$-norm.
\end{definition}


\begin{definition}[Globally $K_{p \to q}$-Lipschitz Continuous]
\label{def:lipschitz_definition_holders_conjugate}
Let:
\begin{align}
1 \le p, q \le \infty    \notag
\end{align}
be two scalars.
A function $f: X \to Y$, with $X \subseteq \mathbb{R}^d$ and $Y \subseteq \mathbb{R}^c$, is said to be \emph{$K_{p \to q}$-Lipschitz continuous} if there exists a constant $K_{p \to q} > 0$ such that:
\begin{equation}
    \|f(u) - f(v)\|_{q} \; \le \; K_{p \to q} \, \|u - v\|_{p},
    \quad \forall\, u, v \in X,
\end{equation}
where $\|\cdot\|_p$ and $\|\cdot\|_q$ denote the $\ell_p$ and $\ell_q$ norms, respectively. Particularly, $K_{2 \to 2}$-Lipschitz continuous reduces to $K$-Lipschitz continuous with respect to $2$-norm.
\end{definition}

\begin{remark}
Definition~\ref{def:lipschitz_definition_holders_conjugate}~(\nameref{def:lipschitz_definition_holders_conjugate}) is non-standard in the mathematical literature; however, it is useful for discussions of certifiable robustness in the context of deep learning.
\end{remark}


\begin{lemma}[Lipschitz Constant Bounds Gradient Norm]
\label{lemma:lipschitz_bounds_gradient}
Let $f: \mathbb{R}^m \to \mathbb{R}$ be a differentiable function. Then $f$ is $K$-Lipschitz continuous (with respect to the 2-norm) if and only if
\begin{equation}
K \geq \sup_{x \in \mathrm{dom}(f)} \|\nabla f(x)\|_2
,
\end{equation}
\citep[Theorem 9.19, \S~9]{rudin1976principles}. In the case $0 < K < 1$, the function $f$ is called a contraction map. In particular, for the case that $\mathrm{dom}(f)$ is a convex set --- any points connected through the \emph{Mean Value Theorem} remain within $\mathrm{dom}(f)$, thus the tight bound is achieved such that:
\begin{equation}
K = \sup_{x \in \mathrm{dom}(f)} \|\nabla f(x)\|_2
.
\end{equation}
\end{lemma}


\begin{remark}
\label{remark:domain_convex}
In Lemma~\ref{lemma:lipschitz_bounds_gradient}~(\nameref{lemma:lipschitz_bounds_gradient}), of the deep learning sense, the domain of a neural network $f: \mathbb{R}^m \to \mathbb{R}$ can be assumed to be a convex set on $\mathbb{R}^m$. Consequently, the tight Lipschitz bound is attained.
\end{remark}

\subsection{$1$-Lipschitz Orthogonal Matrix}
\label{sec:orthogonal_matrix}

\begin{definition}[Skew-Hermitian \& Skew-Symmetric Matrix]
\label{def:skew_hermitian}
A matrix $A$ is referred to as a \emph{skew-hermitian matrix}, if $A$ satisfies:
\begin{align}
    A=-A^\ast
    .
\end{align}
Particularly, if $A$ is a real matrix, then $A$ is also referred to as a \emph{skew-symmetric matrix}.
\end{definition}

\begin{proposition}[Lipschitz Constant of Semi-Orthogonal Matrix]
\label{prop:column_orthogonal_matrix}
If a matrix $W \in \mathbb{R}^{m \times n}$ with:
\begin{align}
    W^\top W = I_n
    \qquad \text{or} \qquad
    W W^\top = I_m
    ,
\end{align}
then $W$ is semi-orthogonal with Lipschitz constant $1$. If $W^\top W = I_n$ (requiring $m \geq n$), $W$ is an isometric map over the entire $\mathbb{R}^n$; if $WW^\top = I_m$ (requiring $m \leq n$), $W$ is non-expansive, acting as an isometry on $\ker(W)^\perp$ and vanishing on $\ker(W)$.
\end{proposition}

\begin{proof}
\begin{enumerate}[label=\textbf{}, leftmargin=*]

\item \textbf{Case 1: $m \geq n$ (Isometric Map).} For $\forall\;x,y \in \mathbb{R}^n$:
\begin{align}
\|W(x-y)\|_2^2
&= (W(x-y))^\top W(x-y) \notag \\
&= (x-y)^\top W^\top W (x-y) \notag \\
&= (x-y)^\top I_n (x-y) \notag \\
&= \|x-y\|_2^2 \notag
,
\end{align}
then by definition:
\begin{align}
    \mathrm{Lip}\left[W\right] =
    \sup_{x \neq y} \frac{\|W(x-y)\|_2}{\|x-y\|_2} = 1
    \notag
    .
\end{align}

\item \textbf{Case 2: $WW^\top = I_m$, $m \leq n$ (Vanishing on Kernel).} Since $WW^\top = I_m$:
\begin{align}
\|W\|_2^2 = \lambda_{\max}(W^\top W) = \lambda_{\max}(WW^\top) = \lambda_{\max}(I_m) = 1 \notag
,
\end{align}
so $\mathrm{Lip}\left[W\right] = \|W\|_2 = 1$. When $m < n$, $\ker(W)$ is non-trivial, and for $\exists \; x-y \in \ker(W)$:
\begin{align}
\|W(x-y)\|_2 = 0 < \|x-y\|_2 \notag
,
\end{align}
so $W$ vanishes on $\ker(W)$ and is thus non-expansive but not an isometry.
\end{enumerate}
\end{proof}

\subsubsection{Matrix Orthogonalization}

We also survey useful matrix orthogonalization algorithms below.

\paragraph{Lie Group Exponential Map.} Let:
\begin{align}
    U(n) = \Bigl\{ 
    A \in \mathbb{C}^{n \times n} \mid A^\ast  A = I
    \Bigr\}
\end{align}
be a unitary group and:
\begin{align}
    \mathfrak{u}(n)=\{B\in\mathbb{R}^{n\times n}\;:\;B=-B^\ast \}
\end{align}
be a \emph{Skew-Hermitian} group. Then there exists an \emph{Lie Exponential Map}:
\begin{align}
    \exp(A): \mathfrak{u}(n) \to U(n)
    ,
\end{align}
connecting the groups $\mathfrak{u}(n)$ and $U(n)$, defined as:
\begin{align}
    \exp(A)=I+A+\frac{1}{2}A^2+\cdots \label{eq:Lie_Exponential_Map}
    ,
\end{align}
which is surjective. For a matrix $W$, its corresponding skew-Hermitian matrix can be constructed by taking:
\begin{align}
    B=W-W^\ast \in \mathfrak{u}(n) \label{eq:skew_Hermitian_conversion}
\end{align}
\citep{lezcano2019cheap}. 

\begin{remark}
The \emph{Lie Exponential Map} (\eqref{eq:Lie_Exponential_Map}) together with the skew-Hermitian matrix conversion (\eqref{eq:skew_Hermitian_conversion}) allow us to map an arbitrary matrix $W$ into the unitary algebra $\mathfrak{u}(n)$ which has Lipschitz constant one. This is particularly useful for architecturally designing $1$-Lipschitz neural networks.  
\end{remark}


\paragraph{Cayley Transform.} If $B \in \mathbb{R}^{n \times n}$ is a \emph{skew-symmetric} matrix, the map:
\begin{align}
    \phi(B)=(I+\frac{1}{2}B)(I-\frac{1}{2}B)^{-1}
\end{align}
is referred to as the \emph{Cayley map} which transforms $B$ to an orthogonal matrix $\phi(B)$ \citep{cayley1846quelques,trockman2021orthogonalizing}. Then the transformed orthogonal matrix $\phi(B)$ has a constant Lipschitz one. The Cayley map is not surjective onto the orthogonal group: its image excludes orthogonal matrices with $-1$ in their spectrum.


\paragraph{\emph{Bj\"orck Orthogonalization} Approximation.} Suppose $W_0 \in \mathbb{R}^{n \times n}$ is not an orthogonal matrix. Let $W_k$ be an iterative sequence such that $W_k$ is the closest orthogonal matrix to $W_0$ as $k \to \infty$. \emph{Bj\"orck Orthogonalization} \citep{bjorck1971} is a differentiable method to iteratively solve the closest orthogonal matrix to a given matrix $W_0$. \citet{chernodub2017normpreservingorthogonalpermutationlinear} use \emph{Bj\"orck Orthogonalization} in an optimization problem for constraining the orthogonality of parameter matrices \citep{chernodub2017normpreservingorthogonalpermutationlinear}. \emph{Bj\"orck Orthogonalization} \citep{bjorck1971} is defined by:
\begin{align}
    W_{k+1} = W_k \Bigl(
    I + \frac{1}{2} Q_k + \cdots + (-1)^p 
    \begin{pmatrix}
        -\frac{1}{2} \\
        p
    \end{pmatrix}
    Q_k^p
    \Bigr)
    ,
\end{align}
where $W_{k}$ is the $k$-th iterative result, $p$ is a chosen hyper-parameter, $\begin{pmatrix}
    -\frac{1}{2}\\
    p
\end{pmatrix}$ is binomial coefficient, and $Q_k$ is:
\begin{align}
    Q_k = I - W_k^\top W_k
    .
\end{align}
As $k \to \infty$, $W_k^\top W_k$ converges to $I_n$. For a rectangular matrix $W_0 \in \mathbb{R}^{m \times n}$, if $\rank(W_0) = n$, the convergence still holds: 
\begin{align}
W_k^\top W_k \to I_n
\notag
,
\end{align}
as $k \to \infty$.


\subsection{Functional Inequalities}

\begin{proposition}[Lipschitz Constant of Function Composition]
\label{prop:lipschitz_composition}
Let $f:X \to Y$ and $g: Y \to Z$ be two bounded functions. Then the Lipschitz constant of their composition $g\;\circ\;f: X \to Z$ admits:
\begin{align}
    \mathrm{Lip}_p \left[ g \circ f \right] \leq \mathrm{Lip}_p \left[ g\right]\;\mathrm{Lip}_p \left[ f\right]
    .
\end{align}
\end{proposition}

\begin{proof}
    \begin{align}
        \mathrm{Lip}_p \left[ g \circ f \right] &=
        \sup_{\|x-y\|_p \neq 0} \frac{\|g(f(x)) - g(f(y))\|_p}{\|x - y\|_p} \notag \\
        &\leq
        \mathrm{Lip}_p \left[ g \right]
        \;
        \sup_{\|x-y\|_p \neq 0} \frac{\|f(x) - f(y)\|_p}{\|x - y\|_p} \notag \\
        &=\mathrm{Lip}_p \left[ g \right]
        \;
        \mathrm{Lip}_p \left[ f \right] \notag
        .
    \end{align}
\end{proof}

\begin{proposition}[Lipschitz Constant of Function Addition]
\label{prop:lipschitz_addition}
Let $f$ and $g$ be two bounded functions on $\mathrm{dom}(g) \; \cap \; \mathrm{dom}(f)$. Then the Lipschitz constant of $g + f$ admits:
\begin{align}
    \mathrm{Lip}_p \left[ g + f \right] \leq \mathrm{Lip}_p \left[ g\right] + \mathrm{Lip}_p \left[ f\right]
    .
\end{align}
\end{proposition}

\begin{proof}
   \begin{align}
       \mathrm{Lip}_p \left[ g + f \right] &=
       \sup_{\|x-y\|_p \neq 0} \frac{\|f(x) + g(x) - \left[f(y) + g(y)\right]\|_p}{\|x - y\|_p}  \notag \\
       &=\sup_{\|x-y\|_p \neq 0} \frac{\|f(x) - f(y) + g(x) - g(y)\|_p}{\|x - y\|_p}  \notag \\
       &\leq
       \sup_{\|x-y\|_p \neq 0} \frac{\|f(x) - f(y)\|_p}{\|x - y\|_p}
       +
       \sup_{\|x-y\|_p \neq 0} \frac{\|g(x) - g(y)\|_p}{\|x - y\|_p} \notag \\
       &= \mathrm{Lip}_p \left[ g\right] + \mathrm{Lip}_p \left[ f\right]
       \notag
       .
   \end{align} 
\end{proof}

\begin{proposition}[Lipschitz Constant of Function Concatenation]
\label{prop:lipschitz_concatenation}
Let $f: \mathbb{R}^d \to \mathbb{R}^m$ and $g: \mathbb{R}^d \to \mathbb{R}^n$ be two Lipschitz continuous functions. Let:
\begin{align}
    (f \oplus g)(x) := \begin{bmatrix}
        f(x) \\
        g(x)
    \end{bmatrix} 
    \in \mathbb{R}^{m+n}
\end{align}
be a function by concatenating the outputs of $f$ and $g$. Then, for $1 \leq p<\infty$, the following inequality holds true:
\begin{align}
    \Bigl(\mathrm{Lip}_p\left[f \oplus g\right]\Bigr)^p \leq \Bigl(\mathrm{Lip}_p\left[f\right]\Bigr)^p + \Bigl(\mathrm{Lip}_p\left[g\right]\Bigr)^p 
    .
\end{align}
\end{proposition}

\begin{proof}
For any $x,y \in \mathbb{R}^d$, we have:
\begin{align}
    \Bigl\|(f \oplus g)(x) - (f \oplus g)(y)\Bigr\|_p^p
    &= \Biggl\|
        \begin{bmatrix}
            f(x) \\
            g(x)
        \end{bmatrix}
        -
        \begin{bmatrix}
            f(y) \\
            g(y)
        \end{bmatrix}
    \Biggr\|_p^p \notag\\
    &=\sum_{i=1}^{m} \Bigl(|f(x)-f(y)|^p\Bigr)_i + \sum_{j=1}^{n} \Bigl(|g(x)-g(y)|^p\Bigr)_j \notag\\
    &\leq \Biggl(\Bigl(\mathrm{Lip}_p\left[f\right]\Bigr)^p  + \Bigl(\mathrm{Lip}_p\left[g\right]\Bigr)^p \Biggr)\|x-y\|_p^p \notag
    .
\end{align}
Hence:
\begin{align}
   \Bigl(\mathrm{Lip}_p\left[f \oplus g\right]\Bigr)^p &= \sup_{x\neq\,y} \frac{\bigl\|(f \oplus g)(x) - (f \oplus g)(y)\bigr\|_p^p}{\|x-y\|_p^p} \notag \\
   &\leq \Bigl(\mathrm{Lip}_p\left[f\right]\Bigr)^p  + \Bigl(\mathrm{Lip}_p\left[g\right]\Bigr)^p
   \notag
   .
\end{align}
\end{proof}


    


\subsection{Sub-Differential Convex Functions}
\label{sec:subdifferential}

For a function that is not differentiable but is locally Lipschitz continuous --- such as the ReLU activation --- the Clarke sub-differential provides a generalized notion of gradient that allows one to analyze and bound local Lipschitz constants \citep{clarke1975generalized}.


\begin{definition}[Generalized Gradient]
Let $f : \mathbb{R}^m \to \mathbb{R}$ be a function on $X$.
The sub-differential of $f$ at a point $x$ is the set
\begin{align}
\partial_s f(x)
=
\left\{
g \in \mathbb{R}^m
\;\middle|\;
f(y) \ge f(x) + \langle g, y - x \rangle,\ \forall y \in X
\right\}.    
\end{align}
If $f$ is convex, then:
\begin{align}
\partial_s f(x) \neq \varnothing 
\qquad
\text{and}
\qquad
\partial_s f(x) = \{\nabla f(x^\ast ) \mid \forall~x^\ast  \to x\}
.
\end{align}

\end{definition}

\begin{definition}[Clarke Sub-Gradient]
Let $f: \mathbb{R}^m \to \mathbb{R}$ be a proper convex function on $X$. If $f$ is locally Lipschitz continuous on $X$, then by Rademacher's theorem it is differentiable almost everywhere. The Clarke sub-differential $f$ at a point $x$ is defined as the convex hull of all limit points of gradients at differentiable points approaching $x$. That is, a vector $g$ lies in the Clarke sub-differential at $x$ if there exists a sequence of points $x_k \to x$ ($k \in \mathbb{N}$) at which $f$ is differentiable such that the gradients $\nabla f(x_k)$ converge to $g$. Then the Clarke sub-differential is a convex hull, satisfying:
\begin{align}
    \partial f(x) = \mathrm{conv}\Bigl\{ 
    g \mid \exists\; \text{a sequence}~(x_k) \to x~\text{as}~k\to \infty, \nabla f(x_k) \to g
    \Bigr\}
\end{align}
\citep[Definition 1.1]{clarke1975generalized}. If $f$ is convex, then $\partial f(x) = \partial_s f(x)$. This definition also extends to vector-valued functions \citep{clarke1990optimization}.
\end{definition}


\begin{lemma}[Local Lipschitz Constant of Sub-Differential Function]
Let $f : \mathbb{R}^m \to \mathbb{R}^n$ be a convex function differentiable almost everywhere on $X$.
Then the $p \to q$ local Lipschitz constant of $f$ on $X$ is given by:
\begin{align}
\mathrm{Lip}_{p \to q}[f; X]
=
\sup_{x \in X} \sup_{G \in \partial f(x)}
\sup_{\|v\|_p \neq 0}
\frac{\|G^\top v\|_q}{\|v\|_p}
=
\sup_{x \in X} \sup_{G \in \partial f(x)}
\sup_{\|v\|_p = 1}
\|G^\top v\|_q,
\end{align}
such that:
\begin{align}
\|f(x) - f(y)\|_q \le \mathrm{Lip}_{p \to q}[f; X] \|x - y\|_p,
\end{align}
for all $x, y \in X$ in the sense of Clarke sub-gradient \citep{jordan2020exactly,boyd2022ee364b}.

\end{lemma}



\subsection{Lipschitz Continuity of Activation Functions}
\label{sec:activation_functions}

An activation function:
\begin{align}
    \rho: \mathbb{R}^d \to \mathbb{R}^d \notag
\end{align}
is a nonlinear mapping applied after neuron's output at a layer, enabling neural networks to learn complex patterns. For example, if $\sigma$ is piecewise defined as:
\begin{align*}
    \rho(x) =
\begin{cases}
x, & \text{if } x > 0, \\
0, & \text{otherwise}
\end{cases}
,
\end{align*}
then the $\rho$ is referred to as \emph{ReLU} activation function \citep{nair2010relu}.


The Lipschitz constants of commonly used activation functions are provided in Table~\ref{tab:lipschitz_activations}. The constants are derived as the supremum of the $2$-norm of the derivatives of activation functions. Proofs are provided in the Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions}. To numerically validate the results, we have conducted experiments by maximizing the gradient norm using Lemma~\ref{lemma:lipschitz_bounds_gradient} for a further sanity check.


\textbf{Notes.} The Lipschitz constant for the \emph{softmax} function reported in the literature~\citep{gouk2021regularisation} and \emph{Sigmoid} function reported in the literature~\citep{virmaux2018lipschitz} as 1. \textcolor{black}{We show in Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Softmax} that the exact Lipschitz constant of \emph{softmax} is indeed $\frac{1}{2}$, validated by our numerical experiment.} This result has been reported in recent concurrent literature \citep{nair2025softmax}. We also show in Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Sigmoid} that exact Lipschitz constant of \emph{sigmoid} is indeed $\frac{1}{4}$, validated by our numerical experiment. For \emph{Leaky ReLU} and \emph{ELU}, the parameter $\alpha$ is typically chosen with $\alpha < 1$, so their effective Lipschitz constants are usually $1$ in practice.

\textbf{Auto-Differentiation based Numerical Method.} Suppose $f: \mathbb{R}^{d} \to \mathbb{R}$ is a first- and second-order differentiable neural network under domain convex condition (Remark~\ref{remark:domain_convex}). Leveraging the autograd mechanism of PyTorch, we use gradient descent --- \eg, Adam \citep{diederik2014adam} --- to numerically approximate the supremum:
\begin{align}
    \mathrm{Lip}[f] = \sup_x \|f'(x)\|_2 \notag
    ,
\end{align}
using Lemma~\ref{lemma:lipschitz_bounds_gradient}.

\begin{table}[H]
\centering

\caption{Lipschitz constants of activation functions.}

\label{tab:lipschitz_activations}
\renewcommand{\arraystretch}{1.2}

\adjustbox{max width=0.9\textwidth}{%
\begin{tabular}{|l|c|c|p{6.2cm}|}
\hline
\textbf{Activation} & \textbf{Definition} & \textbf{Lipschitz Constant \& Proof} & \textbf{Citations} \\
\hline
ReLU & $ \max(0, x) $ & $ 1 $ &\citet[Sec.~2]{nair2010relu}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Leaky ReLU & $ \max(\alpha x, x) $ & $ \max(1, \alpha) $ & \citet[Sec.~2]{maas2013leakyrelu}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Sigmoid & $ \frac{1}{1 + e^{-x}} $ & $ \frac{1}{4} $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Sigmoid}) & \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Tanh & $ \tanh(x) $ & $ 1 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Tanh}) &\citet{cybenko1989approximation}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Softplus & $ \log(1 + e^x) $ & $ 1 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Softplus}) &\citet[Sec.~2]{dugas2001softplus}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
ELU & $ \begin{cases} x & x > 0 \\ \alpha (e^x - 1) & x \leq 0 \end{cases} $ & $ \max(1, \alpha) $ &\citet[Sec.~3]{clevert2015elu}\\
\hline
Swish & $ x \cdot \sigma(x) $ & $ \approx 1.1 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Swish}) &\citet[Sec.~1]{ramachandran2017searching} \\
\hline
GELU & $ \frac{x}{2}\left(1+\mathrm{erf}\left(\frac{x}{\sqrt{2}}\right)\right) $ & $ \approx 1.13 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:GELU}) &\citet[Sec.~2]{hendrycks2016gelu} \\
\hline
Softmax & $ \text{softmax}(x_i) = \frac{e^{x_i}}{\sum_j e^{x_j}} $ & $\frac{1}{2}$ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Softmax}) &\citet[Sec.~3.3]{gouk2021regularisation}\\
\hline
\end{tabular}
}
\end{table}

\subsection{Lipschitz Continuity of Dot-Product Self-Attention}
\label{sec:selfattention_lipschitz}

LLMs \citep{brown2020language, chowdhery2022palm, touvron2023llama,openai2023gpt4,deepseekai2025deepseekr1}, built on transformer architectures \citep{vaswani2017attention}, rely heavily on dot-product self-attention mechanisms, whose Lipschitz continuity governs their sensitivity to input perturbations, such as token-level adversarial attacks. Dot-product self-attention mechanisms form the core of transformer architectures, enabling effective modeling of long-range dependencies in sequences for applications such as natural language processing and vision-language tasks. 

\paragraph{Single-Head Dot-Product Self-Attention.} For an input sequence matrix $x \in \mathbb{R}^{n \times d}$, where $n$ is the sequence length and $d$ is the input dimension, a self-attention layer computes the output as
\begin{align}
\text{Attention}(x) = 
\underbrace{
\mathrm{softmax}\left( \frac{Q K^{\top}}{\sqrt{d_K}} \right)
}_{\text{row-wise softmax}}
V \in \mathbb{R}^{n \times m} 
,\label{eq:shdp_attention}
\end{align}
\citep[Equation~1]{vaswani2017attention} where
\begin{align}
Q = x W_Q \in \mathbb{R}^{n \times m}, \quad K = x W_K \in \mathbb{R}^{n \times m}, \quad V = x W_V \in \mathbb{R}^{n \times m} \label{eq:KQV_def}
,
\end{align}
are the \emph{query}, \emph{key}, and \emph{value} matrices, with weight matrices:
\begin{align}
W_Q, W_K, W_V \in \mathbb{R}^{d \times d_K}\notag
,    
\end{align}
and $d_K$ denotes the key (and query) vector dimension. The softmax is applied row-wise to normalize attention scores. The scaling factor $\frac{1}{\sqrt{d_K}}$ stabilizes the computation numerically. 

\paragraph{Multi-Head Dot-Product Self-Attention.} 
In practice, transformers employ $h$ parallel self-attention heads to jointly attend to information from different representation subspaces \citep{vaswani2017attention}. Each head $i$ has its own projection matrices:
\begin{align}
W_{Q,i}, W_{K,i}, W_{V,i} \in \mathbb{R}^{d \times m_i}\notag
,   
\end{align}
where $m_i = \frac{m}{h}$, $h$ denotes the number of heads, and produces an output for head $i$:
\begin{align}
\mathrm{Attention}_i(x) \in \mathbb{R}^{n \times m_i}
.
\end{align}
The outputs are concatenated:
\begin{align}
\mathrm{Attention}(x) =\bigl[
\mathrm{Attention}_1(x),\mathrm{Attention}_2(x), \cdots, \mathrm{Attention}_h(x)
\bigr]    \in \mathbb{R}^{n \times m} 
,
\end{align}
produces the final output.









\paragraph{Locally Lipschitz Continuous.} Standard dot-product self-attention is locally Lipschitz continuous, and several works have derived explicit upper bounds for its local Lipschitz constant. Let $\mathcal{B}(x_0,\delta)=\{x \mid \|x-x_0\|_2 < \delta \}$ denote a ball centered $x_0$ with a radius $\delta$. \citeauthor{hu2024specformer} show that for the dot-product self-attention layer within a ball $\mathcal{B}_2(x,\delta)$ is locally Lipschitz continuous bounded by:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}; \mathcal{B}_2(x,\delta)\Bigr] 
    \leq
    n(n+1)\Bigl(\|x\|_2 + \delta\Bigr)^2
    \Bigl[
    \|W_V\|_2
    \|W_Q\|_2
    \|W_K^\top\|_2
    +
    \|W_V\|_2
    \Bigr] 
    ,
\end{align}
where $x \in \mathbb{R}^{n \times d}$, $n$ is the sequence length, $d$ is the input dimension, $W_K, W_Q, W_V \in \mathbb{R}^{d \times d_K}$ are the \emph{key}, \emph{query} and \emph{value} parameter matrices, and $\delta$ is a $2$-norm radius \citep[Theorem~2]{hu2024specformer}. \citeauthor{castin2023smooth} provide a tighter bound by $\sqrt{n}$ up to a constant factor, showing that within a ball $\mathcal{B}_2(0, \delta)$, the Lipschitz constant of dot-product self-attention is bounded by:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}; \mathcal{B}_2(0,\delta)\Bigr] 
    \leq
    \sqrt{3} \|W_V\|_2 
    \Biggl[
    \Bigl\|\frac{W_K^\top\,W_Q}{\sqrt{d_K}}\Bigr\|_2^2
    \delta^4
    (4n+1)+n
    \Biggr]^{\frac{1}{2}} 
    ,
\end{align}
where $A$ is the attention score matrix \citep[Theorem~3.3]{castin2023smooth}. 

Most recently, \citet{yudin2025pay} refine the bound by explicitly incorporating the Jacobian of the softmax function, given by:
\begin{align}
\mathcal{M}(P_x) := \nabla \, \mathrm{softmax}\left(x\right) = 
\mathrm{diag}(P_x) - P_x P_x^\top 
,
\end{align}
where:
\begin{align}
    P_x =
    \frac{\mathrm{e}^{x_i}}{\sum_j \mathrm{e}^{x_j}}
    \notag
    ,
\end{align}
showing that the Lipschitz constant for a single head is bounded by:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}\Bigr] 
    \leq
    \|W_V\|_2
    \Biggl(
    \|P\|_2 + 2 \|x\|_2^2 \; \|A\|_2 \; \max_i \|\mathcal{M}(P_{i, :})\|_2
    \Biggr)
\end{align}
with:
\begin{align}
    P = \mathrm{softmax}\Bigl(
    x
    A
    x^\top
    \Bigr) \in \mathbb{R}^{n \times n} \qquad \text{and} \qquad A = \frac{W_QW_K^\top}{\sqrt{d_K}} \in \mathbb{R}^{d \times d} \notag
\end{align}
\citep[Theorem~3]{yudin2025pay}. 




\paragraph{Globally Non-Lipschitz Continuous.} It is worth noting that the Lipschitz constants of both single-head and multi-head dot-product self-attention are usually not globally bounded for arbitrary inputs. This is because the Lipschitz bound for dot-product self-attention grows with the sequence length and input norm itself, implying that the dot-product self-attention is not globally Lipschitz continuous \citep[Theorem~3.1]{kim2021lipschitz}. 










\subsection{Lipschitz Continuity of Neural Networks}
\label{sec:network_lipschitz}

\begin{definition}[Feedforward Network (Compositional Definition)]
Let $f: \mathbb{R}^m \to \mathbb{R}^n$ denote a feedforward neural network consisting of $L$ layers, defined as the composition:
\begin{align}
    f := h^{(L)} \circ \cdots \circ h^{(2)} \circ h^{(1)}, \notag
\end{align}
where each layer $h^{(\ell)}$ is composed of a linear transformation $\phi^{(\ell)}(\cdot)$ followed by a non-linear activation function $\rho^{(\ell)}(\cdot)$:
\begin{align}
    h^{(\ell)} := \rho^{(\ell)} \circ \phi^{(\ell)}. \notag
\end{align}
\end{definition}


\begin{proposition}[Lipschitz Constant of a Linear Layer]
\label{prop:lipschitz_constant_of_linear_unit}
Let $\phi^{(\ell)}: \mathbb{R}^{m_{\ell}} \to \mathbb{R}^{n_{\ell}}$ denote a linear transformation implemented either as a convolutional layer:
\begin{align}
    \phi^{(\ell)}(z^{(\ell-1)}) = \boldsymbol{\theta}^{(\ell)} \circledast z^{(\ell-1)} + b^{(\ell)}, \notag
\end{align}
or as a fully connected (dense) layer:
\begin{align}
    \phi^{(\ell)}(z^{(\ell-1)}) = \boldsymbol{\theta}^{(\ell)} z^{(\ell-1)} + b^{(\ell)},\notag
\end{align}
where $\boldsymbol{\theta}^{(\ell)}$ is the weight matrix (or convolution kernel), $b^{(\ell)}$ is the bias term, $\circledast$ denotes the convolution operator, and $z^{(\ell-1)}$ is the output from the previous layer. The Lipschitz constant of $\phi^{(\ell)}$ with respect to the Euclidean norm is given by:
\begin{align}
    \mathrm{Lip}[\phi^{(\ell)}] = \| \boldsymbol{\theta}^{(\ell)} \|_2,\notag
\end{align}
where $\| \boldsymbol{\theta}^{(\ell)} \|_2$ denotes the spectral-norm of the associated linear operator.
\end{proposition}


\begin{proposition}[Spectral-Norm via Truncated Singular Value Decomposition]
\label{prop:spectralnorm_bound_single_layer}
Let $\boldsymbol{\theta} \in \mathbb{R}^{n \times m}$ be a matrix, admitting a truncated singular value decomposition (SVD):
\begin{align}
\boldsymbol{\theta} = \sum_{i=1}^{r} \sigma_i \boldsymbol{u}_i \boldsymbol{v}_i^\top,
\quad \text{with} \quad \sigma_1 > \sigma_2 > \cdots > \sigma_r > 0,
\quad r = \operatorname{rank}(\boldsymbol{\theta}), \notag
\end{align}
where $\sigma_i$ are the singular values, and $\boldsymbol{u}_i$, $\boldsymbol{v}_i$ are the left and right singular vectors, respectively. Then, the spectral-norm of $\boldsymbol{\theta}$ (\ie, its operator norm induced by the Euclidean norm) is given by the largest singular value:
\begin{align}
    \| \boldsymbol{\theta} \|_2 = \sigma_1 \notag
\end{align}
 \citep[Example 5.6.6, \S~5]{horn2012matrix}.
\end{proposition}

\begin{proposition}[Lipschitz Constant Upper Bound of Feedforward Neural Network]
\label{prop:survey_upper_bound_lipschitz}
Let $f: \mathbb{R}^m \to \mathbb{R}^n$ be an $L$-layer feedforward neural network composed of linear transformations $\phi^{(\ell)}$ and activation functions $\rho^{(\ell)}$. The Lipschitz constant of $f$ with respect to the Euclidean norm is defined as:
\begin{align}
\mathrm{Lip}[f] = \sup_{\forall~u \neq v} \frac{\|f(u) - f(v)\|_2}{\|u - v\|_2},
\end{align}
which immediately admits an upper bound by applying Proposition~\ref{prop:lipschitz_composition}~(\nameref{prop:lipschitz_composition}):
\begin{align}
    \mathrm{Lip}[f] 
    \leq 
    \prod_{\ell=1}^{L} \; \mathrm{Lip}[\rho^{(\ell)}] 
    \;
    \prod_{\ell=1}^{L} \; \mathrm{Lip}[\phi^{(\ell)}]
\end{align}
\citep[Proposition 8, \S~5]{luo2025lipschitz}. 
\end{proposition}

\begin{corollary}[Spectral-Norm Upper Bound of Feedforward Neural Network]
For an $\ell$-layer feedforward network $f$ with only linear or convolutional layers and $1$-Lipschitz activation functions, combining
Proposition~\ref{prop:lipschitz_constant_of_linear_unit} and Proposition~\ref{prop:survey_upper_bound_lipschitz} immediately yields a spectral-norm product bound:
\begin{align}
    \mathrm{Lip}\left[f\right] \leq \prod_{\ell=1}^{L} \| \theta^{(\ell)} \|_2
    ,
\end{align}
where $\theta^{(\ell)}$ is the $\ell$-th layer parameter matrix. 
\end{corollary}



\subsubsection{Lipschitz Continuity for a Directed Acyclic Graph (DAG)}


\begin{figure}[t!]
  \centering
  \begin{tikzpicture}[
    ->, 
    node distance=1.8cm and 2cm,
    every node/.style={circle, draw, minimum size=10mm},
    shorten >=1pt]

\node (s)  at (0, 0)       {$s$};
\node (u1) at (2, 2.5)     {$u_1$};
\node (u2) at (2, 0.8)     {$u_2$};
\node (u3) at (2, -0.8)    {$u_3$};
\node (v)  at (4, 0)       {$v$};
\node (t)  at (6, 0)       {$t$};

\draw (s) to[out=90, in=180] (u1);
\draw (s) to[out=45, in=180] (u2);
\draw (s) to[out=-45, in=180] (u3);

\draw (u1) to[out=0, in=90] (v);
\draw (u2) to[out=0, in=130] (v);
\draw (u3) to[out=0, in=220] (v);

\draw (v) -- (t);

\draw (s) to[out=-90, in=-90] (t);

\end{tikzpicture}

  \caption[Example of Feedforward DAG Network]{Example of Feedforward DAG Network. There are four computational paths: $s\to u_1 \to v \to t$, $s\to u_2 \to v \to t$, $s\to u_3 \to v \to t$, and $s\to t$. A node is a module in the DAG neural network $f$.}
  
  \label{fig:dag_network}
\end{figure}

To the best of our knowledge, the existing literature does not present an explicit Lipschitz bound for a general feedforward network with skip connections. Prior literature such as \citep{virmaux2018lipschitz} focuses strictly on sequential architectures, while norm-based capacity measures such as the path norm \citep{neyshabur2015norm} implicitly involve path enumeration but are not formulated as direct Lipschitz bounds. More recent path-metric bounds \citep{gonon2024_rescaling_invariant} apply to arbitrary DAGs but are expressed in a rescaling-invariant metric form rather than the simple sum-over-paths structure we consider. 

Figure \ref{fig:dag_network} provides an illustrative example of a DAG network. To complement the survey, we derive an explicit bound in Theorem \ref{thm:path_lipschitz_general} using graph-theoretic method. To the best of our knowledge, this result has not previously appeared in the literature.



\begin{theorem}[Lipschitz Bound for DAG Network]
\label{thm:path_lipschitz_general}
Let $G=(V,E)$ be a finite directed acyclic graph (DAG) representing a feedforward neural network with unique input node $s\in V$ and output node $t\in V$.  
Each node $v \in V$ is a module $h_v$ that is Lipschitz continuous with constant $\mathrm{Lip}[h_v]$.  
An edge $(u \to v) \in E$ represents the computation of $h_v$ immediately after $h_u$. Let $x_{v_i}: x \to x_{v_i}(x)$ represent the output at a node $v_i \in V$. The network is evaluated additively along incoming edges:
\begin{align}
\begin{cases}
x_s(x) = x  &\\
x_v(x) = \sum_{(u\to v)\in E} h_v\!\big(x_u(x)\big), &\text{if} \quad v\neq s 
\end{cases}
.
\end{align}

A \emph{computational path} $p$ from $s$ to $t$ is an ordered sequence of nodes
\begin{align}
p = (v_0=s, v_1, \dots, v_{L_p}=t), \notag
\end{align}
where $(v_{i-1} \to v_i) \in E$ for all $i=1,\dots,L_p$.
Define for each edge $(u\to v)$ the constant
\begin{align}
C_{(u\to v)} := \mathrm{Lip}[h_v], 
\end{align}
and for a path $p$ set
\begin{align}
C_p := \prod_{i=1}^{L_p} \mathrm{Lip}[h_{v_i}]
= \prod_{i=1}^{L_p} C_{(v_{i-1}\to v_i)}. 
\end{align}
Let $\mathcal{P}$ be the set of all such paths from $s$ to $t$.  
Then the Lipschitz constant of the overall network $f(x):=x_t(x)$ satisfies
\begin{align}
\mathrm{Lip}[f] \;\le\; \sum_{p \in \mathcal{P}} C_p.
\end{align}
\end{theorem}





\begin{proof}
Fix any topological order of $V$. For $v\in V$, define the scalar
\begin{align}
S(v) := 
\begin{cases}
1, & v=s,\\[2pt]
\displaystyle \sum_{(u\to v)\in E} C_{(u\to v)}\, S(u), & v\neq s.
\end{cases}
\end{align}
\emph{Claim:} for all $v\in V$,
\begin{align}
\label{eq:node_lip_bound}
\mathrm{Lip}[x_v] \;\le\; S(v).
\end{align}
We prove \eqref{eq:node_lip_bound} by induction along the topological order.

\paragraph{Base case ($v=s$).} Considering $x_s(x)=x$, hence base case holds true:
\begin{align}
\mathrm{Lip}[x_s]=1=S(s) 
.\notag
\end{align}


\paragraph{Inductive step.} Let $v\neq s$ and assume \eqref{eq:node_lip_bound} holds for all predecessors $u$ of $v$. Applying Minkowski inequality, for any $x,y$ in the input space,
\begin{align}
\|x_v(x)-x_v(y)\|
&= \left\| \sum_{(u\to v)} h_v\big(x_u(x)\big) - \sum_{(u\to v)} h_v\big(x_u(y)\big) \right\| \notag\\
&\le \sum_{(u\to v)} \big\| h_v\big(x_u(x)\big) - h_v\big(x_u(y)\big) \big\| \notag\\
&\le \sum_{(u\to v)} \mathrm{Lip}[h_v] \,\big\| x_u(x) - x_u(y) \big\| \notag\\
&\le \sum_{(u\to v)} \mathrm{Lip}[h_v] \,\mathrm{Lip}[x_u] \,\|x-y\| \notag\\
&= \sum_{(u\to v)} C_{(u\to v)}\, \mathrm{Lip}[x_u] \,\|x-y\| \notag\\
&\le \left( \sum_{(u\to v)} C_{(u\to v)}\, S(u) \right) \|x-y\| = S(v)\,\|x-y\| \notag
,
\end{align}
since inductive hypothesis:
\begin{align}
\mathrm{Lip}[x_u] \le S(u) \notag
,
\end{align}
so that $\mathrm{Lip}[x_v]\le S(v)$. In particular,
\begin{align}
\mathrm{Lip}[f]=\mathrm{Lip}[x_t] \;\le\; S(t). \notag
\end{align}

It remains to show $S(t)=\sum_{p\in\mathcal P} C_p$. More generally:

\begin{lemma}[Lemma (Path expansion of $S$)]
\label{lemma:path-expansion}
For every $v\in V$, the path extension of $S$ holds:
\begin{align}
\label{eq:path-expansion}
S(v) = \sum_{p\in\mathcal P(s\to v)} \prod_{e\in p} C_e , 
\end{align}
where $\mathcal P(s\to v)$ is the set of all directed paths from $s$ to $v$.    
\end{lemma}

\begin{proof}
Proceed again by induction in topological order. For $v=s$, $\mathcal P(s\to s)$ contains only the empty path with product $1$, so \eqref{eq:path-expansion} holds.
Assume \eqref{eq:path-expansion} holds for all predecessors $u$ of $v$. Then
\begin{align}
S(v)
&= \sum_{(u\to v)} C_{(u\to v)}\, S(u) \\
&= \sum_{(u\to v)} C_{(u\to v)} \left( \sum_{p\in\mathcal P(s\to u)} \prod_{e\in p} C_e \right) \notag\\
&= \sum_{(u\to v)} \sum_{p\in\mathcal P(s\to u)} \left( \prod_{e\in p} C_e \right) C_{(u\to v)}. \notag
\end{align}
Concatenating each $p\in\mathcal P(s\to u)$ with the edge $(u\to v)$ yields a bijection onto $\mathcal P(s\to v)$, and multiplies the edge constants accordingly; thus \eqref{eq:path-expansion} holds for $v$.
\end{proof}

Applying Lemma~\ref{lemma:path-expansion} at $v=t$ gives $S(t)=\sum_{p\in\mathcal P} C_p$, and hence
\begin{align}
\mathrm{Lip}[f] \;\le\; S(t) = \sum_{p\in\mathcal P} \prod_{i=1}^{L_p} \mathrm{Lip}[h_{v_i}] \notag
,
\end{align}
which is the claim as demonstrated.
\end{proof}

\begin{figure}[t!]
  \centering
  \resizebox{0.9\linewidth}{!}{
  \begin{tikzpicture}[
    ->, 
    node distance=1.8cm and 2cm,
    every node/.style={circle, draw, minimum size=10mm},
    shorten >=1pt]


    \node[circle, fill=gray!20, inner sep=10pt] (S1) {$S_1$};
    
    \node[circle, inner sep=1.5pt, right = of S1, xshift=-1cm] (a1) {$a_1$};

    \node[circle, fill=gray!20, inner sep=10pt, right=of a1,xshift=-1cm] (S2) {$S_2$};

    \node[circle, inner sep=1.5pt, right = of S2,xshift=-1cm] (a2) {$a_2$};


    \node[circle, inner sep=1.5pt, right = of a2] (aLminusOne) {$a_{L-1}$};
    
    \node[circle, fill=gray!20, inner sep=10pt, right=of aLminusOne,xshift=-1cm] (SL) {$S_L$};


    \draw (S1) -- (a1);
    \draw (a1) -- (S2);
    \draw (S2) -- (a2);
    \draw[dashed] (a2) -- (aLminusOne);
    \draw (aLminusOne) -- (SL);
    
\end{tikzpicture}
}

  \caption[Non-Biconnected DAG Network]{Topology of non-biconnected DAG network. If a DAG is separated into two sub-DAGs by the removal of a vertex $a_i$, then $a_i$ is referred to as a \emph{cut vertex} (or \emph{articulation point}), and the DAG is said to be \emph{non-biconnected}. This diagram shows the topology for a DAG that contains $L-1$ articulation points $a_1, a_2, \dots, a_{L-1}$ and $L$ corresponding sub-DAGs $S_1, S_2, \dots, S_L$.}
  
  \label{fig:nonbiconnected_dag_network}
\end{figure}

\subsubsection{Lipschitz Constant of Non-Biconnected DAG}


If a DAG is separated into two disconnected sub-DAGs by the removal of a vertex, then the removed vertex is referred to as \emph{cut vertex} or \emph{articulation point}. Modern deep learning architectures often give rise to computation DAGs that are not biconnected: the DAGs can be separated into multiple subgraphs by removing a small set of vertices. 


\begin{theorem}[Lipschitz Bound for Non-Biconnected DAG Network]
\label{thm:nonbiconnected_dag_lipschitz}
Figure~\ref{fig:nonbiconnected_dag_network} shows the typical non-biconnected DAG topology found in modern deep learning architectures. The DAG contains a set of cut vertices $a_1,a_2, \cdots, a_{L-1}$ and biconnected DAGs $S_1,S_2,\cdots,S_L$. Suppose the DAG network $f$ in Figure~\ref{fig:nonbiconnected_dag_network} is:
\begin{align}
    f= S_L\,\circ\,a_{L-1}\,\cdots\,a_2\,\circ\,S_2\,\circ\,a_1\,\circ\,S_1 \notag
    ,
\end{align}
then it is not difficult to show that the Lipschitz constant bound of this DAG is:
\begin{align}
\label{equ:nonbiconnected_dag_lipschitz}
\mathrm{Lip}\left[ f \right] \leq 
\Biggl(
\prod_{i=1}^{L}    \mathrm{Lip}\left[ S_i \right] 
\Biggr)
\Biggl(
\prod_{j=1}^{L-1}    \mathrm{Lip}\left[ a_j \right]
\Biggr) 
,
\end{align}
where the Lipschitz bound of each sub-DAG $\mathrm{Lip}\left[ S_i \right]$ is given by Theorem~\ref{thm:path_lipschitz_general} (\nameref{thm:path_lipschitz_general}).
\end{theorem}

\begin{remark}
Theorem~\ref{thm:nonbiconnected_dag_lipschitz} (\nameref{thm:nonbiconnected_dag_lipschitz}) is particularly valuable for estimating the Lipschitz bound of a deep model. In contrast to path-based bound of Theorem~\ref{thm:path_lipschitz_general} (\nameref{thm:path_lipschitz_general}), which can be quite loose due to its combinatorial dependence on the number of paths, Theorem~\ref{thm:nonbiconnected_dag_lipschitz} yields significantly tighter and more structurally informed bounds.
\end{remark}



\subsubsection{Lipschitz Constant of Residual Network}
\label{sec:lipschitz_of_residual_module}

Residual networks \citep{he2016deep} address the optimization challenges of very deep neural architectures by introducing \emph{residual modules}, which are illustrated in Figure~\ref{fig:residual_module}. Each module $m_{\mathrm{res}}$ has the structure:
\begin{align}
    m_{\mathrm{res}}(x) = x + \phi(x), \notag
\end{align}
which consists of a non-identity unit $\phi$ and an identity skip connection. The resulting residual mapping $m_{\mathrm{res}}(x)$ maintains stable gradient flow, mitigates vanishing-gradient effects, and enables the training of substantially deeper networks without degradation. This simple architectural principle has proven highly effective and forms the backbone of many state-of-the-art deep learning models. Using Theorem~\ref{thm:path_lipschitz_general} (\nameref{thm:path_lipschitz_general}), it is not difficult to show that the Lipschitz constant bound of this structure is:
\begin{align}
    \mathrm{Lip}\left[m_{\mathrm{res}}\right] \leq 
    \mathrm{Lip}\left[s\right] +\mathrm{Lip}\left[\phi\right] = 
    1 + \mathrm{Lip}\left[\phi\right] \notag
    ,
\end{align}
which recovers the same results in \citep[Lemma 2, \S~2]{Behrmann2019InvertibleResidual}, \citep[\S~3.4]{gouk2021regularisation} and Proposition~\ref{prop:lipschitz_composition}~(\nameref{prop:lipschitz_composition}) by setting $s$ to an identity map.

\begin{figure}[t!]
    \centering

    \begin{tikzpicture}[>=latex, node distance=2.5cm, thick]

  \node (x) {$x$};

  \node[circle, fill=black, inner sep=1.5pt, right=of x, xshift=-1.5cm] (input) {};
  
  \node[draw, rectangle, minimum width=1.5cm, minimum height=1cm, right=of input, xshift=-1.5cm] (phi) {$\phi$};
  
  \node[circle, draw, right=of phi, inner sep=1pt, minimum size=0.6cm, xshift=-1.5cm] (sum) {$+$};
  
  \node[right=of sum, xshift=-1.5cm] (z) {$z$};

  \draw[->] (x) -- (phi);
  \draw[->] (phi) -- (sum);

  \draw[->] ($(input) + (0,0)$) |- ([yshift=0.8cm]sum.north) -- node[above, xshift=-2.cm,yshift=0.4cm] {$s$} (sum);

  \draw[->] (sum) -- (z);

\end{tikzpicture}


    \caption[Structure of Residual Module]{A residual module $m(x)=x + \phi(x)$ consists of a non-identity unit $\phi: x \mapsto \phi(x)$ and an identity skip connection unit $s: x \mapsto x$.}
    
    \label{fig:residual_module}
    
\end{figure}





\subsection{Complexity-Theoretic Generalization Bound}
\label{sec:generalization_bounds}


\paragraph{Notations.} Let $\mathcal{H}$ be a hypothesis family and $\mathcal{H} \ni h: X \to Y$ be a hypothesis. Let $\ell: Y \times Y \to \mathbb{R}$ be a loss function. For each $\ell(h(x), y)$, we can associate $\ell$ and $h$ with a map $G \ni g: X \times Y \to \mathbb{R}$, where $G$ is the family of loss functions associated with the hypothesis family $\mathcal{H}$.

%The generalization capacity of a neural network is fundamentally governed by its Lipschitz constant \citep{mohri2018foundations}. 

Lipschitz constants can enter complexity--theoretic generalization bounds and often interact with capacity, robustness, and smoothness~\citep{mohri2018foundations}. To quantify this capacity for a hypothesis, the concept of \emph{generalization gap} is often used to measure the error between \emph{true risk} and \emph{empirical risk} (Definition~\ref{def:generalization_gap}). This gap for a model $h \in \mathcal{H}$ is proportional to its empirical Rademacher complexity of the hypothesis family $\mathcal{H}$, and the empirical Rademacher complexity is proportional to the Lipschitz constant $\mathrm{Lip}\left[\mathcal{H}\right]:=\sup_{h \in \mathcal{H}} \mathrm{Lip}\left[h\right]$ of the hypothesis family:
\begin{align}
\text{Generalization gap of $h$} \sim \text{Rademacher complexity} \sim O(\mathrm{Lip}\left[\mathcal{H}\right]) \notag
\end{align}
(\citealp[\S~3]{mohri2018foundations}; \citealp[Part IV]{shalev2014understanding}). A smaller Lipschitz constant enforces smoother mappings, reducing the complexity of the function class and mitigating overfitting, thereby enhancing robustness to noise and adversarial perturbations \citep{neyshabur2015norm,gouk2021regularisation,castin2023smooth}. 



\begin{definition}[Generalization Gap]
\label{def:generalization_gap}
Let $S:=\{(x_i,y_i)\}_{i=1}^m$ be a dataset where $(x_i,y_i)$ is sampled \emph{i.i.d.} from an unknown distribution $\mathcal{D}_X$. The true (population) risk for hypothesis $h$ is defined as:
\begin{align}
    R(h) := \mathbb{E}_{(x,y)\sim\mathcal{D}_X}[\ell(h(x),y)]
    ,\notag
\end{align}
and the empirical risk on $S$ is defined as:
\begin{align}
   R_S(h) :=  \frac{1}{m} \sum_{i=1}^m \ell(h(x_i), y_i)  \notag
\end{align}
(\citealp[\S~3]{mohri2018foundations}; \citealp[Part IV]{shalev2014understanding}). Accordingly, the generalization gap on $S$ is given by:
\begin{align}
     R(h) - R_S(h). \notag
\end{align}

\end{definition}







\subsubsection{Rademacher Complexity and its Bounds}


In learning theory, \emph{Rademacher complexity} quantifies the expressiveness of a hypothesis family $G:=\{g: X \to \mathbb{R}\}$ by measuring how well the $G$ can fit data associated with random labels \citep[\S~3.1]{mohri2018foundations}. Let $S = (x_1, x_2, \dots, x_m)$ be a dataset of size $m$ with each $x_i \in X$ drawn i.i.d. from an unknown distribution $\mathcal{D}_X$. Let $h : X \to \mathbb{R}$ be a hypothesis that assigns a real-valued score to each input. Let $\sigma_1, \dots, \sigma_m$ be $m$ independent \emph{Rademacher variables}, \ie, random variables uniformly distributed over $\{-1, +1\}$ \citep[\S~3.1]{mohri2018foundations}. For random labels $\sigma_1, \dots, \sigma_m$ assigned to $S$, the maximal correlation between the labels and the predictions of hypotheses in $\mathcal{H}$ is given by
\begin{align}
    \sup_{g \in G} \frac{1}{m} \sum_{i=1}^m \sigma_i g(x_i). \notag
\end{align}
By assigning all possible random labels to the dataset $S$, we can thus define \emph{Rademacher Complexity} for hypothesis family $\mathcal{G}$, stated in Definition~\ref{def:empirical_rademacher} (\nameref{def:empirical_rademacher}).


\begin{definition}[Rademacher Complexity {\citep[Definition 3.1, \S~3]{mohri2018foundations}}]
\label{def:empirical_rademacher}
The \emph{empirical Rademacher complexity} of $G$ with respect to $S$ is defined as
\begin{align}
\widehat{\mathfrak{R}}_S(G)
:= \mathbb{E}_{\sigma} \left[ \sup_{g \in G} \frac{1}{m} \sum_{i=1}^m \sigma_i g(x_i) \right], \notag
\end{align}
and the (expected) \emph{Rademacher complexity} is the expectation of $\widehat{\mathfrak{R}}_S(G)$ over all dataset $S$ of size $m$:
\begin{align}
\mathfrak{R}_m(G)
:= \mathbb{E}_{S \sim \mathcal{D}_X^m} \left[ \widehat{\mathfrak{R}}_S(G) \right]
,\notag
\end{align}
where $S \sim \mathcal{D}_X^m$ denotes $m$ samples i.i.d. drawn from $\mathcal{D}$. 
\end{definition}


In the paradigm of machine learning, for the case of the hypothesis family $\ell\circ \mathcal{H}$ is the composition of a model $h \in \mathcal{H}:=\{h:\mathbb{R}^n \to \mathbb{R} \}$ and loss function $\ell: \mathbb{R} \to \mathbb{R}$:
\begin{align}
    \ell\circ \mathcal{H} := \{\ell\circ h \mid h \in \mathcal{H}\}, \notag
\end{align}
by Talagrand's Contraction Lemma \citep[Lemma 4.2, \S~4]{mohri2018foundations}, the empirical Rademacher complexity of $\ell\circ \mathcal{H}$ on $S$ admits:
\begin{align}
    \widehat{\mathfrak{R}}_S(\ell\circ \mathcal{H}) \leq 
    \mathrm{Lip}\left[\ell\right] \;\widehat{\mathfrak{R}}_S(\mathcal{H}) 
    . \notag
\end{align}

For any $\delta > 0$, with probability at least $1-\delta$, the generalization gap for $h \in \mathcal{H}$ on $S$ is bounded by empirical Rademacher complexity of $\ell\circ \mathcal{H}$:
\begin{align}
    R(h) - R_S(h) \leq 2 \;\widehat{\mathfrak{R}}_S(\ell\circ\mathcal{H}) + 
    3 \sqrt{\frac{\log{\frac{2}{\delta}}}{2m}}
    \leq
    2\; \mathrm{Lip}\left[\ell\right] \;\widehat{\mathfrak{R}}_S(\mathcal{H}) + 3 \sqrt{\frac{\log{\frac{2}{\delta}}}{2m}}
\end{align}
\citep[Theorem 3.1 \& Theorem 3.3, \S~3]{mohri2018foundations}.


For general vectorized function, let:
\begin{align}
\Phi:=\{\phi: \mathbb{R}^n \to \mathbb{R}^n \mid \phi~\text{is a coordinate-wise identity map}\}   
\notag
\end{align}
be a coordinate-wise identity family. For vectorized function $h: \mathbb{R}^n \to \mathbb{R}^k$ and compositional hypothesis $h \circ \Phi$, suppose $h_i$ is $K$-Lipschitz continuous, using vector contraction theorem \citep[Equation 1 \& Corollary 4]{Maurer2016Contraction} yields:
\begin{align}
\widehat{\mathfrak{R}}_S(h \circ \Phi)  
&\leq
\sqrt{2} \; K \; \frac{1}{m} \; \mathbb{E}\Bigl[ \sup_{\phi \in \Phi} \sum_{i=1}^m \sum_{j=1}^n \sigma_{ij} \phi_j(x_i)\Bigr] \notag\\
&\leq \sqrt{2} \; K \; \frac{1}{m} \; \sum_{i=1}^m \sum_{j=1}^n 
\bigl|\phi_j(x_i)\bigr| = \sqrt{2} \; K \; \frac{1}{m} \; \sum_{i=1}^m \Biggl(\sum_{j=1}^n 
\bigl|x_{i:j}\bigr| \Biggr) = \sqrt{2} \; K \; \frac{1}{m} \; \sum_{i=1}^m \bigl\|x_i\bigr\|_1 \notag \\
&\leq \sqrt{2} \; K \; \frac{1}{m} \; m \; \sup_{x \in S} \bigl\| x \bigr\|_1 = \sqrt{2} \; K \; \sup_{x \in S} \bigl\| x \bigr\|_1
,
\end{align}
where $\sigma_{ij}$ are an $m \times n$ matrix of independent Rademacher variables, $x_{i:j}$ denotes the $j$-th component of the $i$-th data point, and $\sup_{x \in S} \bigl\| x \bigr\|_1$ is the $1$-norm dataset diameter. This result implies that Lipschitz constant of $h$ controls its generalization bound:
\begin{align}
    R(h) - R_S(h) \leq \mathcal{O}(K)
    .
\end{align}



































\subsection{Training Dynamics of Lipschitz Continuity}
\label{sec:optimization_induced_dynamics}



The Lipschitz continuity of a parameterized network evolves as optimization updates its parameters. Consequently, the optimization process induces the dynamics of the network's Lipschitz continuity. While existing work in deep learning theory has largely focused on bounding the Lipschitz constants of neural networks, understanding how Lipschitz continuity evolves throughout training remains an open problem. Only a few studies have begun to explore this aspect. In particular, \citet{luo2025lipschitz} introduces the concept of \emph{optimization-induced dynamics} and establishes a continuous-time stochastic framework that explicitly links the optimization process to the time-varying Lipschitz continuity bound of deep networks. The literature \citep{luo2025lipschitz} uses the operator-theoretical results regarding how the largest singular values of parameter matrices vary with respect to perturbations from the literature \citep{luo2025spectralvariation}, along with the theory from high-dimensional stochastic differential equations (SDEs) from stochastic analysis, for establishing a mathematical framework modeling the evolution of a spectral-norm based Lipschitz continuity upper bound. They further validate their theoretical framework with experiments across datasets and regularization scenarios.






Consider an $L$-layer feed-forward neural network $f: \mathbb{R}^m \to \mathbb{R}$ with 1-Lipschitz activation functions (\eg, ReLU). Let $\boldsymbol{\theta}^{(\ell)}(t) \in \mathbb{R}^{m_\ell \times n_\ell}$ be the $\ell$-layer parameter matrix at time $t$ and $\boldsymbol{\theta}(t)$ be the collection of $\boldsymbol{\theta}^{(\ell)}(t)$ for all layers. Let $\mathcal{L}_f(\boldsymbol{\theta}^{(\ell)}(t))$ be the loss expectation for the $f$ with parameters $\boldsymbol{\theta}(t)$ at time $t$. Suppose that $\boldsymbol{\Sigma}_t^{(\ell)} \in \mathbb{R}^{(m_\ell n_\ell) \times (m_\ell n_\ell)}$ is the layer-wise covariance matrix of stochastic gradient noise, arising from mini-batch sampling. Let $K^{(\ell)}(t)$ be the Lipschitz constant at layer $\ell$. Let $K(t)$ be the network Lipschitz spectral-norm bound. \citet{luo2025lipschitz} show that the continuous-time dynamics of the parameters under stochastic gradient descent (SGD) with a sufficiently small learning rate $\eta > 0$ are given by a system of SDEs \citep[Definition 10]{luo2025lipschitz}:

\begin{align}
\begin{cases}
\dd \mathrm{vec}(\boldsymbol{\theta}^{(\ell)}(t)) = - \mathrm{vec}\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right]  \, \dd t   + \sqrt{\eta} \left[\boldsymbol{\Sigma}_t^{(\ell)} \right]^{\frac{1}{2}} \, \dd \boldsymbol{B}_t^{(\ell)} \\
    K^{(\ell)}(t)=\|\boldsymbol{\theta}^{(\ell)}(t)\|_{op}  \\
    Z(t)  = \sum_{l=1}^L \log K^{(\ell)}(t) \\
    K(t) = \mathrm{e}^{Z(t)} 
    \end{cases}
\end{align}
where:
\begin{itemize}
    \item $\mathrm{vec}: \mathbb{R}^{m \times n} \to \mathbb{R}^{mn}$ represents major-column vectorization operator.

    \item $\|\cdot\|_{op}$ the matrix operator (spectral) norm.

    
    \item $\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))$ is the gradient of the loss with respect to the $\ell$-th layer parameters.

    
    \item $\boldsymbol{B}_t^{(\ell)}$ is a standard $(m_\ell n_\ell)$-dimensional Wiener process adapted to the filtration induced by mini-batch sampling.

\end{itemize}


This stochastic dynamical system characterizes, in continuous time, the evolution of both layer-wise and network-level Lipschitz continuity bounds induced by the optimization process. \citet[Theorem 15]{luo2025lipschitz} show that the layer-wise dynamics decompose into three \emph{driving forces}:
\begin{align}
\frac{\dd K^{(\ell)}(t)}{K^{(\ell)}(t)}  = \left( \mu^{(\ell)}(t) + \kappa^{(\ell)}(t) \right) \,  \dd t + \boldsymbol{\lambda}^{(\ell)}(t)^\top \, \dd \boldsymbol{B}_t^{(\ell)} 
, 
\end{align}    
where $\dd\,\boldsymbol{B}_t^{(\ell)} \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{\mathrm{I}}_{m_{\ell}n_{\ell}} \dd t)$ represents the increment of a standard Wiener process in $\mathbb{R}^{m_{\ell}n_{\ell}}$,
and the three \emph{driving forces} are:
\begin{enumerate}
    \item \textbf{Optimization-induced drift}:
    \begin{align}
    \mu^{(\ell)}(t) 
    &= \frac{\left\langle \boldsymbol{J}_{op}^{(\ell)}(t), -\mathrm{vec}\!\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right] \right\rangle}
            {\sigma_{1}^{(\ell)}(t)},
    \end{align}
    where $\boldsymbol{J}_{op}^{(\ell)}(t)$ is the Jacobian of the operator norm with respect to $\mathrm{vec}(\boldsymbol{\theta}^{(\ell)}(t))$ and $\sigma_{1}^{(\ell)}(t)$ is its largest singular value. This term captures the deterministic component of Lipschitz evolution driven by the mean gradient flow. This shows that the alignment of the gradient $\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))$ and principal direction of the $\ell$-th layer parameter matrix $\boldsymbol{J}_{op}^{(\ell)}(t)$ at time $t$ determines the contribution of the optimization to the increment of the layer-wise Lipschitz constant.

    \item \textbf{Noise--curvature entropy production}:
    \begin{align}
    \kappa^{(\ell)}(t) 
    &= \frac{\eta}{2\,\sigma_{1}^{(\ell)}(t)}
       \left\langle \boldsymbol{H}_{op}^{(\ell)}(t), \boldsymbol{\Sigma}_t^{(\ell)} \right\rangle \ge 0,
    \end{align}
    where $\boldsymbol{H}_{op}^{(\ell)}(t)$ is the Hessian of the operator norm and $\boldsymbol{\Sigma}_t^{(\ell)}$ is the gradient-noise covariance. This non-negative term quantifies irreversible growth of the Lipschitz bound due to the interaction between stochastic gradient noise and curvature.

    \item \textbf{Diffusion-modulation intensity}:
    \begin{align}
    \boldsymbol{\lambda}^{(\ell)}(t) 
    &= \frac{\sqrt{\eta}}{\sigma_{1}^{(\ell)}(t)}
       \left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{1/2\top} \boldsymbol{J}_{op}^{(\ell)}(t),
    \end{align}
    which controls the variance of Lipschitz evolution by scaling the Wiener noise term from mini-batch sampling.
\end{enumerate}

\citet[Theorem 16]{luo2025lipschitz} show that, at the network level, these quantities aggregate as:
\begin{align}
\mu_Z(t) = \sum_{\ell=1}^L \mu^{(\ell)}(t) 
,\qquad
\kappa_Z(t) = \sum_{\ell=1}^L \kappa^{(\ell)}(t)
,  \qquad
\lambda_Z(t) = \left[\sum_{\ell=1}^L \|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2\right]^{\frac{1}{2}}
,
\end{align}
governing the deterministic trend, irreversible growth, and stochastic fluctuations of the overall Lipschitz bound $K(t)$.


Their framework is particularly useful for interpreting the behaviors of neural networks, such as the near-convergence behavior, noisy supervision and mini-batch sampling trajectories. \citet[\S~8]{luo2025lipschitz} show that:
\begin{enumerate}
    \item The Lipschitz constant bound irreversibly increases since the term \emph{noise-curvature entropy production} $\boldsymbol{\kappa}_Z(t)$ is \emph{non-negative}, which increases the system entropy \citep[\S~8.3]{luo2025lipschitz}.

    \item The magnitude of uniform label noise affects the Lipschitz bound \citep[\S~8.4 \& 8.5]{luo2025lipschitz}. In particular, larger supervision noise leads to a lower Lipschitz bound for the network. This is because the supervision noise shrinks the \emph{optimization-induced drift} $\boldsymbol{\mu}_Z(t)$.

    \item Mini-batch trajectories do not affect the variance of the Lipschitz bound if batch size is sufficiently large \citep[\S~8.6]{luo2025lipschitz}.
    
\end{enumerate}

\begin{remark}
The dynamical analysis of Lipschitz continuity in deep learning models remains an open research problem. For instance, the dynamics under small-batch training remains poorly understood.
\end{remark}



\section{Estimation Methods}
\label{sec:estimating_lipschitz}


Proposition~\ref{prop:survey_upper_bound_lipschitz} gives an upper bound of the Lipschitz constant of a network \citep{miyato2018spectral,luo2025lipschitz}. However, exact computation of the Lipschitz constant
\begin{align}
K = \sup_{x \neq y} \frac{\|f(x) - f(y)\|_2}{\|x - y\|_2}
= \sup_{x} \|\nabla f(x)\|_2 \notag
\end{align}
is generally NP-hard \citep{virmaux2018lipschitz}, and even inapproximable under the Exponential Time Hypothesis \citep{jordan2020exactly}. This section surveys major estimation and bounding techniques, ranging from statistical sampling to certified convex relaxations.  
We group them into \emph{Power Iteration}, \emph{Extreme Value Theory}, \emph{Derivative Bound Propagation}, \emph{Spectral Alignment}, \emph{Convex Optimization Relaxations}, and \emph{Exact/Relaxed MILP formulations}. 

\subsection{Power Iteration for Single Linear Unit}
\label{sec:estimation:power_iteration}



\textbf{Power Iteration \citep{mises1929praktische}} is also known as the Von Mises iteration \citep{mises1929praktische}. It is the standard way to estimate the Lipschitz constant for a linear layer --- fully-connected or convolutional, by approximating the spectral-norm of weight matrices, which bounds the layer Lipschitz constant (Proposition~\ref{prop:lipschitz_constant_of_linear_unit}) \citet{yoshida2017spectral,miyato2018spectral,sedghi2019singular,kim2021lipschitz,luo2025lipschitz}. Another desirable property of \emph{power iteration} in optimization is that \emph{power iteration} is differentiable. For example, \citet{yoshida2017spectral} and \citet{miyato2018spectral} use \emph{power iteration} for computing the largest singular values of parameter matrices, in which the differentiability of \emph{power iteration} allows the gradient propagation for gradient based optimization.


Suppose that $W \in \mathbb{R}^{m \times m}$ is the parameter matrix of a fully-connected layer or a convolutional layer, then the largest singular value $\sigma_1(W)$ is its operator norm:
\begin{align}
    \mathrm{Lip}[W] = \sigma_1(W)
    .
\end{align}
Computing the exact value of $\sigma_1(W)$ for a large $m \times m$ matrix $W$ is computationally expensive, as classical algorithms require $O(m^3)$ time. However, the largest singular value can be approximated using \emph{power iteration} by assuming the existence of a uniquely dominant singular value \citep[\S~7.3]{golub2013matrix}. Starting with random unit vectors $u_0, v_0$, one step of power iteration updates
\begin{align}
v_{k+1} \;\leftarrow\; \frac{W^\top u_k}{\|W^\top u_k\|_2},
\qquad
u_{k+1} \;\leftarrow\; \frac{W v_k}{\|W v_k\|_2}
,
\end{align}
and uses 
\begin{align}
\hat{\sigma}_1^{(k+1)} = u_{k+1}^\top W v_{k+1}    
\end{align}
as a differentiable estimate of $\sigma_1(W)$ at step $k+1$. At the iteration number $T$, the estimated Lipschitz constant of $W$ is approximated as:
\begin{align}
    \mathrm{Lip}[W] \approx 
    u_{T}^\top W v_T
    ,
\end{align}
where $T$ is the number of iterations. The estimation error is proportional to:
\begin{align}
    |\sigma_1 - \hat{\sigma}_1^{(T)} | = O\Bigl( \Bigl[ \frac{\sigma_2}{\sigma_1} \Bigr]^T \Bigr)
    ,
\end{align}
where $\sigma_1$ and $\sigma_2$ are the largest, and second largest singular values, respectively \citep[Equation 7.3.5, \S~7.3]{golub2013matrix}.









\subsection{Extreme Value Theory}
\label{sec:estimation:extreme_value_theory}

\textbf{CLEVER \citep{weng2018clever}} --- \emph{Cross-Lipschitz Extreme Value for nEtwork Robustness} --- converts the problem of estimating the attack-independent robustness into the problem of estimating the \emph{local} Lipschitz constant by sampling gradient norms in a neighborhood of the input \citep{weng2018clever}. This is because the $q$-norm Lipschitz constant of a network $g: \mathbb{R}^m \to \mathbb{R}$ is determined by:
\begin{align}
    \mathrm{Lip}_q\left[g\right] = \sup_x \|\nabla\; g(x) \|_q
    , 
\end{align}
so that, for any inputs $x$ and $y$, the inequality holds:
\begin{align}
    |g(x) - g(y)| \leq \mathrm{Lip}_q\left[f\right] \|x-y\|_p \notag
    ,
\end{align}
\citep[Lemma 3.1]{weng2018clever} where $1 \leq p, q \leq \infty$ satisfy the H\"older conjugacy relation \citep[\S~6]{rudin1976principles}:
\begin{align}
\frac{1}{p} + \frac{1}{q} = 1
. \notag
\end{align}



\paragraph{Adversarial Perturbation Bound.} \citet{weng2018clever} further show that the local Lipschitz constant can be used for deriving the adversarial perturbation bound. Let 
\begin{align}
f: \mathbb{R}^m \to \mathbb{R}^k    \notag
\end{align}
be a $k$-class classifier and $f_i$ be the $i$-th prediction. Let:
\begin{align}
    c(x) = \argmax_{1 \leq i \leq k} f_i(x) \notag
\end{align}
be the prediction. Then the $p$-norm adversarial perturbation $\|\delta\|_p$ to an input $x_0$ is bounded above by:
\begin{align}
    \|\delta\|_p \leq \min_{j \neq c} \frac{f_c(x_0) - f_j(x_0)}{\mathrm{Lip}_q\left[f_c - f_j\right]}
    ,\notag
\end{align}
where the local Lipschitz constant $\mathrm{Lip}_q\left[f_c - f_j\right]$ can be estimated through:
\begin{align}
    \mathrm{Lip}_q\left[f_c - f_j\right] = \max_{x \in B_p(x_0, \delta)} \|\nabla\; (f_c - f_j)(x) \|_q 
\end{align}
and $B_p(x_0, \delta)$ is a $p$-norm ball centered at $x_0$ with a radius $\delta$ \citep[Theorem 3.2]{weng2018clever}.

\paragraph{Distribution of Extreme Value $\max_{x \in B_p(x_0, \delta)} \|\nabla\; (f_c - f_j)(x) \|_q$.} Estimating:
\begin{align}
\max_{x \in B_p(x_0, \delta)} \|\nabla_x\; (f_c - f_j)(x) \|_q
\end{align}
can be through sampling $x \in B_p(x_0, \delta)$. Suppose the $n$ samples are $\{x^{(1)}, x^{(2)}, \cdots, x^{(n)} \}$. Their gradient $q$-norms are $\{\|\nabla\; (f_c - f_j)(x^{(1)}) \|_q, \|\nabla\; (f_c - f_j)(x^{(2)}) \|_q, \cdots, \|\nabla\; (f_c - f_j)(x^{(n)}) \|_q\}$. \citet{weng2018clever} show that the extreme value of the gradient $q$-norm:
\begin{align}
  Y := \lim_{n \to \infty} \; \max_{x^{(i)} \in B_p(x_0, \delta)} \Bigl\{\|\nabla\; (f_c - f_j)(x^{(1)}) \|_q, \|\nabla\; (f_c - f_j)(x^{(2)}) \|_q, \cdots, \|\nabla\; (f_c - f_j)(x^{(n)}) \|_q \Bigr\} 
\end{align}
can only be a distribution $P_Y$ of three distribution classes:
\begin{itemize}
    \item \textbf{Type I}: \emph{Gumbel class},
    \item \textbf{Type II}: \emph{Fr\'echet class},
    \item \textbf{Type III}: \emph{Reverse Weibull class},
\end{itemize}
according to Fisher-Tippett-Gnedenko Theorem \citep[Theorem 4.1]{weng2018clever}. The extreme value $\max\|\nabla\; (f_c - f_j)(x^{(1)}) \|_q$ is thus converted to estimating the right end-point (the location parameter $a_W$) of the reverse Weibull distribution $P_Y$:
\begin{align}
     \mathrm{Lip}_q\left[f_c - f_j\right] \approx a_W
     .
\end{align}


\subsection{Coordinate-Wise Gradient}
\label{sec:estimation:coordinate_wise_gradient}


\textbf{Fast-Lip \citep{weng2018fastlip}} derives an upper bound of local Lipschitz constant in the form of coordinate-wise gradients by analyzing the activation patterns of ReLU networks. Let $n_k$ denote the number of neurons at the $k$-th layer of an $m$-layer network and Let $n_0$ be the input dimension. Let $\phi_k: \mathbb{R}^{n_0} \to \mathbb{R}^{n_k}$ be the map from input to the output of $k$-th layer. Let $\rho$ be the coordinate-wise activation function. Then the relation between the $(k-1)$-th layer and the $k$-th layer can be written as:
\begin{align}
    \phi_k(x) = \rho\Bigl(
    W^{(k)} \phi_{k-1}(x) + b^{(k)}
    \Bigr)
    ,
\end{align}
where $W^{(k)} \in \mathbb{R}^{n_k \times n_{k-1}}$ is the $k$-th layer parameter matrix, and $b^{(k)} \in \mathbb{R}^{n_k}$ is the bias. Set $f(x) = \phi_m(x)$ and let $f_j(x)$ denote the $j$-th output of $f$. \citet{weng2018fastlip} start from analyzing the ReLU activation patterns and then deriving gradient bounds under this setting for bounding local Lipschitz constant.


\paragraph{Activation Patterns of ReLU Networks.} Let $l_r^{(k)}$ and $u_r^{(k)}$ denote the lower and upper bound for the $r$-th neuron in the $k$-th layer and let $z_r^{(k)}$ be the pre-activation at the $k$-th layer, given as:
\begin{align}
    z_r^{(k)} = W_{r,:}^{(k)} \phi_{k-1}(x) + b_r^{(k)}
    ,
\end{align}
where $W_{r,:}^{(k)}$ denotes the $r$-th row of $W^{(k)}$ \citep[\S~3.2]{weng2018fastlip}. For the neurons indexed by $[n_k]:=\{1, 2, \cdots, n_k\}$, then there are only three activation patterns:
\begin{enumerate}
    \item \textbf{Always Activated.} Neurons are always activated: $\mathcal{I}_k^+ := \{ r \in [n_k] \mid u_r^{(k)} \geq l_r^{(k)} \geq 0\}$.
    
    \item \textbf{Always Inactivated.} Neurons are always inactivated: $\mathcal{I}_k^- := \{ r \in [n_k] \mid l_r^{(k)} \leq u_r^{(k)} \leq 0\}$.
    
    \item \textbf{Either Activated or Inactivated.} Neurons are either activated or inactivated: $\mathcal{I}_k := \{ r \in [n_k] \mid l_r^{(k)} \leq 0 \leq u_r^{(k)} \}$.
\end{enumerate}


\paragraph{Gradient Analysis of ReLU Networks.} Gradient norm carries the information for local Lipschitz constant. \citet{weng2018fastlip} then analyze the coordinate-wise gradients of ReLU networks with a manner of layer-wise. Using the activation patterns of ReLU networks, the $k$-th layer output can be rewritten into:
\begin{align}
    \phi_k(x) = \Lambda^{(k)} \Bigl(
    W^{(k)}\phi_{k-1}(x) + b^{(k)}
    \Bigr)
    ,
\end{align}
where $\Lambda^{(k)}$ is the activation pattern matrix:
\begin{align}
    \Lambda^{(k)}_{r,r} = \begin{cases}
        1~\text{or}~0, &\text{if}~r \in \mathcal{I}_k \\
        1, &\text{if}~r \in \mathcal{I}_k^+ \\
        0, &\text{if}~r \in \mathcal{I}_k^-
    \end{cases}
    .
\end{align}
Let $\Lambda^{(k)}_{a}$ be the diagonal activation matrix for neurons in the $k$-th layer that are always activated and set $\Lambda^{(k)}_{u}: = \Lambda^{(k)} - \Lambda^{(k)}_{a}$. Starting by analyzing the bound of the gradient $\nabla \phi_k(x)$ coordinate-wisely in a $2$-layer ReLU network, \citet{weng2018fastlip} show that an inequality for gradient $q$-norm holds:
\begin{align}
    \max_{x \in B_p(x_0, \epsilon)}
    \;
    \Bigl| \left[ \nabla f_j(x) \right]_k \Bigr|
    \leq
    \max \Bigl( 
    C_{j,k}^{(1)} + L_{j,k}^{(1)}
    ,\;
    C_{j,k}^{(1)} + U_{j,k}^{(1)}
    \Bigr)
    ,
\end{align}
where:
\begin{align}
    C_{j,k}^{(1)} = W_{j,:}^{(2)} \Lambda^{(1)}_{a} W_{:,k}^{(1)}
    , \quad 
    L_{j,k}^{(1)} = \sum_{i \in \mathcal{I}_1, W_{j,i}^{(2)}W_{i,k}^{(2)} < 0} W_{j,i}^{(2)}W_{i,k}^{(2)}, 
    \quad
    \text{and}
    \quad
    U_{j,k}^{(1)} = \sum_{i \in \mathcal{I}_1, W_{j,i}^{(2)}W_{i,k}^{(2)} > 0} W_{j,i}^{(2)}W_{i,k}^{(2)}
    .
\end{align}
Then the gradient $q$-norm can be bounded above by:
\begin{align}
\mathrm{Lip}_q\left[f_j; B_p(x_0, \epsilon)\right]
=
\max_{x \in B_p(x_0, \epsilon)} \| \nabla f_j(x) \|_q 
\leq
\Biggl[ 
\sum_k
\Bigl(
\max_{x \in B_p(x_0,\epsilon)}
\bigl| [\nabla f_j(x)]_k \bigr|
\Bigr)^{q}
\Biggr]^{\frac{1}{q}}
,
\end{align}
yielding a local Lipschitz constant upper bound. This method is referred to as \textbf{Fast-Lip} in \citet{weng2018fastlip}.





\subsection{Spectral Alignment}
\label{sec:estimation:spectral_alignment}

\textbf{SeqLip \citep{virmaux2018lipschitz}} refines the upper bound of an $L$-layer sequential network $f \in \mathbb{R}^{n_1} \to \mathbb{R}^{n_L}$ with $1$-Lipschitz activation functions:
\begin{align}
    \mathrm{Lip}\left[f\right]^+ = \prod_{\ell=1}^{L} \|W^{(\ell)}\|_2
    ,
\end{align}
where $W^{(\ell)} \in \mathbb{R}^{n_{\ell} \times n_{\ell+1}}$ is the $\ell$-th layer parameter matrix, and $\mathrm{Lip}\left[f\right]^+$ is referred to as \textbf{AutoLip} bound in \citet{virmaux2018lipschitz}. By taking into account the spectral alignment between the parameter matrices of two consecutive layers, the bound is then refined as:
\begin{align}
  \mathrm{Lip}\left[f\right] \leq 
  \mathrm{Lip}\left[f\right]^+
  \Biggl(
  \underbrace{
  \prod_{\ell}^{L-1}
  \sqrt{
  (1 - r_{\ell} - r_{\ell+1})
  \max_{t^{(\ell)} \in [0,1]^{n_\ell}} 
  \langle
  t^{(\ell)} \cdot 
  v_1^{(\ell+1)}
  ,\;
  u_1^{(\ell)}
  \rangle^2
  +r_{\ell} + r_{\ell+1} + r_{\ell}r_{\ell+1}
  }
  }_{\text{spectral alignment}}
  \Biggr)
  ,
\end{align}
where $t^{(\ell)} \in [0,1]^{n_\ell}$ represents the $\ell$-th layer gradient patterns from activation functions for $n_{\ell}$ neurons --- the coordinate-wise gradient of an activation function such as ReLU falls in $[0, 1]$, $u_1^{(\ell)}$ is the first left-singular vector for $W^{(\ell)}$, $v_1^{(\ell+1)}$ is the first right-singular vector for $W^{(\ell+1)}$, and $r_{\ell}=\frac{\sigma_2^{(\ell)}}{\sigma_1^{(\ell)}}$ is the ratio of the second largest singular value to the first largest singular value for $W^{(\ell)}$ \citep[Theorem 3]{virmaux2018lipschitz}.


\citet{virmaux2018lipschitz} also show that, if $u, v \in \mathbb{R}^n$ are two independent random vectors taken uniformly from $\mathbb{S}^{n-1}=\{ x \in \mathbb{R}^n \mid \|x\|_2=1\}$, the following limit:
\begin{align}
    \lim_{n \to \infty}\;
    \max_{t \in [0,1]^n} \Bigl | 
    \langle
    t \cdot u 
    \;,
    v
    \rangle
    \Bigr |
    =\frac{1}{\pi}
\end{align}
holds \emph{almost surely}. Under this independent assumption, the bound reduces to:
\begin{align}
    \mathrm{Lip}\left[f\right] \approx \frac{\mathrm{Lip}\left[f\right]^+}{\pi^{L-1}}
\end{align}
\citep[Lemma 2]{virmaux2018lipschitz}. In real setting, the singular vectors are not independent across layers. 

\subsection{Convex Optimization Relaxation}
\label{sec:estimation:convex_optimization_relaxation}

\textbf{LipSDP \citep{fazlyab2019efficient}} interprets activation functions as gradients of convex potential functions, satisfying certain properties described by quadratic constraints. Therefore, Lipschitz constant estimation problem is treated as a semi-definite program (SDP) problem.

Let $f: \mathbb{R}^{n_0} \to \mathbb{R}^{n_L}$ be an $L$-layer feed-forward network, recursively defined as:
\begin{align}
    \begin{cases}
        x^{(0)} = x \\
        x^{(k+1)} = \rho \Bigl( W^{(k)} x^{(k)} + b^{(k)} \Bigr)
    \end{cases}
    ,
\end{align}
where $x^{(\ell)}$ is the output at the $\ell$-th layer, $W^{(\ell)} \in \mathbb{R}^{n_{\ell+1} \times n_{\ell}}$ is the parameter matrix at the $\ell$-th layer, $b^{(\ell)} \in \mathbb{R}^{n_{\ell+1}}$ is the bias at the $\ell$-th layer, and $\rho$ is the coordinate-wise activation function. For a single layer network:
\begin{align}
f(x) = W^{(1)} \rho \bigl(
W^{(0)}x + b^{(0)} + b^{(1)}
\bigr) 
,
\end{align}
\citet{fazlyab2019efficient} shows that the Lipschitz constant of $f$ is given by a SDP problem:
\begin{align}
    \mathrm{Lip}\left[f\right] \leq \sqrt{t}
    ,
\end{align}
defined by:
\begin{align}
    \text{minimize}    \qquad &t \\
    \text{subject to}  \qquad &M(t, T) \preceq 0 \quad T \in T_n,
\end{align}
where $\rho$ is \emph{slope-restricted} on $[\alpha, \beta]$ \citep[Definition 1]{fazlyab2019efficient}:
\begin{align}
    \alpha \leq \frac{\rho_j(x) - \rho_j(y)}{x-y} \leq \beta \qquad \forall x,y \in \mathbb{R}
,
\end{align}
$T_n$ is a convex set \citep[Lemma 1]{fazlyab2019efficient}:
\begin{align}
T_n:= \bigl\{ T \in \mathbb{S}^n \mid T = \sum_{i=1}^n \lambda_{ii}e_ie_i^\top, \lambda_{ii} \geq 0 \bigr\}
    ,
\end{align}
and:
\begin{align}
   M(t, T) :=
   \begin{bmatrix}
       -2\alpha\beta (W^{(0)})^\top T W^{(0)} - t I_{n_0} &(\alpha + \beta)(W^{(0)})^\top T \\
       (\alpha + \beta) T W^{(0)} & -2T + (W^{(1)})^\top W^{(1)}
   \end{bmatrix} 
   \preceq 0
\end{align}
holds true for $T \in T_n$ \citep[Theorem 1]{fazlyab2019efficient}. For more general $L$-layer fully-connected network, \citet{fazlyab2019efficient} show that $M(t, T)$ is:
\begin{align}
    M(t, T) = 
    \begin{bmatrix}
        A \\
        B
    \end{bmatrix}^\top
    \begin{bmatrix}
        -2\alpha\beta\,T & (\alpha + \beta)T \\
        (\alpha + \beta)T & -2T
    \end{bmatrix}
    \begin{bmatrix}
        A \\
        B
    \end{bmatrix}
    +
    \begin{bmatrix}
        -t I_{n_0} &0 &\cdots &0 \\
        0             &0 &\cdots &0 \\
        \vdots        &\vdots &\ddots &\vdots \\
        0             &0 &\cdots &(W^{(L)})^\top\,W^{(L)}
    \end{bmatrix}
    \preceq 0
    ,
\end{align}
where:
\begin{align}
    A=\begin{bmatrix}
        W^{(0)} &0 &\cdots &0 &0 \\
        0        &W^{(1)} &\cdots &0 &0 \\
        \vdots &\vdots &\ddots &\vdots &\vdots \\
        0 &0 &\cdots &W^{(L-1)} & 0
    \end{bmatrix}
    , \qquad
    B=\begin{bmatrix}
        0 &I_{n_1} &0 &\cdots &0 \\
        0  &0 &I_{n_2} &\cdots &0 \\
        \vdots &\vdots &\vdots &\ddots &\vdots \\
        0 &0 &0 &\cdots &I_{n_L}
    \end{bmatrix}
    ,
\end{align}
and:
\begin{align}
    C=\begin{bmatrix}
        0 &\cdots &0 &W^{(L)}
    \end{bmatrix}
    ,
    \qquad
    b=\begin{bmatrix}
        (b^{(0)})^\top \cdots (b^{(L-1)})^\top
    \end{bmatrix}^\top
\end{align}
\citep[Theorem 2]{fazlyab2019efficient}.





\subsection{Integer Programming for ReLU Networks}
\label{sec:estimation:integer_programming_for_relu_networks}

It is well known that computing the Lipschitz constant of an arbitrary scalar- or vector-valued function is NP-hard \citep{virmaux2018lipschitz}, and even inapproximable under the Exponential Time Hypothesis \citep{jordan2020exactly}. A common approximation is to estimate the Lipschitz constant using gradient norms, where the Jacobians can be explicitly derived via the chain rule. However, nondifferentiabilities, \eg, those arising in ReLU networks, can introduce inaccuracies into these estimates. An alternative approach is to formulate the Lipschitz bounding problem as an integer programming problem, which avoids such inaccuracies by directly bounding the Jacobians.


\textbf{LipMIP \citep{jordan2020exactly}} is a method that provably exactly compute
$\ell_1$- and $\ell_\infty$-norm Lipschitz constants of non-smooth ReLU networks. We summarize their method by simplifying their notations. Let $f: \mathbb{R}^d \to \mathbb{R}$ be a ReLU network. Let $\rho$ be activation function. Then, an $L$-layer ReLU network is recursively defined as:
\begin{align}
    \begin{cases}
        f(x) = \rho(Z_L(x)) \\
        Z^{(\ell)}(x) = W^{(\ell)}\;\rho\Bigl(Z^{(\ell-1)}(x)\Bigr) + b^{(\ell)} \\
        Z^{(0)} = x
    \end{cases}
,
\end{align}
where $W^{(\ell)} \in \mathbb{R}^{n_{\ell} \times n_{\ell-1}}$ is the $\ell$-th layer parameter matrix, and $Z^{(\ell)}(x)$ is the output of the $\ell$-th layer neurons. Let $\partial f(x)$ be the Clarke sub-differential convex hull of $f$ at point $x$ --- see Section~\ref{sec:subdifferential}~(\nameref{sec:subdifferential}). For example:
\begin{align}
 \partial \rho(0)=[0,1]   
 .
\end{align}

\paragraph{Pushforward Sub-Differential Hull Set.} However, in practice, PyTorch implementations often set $\partial \rho(0) = 1$, which can lead to inaccuracies in estimating the Lipschitz constant. To correctly estimate the Lipschitz constant of a ReLU network, the analysis must be carried out in the sense of sub-differentials. Let $\partial f(X)$:
\begin{align}
    \partial f(X) = \Bigl\{
    g \mid\; g \in \partial f(x), x \in X
    \Bigr\}
\end{align}
be the set-valued Clarke sub-differentials at set $X$. Let $\nabla^{\sharp} f(\bullet)$ be the pushforward set that the sub-gradients of ReLU activation at value $0$ come from the hull set $\partial \rho(0)$:
\begin{align}
    \nabla^{\sharp} f(\bullet) =\Bigl\{
    \nabla f(\bullet) \mid \text{the sub-differentials of activations come from the hull set}~\partial\rho(0)
    \Bigr\}
    .
\end{align}
Thus for a ReLU network, the \emph{feasible set} for its gradients on $X$ is given as:
\begin{align}
\nabla^{\sharp} f(X) =
  \Bigl\{   
    G \in \nabla^{\sharp} f(x) \mid x \in X 
  \Bigr\}
  .
\end{align}

Theoretically, \citep{jordan2020exactly} show that the push forward set sub-gradient $\nabla^{\sharp} f(x)$ is the Clarke sub-gradient hull $\partial f(x)$, that is:
\begin{align}
    \nabla^{\sharp} f(x) = \partial f(x)
\end{align}
\citep[Theorem 2]{jordan2020exactly} with all gradients come from $\partial \rho(0)$. Then the local $p \to q$ Lipschitz constant of $f$ on $X$ is given as:
\begin{align}
    \mathrm{Lip}_{p \to q}\left[f;X\right] =\sup_{G \in \nabla^{\sharp} f(X)} \sup_{\|v\|_p \leq 1} \frac{\|G^\top\,v\|_{q}}{\|v\|_p}
    = \sup_{G \in \nabla^{\sharp} f(X)} \|G^\top \|_q
    .
\end{align}
Finding the Lipschitz constant on $X$ can be formulated as an integer programming problem on the feasible set $\nabla^{\sharp} f(X)$.

\paragraph{Solving the Supremum of Sub-Differential Hull Set.} The problem:
\begin{align}
    \sup_{G \in \nabla^{\sharp} f(X)} \; \Bigl\{
    \|G^\top\|_q \mid G \in \nabla^{\sharp} f(X)
    \Bigr\}
\end{align}
is then represented as a \emph{mixed-integer polytope}, which is a mixed-integer programming problem for maximizing $\|G^\top\|_q$ by solving the combinations of input $x \in X$ and ReLU's sub-gradient $a \in [0, 1]^n$ in $X \times [0, 1]^n$ \citep[Definition 6 \& Lemma 1]{jordan2020exactly}. This problem can be solved by off-the-shelf MIP solvers.















\subsection{Remarks}

The estimation methods surveyed above involve an inherent trade-off between computational efficiency, tightness, and scalability. Power iteration \citep{mises1929praktische,yoshida2017spectral,miyato2018spectral} (see Section~\ref{sec:estimation:power_iteration}) is lightweight and differentiable, but it only provides a layer-wise upper-bound estimate of the spectral norm, and therefore may induce a loose network-level upper bound when combined across layers (see Proposition~\ref{prop:lipschitz_constant_of_linear_unit} and Proposition~\ref{prop:survey_upper_bound_lipschitz}). Extreme-value-theoretic approaches such as CLEVER \citep{weng2018clever} (see Section~\ref{sec:estimation:extreme_value_theory}) are scalable and often yield tight empirical estimates of local Lipschitz behavior by leveraging the extreme value distributions of observed Lipschitz constants (see Lemma~\ref{lemma:lipschitz_bounds_gradient}), yet they do not provide formal certificates. Methods based on coordinate-wise gradient propagation and spectral alignment, such as Fast-Lip \citep{weng2018fastlip} (see Section~\ref{sec:estimation:coordinate_wise_gradient}) and SeqLip \citep{virmaux2018lipschitz} (see Section~\ref{sec:estimation:spectral_alignment}), improve upon spectral-norm product bounds by exploiting architectural structure (see Proposition~\ref{prop:survey_upper_bound_lipschitz}), but they remain approximate and are typically tailored to specific network classes. In contrast, convex relaxation methods such as LipSDP \citep{fazlyab2019efficient} (see Section~\ref{sec:estimation:convex_optimization_relaxation}) and mixed-integer formulations such as LipMIP \citep{jordan2020exactly} (see Section~\ref{sec:estimation:integer_programming_for_relu_networks}) offer substantially stronger guarantees, with the latter being exact for ReLU networks on bounded domains by working directly with the feasible Jacobian or sub-differential set (see Section~\ref{sec:subdifferential}); however, these methods are considerably more computationally expensive and generally require additional architectural information to remain tractable.





\section{Regularization Approaches}
\label{sec:lipschitz_regularizations}


A variety of techniques have been developed to explicitly or implicitly enforce Lipschitz continuity in deep neural networks. These approaches can be categorized into:
\begin{enumerate}[label=(\roman*)]
    \item Section~\ref{sec:lipschitz_regularizations:weight}: \textbf{\nameref{sec:lipschitz_regularizations:weight}} --- constraining or regularizing weight matrices during initialization and training;
    
    \item Section~\ref{sec:lipschitz_regularizations:gradient}: \textbf{\nameref{sec:lipschitz_regularizations:gradient}} --- penalizing or normalizing gradient norms during training;

    \item Section~\ref{sec:lipschitz_regularizations:activation}: \textbf{\nameref{sec:lipschitz_regularizations:activation}} --- designing or constraining activation functions to be Lipschitz-bounded; 


    \item Section~\ref{sec:lipschitz_regularizations:class_margin}: \textbf{\nameref{sec:lipschitz_regularizations:class_margin}} --- implicitly enforcing Lipschitz constraints via maximizing class decision boundaries;


    \item Section~\ref{sec:lipschitz_regularizations:architecture}: \textbf{\nameref{sec:lipschitz_regularizations:architecture}} --- enforcing Lipschitz constraints by designing architectures, particularly for transformers.


\end{enumerate}


\subsection{Weight Regularization}
\label{sec:lipschitz_regularizations:weight}


This subsection reviews methods that control the Lipschitz constant by directly constraining or regularizing the network's weight parameters, either at initialization or during training.





\subsubsection{Weight Clipping}
Weight clipping is a straightforward method to enforce Lipschitz continuity by limiting the magnitude of weight matrices. This is because for a matrix $W$, the operator-norm variation $\|W\|_{op}$ in $\ell_2$ for $W$ under perturbation $\Delta\,W$ is bounded above by:
\begin{align}
    \|W\|_{op} = \sigma_1(W) = \langle u_1 v_1^\top,\; \Delta W \rangle \leq \|u_1 v_1^\top\|_2\; \|\Delta\,W\|_2
    ,
\end{align}
with Cauchy--Schwarz inequality, where $\sigma_1(W)$ is the largest singular value of $W$, $u_1, v_1$ are the left- and right-singular vectors corresponding to the largest singular value \citep[Lemma 5.1]{luo2025spectralvariation}.

In the setting of generative adversarial networks (GANs), \citet{arjovsky2017wasserstein} showthat the discriminator $f$ of a GAN evaluates the Wasserstein distance $W\left(\mathbb{P}, \mathbb{Q}\right)$ between two distributions $\mathbb{P}$ and $\mathbb{Q}$. The Kantorovich-Rubinstein duality \citep{villani2008optimal} tells that:
\begin{align}
    W\left(\mathbb{P}, \mathbb{Q}\right) = \frac{1}{K} \; \sup_{\mathrm{Lip}\left[f\right] \leq K} \;
    \mathbb{E}_{x \sim \mathbb{P}}\bigl[f(x)\bigr] - \mathbb{E}_{y \sim \mathbb{Q}}\bigl[f(y)\bigr]
\end{align}
\citep{arjovsky2017wasserstein}. Therefore reducing the Lipschitz constant $K$ can reduce the Wasserstein distance $W\left(\mathbb{P}, \mathbb{Q}\right)$. \citet{arjovsky2017wasserstein} propose clipping weights to a fixed range:
\begin{align}
W \leftarrow \text{clip}(W, -c, +c)
\end{align}
\citep[Algorithm 1]{arjovsky2017wasserstein}, where $c$ is a small positive constant (\eg, $c=0.01$). Weight clipping is computationally efficient, but can lead to exploding or vanishing gradients if $c$ is too small, reducing model capacity, as criticized in later literature \citep{gulrajani2017improved}. 




\subsubsection{Spectral Normalization and Regularization}


\paragraph{Explicit Regularization by Penalizing Spectral Norm.}
Referring to Propositions~\ref{prop:lipschitz_constant_of_linear_unit} (\nameref{prop:lipschitz_constant_of_linear_unit}) and~\ref{prop:survey_upper_bound_lipschitz} (\nameref{prop:survey_upper_bound_lipschitz}), the product of the spectral norms of the parameter matrices gives rise to an upper bound on the Lipschitz constant of a neural network. To penalize this Lipschitz bound during training and thereby improve generalization, \citeauthor{yoshida2017spectral} propose, for an $L$-layer network parameterized by:
\begin{align}
W:=(W^{(1)},W^{(2)},\cdots,W^{(L)})
,\notag
\end{align}
the following regularization objective:
\begin{align}
    \min_{W} \mathscr{L}_{\mathrm{task}}(\xi;W) + \frac{\lambda}{2}\sum_{\ell=1}^L \big(\sigma_1^{(\ell)}\big)^2,
\end{align}
where $\mathscr{L}_{\mathrm{task}}(\xi;W)$ represents the task loss evaluated on mini batch $\xi$, $\lambda$ denotes regularization coefficient and $\sigma_1^{(\ell)}$ denotes the largest singular value of the $\ell$-th parameter matrix \citep[Equation 1]{yoshida2017spectral}. In implementation, each $\sigma_1^{(\ell)}$ is estimated using power iteration (see Section~\ref{sec:estimation:power_iteration}).



\paragraph{Implicit Regularization by Normalizing Spectral Norm.} A challenge for Generative Adversarial Networks (GANs) \citep{goodfellow2014generative} is that the prediction of discriminator is often inaccurate and unstable during training \citep{arjovsky2017towards,miyato2018spectral}. \citet{miyato2018spectral} propose normalizing the weight matrix $W$ of a linear layer by:
\begin{align}
W \leftarrow \frac{W}{\|W\|_2} = \frac{W}{\sigma_1}
,
\end{align}
where $\sigma_1$ is the largest singular value of parameter matrix $W$, for ensuring a Lipschitz constant of at most $1$ for the layer \citep[Equation 8]{miyato2018spectral}. Readers can also refer to Proposition~\ref{prop:spectralnorm_bound_single_layer}. This method was proposed by \citeauthor{miyato2018spectral} for training generative adversarial networks (GANs) \citep{goodfellow2014generative}, improving the generations \citep[\S~2.1]{miyato2018spectral}. 






\subsubsection{Orthogonal Weight}

\paragraph{Parseval Networks \citep{cisse2017parseval}.} Parseval networks enforce approximate orthonormality on weight matrices to bound their spectral-norms \citep{cisse2017parseval}. For a weight matrix $W^{(\ell)}$ in layer $\ell$, \citet{cisse2017parseval} minimize the $2$-norm of the deviation from orthonormality:
\begin{align}
\|W^{(\ell)\top} W^{(\ell)} - \mathrm{I}\|_F,
\end{align}
ensuring $\|W^{(\ell)}\|_2 \leq 1$ \citep[\S~4.2]{cisse2017parseval}. For a feedforward network with $L$ layers and 1-Lipschitz activations (\eg, ReLU), the global Lipschitz constant is bounded by:
\begin{align}
K \leq \prod_{\ell=1}^L \|W^{(\ell)}\|_2 \leq 1
,
\end{align} 
(see Proposition~\ref{prop:survey_upper_bound_lipschitz} (\nameref{prop:survey_upper_bound_lipschitz})). \citep{cisse2017parseval} argue that the robustness to adversarial attacks is enhanced by the reduced sensitivity to perturbations. %This regularization for orthogonal weights is also used in \citep{brock2017neuralphotoeditingintrospective} for training GANs.







\subsection{Gradient Regularization}
\label{sec:lipschitz_regularizations:gradient}


Gradient-based regularization methods enforce Lipschitz continuity by constraining the gradient norm of the loss function or network output with respect to inputs, ensuring smooth decision boundaries and robustness. Note that, for a network $f$ on convex $X$, its $2$-norm Lipschitz constant on $X$ is given by:
\begin{align}
    \mathrm{Lip}\left[f\right] = \sup_{x \in X} \|\nabla\,f(x)\|_2
    ,
\end{align}
(see Lemma~\ref{lemma:lipschitz_bounds_gradient} (\nameref{lemma:lipschitz_bounds_gradient})). Theoretically, constraining $\|\nabla\,f(x)\|_2$ can bound Lipschitz constant of $f$. 

For example, \citet{gulrajani2017improved} argue that bounding Lipschitz constant by weight clipping can lead to exploding or vanishing gradients, and reduce capacity of the critic in a GAN. They then introduce a regularization method by directly bounding the gradients of the critic network $D$ through:
\begin{align}
    \mathbb{E}_{x\,\sim\,\mathbb{P}_X}
    \Bigl[
    \bigl(
    \|\nabla\,D(x)\|_2 -1
    \bigr)^2
    \Bigr]
    ,
\end{align}
where $\mathbb{P}_X$ is the distribution of training sample set $X$ \citep[\S~4]{gulrajani2017improved}. 






\subsection{Activation Regularization}
\label{sec:lipschitz_regularizations:activation}

Activation regularization methods modulate Lipschitz continuity by constraining the properties of activation functions or their outputs. Such approaches may impose explicit norm bounds, design activations that are inherently norm-preserving, or apply penalties to activation magnitudes, thereby limiting the contribution of nonlinearities to the overall Lipschitz constant of the network.

\subsubsection{Group-Sorting Activation}

Bounding the Lipschitz constant of a network by ensuring $1$-Lipschitz for affine units through spectral-norm constraints can improve robustness \citep{yoshida2017spectral,miyato2018spectral}. However, this often comes at the cost of reduced expressiveness \citep{anil2019sorting}. \citet{anil2019sorting} first show that, to remain expressive in a spectral-norm constrained network, the network must preserve the gradient norms at each layer \citep{anil2019sorting}. ReLU networks can only satisfy this for positive values, this is because:
\begin{align}
    \frac{\partial\,\mathrm{ReLU}(x)}{\partial\,x} = \begin{cases}
        1, &x > 0\\
(0,1), &\text{in sub-differential sense} \\ 
        0, &x < 0
    \end{cases}
    .
\end{align}
To preserve the gradient norms at activation layer, \citet{anil2019sorting} use a general purpose $1$-Lipschitz
activation function $\textbf{GroupSort}(x)$ which is homogeneous: 
\begin{align}
\textbf{GroupSort}(\alpha\,x)=\alpha\,\textbf{GroupSort}(x)    
\end{align}
\citep{anil2019sorting}. \textbf{GroupSort} activation separates
a pre-activation $x$ into $k$ groups:
\begin{align}
    x = (
    \underbrace{
    x_1, \cdots, x_{g_1}
    }_{\text{group 1}}
    ,\, 
    \underbrace{
    x_{g_1+1}, \cdots, x_{g_2}
    }_{\text{group 2}}
    ,\cdots\,
    \underbrace{
    x_{g_{k-1}+1}, \cdots, x_{g_k}
    }_{\text{group k}}
    )
    ,
\end{align}
and sorts each group into ascending order:
\begin{align}
    \textbf{GroupSort}(x) = (
    \underbrace{
    x_{s_1}, \cdots, x_{s_{g_1}}
    }_{\text{group 1}}
    ,\, 
    \underbrace{
    x_{s_{g_1}+1}, \cdots, x_{s_{g_2}}
    }_{\text{group 2}}
    ,\cdots\,
    \underbrace{
    x_{s_{g_{k-1}}+1}, \cdots, x_{s_{g_k}}
    }_{\text{group k}}
    )
,
\end{align}
where the $i$-th sorted group satisfies:
\begin{align}
x_{s_{g_{i-1}}+1} \leq
x_{s_{g_{i-1}}+2} \leq
\cdots \leq
x_{s_{g_{i}}}
\end{align}
\citep{anil2019sorting}. For the pre-activation in a linear unit:
\begin{align}
   Wx 
\end{align}
where $W \in \mathbb{R}^{m \times n}$ and $x \in \mathbb{R}^n$, if the linear unit is with spectral-norm constraint such that:
\begin{align}
    \|W\|_2 = 1
    ,
\end{align}
\textbf{GroupSort} activation directly gives rise to a $1$-Lipschitz constant activation:
\begin{align}
    \sup_{\|x\|_2=1} \| \textbf{GroupSort}(Wx) \|_2
    = \sup_{\|x\|_2=1} \| Wx \|_2 = \|W\|_2.
\end{align}
When the group size is $2$, \citet{anil2019sorting} refers to this special case as \textbf{MaxMin}, which is equivalent to the Orthogonal Permutation Linear Unit (OPLU) \citep{chernodub2017normpreservingorthogonalpermutationlinear}; when the group size is the entire input, this is referred to as \textbf{FullSort} in the literature \citep{chernodub2017normpreservingorthogonalpermutationlinear}.

To train a network with \textbf{GroupSort} activations and guarantee that all linear units are exactly $1$-Lipschitz during optimization instead of bounded by $1$ \citep{cisse2017parseval,gulrajani2017improved}, \citet{chernodub2017normpreservingorthogonalpermutationlinear} approximate the updated parameter matrix $W_0$ with a closest orthogonal matrix through a differentiable, iterative algorithm, referred to as \emph{Bj\"orck Orthogonalization} \citep{bjorck1971}. This algorithm is defined by:
\begin{align}
    W_{k+1} = W_k \Bigl(
    I + \frac{1}{2} Q_k + \cdots + (-1)^p 
    \begin{pmatrix}
        -\frac{1}{2} \\
        p
    \end{pmatrix}
    Q_k^p
    \Bigr)
    ,
\end{align}
where $W_{k}$ is the $k$-th iterative result, $p$ is a chosen hyper-parameter and $Q_k$ is:
\begin{align}
    Q_k = I - W_k^\top W_k
\end{align}
\citep[\S~4.2.1]{chernodub2017normpreservingorthogonalpermutationlinear}. As a result, the iteration at step $T$ leads to:
\begin{align}
    W_T^\top W_T \approx I
    ,
\end{align}
which provably ensures the linear unit with parameter matrix $W$ is $1$-Lipschitz continuous:
\begin{align}
    \|W_T\|_2 \approx 1.
\end{align}


\subsubsection{Contraction Activation and Invertible Residual Map}


Flow-based models or flows learn to transform a source distribution $p_X$ to target distribution $p_Z$, consisting of invertible networks \citep{Rezende2015VariationalNormalizingFlows}. Ensuring that the transformation is invertible and its Jacobian is computable is a straightforward way for ensuring invertibility:
\begin{align}
    \log\,p_X(x) = \log\,p_Z(z) + \log\, \left| \det J_F(x) \right|
\end{align}
where $F: \mathbb{R}^m \to \mathbb{R}^m$ is an invertible map and $J_F(x)$ is the Jacobian of $F$ at $x$ \citep{berg2018sylvester,dinh2017density}. Different from explicit computation of Jacobian, \citet{Behrmann2019InvertibleResidual} propose a method for inverting residual networks \citep{he2016deep} by ensuring the Lipschitz constants be less than $1$, so that the residual networks are \emph{contraction maps} \citep{Behrmann2019InvertibleResidual,perugachi2021invertible}. 

\paragraph{Inverting Residual Layer.} Let 
\begin{align}
    F(x) = x + g(x)
\end{align}
be a residual layer where $F: \mathbb{R}^m \to \mathbb{R}^m$, $g: \mathbb{R}^m \to \mathbb{R}^m$ and $x \in \mathbb{R}^m$. Let $g$ be a contraction map so that:
\begin{align}
    \mathrm{Lip}\left[g\right] < 1
    .
\end{align}
Suppose that the inversion $F^{-1}$ exists and set $y =F(x)$, so that:
\begin{align}
x = F^{-1}(y) =  y - g(x).
\end{align}
A \textbf{sufficient condition} for inverting $F(x)$ is that $g$ is a contraction map:
\begin{align}
    \mathrm{Lip}\left[g\right] < 1
\end{align}
\citep[Theorem 1]{Behrmann2019InvertibleResidual}. Set:
\begin{align}
    T(x) = F^{-1}(y) = y - g(x)
    ,
\end{align}
then the inversion of $y$ is a fixed-point problem for solving:
\begin{align}
    x = T(x)
    .
\end{align}
Using \emph{Banach contraction principle} or \emph{Banach fixed-point theorem}, set $x_0=y$, the $F^{-1}(y)$ can be approximated through:
\begin{align}
    x_{k+1} = y - g(x_k)
\end{align}
iteratively. 


\paragraph{Contraction Activation.} \citet{chen2019residualflows} first introduce \textbf{LipSwish} activation function for inverting residual networks, defined as:
\begin{align}
    \textbf{LipSwish}(x) = \frac{x\sigma(\beta\,x)}{1.1}
    ,
\end{align}
where $\sigma$ is the sigmoid function, and $\beta > 0$ is a learnable positive constant (kept positive via softplus), initialized with $0.5$. $\textbf{LipSwish}$ has a Lipschitz constant at most $1$. However, the negative axis of $\textbf{LipSwish}$ has zero gradients almost everywhere. In a $1$-Lipschitz continuous network, the Jacobian norm across two consecutive layers is reduced to be at most one, which limits the network's expressiveness and referred to as \emph{gradient norm attenuation} problem \citep{anil2019sorting,li2019preventinggradientattenuation}. To mitigate this problem, \citet{perugachi2021invertible} use specially designed activation function \textbf{CLipSwish} by concatenating two \textbf{LipSwish} functions. The \textbf{CLipSwish} is therefore given as:
\begin{align}
    \Phi(x)=
    \begin{bmatrix}
        \textbf{LipSwish}(x) \\
        \textbf{LipSwish}(-x)
    \end{bmatrix}
    ,
    \qquad
    \textbf{CLipSwish}(x)= \frac{\Phi(x)}{\mathrm{Lip}\left[\Phi\right]} \leq 1
    ,
\end{align}
where $\mathrm{Lip}\left[\Phi\right] \approx 1.004$ \citep[\S~3.4]{perugachi2021invertible}. This concatenation overcomes the gradient attenuation problem introduced by $\textbf{LipSwish}$ since the negative axis has zero gradients almost everywhere while ensuring the activation is a contraction map. 


\subsection{Class-Margin Regularization}
\label{sec:lipschitz_regularizations:class_margin}


\paragraph{Input Margin.} The goal of adversarial defense in classification task is to ensure that, for a $k$-class classifier $f: \mathbb{R}^d \to \mathbb{R}^k$, and an input $x \in \mathbb{R}^d$, a bounded perturbation $\|\delta_x\|_2 < c$ does not alter the prediction:
\begin{align}
    \hat{y} = \argmax\limits_{i \in [k]=\{1,2,\cdots,k\}} \;f_i(x+\delta_x),
\end{align}
where $f_j(x)$ denotes the output at the $j$-th coordinate, and the $\delta_x$ giving rise to the minimal $\|\delta_x\|_2$ is often referred to as $2$-norm \emph{input margin} \citep{Jonas2024marginconsistency}. More generally, \emph{input margin} can also be discussed with respect to $p$-norm ($1\leq p \leq \infty$). The $p$-norm \emph{input margin} represents the decision boundary in the input space with respect to the topology induced by $p$-norm.




\paragraph{Class/Logit Margin.} Of the same setting, the \emph{class margin} (\ie~\emph{logit margin}) $m(x)$ is defined as:
\begin{align}
    m(x) = f_i(x) - \max_{j \neq i} f_j(x)
    , \label{eq:classmargin_mx}
\end{align}
where $i$ is the ground-truth \citep[\S~4.1]{tsuzuku2018lipschitz}. By writing equation~(\eqref{eq:classmargin_mx}) into:
\begin{align}
m(x) = (e_i - e_j)^\top
    \begin{bmatrix}
        f_i(x) \\
        \max_{j \neq i} f_j(x)
    \end{bmatrix}
    ,
\end{align}
where $e_i$ and $e_j$ are one-hot basis, for $2$-norm, applying Proposition~\ref{prop:lipschitz_concatenation} (\nameref{prop:lipschitz_concatenation}) immediately yields:
\begin{align}
\mathrm{Lip}\left[m\right]^2 \leq  \mathrm{Lip}\left[f\right]^2 + \mathrm{Lip}\left[f\right]^2 \Longrightarrow \mathrm{Lip}\left[m\right] \leq \sqrt{2} \; \mathrm{Lip}\left[f\right]
.
\end{align}
Therefore, a guaranteed $2$-norm perturbation $\delta_x$ does not alter the prediction, if:
\begin{align}
\label{eq:2norm_perturbation_deltax}
    \|\delta_x\|_2 \leq \frac{m(x)}{\mathrm{Lip}\left[m\right]} = \frac{m(x)}{\sqrt{2} \;\mathrm{Lip}\left[f\right]}
\end{align}
\citep[also see][Proposition 1 \& 2]{tsuzuku2018lipschitz}, which implies that the class margin must be at least:
\begin{align}
    m(x) = f_i(x) - \max_{j \neq i} f_j(x) \geq \sqrt{2} \,c\, \mathrm{Lip}\left[f\right]
    .
\end{align}



\paragraph{Lipschitz-Margin Training.} Of the same setting, in training stage, \citet{tsuzuku2018lipschitz} adjust each class margin $j \neq i$ by:
\begin{align}
    f_j(x) \leftarrow f_j(x) + \sqrt{2}\,c\,\mathrm{Lip}\left[f\right]
    ,
\end{align}
where $c$ is a guaranteed perturbation bound \citep[Algorithm 1]{tsuzuku2018lipschitz}. For each linear unit $\phi: \mathbb{R}^m \to \mathbb{R}^n$ in the network, and let $u \in \mathbb{R}^m$ be drawn i.i.d. from $\mathcal{N}(0,1)$. \citet{tsuzuku2018lipschitz} use a general method for estimating the Lipschitz constant of $\phi$ iteratively by:
\begin{align}
    u \leftarrow \frac{u}{\|u\|_2}, \qquad
    v \leftarrow \phi(u), \qquad
    \sigma \leftarrow \|v\|_2, \qquad
    u \leftarrow \frac{1}{2}\frac{\partial\,\|v\|_2^2}{\partial\,u}
\end{align}
\citep[Theorem 1 \& Algorithm 2]{tsuzuku2018lipschitz}. At the end of the iteration $T$, the Lipschitz constant of $\phi$ is given by:
\begin{align}
    \mathrm{Lip}\left[\phi\right] \approx \sigma
,
\end{align}
almost surely.



\subsection{Architectural Regularization}
\label{sec:lipschitz_regularizations:architecture}

Lipschitz continuity can also be constrained through architectural design choices, including activation functions, parameter structures, initialization schemes, and optimization. As a complement to regularization approaches that do not fall into one single category, we survey these approaches in this section.

\subsubsection{Orthogonalizing Convolution}


Parameter orthogonality in neural networks can directly yield $1$-Lipschitz continuous (Proposition~\ref{prop:column_orthogonal_matrix})~(\nameref{prop:column_orthogonal_matrix})). This is because, for a matrix $W \in \mathbb{R}^{m \times n}$, a semi-orthogonal matrix $W$ preserves the $2$-norm:
\begin{align}
    W^\top\,W = I_n
    \quad \text{or} \quad
    WW^\top = I_m
    \quad
    \Longrightarrow 
    \quad
    \mathrm{Lip}\left[ W \right]=1
    ,
\end{align}
if $m \geq n$ and $W^\top W=I_n$, $W$ is an isometric map; if $m < n$ and $WW^\top = I_m$, $W$ is non-expansive, vanishing on the kernel $\ker(W)$ (Proposition~\ref{prop:column_orthogonal_matrix})~(\nameref{prop:column_orthogonal_matrix})).

\paragraph{Extending Semi-Orthogonality to Convolution.} Let $W \in \mathbb{R}^{c_{out} \times c_{in} \times n \times n}$ be a convolutional filter where $c_{out}$ is the number of output channels, $c_{in}$ is the number of input channels, and $n \times n$ are the input dimensions. The action on an input $x \in \mathbb{R}^{c_{in} \times n \times n}$ is denoted by:
\begin{align}
    W \circledast x: \mathbb{R}^{c_{in} \times n \times n} \to \mathbb{R}^{c_{out} \times n \times n}.
\end{align}
Using the norm preserving concept for $1$-Lipschitz maps on $\ell_2$, for $\forall\;x \in \mathbb{R}^{c_{in} \times n \times n}$, if the $2$-norms are preserved:
\begin{align}
    \|W \circledast x\|_2 = \|x\|_2
    ,
\end{align}
then the convolutional filter $W$ is referred to as semi-orthogonal \citep{trockman2021orthogonalizing}.


\paragraph{Filter Orthogonalization via Cayley Transform.} However, convolutional operation is not matrix multiplication, to apply the existing results from matrix theory, \citet{trockman2021orthogonalizing} harness the \emph{Convolutional Theorem} \citep{jain1989fundamentals} for converting the convolutional operation in spatial domain to multiplication in frequency domain by:
\begin{align}
    \mathscr{F}\left[W \circledast x\right][:,i,j] =\mathscr{F}\left[W\right][:,:,i,j] \; \mathscr{F}\left[x\right][:,:,i,j] = \widehat{W}[:,i,j]\widehat{x}[:,i,j]
    ,
\end{align}
where $\mathscr{F}$ represents Fourier transform, $\widehat{W}=\mathscr{F}\left[W\right]$, $\widehat{x}=\mathscr{F}\left[x\right]$, $[:,:,i,j]$ and $[:,i,j]$ are slicing operations by fixing indices $(i,j)$) \citep[Equation 3 \& 4, \S~4]{trockman2021orthogonalizing}. Note that $\widehat{W}[:,:,i,j]$ is not orthogonal or semi-orthogonal, \citet{trockman2021orthogonalizing} use a bijective \emph{Cayley Transform} for deriving an orthogonal matrix $Q[:,:,i,j]$ from $\widehat{W}[:,:,i,j]$ by:
\begin{align}
    Q[:,:,i,j] = (I - A[:,:,i,j])(I + A[:,:,i,j])^{-1},
\end{align}
where:
\begin{align}
    A[:,:,i,j] = \widehat{W}[:,:,i,j] - \widehat{W}[:,:,i,j]^\ast 
    ,
\end{align}
and $A[:,:,i,j]$ is referred to as \emph{skew-Hermitian} matrix \citep{trockman2021orthogonalizing}. Conceptually, the convolution on frequency domain is then computed through:
\begin{align}
    \mathscr{F}\left[W \circledast x \right][:,i,j] &= Q[:,:,i,j] \; \widehat{x}[:,i,j] \\
    &=(I - A[:,:,i,j])(I + A[:,:,i,j])^{-1} \;\widehat{x}[:,i,j]
    ,
\end{align}
then $Q[:,:,i,j] \; \widehat{x}[:,i,j]$ is inverted back to spatial domain by:
\begin{align}
    \mathscr{F}^{-1}\left[ Q[:,:,i,j] \; \widehat{x}[:,i,j]\right],
\end{align}
which leads to the convolution $1$-Lipschitz continuous.


\subsubsection{Orthogonality with Lie Unitary Group}


\citet{lezcano2019cheap} introduce a method, stemming from Lie group theory, through the exponential map, for ensuring $1$-Lipschitz by construction. Orthogonal
constraints networks can improve the robustness and generalization capabilities \citep{huang2018orthogonalweight,Bansal2018orthogonality}. For a matrix $A$, if $AA^\ast =I$, then the matrix $A$ is referred to as a unitary matrix. Unitary matrices allow to solve the exploding or vanish gradients \citep{Arjovsky2016unitary,arjovsky2017wasserstein}. In the sense of Lie algebra, these unitary matrices form a special orthogonal group on field $\mathbb{R}$:
\begin{align}
    SO(n) = \Bigl\{ 
    A \in \mathbb{R}^{n \times n} \mid A^\top A = I
    \Bigr\}
\end{align}
and unitary group on field $\mathbb{C}$:
\begin{align}
    U(n) = \Bigl\{ 
    A \in \mathbb{C}^{n \times n} \mid A^\ast  A = I
    \Bigr\}
\end{align}
\citep[\S~3.1]{lezcano2019cheap}. We are interested in converting a parameter matrix $W \in \mathbb{R}^{n \times n}$ to $SO(n)$ or $U(n)$. \citet{lezcano2019cheap} harness the concept of \emph{skew-symmetric matrix} group (Definition~\ref{def:skew_hermitian}~(\nameref{def:skew_hermitian})) as a bridge:
\begin{align}
    \mathfrak{so}(n)=\{B\in\mathbb{R}^{n\times n}\;:\;B=-B^\top\}
\end{align}
and:
\begin{align}
    \mathfrak{u}(n)=\{B\in\mathbb{R}^{n\times n}\;:\;B=-B^\ast \}
    .
\end{align}
Taking:
\begin{align}
    B=W - W^\top
\end{align}
can easily send a parameter matrix $W$ to $\mathfrak{u}(n)$. 

\paragraph{Connecting to Lie Orthogonal Group.} Then there exists an exponential \emph{surjective} map between two groups:
\begin{align}
    \exp: \mathfrak{so}(n) \to SO(n)
\end{align}
and:
\begin{align}
    \exp: \mathfrak{u}(n) \to U(n)
,
\end{align}
which is defined as:
\begin{align}
    \exp(B) = I + B + \frac{1}{2}B^2 + \cdots
\end{align}
\citep[\S~3.2]{lezcano2019cheap}. Then a network $f(x; W)$ is parameterized on the Lie group $SO(n)$ by an algebraic mapping chain:
\begin{align}
    W \in \mathbb{R}^{n \times n} 
    \xlongrightarrow[]{B=W-W^\top}  B \in \mathfrak{so}(n) \xlongrightarrow[]{A=\exp(B)}  A \in SO(n)
    ,
\end{align}
and the optimization problem becomes:
\begin{align}
    \min_{A}~f(x; A) \Longleftrightarrow \min_{B}~f(x; \exp(B))
\end{align}
\citep[\S~3.3]{lezcano2019cheap}. 


\paragraph{Optimizing on Lie Orthogonal Group.} The Lie group $SO(n)$ forms a Riemannian manifold, to optimize a function $f$ on the Riemannian manifold $SO(n)$:
\begin{align}
    f: \mathcal{X} \times SO(n) \to \mathbb{R}
    ,
\end{align}
where $\mathcal{X}$ is input space, one may use \emph{Riemannian gradient descent} \citep{absil2009optimization}. Given a point on the manifold $A \in SO(n)$, $\mathcal{T}_A\,SO(n)$ is the tangent space at $A$ with induced metric, and a gradient $\Omega \in \mathcal{T}_A\,SO(n)$, then the geodesic update is:
\begin{align}
    A \leftarrow A \, \exp\left(-\eta\,A^\ast  \, \Omega\right)
    ,
\end{align}
where $\eta$ is a learning rate $\eta > 0$ \citep{lezcano2019cheap}. Computing the Riemannian exponential map is expensive; a cheaper first-order approximation, the \emph{Cayley map}, may be used for the update instead:
\begin{align}
    A \leftarrow A \, \phi\left(-\eta\,A^\ast  \, \Omega\right)
    ,
\end{align}
where $\phi$ is the \emph{Cayley map}:
\begin{align}
    \phi(A) = (I+\frac{1}{2}A)(I-\frac{1}{2}A)^{-1}    
\end{align}
\citep{Wisdom2016FullCapacity,Vorontsov2017Orthogonality}. Finally, this induces an update rule on $B \in \mathfrak{so}(n)$:
\begin{align}
    \exp(B) \leftarrow \exp\Bigl(B-\eta\,\nabla\,f\left(x;\exp(B)\right)\Bigr)\,
\end{align}
where $\nabla\,f\left(x;\exp(B)\right)$ is the usual gradient with Euclidean metric. In a specially designed recurrent neural network (RNN), \citet{lezcano2019cheap} transform the matrix exponential maps skew-symmetric matrices to orthogonal matrices transforming an optimization problem with orthogonal constraints \citep{lezcano2019cheap}. Particularly, \citet{lezcano2019cheap} use Pad\'e approximants and the scale-squaring trick to compute machine-precision approximations of the matrix exponential and its gradient \citep{lezcano2019cheap}. As a result, the optimization remains in the group and the Lipschitz constants of the updated matrices remain $1$ by design.


\subsubsection{Lipschitz Continuous Transformers}


\paragraph{$L_2$ Self-Attention Transformer.} \citeauthor{kim2021lipschitz} have shown that dot-product self-attention is non-globally Lipschitz continuous \citep[Theorem 3.1.]{kim2021lipschitz}. Referring to \eqref{eq:shdp_attention} and \eqref{eq:KQV_def} in Section~\ref{sec:selfattention_lipschitz}, recall that the distance matrix for \emph{query} $Q$ and \emph{key} $K$ in multi-head dot-product attention matrix are computed through their row-wise dot-product:
\begin{align}
    P:= \mathrm{Softmax}\Bigl( \frac{QK^\top}{\sqrt{d_K}} \Bigr) = \mathrm{Softmax}\Bigl( \frac{xW_Q(xW_K)^\top}{\sqrt{d_K}} \Bigr) \propto \exp{\Bigl(\frac{xW_Q(xW_K)^\top}{\sqrt{d_K}}\Bigr)}
    ,
\end{align}
which leads to unbounded Jacobian norm. To solve the issue caused by dot-product attention computation, \citeauthor{kim2021lipschitz} propose to use $L_2$ distance instead by:
\begin{align}
    P_{ij} \propto \exp{\Bigl(\frac{-\|x_iW_Q - x_jW_K\|_2^2 }{\sqrt{d_K}}\Bigr)}
    ,
\end{align}
where $x_i$ and $x_j$ are the $i$-th and $j$-th tokens of $x$, and $P_{ij}$ represents their attention score \citep[Equation 8]{kim2021lipschitz}. 

\citeauthor{kim2021lipschitz} further show that, for a sequence length $n$, input dimension $d$, and $h$ heads, its $2$-norm Lipschitz bound is:
\begin{align}
\mathrm{Lip}\left[L_2\mathrm{-Attention}\right]
\leq
\frac{\sqrt{n}}{\sqrt{d_K}}
\Bigl[
4\phi^{-1}(n-1)+1
\Bigr]
\Biggl(
\sqrt{
\sum_{h_i} 
\|W_{Q,h_i}\|_2^2\;
\|W_{V,h_i}\|_2^2\;
}
\Biggr)
\|W_O\|_2 
, \label{equ:kims_dotproduct_bound:l2}
\end{align}
and the $\infty$-norm Lipschitz bound:
\begin{align}
\mathrm{Lip}_{\infty}\left[L_2\mathrm{-Attention}\right]
\leq 
\Biggl[
4\phi^{-1}(n-1) + \frac{1}{\sqrt{d_K}}
\Biggr]
\;
\|W_O^\top\|_{\infty}
\;
\max_{h_i} 
\|W_{Q,h_i}\|_{\infty}
\|W_{Q,h_i}^\top\|_{\infty}
\;
\max_{h_j}  \|W_{V,h_j}^\top\|_{\infty} 
, \label{equ:kims_dotproduct_bound:linfty}
\end{align}
where:
\begin{align}
\phi(x)=x\exp(x+1)    \notag
\end{align}
is an invertible univariate function on $x>0$,
$W_{Q,h_i}$ is the \emph{query} parameter matrix for head $h_i$, $W_{V,h_i}$ is the \emph{value} parameter matrix for head $h_i$, and $W_O \in \mathbb{R}^{d \times d}$ is the projection parameter matrix; the per-head key dimension is $d_K = d/h$ \citep[Theorem~3.2]{kim2021lipschitz}. They further conclude that their results can lead that the $2$-norm Lipschitz bound is at the scale:
\begin{align}
\mathrm{Lip}[\mathrm{Attention}] \sim O(\sqrt{n} \log n) 
,    
\end{align}
and the $\infty$-norm Lipschitz bound is at the scale:
\begin{align}
\mathrm{Lip}_{\infty}[\mathrm{Attention}] \sim
O(\log n)
\end{align}
\citep[Theorem~3.2]{kim2021lipschitz}. The bounds in \citep[Theorem~3.2]{kim2021lipschitz} are complemented by concurrent work \citep{vuckovic2020mathematical} with a measure-theoretical framework. \citeauthor{vuckovic2020mathematical} show that the $1$-norm Lipschitz bound is at the scale:
\begin{align}
\mathrm{Lip}_1[\mathrm{Attention}] \sim O(\sqrt{\log{n}})
\end{align}
\citep[Theorem 29 \& Corollary 30]{vuckovic2020mathematical}.

\begin{remark}
The Lipschitz constant bound of an $L_2$ self-attention layer remains dependent on the sequence length $n$ but is independent of the input norm. 
\end{remark}




\paragraph{LipsFormer.} \citet{qi2023lipsformer} demonstrate that enforcing Lipschitz continuity in Transformer architecture \citep{vaswani2017attention} is more crucial for ensuring training stability in contrast to the tricks such as \emph{learning rate warmup}, \emph{layer normalization}, \emph{attention formulation}, and \emph{weight initialization} \citep{qi2023lipsformer}. Their proposed method, referred to as \textbf{LipsFormer}, replaces the Transformer parts with their Lipschitz continuous counterparts: \emph{CenterNorm} for \emph{LayerNorm}, \emph{spectral initialization} for \emph{Xavier initialization}, \emph{scaled cosine similarity attention} for \emph{dot-product attention}, and \emph{weighted residual shortcut} for \emph{residual connection} \citep{qi2023lipsformer}. These modifications result in a Transformer architecture with a provably bounded Lipschitz constant. Their key architectural design elements are summarized as follows:
\begin{enumerate}[left=1em]
    \item \textbf{CenterNorm instead of LayerNorm.} LayerNorm \citep{ba2016layer} is widely used in Transformer, defined as:
\begin{align}
    \mathrm{LN}(x) = \gamma \, \odot \, z + \beta
    ,
\end{align}
and:
\begin{align}
    z = \frac{y}{\mathrm{std}(y)}, \qquad y = \Bigl(I_d - \frac{1}{d}\boldsymbol{1}_d\boldsymbol{1}_d^\top\Bigr)x
    ,
\end{align}
where $x \in \mathbb{R}^d$ is input, $I_d$ is an identity matrix in $\mathbb{R}^{d \times d}$, $\boldsymbol{1}_d$ is an all-ones vector in $\mathbb{R}^d$, $\mathrm{std}(y)$ is the standard deviation of $y$, $\odot$ is element-wise product, $\gamma$ and $\beta$ are learnable parameters initialized to $1$ and $0$ respectively \citep{qi2023lipsformer}. The Jacobian of $z$ with respect to $x$ is given as:
\begin{align}
    \frac{\partial\,z}{\partial\,x} = \frac{1}{\mathrm{std}(y)} 
    \Bigl(I_d - \frac{1}{d}\boldsymbol{1}_d\boldsymbol{1}_d^\top\Bigr)
    \Bigl(
    I_d - \frac{yy^\top}{\|y\|_2^2}
    \Bigr)
    ,
\end{align}
which shows that \textbf{LayerNorm} is not Lipschitz continuous when $\mathrm{std}(y) \to 0$. To address this problem, \citet{qi2023lipsformer} introduce \textbf{CenterNorm}, defined as:
\begin{align}
    \mathrm{CN}(x) = \gamma\,\odot\,\frac{d}{d-1}
    \Bigl(I_d-\frac{1}{d}\boldsymbol{1}_d\boldsymbol{1}_d^\top\Bigr)x + \beta
    ,
\end{align}
which admits a Lipschitz constant:
\begin{align}
    \mathrm{Lip}\left[\mathrm{CN}\right] = \frac{d}{d-1} \approx 1
\end{align}
for sufficient large $d$, $\gamma=1$, and $\beta=0$ \citep{qi2023lipsformer}.


\item \textbf{Scaled Cosine Similarity Attention (SCSA).} \citet{kim2021lipschitz} show that standard dot-product self-attention is not Lipschitz continuous since the Lipschitz constant depends on sequence length which is not bounded \citep{kim2021lipschitz}, see also Section~\ref{sec:selfattention_lipschitz} (\nameref{sec:selfattention_lipschitz}). To address this problem, \citet{qi2023lipsformer} replace standard dot-product attention part with \textbf{SCSA}, defined as:
\begin{align}
    \mathrm{SCSA}(x;\nu,\tau)=\nu PV, \qquad P = \mathrm{softmax}(\tau\,QK^\top),
\end{align}
where $\nu$ and $\tau$ are learnable scalars, and $K,Q,V$ are row-wise normalized in $\ell_2$ \citep[\S~4.1.2]{qi2023lipsformer}. 

\begin{remark}
It is worth noting that their method reduces the Lipschitz constant of the attention module; however, the module remains not globally Lipschitz continuous since the Lipschitz constant still depends on sequence length $n$:
\begin{align}
    \mathrm{Lip}_2\left[SCSA\right] \leq O(n^2), \qquad \text{and} \qquad \mathrm{Lip}_{\infty}\left[SCSA\right] \leq O(n^2)
\end{align}
\citep[Theorem 1]{qi2023lipsformer}.
\end{remark}


\item \textbf{Weighted Residual Shortcut.} For a residual module:
\begin{align}
    h(x) = x + g(x)
    ,
\end{align}
where $g: \mathbb{R}^d \to \mathbb{R}^d$, $h: \mathbb{R}^d \to \mathbb{R}^d$ and $x \in \mathbb{R}^d$, the Lipschitz constant of $h$ is bounded by:
\begin{align}
    \mathrm{Lip}\left[h\right] \leq  1 + \mathrm{Lip}\left[g\right]
    ,
\end{align}
see Section~\ref{sec:lipschitz_of_residual_module} (\nameref{sec:lipschitz_of_residual_module}). To further reduce the Lipschitz constant introduced by residual module, \citet{qi2023lipsformer} replace the standard residual module with:
\begin{align}
    \mathrm{WRS}(x) = x + \alpha \, \odot\, g(x)
    ,
\end{align}
where $\alpha$ is a learnable parameter, initialized to a small value $[0.1, 0.2]$ \citep{qi2023lipsformer}. Assuming the residual branch $g$ is $1$-Lipschitz, the Lipschitz constant of $\mathrm{WRS}$ in residual module is bounded by:
\begin{align}
\mathrm{Lip}\left[\mathrm{WRS}\right] \leq 1 + \max(\alpha)
.
\end{align}



\item \textbf{Spectral-based Weight Initialization.} \citet{qi2023lipsformer} further normalize the parameters at initialization by spectral-norm. Let $W$ be a parameter matrix, the $W$ is normalized by:
\begin{align}
    W \leftarrow \frac{W}{\|W\|_2}
\end{align}
\citep[\S~4.1.4]{qi2023lipsformer}.


\end{enumerate}











\subsubsection{Jacobian Norm Minimization}



Constraining the Lipschitz constant of Transformer architecture for stable optimization and robustness remains an open research problem. \citet{yudin2025pay} first derive an explicit tight local Lipschitz constant for self-attention module in Transformer architecture by analyzing the Jacobian of softmax \citep{yudin2025pay}. Building on top of the Jacobian analysis, they present \textbf{JaSMin} (\textbf{Ja}cobian \textbf{S}oftmax norm \textbf{Min}imization) for enhancing Transformer's robustness by constraining the local Lipschitz constant \citep{yudin2025pay}.


\paragraph{Bounding Lipschitz through Softmax Jacobian.} Consider the softmax function:
\begin{align}
    \mathrm{softmax}: \mathbb{R}^d \to \mathbb{R}^d
    ,
\end{align}
then the Jacobian of the softmax function is:
\begin{align}
\mathcal{M}(P_x) := \nabla \, \mathrm{softmax}\left(x\right) = 
\mathrm{diag}(P_x) - P_x P_x^\top,
\end{align}
where:
\begin{align}
    P_x = \Biggl( \frac{\mathrm{e}^{x_i}}{\sum_j \mathrm{e}^{x_j}} \Biggr) 
    .
\end{align}
\citet{yudin2025pay} incorporate this Jacobian expression of the softmax function into self-attention, leading to a Lipschitz constant bound for a single head:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}\Bigr] 
    \leq
    \|W_V\|_2
    \Biggl(
    \|P\|_2 + 2 \|x\|_2^2 \; \|A\|_2 \; \max_i \|\mathcal{M}(P_{i, :})\|_2
    \Biggr)
\end{align}
with:
\begin{align}
    P = \mathrm{softmax}\Bigl(
    x
    A
    x^\top
    \Bigr) \in \mathbb{R}^{n \times n} \qquad \text{and} \qquad A = \frac{W_QW_K^\top}{\sqrt{d_K}} \in \mathbb{R}^{d \times d}
\end{align}
\citep[Theorem~3]{yudin2025pay}. It is worth noting that the local Lipschitz constant contains a term:
\begin{align}
 \mathrm{Lip}\Bigl[\mathrm{Attention}\Bigr] \leq
 O\Bigl(
 \max_i \|\mathcal{M}(P_{i, :})\|_2
 \Bigr)
 ,
\end{align}
which shows that softmax Jacobian norm determines an upper bound of the local Lipschitz constant.

\paragraph{Jacobian Softmax Norm Minimization.} To approximate the Jacobian norm more efficiently, \citet{yudin2025pay} introduce a surrogate function $g$ that captures the partial ordering of the singular values of softmax mappings. For $x \in \mathbb{R}_{>0}^n$, let $x_{(k)}$ be the $k$-th largest component of $x$. Define:
\begin{align}
    g_k(x) := x_{(k)}(1 - x_{(k)} + x_{(k+1)})
,
\end{align}
for $k=1,2,\cdots,n-1$ \citep[Definition 1]{yudin2025pay}. Let $A = \mathrm{diag}(x) - xx^\top$, then the following inequality holds true:
\begin{align}
    x_{(1)} \geq g_1(x) \geq \sigma_1(A)
    \geq
    x_{(2)} \geq g_2(x) \geq \sigma_2(A)
    \geq
    x_{(n)} \geq g_n(x) \geq \sigma_n(A)
    \geq 0
\end{align}
\citep[Theorem 4]{yudin2025pay}.

Building on the derived bound, \citet{yudin2025pay} propose an efficient regularization loss expressed in terms of the function $g$ with two forms:
\begin{align}
    \mathcal{L}_{\mathrm{JaSMin}(k=0)}
    = \sum_{\ell=1}^{L}
    \sum_{h_i=1}^{h}
    \max_j\log
    \Bigl[
    g_1\Bigl(
    P_{j,:}^{\ell, i}
    \Bigr)
    \Bigr]
    ,
\end{align}
and:
\begin{align}
    \mathcal{L}_{\mathrm{JaSMin}(k)}
    = \sum_{\ell=1}^{L}
    \sum_{h_i=1}^{h}
    \max_j\log
    \Biggl[
    \frac{
    g_1\Bigl(
    P_{j,:}^{\ell, i}
    \Bigr)
    }{
    g_k\Bigl(
    P_{j,:}^{\ell, i}
    \Bigr)
    }
    \Biggr]
    ,
\end{align}
where $P_{j,:}^{\ell, i}$ represents the softmax map for the $\ell$-th attention module ($1\leq \ell \leq L$), $i$-th head ($1 \leq i \leq h$), and the $j$-th row of the map \citep[\S~4]{yudin2025pay}. They also show that for $\sfrac{g_1}{g_k}$ is bounded below $\gamma$:
\begin{align}
    \frac{
    g_1\Bigl(P_{j,:}^{\ell,i}\Bigr)
    }{
    g_k\Bigl(P_{j,:}^{\ell,i}\Bigr)
    } \leq \gamma
,
\end{align}
for $1 \leq \gamma \leq \frac{k}{4}$. Then the softmax Jacobian $2$-norm is bounded by:
\begin{align}
   \| \mathcal{M}(P_{j,:}^{\ell,i}) \|_2 \leq
   O\Bigl(\frac{\gamma}{k}\Bigr)
\end{align}
\citep[Proposition 1]{yudin2025pay}.

\subsection{Remarks}

The regularization approaches surveyed above also involve a trade-off between enforceability, computational cost, expressive power, and guarantee strength. Weight-based methods such as weight clipping \citep{arjovsky2017wasserstein} (see Section~\ref{sec:lipschitz_regularizations:weight}) and spectral normalization \citep{miyato2018spectral,yoshida2017spectral} (see Section~\ref{sec:lipschitz_regularizations:weight}) are simple to implement and scale well to large models, but they typically control only upper bounds induced by layer norms rather than the exact network Lipschitz constant (see Proposition~\ref{prop:lipschitz_constant_of_linear_unit} and Proposition~\ref{prop:survey_upper_bound_lipschitz}). Gradient-based methods \citep{gulrajani2017improved} (see Section~\ref{sec:lipschitz_regularizations:gradient}) act more directly on the input--output sensitivity by penalizing gradient norms (see Lemma~\ref{lemma:lipschitz_bounds_gradient}), yet they are often local in nature and can be computationally expensive due to repeated differentiation. Activation- and architecture-based approaches, such as GroupSort \citep{anil2019sorting}, invertible residual constructions \citep{Behrmann2019InvertibleResidual,perugachi2021invertible}, and Lipschitz-continuous transformer variants \citep{kim2021lipschitz,qi2023lipsformer,yudin2025pay} (see Sections~\ref{sec:lipschitz_regularizations:activation} and~\ref{sec:lipschitz_regularizations:architecture}), provide stronger structural control by design, but may restrict architectural flexibility or reduce expressive efficiency. Class-margin regularization \citep{tsuzuku2018lipschitz} (see Section~\ref{sec:lipschitz_regularizations:class_margin}) connects Lipschitz control to certifiable robustness more directly through margin-based objectives, although its effectiveness still depends on the quality of the underlying Lipschitz bound (see Equation~\eqref{eq:2norm_perturbation_deltax}). 



\section{Certifiable Robustness}
\label{sec:certifiable_robustness}


Certifiable robustness, a cornerstone of trustworthy deep learning, guarantees that a neural network's predictions remain consistent under adversarial perturbations within a specified norm ball. Unlike empirical defenses like adversarial training, which lack formal guarantees, Lipschitz-based certification methods leverage the Lipschitz constant to bound sensitivity to input changes, ensuring provable robustness. While some literature, such as \citep{clevert2015elu}, have been introduced previously from the perspectives --- such as \textbf{theoretical foundations}, \textbf{estimation methods} and \textbf{regularization approaches}, we may revisit some of them in this section from the perspective of \textbf{certifiable robustness}.



\subsection{Formal Robustness Guarantees}


To complement the results in Section~\ref{sec:lipschitz_regularizations:class_margin}, we now discuss formal robustness guarantees for the general case. In the setting of a $k$-class classifier $f$ with Lipschitz constant $K$, a central question in adversarial defense is to determine the largest perturbation norm that leaves the prediction unchanged.

\begin{theorem}[$p$-Norm Lipschitz Margin Robustness Radius]
Let $f:\mathbb{R}^d\to\mathbb{R}^k$ be a classifier. Let $f_i$ be the $i$-th output. Let $c=\arg\max_i f_i(x)$ be the predicted class for $x$. Define the (one-versus-rest) margin
\begin{align}
m(x)\;:=\;f_c(x)-\max_{j\ne c} f_j(x).
\end{align}
Let $f$ be Lipschitz continuous from the input $\ell_p$ norm to the output $p$-norm, \ie,
\begin{align}
\|f(x)-f(y)\|_p \;\le\; \mathrm{Lip}_p[f]\,\|x-y\|_p \quad \text{for all } x,y.
\end{align}

Then for any perturbation $\delta_x$ with
\begin{align}
\|\delta_x\|_p \;<\; \frac{m(x)}{2^{1-\frac{1}{p}}\,\mathrm{Lip}_p[f]},
\end{align}
the prediction is unchanged: 
\begin{align}
 \arg\max_i f_i(x+\delta_x)=c
 .
\end{align}
\end{theorem}

\begin{remark}
This result is particularly useful for analyzing the adversarial defense problem. Similar results have been discussed in the literature~\citep{szegedy2014intriguing,hein2017formal,cisse2017parseval,tsuzuku2018lipschitz}.
\end{remark}

\begin{proof}
By writing \eqref{eq:classmargin_mx} into:
\begin{align}
m(x) = (e_c - e_j)^\top
    \begin{bmatrix}
        f_c(x) \\
        \max_{j \neq c} f_j(x)
    \end{bmatrix}
    ,\notag
\end{align}
where $e_c$ and $e_j$ are one-hot basis, for $p$-norm, applying H\"older's inequality with the conjugate exponent $q$ ($\frac{1}{p} + \frac{1}{q} = 1$) immediately yields:
\begin{align}
\mathrm{Lip}_p\left[m\right] \leq \left\| e_c - e_j \right\|_{q} \; \mathrm{Lip}_p\left[f\right] = 2^{\frac{1}{q}} \; \mathrm{Lip}_p\left[f\right] = 2^{1-\frac{1}{p}} \; \mathrm{Lip}_p\left[f\right]
,\notag
\end{align}
so that a guaranteed $p$-norm perturbation $\delta_x$ does not alter the prediction, if:
\begin{align}
\|\delta_x\|_p \leq \frac{m(x)}{\mathrm{Lip}_p\left[m\right]} = \frac{m(x)}{2^{1-\frac{1}{p}} \;\mathrm{Lip}_p\left[f\right]}
,\notag
\end{align}
which recovers \eqref{eq:2norm_perturbation_deltax} in Section~\ref{sec:lipschitz_regularizations:class_margin} with $p=2$.







\end{proof}







  




\subsection{Certifiable Robustness via Global Lipschitz Bound}

For a network $f$ with 1-Lipschitz activations and $W^{(\ell)}$ is the $\ell$-th layer parameter matrix, the spectral-norm product bounds the Lipschitz constant of $f$ globally:
\begin{align}
\mathrm{Lip}[f] \le \prod_{\ell=1}^L \|W^{(\ell)}\|_2,\notag
\end{align}
providing a \emph{certified global bound}. This is computationally cheap but typically loose. \textbf{SeqLip} \citep{virmaux2018lipschitz} refines this spectral product by incorporating singular-vector alignment between layers, also producing certified global bounds. \textbf{LipSDP} \citep{fazlyab2019efficient} interprets activation functions as gradients of convex potential functions, satisfying certain properties described by quadratic constraints. Therefore, Lipschitz constant estimation problem is treated as a semi-definite program (SDP) problem. 

\subsection{Certifiable Robustness via Local Lipschitz Bound}

Local Lipschitz bounds are computed over a neighborhood. \textbf{Fast-Lip} \citep{weng2018fastlip} analyze the activation patterns of ReLU networks and derive a gradient norm based local Lipschitz bound. \textbf{CLEVER} \citep{weng2018clever} estimates local constants via extreme value theory on sampled gradient norms; this improves tightness but does not yield a formal certificate. MILP-based methods \citep{jordan2020exactly} encode the exact piecewise-linear constraints of ReLU networks within the ball, yielding exact local Lipschitz constants (and thus exact certified radii), but are limited to small networks.  



\subsection{Certifiable Robustness in Language Models}


\paragraph{Proper Distance Metrics for Text.} Language models typically operate on text sequences as inputs, for which the conventional notion of a Lipschitz constant over $\mathbb{R}$ with $\ell_p$ norm does not directly apply. The \emph{Levenshtein distance} \citep{levenshtein1966binary} measures the number of character replacements, insertions or deletions needed in order to transform a sequence $x$ to sequence $y$. It is a proper metric that satisfies all axioms of a metric space:
\begin{enumerate}
    \item \textbf{Non-Negativity.} $d_{\mathrm{lev}}(x,y) \geq 0$;
    \item \textbf{Identity.} $d_{\mathrm{lev}}(x,y) = 0 \Longleftrightarrow x =y$;
    \item \textbf{Symmetry.} $d_{\mathrm{lev}}(x,y) = d_{\mathrm{lev}}(y,x)$;
    \item \textbf{Triangle Inequality.} $d_{\mathrm{lev}}(x,z) \leq d_{\mathrm{lev}}(x,y) + d_{\mathrm{lev}}(y,z)$;
\end{enumerate}
where $d_{\mathrm{lev}}(x,y)$ denotes the Levenshtein distance between two sequences $x$ and $y$. Thereby it provides a principled foundation for discussing Lipschitz continuity in the context of language models. For tokenized text --- where each vocabulary item is represented as a one-hot vector --- a variant of the \emph{Levenshtein distance}, known as the \emph{ERP distance}, has been proposed for comparing sequences of one-hot vectors \citep{chen2004editdistance}.



\citet{rocamora2025certified} introduce \textbf{LipsLev}, a method for training convolutional text classifiers that are \emph{1-Lipschitz} in the sense of Levenshtein distance for Lipschitz constant based defense \citep{rocamora2025certified}. That is, for a classifier $f: S \to \mathbb{R}^c$, two one-hot vector-valued sequences $x \in \mathbb{R}^{n \times d} \subset S $ and $y \in \mathbb{R}^{m \times d} \subset S$ where $n,m$ are sequence lengths and $d$ is one-hot vector dimension, the classification margin must hold:
\begin{align}
    | f_i(x) - f_j(y)| \leq K_{\mathrm{lev}} \; d_{\mathrm{lev}}(x, y)
\end{align}
for a constant $K_{\mathrm{lev}} \leq 1$, so that the prediction does not change under perturbation radius $d_{\mathrm{lev}}(x, y) < R$ \citep[Theorem 4.3 \& Corollary 4.4]{rocamora2025certified}. They then train a 1-Lipschitz classifier over text sequences --- in the sense of the Levenshtein distance --- by normalizing each layer's outputs through division by its corresponding Lipschitz constant \citep[\S~4.3]{rocamora2025certified}.










\section{Conclusions}

Lipschitz continuity serves as a cornerstone for enhancing the robustness, generalization, and optimization stability of deep neural networks, providing a rigorous mathematical framework to quantify and control sensitivity to input perturbations. This comprehensive survey synthesizes key insights across theoretical foundations, estimation techniques, regularization approaches, and certifiable robustness, highlighting their interconnections and practical implications. By unifying disparate research threads, we address a critical gap in the literature, offering a cohesive resource for researchers and practitioners. Challenges remain in balancing bound tightness with computational scalability, preserving model expressivity under constraints, and extending certifications to diverse norms and large-scale architectures like transformers, paving the way for future advancements in trustworthy deep learning systems.




==> main_matter/chapters/LiteratureReview/text_v2.tex <==

\section{Introduction}
\label{sec:intro}


\lettrine[lines=3]{D}{eep} learning has achieved remarkable success across various domains, including computer vision, natural language processing, and graph-based learning. Advances in state-of-the-art architectures, such as convolutional neural networks (CNNs) \citep{krizhevsky2012imagenet}, transformers \citep{vaswani2017attention, brown2020language}, and graph neural networks (GNNs) \citep{kipf2017semi}, as well as their large-scale applications, including large language models (LLMs) \citep{brown2020language, chowdhery2022palm, touvron2023llama,openai2023gpt4,deepseekai2025deepseekr1} and large vision-language models (LVLMs) \citep{radford21aclip,li22nblip,geminiteam2025}, have significantly expanded the frontiers of deep learning, enabling powerful capabilities across a wide range of tasks.

Beyond their remarkable success, ensuring safety, robustness \citep{madry2018towards} and generalization, remains a critical challenge. These properties are intrinsically linked to the sensitivity of neural networks to input perturbations \citep{madry2018towards,tsipras2018robustness,hendrycks2019benchmarking,amerehi25alabelaugmentation}, which can significantly impact their reliability in real-world applications. For instance, adversarial vulnerabilities \citep{goodfellow2014explaining, carlini2017towards}, and out-of-distribution (OOD) generalization \citep{sokolic2017robust,Neyshabur2017nips,bartlett2017spectrally,hendrycks2021many} are major concerns in developing reliable deep learning models. A fundamental mathematical concept that characterizes network sensitivity and governs these properties is \textbf{Lipschitz continuity}, which measures the upper bound of the outputs of neural networks to inputs.

Although numerous studies have explored Lipschitz continuity from both theoretical \citep{bartlett2017spectrally, luo2025lipschitz} and applied \citep{arjovsky2017wasserstein, gulrajani2017improved, miyato2018spectral} perspectives, a unified survey that consolidates these insights is still lacking. Existing works primarily focus on isolated aspects, such as adversarial robustness \citep{szegedy2014intriguing, madry2018towards, weng2018clever}, regularization \citep{arjovsky2017wasserstein, gulrajani2017improved}, or theoretical bounds without practical considerations \citep{bartlett2017spectrally}. The absence of a comprehensive survey integrating these perspectives leaves a critical gap in the literature. To address this, we provide a systematic review of Lipschitz continuity in deep learning, covering its \textbf{theoretical foundations},  \textbf{estimation methods}, \textbf{regularization approaches in optimization and architecture}, and \textbf{certifiable robustness}. By synthesizing key findings across these domains, this survey serves as a valuable resource for researchers and practitioners seeking a deeper understanding of Lipschitz continuity and its role in trustworthy learning systems. Beyond conducting a survey, we also critically distill the existing knowledge, present it in a more accessible manner, and provide the results or proofs \textbf{missing} or \textbf{incorrect} in the literature.

\subsection{Scope}

This survey aims to consolidate existing knowledge across these domains, providing a comprehensive resource for researchers and practitioners seeking to understand and leverage Lipschitz continuity in deep learning. To ensure a high-quality review, we focus primarily on the literature published in prestigious and other well-regarded sources. The scope of this survey is organized as below:

\begin{enumerate}

    \item Section~\ref{sec:theory}:~\nameref{sec:theory}  
    presents the formal definitions and fundamental properties of Lipschitz continuity, followed by key theoretical developments in deep learning. It covers the mathematical foundations, Lipschitz properties of activation functions and neural networks, Lipschitz analysis of multi-head self-attention, complexity-theoretic generalization bounds, and advances in training dynamics.

    \item Section~\ref{sec:estimating_lipschitz}:~\nameref{sec:estimating_lipschitz}  
    surveys the principal methods for estimating the Lipschitz constants of neural networks, including derivative bound propagation, spectral alignment, convex optimization relaxations, and relaxed integer programming approaches.


    \item Section~\ref{sec:lipschitz_regularizations}:~\nameref{sec:lipschitz_regularizations}  
    reviews approaches for enforcing Lipschitz continuity in neural networks through both optimization-based and architectural approaches, covering weight regularization, gradient regularization, activation regularization, and class-margin regularization.
    

    \item Section~\ref{sec:certifiable_robustness}:~\nameref{sec:certifiable_robustness}  
    examines methods for achieving certifiable robustness through Lipschitz bounds, including the theoretical foundations of Lipschitz-margin robustness radii, certification via global Lipschitz bounds, certification via local Lipschitz bounds and certificated robustness in LLMs.
    
\end{enumerate}





\subsection{Contributions}


Our key contributions are as follows:
\begin{enumerate}

    \item \textbf{A Unified Systematic Review}. We close a critical gap in the literature by conducting a comprehensive survey of Lipschitz continuity in deep learning. Our review unites disparate research threads --- spanning theoretical foundations, estimation methods, regularization approaches, architectural designs, and certified robustness --- into a coherent framework that highlights their interconnections from the lens of Lipschitz continuity.
    

    \item \textbf{Comprehensive Analysis}. We provide in‐depth examinations of existing techniques organized into four categories:
    \begin{itemize}
        \item \textbf{Theoretical Foundations}. We review the formal definitions and properties of Lipschitz continuity, analyze Lipschitz behavior of activations and network architectures, and synthesize key results on generalization bounds, optimization convergence, and training‐induced Lipschitz dynamics. 
        
        \item \textbf{Estimation Methods}. From power‐iteration spectral‐norm approximations and extreme‐value theory to randomized and interval‐analysis approaches, we compare each method's tightness, computational overhead, and scalability to modern architectures.
        
        \item \textbf{Regularization Approaches}. We critically assess gradient‐based penalties, spectral normalization, orthogonal and Parseval constraints, and novel Lipschitz bounded activations, examining their theoretical guarantees, implementation trade‐offs, and empirical effects on robustness, generalization, and training dynamics.
        
        \item \textbf{Certifiable Robustness}. We survey Lipschitz‐based certification frameworks --- covering global and local Lipschitz bounds, path‐based and convex‐relaxation certificates, randomized smoothing, and Lipschitz constrained architectures --- analyzing their provable guarantees, computational requirements, and applicability to real‐world deep models.
    \end{itemize}

   
 
    % \item \textbf{Results and Proofs}. \textcolor{blue}{We contribute new and complementary results, including:}
    % \begin{itemize}
    %     \item \textbf{Results for Common Activation Functions} --- we correct Lipschitz constants for common activation functions (\eg, \emph{softmax} and \emph{sigmoid}) that are not accurate in prior literature, and validate by our numerical experiments. We also provide 

    %     \item \textbf{Results for Directed Acyclic Graphs (DAGs)} --- we derive a Lipschitz continuity bound for arbitrary neural networks represented as directed acyclic graphs (DAGs). 

    %     \item \textbf{Proofs} ---
    %     Furthermore, we provide theoretical results missing from prior work, such as rigorous proofs of the closed-form expressions for the Lipschitz constants of common activation functions and a general perturbation bound for certifiable robustness based on H\"older's conjugacy relation.
    % \end{itemize}
    

    
    \item \textbf{Results and Proofs}. We contribute new and complementary results, including corrected Lipschitz constants for common activation functions (validated by our numerical experiments) and a Lipschitz continuity bound for arbitrary neural networks represented as directed acyclic graphs (DAGs). Furthermore, we provide theoretical results \textbf{missing or incorrect} from prior work, such as rigorous proofs of the closed-form expressions for the Lipschitz constants of common activation functions and a general perturbation bound for certifiable robustness based on H\"older's conjugacy relation.
    
\end{enumerate}

 




\section{Theoretical Foundations}
\label{sec:theory}


Lipschitz continuity is a foundational concept in deep learning theory, offering a rigorous framework for quantifying a neural network's sensitivity to input perturbations. It plays a central role in understanding robustness, generalization, and optimization dynamics. Throughout, we use operator $\mathrm{Lip}_p\left[ \bullet \right]$ to denote the $p$-norm Lipschitz constant for $\bullet$, and use operator $\mathrm{Lip}\left[ \bullet \right]$ to denote the $2$-norm Lipschitz constant for $\bullet$.





\subsection{Preliminaries}
\label{sec:preliminaries}

\begin{definition}[$p$-Norm in Finite-Dimensional Vector Spaces]
Let $V \subseteq \mathbb{R}^d$ be a finite-dimensional vector space. The $p$-norm (\ie~$\ell_p$-norm) in $V$ is defined as:
\begin{equation}
    \|z\|_p =
    \begin{cases}
        \left( \sum\limits_{i=1}^d |z_i|^p \right)^{1/p}, & \text{if } 1 \leq p < \infty, \\
        \quad \\
        \max\limits_{i=1,\dots,d} |z_i|, & \text{if } p = \infty,
    \end{cases}
\end{equation}
where $z = (z_1, z_2, \dots, z_d) \in V$ \citep[Definition~3.6, \S~3]{rudin1987real}.
\end{definition}



\begin{definition}[Globally $K$-Lipschitz Continuous]
\label{def:lipschitz_definition}
Let $f: X \mapsto Y$ be a function, where $X \subseteq \mathbb{R}^d$ and $Y \subseteq \mathbb{R}^c$. The function $f$ is said to be \emph{globally $K$-Lipschitz continuous} (with respect to the 2-norm) if there exists a constant scalar $K > 0$ such that:
\begin{equation}
    \|f(u) - f(v)\|_2 \leq K \|u - v\|_2, \quad \forall\, u, v \in X
    ,
\end{equation}
\citep[Theorem 9.19, \S~9]{rudin1976principles}. Throughout, unless specified otherwise, the \emph{Lipschitz norm} is assumed to be the $2$-norm.
\end{definition}


\begin{definition}[Globally $K_{p \to q}$-Lipschitz Continuous]
\label{def:lipschitz_definition_holders_conjugate}
Let:
\begin{align}
1 \le p, q \le \infty    
\end{align}
be two scalars.
% satisfy the H\"older conjugacy relation \citep[\S~6]{rudin1976principles}:
% \begin{align}
% \frac{1}{p} + \frac{1}{q} = 1
% .
% \end{align}
A function $f: X \to Y$, with $X \subseteq \mathbb{R}^d$ and $Y \subseteq \mathbb{R}^c$, is said to be \emph{$K_{p \to q}$-Lipschitz continuous} if there exists a constant $K_{p \to q} > 0$ such that:
\begin{equation}
    \|f(u) - f(v)\|_{q} \; \le \; K_{p \to q} \, \|u - v\|_{p},
    \quad \forall\, u, v \in X,
\end{equation}
where $\|\cdot\|_p$ and $\|\cdot\|_q$ denote the $\ell_p$ and $\ell_q$ norms, respectively. Particularly, $K_{2 \to 2}$-Lipschitz continuous reduces to $K$-Lipschitz continuous with respect to $2$-norm.
\end{definition}

\begin{remark}
Definition~\ref{def:lipschitz_definition_holders_conjugate}~(\nameref{def:lipschitz_definition_holders_conjugate}) is non-standard in the mathematical literature; however, it is useful for discussions of certifiable robustness in the context of deep learning.
\end{remark}

%{\color{blue}

\begin{lemma}[Lipschitz Constant Bounds Gradient Norm]
\label{lemma:lipschitz_bounds_gradient}
Let $f: \mathbb{R}^m \to \mathbb{R}$ be a differentiable function. Then $f$ is $K$-Lipschitz continuous (with respect to the 2-norm) if and only if
\begin{equation}
K \geq \sup_{x \in \mathrm{dom}(f)} \|\nabla f(x)\|_2,
\end{equation}
\citep[Theorem 9.19, \S~9]{rudin1976principles}. In the case $0 < K < 1$, the function $f$ is called a contraction map. In particular, for the case that $\mathrm{dom}(f)$ is a convex set --- any points connected through the \emph{Mean Value Theorem} remain within $\mathrm{dom}(f)$, thus the tight bound is achieved such that:
\begin{equation}
K = \sup_{x \in \mathrm{dom}(f)} \|\nabla f(x)\|_2.
\end{equation}
\end{lemma}


\begin{remark}
\label{remark:domain_convex}
In Lemma~\ref{lemma:lipschitz_bounds_gradient}~(\nameref{lemma:lipschitz_bounds_gradient}), of the deep learning sense, the domain of a neural network $f: \mathbb{R}^m \to \mathbb{R}$ can be assumed to be a convex set on $\mathbb{R}^m$. Consequently, the tight Lipschitz bound is attained.
\end{remark}

\subsection{$1$-Lipschitz Orthogonal Matrix}
\label{sec:orthogonal_matrix}

\begin{definition}[Skew-Hermitian \& Skew-Symmetric Matrix]
\label{def:skew_hermitian}
A matrix $A$ is referred to as a \emph{skew-hermitian matrix}, if $A$ satisfies:
\begin{align}
    A=-A^*
    .
\end{align}
Particularly, if $A$ is a real matrix, then $A$ is also referred to as a \emph{skew-symmetric matrix}.
\end{definition}

\begin{proposition}[Lipschitz Constant of Semi-Orthogonal Matrix]
\label{prop:column_orthogonal_matrix}
If a matrix $W \in \mathbb{R}^{m \times n}$ with:
\begin{align}
    W^\top W = I_n
    \qquad \text{or} \qquad
    W W^\top = I_m
    ,
\end{align}
then $W$ is semi-orthogonal with Lipschitz constant $1$. If $m \geq n$, $W$ is an isometric map over the entire $\mathbb{R}^n$; if $m < n$, $W$ is a contraction map on $\ker(W)$ strictly.
\end{proposition}

\begin{proof}
\begin{enumerate}[label=\textbf{}, leftmargin=*]

\item \textbf{Case 1: $m \geq n$ (Isometric Map).} For $\forall\;x,y \in \mathbb{R}^n$:
\begin{align}
\|W(x-y)\|_2^2
&= (W(x-y))^\top W(x-y) \\
&= (x-y)^\top W^\top W (x-y)\\
&= (x-y)^\top I_n (x-y) \\
&= \|x-y\|_2^2
,
\end{align}
then by definition:
\begin{align}
    \mathrm{Lip}\left[W\right] =
    \sup_{x \neq y} \frac{\|W(x-y)\|_2}{\|x-y\|_2} = 1.
\end{align}

\item \textbf{Case 1: $m < n$ (Contraction on Kernel).} For $\exists \; x-y \in \ker(W)$, such that:
\begin{align}
\|W(x-y)\|_2 = 0 < \|x-y\|_2
,
\end{align}
then $W$ is a contraction map on the kernel $\ker(W)$ strictly.
\end{enumerate}
\end{proof}

\subsubsection{Matrix Orthogonalization}

We also survey useful matrix orthogonalization algorithms below.

\paragraph{Lie Group Exponential Map.} Let:
\begin{align}
    U(n) = \Bigl\{ 
    A \in \mathbb{C}^{n \times n} \mid A^* A = I
    \Bigr\}
\end{align}
be an unitary group and:
\begin{align}
    \mathfrak{u}(n)=\{B\in\mathbb{R}^{n\times n}\;:\;B=-B^*\}
\end{align}
be a \emph{Skew-Hermitian} group. Then the \emph{Lie Exponential Map} connects $\mathfrak{u}(n)$ and $U(n)$:
\begin{align}
    \exp(A)=I+A+\frac{1}{2}A^2+\cdots
    ,
\end{align}
which is surjective. For a matrix $W$, its corresponding skew-Hermitian matrix can be constructed by taking:
\begin{align}
    B=W-W^*
\end{align}
\citep{lezcano2019cheap}.

\paragraph{Cayley Transform.} If $B \in \mathbb{R}^{n \times n}$ is a \emph{skew-symmetric} matrix, the surjective map:
\begin{align}
    \phi(B)=(I+\frac{1}{2}B)(I-\frac{1}{2}B)^{-1}
\end{align}
is referred to as the \emph{Cayley map} which transforms $B$ to an orthogonal matrix $\phi(B)$ \citep{cayley1846quelques,trockman2021orthogonalizing}.

%\paragraph{Newton–Schulz Iteration.} 

\paragraph{\emph{Bj\"orck Orthogonalization} Approximation.} Suppose $W_0 \in \mathbb{R}^{n \times n}$ is not an orthogonal matrix. Let $W_k$ be an iterative sequence such that $W_k$ is the closest orthogonal matrix to $W_0$ as $k \to \infty$. \emph{Bj\"orck Orthogonalization} \citep{bjorck1971} is a differentiable method to iteratively solve the closest orthogonal matrix to a given matrix $W_0$. \citet{chernodub2017normpreservingorthogonalpermutationlinear} use \emph{Bj\"orck Orthogonalization} in an optimization problem for constraining the orthogonality of parameter matrices \citep{chernodub2017normpreservingorthogonalpermutationlinear}. \emph{Bj\"orck Orthogonalization} \citep{bjorck1971} is defined by:
\begin{align}
    W_{k+1} = W_k \Bigl(
    I + \frac{1}{2} Q_k + \cdots + (-1)^p 
    \begin{pmatrix}
        -\frac{1}{2} \\
        p
    \end{pmatrix}
    Q_k^p
    \Bigr)
    ,
\end{align}
where $W_{k}$ is the $k$-th iterative result, $p$ is a chosen hyper-parameter, $\begin{pmatrix}
    -\frac{1}{2}\\
    p
\end{pmatrix}$ is binomial coefficient, and $Q_k$ is:
\begin{align}
    Q_k = I - W_k^\top W_k
    .
\end{align}
As $n \to \infty$, $W_k^\top W_k$ converges to $I_n$. For a rectangular matrix $W_0 \in \mathbb{R}^{m \times n}$, if $\rank(W_0) = n$, the convergence still holds: 
\begin{align}
W_k^\top W_k \to I_n \qquad \text{as} \qquad
n \to \infty
.
\end{align}



\subsection{Functional Inequalities}

\begin{proposition}[Lipschitz Constant of Function Composition]
\label{prop:lipschitz_composition}
Let $f:X \to Y$ and $g: Y \to Z$ be two bounded functions. Then the Lipschitz constant of their composition $g\;\circ\;f: X \to Z$ admits:
\begin{align}
    \mathrm{Lip}_p \left[ g \circ f \right] \leq \mathrm{Lip}_p \left[ g\right]\;\mathrm{Lip}_p \left[ f\right].
\end{align}
\end{proposition}

\begin{proof}
    \begin{align}
        \mathrm{Lip}_p \left[ g \circ f \right] &=
        \sup_{\|x-y\|_p \neq 0} \frac{\|f(g(x)) - f(g(y))\|_p}{\|x - y\|_p} \\
        &\leq 
        \mathrm{Lip}_p \left[ f \right]
        \;
        \sup_{\|x-y\|_p \neq 0} \frac{\|g(x) - g(y)\|_p}{\|x - y\|_p} \\
        &=\mathrm{Lip}_p \left[ f \right]
        \;
        \mathrm{Lip}_p \left[ g \right]
        .
    \end{align}
\end{proof}

\begin{proposition}[Lipschitz Constant of Function Addition]
\label{prop:lipschitz_addition}
Let $f$ and $g$ be two bounded functions on $\mathrm{dom}(g) \; \cap \; \mathrm{dom}(f)$. Then the Lipschitz constant of $g + f$ admits:
\begin{align}
    \mathrm{Lip}_p \left[ g + f \right] \leq \mathrm{Lip}_p \left[ g\right] + \mathrm{Lip}_p \left[ f\right].
\end{align}
\end{proposition}

\begin{proof}
   \begin{align}
       \mathrm{Lip}_p \left[ g + f \right] &=
       \sup_{\|x-y\|_p \neq 0} \frac{\|f(x) + g(x) - \left[f(y) + g(y)\right]\|_p}{\|x - y\|_p}  \\
       &=\sup_{\|x-y\|_p \neq 0} \frac{\|f(x) - f(y) + g(x) - g(y)\|_p}{\|x - y\|_p}  \\
       &\leq
       \sup_{\|x-y\|_p \neq 0} \frac{\|f(x) - f(y)\|_p}{\|x - y\|_p}
       +
       \sup_{\|x-y\|_p \neq 0} \frac{\|g(x) - g(y)\|_p}{\|x - y\|_p} \\
       &= \mathrm{Lip}_p \left[ g\right] + \mathrm{Lip}_p \left[ f\right].
   \end{align} 
\end{proof}

\begin{proposition}[Lipschitz Constant of Function Concatenation]
\label{prop:lipschitz_concatenation}
Let $f: \mathbb{R}^d \to \mathbb{R}^m$ and $g: \mathbb{R}^d \to \mathbb{R}^n$ be two Lipschitz continuous functions. Let:
\begin{align}
    (f \oplus g)(x) := \begin{bmatrix}
        f(x) \\
        g(x)
    \end{bmatrix}
    \in \mathbb{R}^{m+n}
\end{align}
be a function by concatenating the outputs of $f$ and $g$. Then, the following inequality holds true:
\begin{align}
    \Bigl(\mathrm{Lip}_p\left[f \oplus g\right]\Bigr)^p \leq \Bigl(\mathrm{Lip}_p\left[f\right]\Bigr)^p + \Bigl(\mathrm{Lip}_p\left[g\right]\Bigr)^p
    .
\end{align}
\end{proposition}

\begin{proof}
For any $x,y \in \mathbb{R}^d$, we have:
\begin{align}
    \bigl\|(f \oplus g)(x) - (f \oplus g)(y)\bigr\|_p^p
    &= \left\|
        \begin{bmatrix}
            f(x) \\
            g(x)
        \end{bmatrix}
        -
        \begin{bmatrix}
            f(y) \\
            g(y)
        \end{bmatrix}
    \right\|_p^p \\
    &=\sum_{i=1}^{m} \Bigl(|f(x)-f(y)|^p\Bigr)_i + \sum_{j=1}^{n} \Bigl(|g(x)-g(y)|^p\Bigr)_j\\
    &\leq \Biggl(\Bigl(\mathrm{Lip}_p\left[f\right]\Bigr)^p  + \Bigl(\mathrm{Lip}_p\left[g\right]\Bigr)^p \Biggr)\|x-y\|_p^p 
    .
\end{align}
Hence:
\begin{align}
   \Bigl(\mathrm{Lip}_p\left[f \oplus g\right]\Bigr)^p &= \sup_{x\neq\,y} \frac{\bigl\|(f \oplus g)(x) - (f \oplus g)(y)\bigr\|_p^p}{\|x-y\|_p^p}  \\
   &\leq \Bigl(\mathrm{Lip}_p\left[f\right]\Bigr)^p  + \Bigl(\mathrm{Lip}_p\left[g\right]\Bigr)^p
   .
\end{align}

\end{proof}


% \begin{theorem}[Rademacher's Theorem]
    
% \end{theorem}

%The (Clarke) generalized Jacobian
%Frank H Clarke. Generalized gradients and applications. Transactions of the American Mathematical Society, 205:247–262, 1975.

%Exactly Computing the Local Lipschitz Constant of ReLU networks
%
\subsection{Sub-Differential Convex Functions}
\label{sec:subdifferential}

For a function that is not differentiable but is locally Lipschitz continuous --- such as the ReLU activation --- the Clarke sub-differential provides a generalized notion of gradient that allows one to analyze and bound local Lipschitz constants \citep{clarke1975generalized}.

%For a non-differentiable convex function --- such as the ReLU activation --- the notion of a generalized gradient (\ie, the Clarke subgradient) is used to discuss the local Lipschitz constant on convex hulls in the sense of sub-differentiability \citep{clarke1975generalized}.

%https://pages.cs.wisc.edu/~yliang/cs839_spring22/documents/0222-lec9-Clarke.pdf
\begin{definition}[Generalized Gradient]
Let $f: \mathbb{R}^m \to \mathbb{R}$ be a function on $X$. The sub-differential of $f$ at point $x$ is a set, satisfying:
\begin{align}
    \partial_s f(x) = \Bigl\{
    g \mid \forall x,y \in X,\, \exists\, g \in \mathbb{R}^m\; \text{s.t.}~f(y) \geq f(x) + \langle g, y -x\rangle
    \Bigr\}
    .
\end{align}
If $f$ is convex, then:
\begin{align}
\partial_s f(x) \neq \varnothing 
\qquad
\text{and}
\qquad
\partial_s f(x) = \{\nabla f(x^*) \mid \forall~x^* \to x\}
.
\end{align}

\end{definition}

\begin{definition}[Clarke Sub-Gradient]
Let $f: \mathbb{R}^m \to \mathbb{R}$ be a proper convex function on $X$. If $f$ is locally Lipschitz continuous on $X$, then by Rademacher’s theorem it is differentiable almost everywhere. The Clarke sub-differential $f$ at a point $x$ is defined as the convex hull of all limit points of gradients at differentiable points approaching $x$. That is, a vector $g$ lies in the Clarke sub-differential at $x$ if there exists a sequence of points $x_k \to x$ ($k \in \mathbb{N}$) at which $f$ is differentiable such that the gradients $\nabla f(x_k)$ converge to $g$. Then the Clarke sub-differential is a convex hull, satisfying:
\begin{align}
    \partial f(x) = \mathrm{conv}\Bigl\{ 
    g \mid \exists\; \text{a sequence}~(x_k) \to x~\text{as}~k\to \infty, \nabla f(x_k) \to g
    \Bigr\}
\end{align}
\citep[Definition 1.1]{clarke1975generalized}. If $f$ is convex, then $\partial f(x) = \partial_s f(x)$. This definition also extends to vector-valued functions \citep{clarke1990optimization}.
\end{definition}


\begin{lemma}[Local Lipschitz Constant of Sub-Differential Function]
%https://abel.math.harvard.edu/archive/212b_spring_05/handouts/Rademacher.pdf
Let $f: \mathbb{R}^m \to \mathbb{R}^n$ be a convex function differentiable almost everywhere on $X$. Then the $p \to q$ local Lipschitz constant of $f$ on $X$ is given as:
\begin{align}
    \mathrm{Lip}_{p \to q}\left[f; X\right] = \sup_{G \in \partial f(x)} \; \sup_{\|v\|_p \neq 0} \; \frac{\| G^\top\,v \|_q}{\|v\|_p} =
    \sup_{G \in \partial f(x)} \; \sup_{\|v\|_p = 1} \; \| G^\top \|_q
    ,
\end{align}
such that:
\begin{align}
    \|f(x) - f(y)\|_q \leq 
    \mathrm{Lip}_{p \to q}\left[f; X\right] \; \|x - y\|_p
    ,
\end{align}
for $\forall\;x,y \in X$ in the sense of Clarke sub-gradient \citep{jordan2020exactly,boyd2022ee364b}.
\end{lemma}

% 

%then use rademacher's theorem we can bound.

\subsection{Lipschitz Continuity of Activation Functions}
\label{sec:activation_functions}

An activation function:
\begin{align}
    \phi: \mathbb{R}^d \to \mathbb{R}^d
\end{align}
is a nonlinear mapping applied after neuron's output at a layer, enabling neural networks to learn complex patterns. For example, if $\phi$ is piecewise defined as:
\begin{align*}
    \phi(x) =
\begin{cases}
x, & \text{if } x > 0, \\
0, & \text{otherwise}
\end{cases}
,
\end{align*}
then the $\phi$ is referred to as \emph{ReLU} activation function \citep{nair2010relu}.


%W5. The language around the use of Lemma 2.4 to "verify the results" needs to be appropriately qualified. The autograd-based method does not provide any sort of guarantee / verification, as the maximizing solution to (7) may not be found in practice. This is at best a sanity check for the Lipschitz bounds, but certainly not any guarantee.
The Lipschitz constants of commonly used activation functions are provided in Table~\ref{tab:lipschitz_activations}. The constants are derived as the supremum of the $2$-norm of the derivatives of activation functions. Proofs are provided in the Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions}. To numerically validate the results, we have conducted experiments by maximizing the gradient norm using Lemma~\ref{lemma:lipschitz_bounds_gradient} for a further sanity check.


\textbf{Notes.} The Lipschitz constant for the \emph{softmax} function reported in the literature~\citep{gouk2021regularisation} and \emph{Sigmoid} function reported in the literature~\citep{virmaux2018lipschitz} as 1. \textcolor{black}{We show in Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Softmax} that the exact Lipschitz constant of \emph{softmax} is indeed $\frac{1}{2}$, validated by our numerical experiment.} This result has been reported a recent concurrent literature \citep{nair2025softmax}. We also show in Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Sigmoid} that exact Lipschitz constant of \emph{sigmoid} is indeed $\frac{1}{4}$, validated by our numerical experiment. For \emph{Leaky ReLU} and \emph{ELU}, the parameter $\alpha$ is typically chosen with $\alpha < 1$, so their effective Lipschitz constants are usually $1$ in practice.

\textbf{Auto-Differentiation based Numerical Method.} Suppose $f: \mathbb{R}^{d} \to \mathbb{R}$ be a first- and second-order differentiable neural network under domain convex condition (Remark~\ref{remark:domain_convex}). Leverage the autograd mechanism of PyTorch, we use gradient descent --- \eg, Adam \citep{diederik2014adam} --- to numerically approximate the supremum:
\begin{align}
    \mathrm{Lip}[f] = \sup_x \|f'(x)\|_2
    ,
\end{align}
using Lemma~\ref{lemma:lipschitz_bounds_gradient}.

\begin{table}[H]
\centering

\caption{Lipschitz constants of activation functions.}

\label{tab:lipschitz_activations}
\renewcommand{\arraystretch}{1.2}

%\resizebox{0.95\linewidth}{!}{ 
\adjustbox{max width=0.9\textwidth}{%
\begin{tabular}{|l|c|c|p{6.2cm}|}
\hline
\textbf{Activation} & \textbf{Definition} & \textbf{Lipschitz Constant \& Proof} & \textbf{Citations} \\
\hline
ReLU & $ \max(0, x) $ & $ 1 $ &\citet[Sec.~2]{nair2010relu}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Leaky ReLU & $ \max(\alpha x, x) $ & $ \max(1, \alpha) $ & \citet[Sec.~2]{maas2013leakyrelu}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Sigmoid & $ \frac{1}{1 + e^{-x}} $ & $ \frac{1}{4} $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Sigmoid}) & \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Tanh & $ \tanh(x) $ & $ 1 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Tanh}) &\citet{cybenko1989approximation}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
Softplus & $ \log(1 + e^x) $ & $ 1 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Softplus}) &\citet[Sec.~2]{dugas2001softplus}; \citet[Sec.~5]{virmaux2018lipschitz} \\
\hline
ELU & $ \begin{cases} x & x > 0 \\ \alpha (e^x - 1) & x \leq 0 \end{cases} $ & $ \max(1, \alpha) $ &\citet[Sec.~3]{clevert2015elu}\\
\hline
Swish & $ x \cdot \sigma(x) $ & $ \approx 1.1 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Swish}) &\citet[Sec.~1]{ramachandran2017searching} \\
\hline
GELU & $ \frac{x}{2}\left(1+\mathrm{erf}\left(\frac{x}{\sqrt{2}}\right)\right) $ & $ \approx 1.1 $ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:GELU}) &\citet[Sec.~2]{hendrycks2016gelu} \\
\hline
Softmax & $ \text{softmax}(x_i) = \frac{e^{x_i}}{\sum_j e^{x_j}} $ & $\frac{1}{2}$ (Appendix~\ref{appendix:proofs_lipschitz_constants_of_activation_functions:Softmax}) &\citet[Sec.~3.3]{gouk2021regularisation}\\
\hline
\end{tabular}
}
\end{table}

\subsection{Lipschitz Continuity of Dot-Product Self-Attention}
\label{sec:selfattention_lipschitz}

LLMs \citep{brown2020language, chowdhery2022palm, touvron2023llama,openai2023gpt4,deepseekai2025deepseekr1}, built on transformer architectures \citep{vaswani2017attention}, rely heavily on dot-product self-attention mechanisms, whose Lipschitz continuity governs their sensitivity to input perturbations, such as token-level adversarial attacks. Dot-product self-attention mechanisms form the core of transformer architectures, enabling effective modeling of long-range dependencies in sequences for applications such as natural language processing and vision-language tasks. 

\paragraph{Single-Head Dot-Product Self-Attention.} For an input sequence matrix $x \in \mathbb{R}^{n \times d}$, where $n$ is the sequence length and $d$ is the input dimension, a self-attention layer computes the output as
\begin{align}
\text{Attention}(x) = 
\underbrace{
\mathrm{softmax}\left( \frac{Q K^{\top}}{\sqrt{d}} \right)
}_{\text{row-wise softmax}}
V \in \mathbb{R}^{n \times m},
\end{align}
\citep[Equation~1]{vaswani2017attention} where
\begin{align}
Q = x W_Q \in \mathbb{R}^{n \times m}, \quad K = x W_K \in \mathbb{R}^{n \times m}, \quad V = x W_V \in \mathbb{R}^{n \times m},
\end{align}
are the \emph{query}, \emph{key}, and \emph{value} matrices, with weight matrices:
\begin{align}
W_Q, W_K, W_V \in \mathbb{R}^{d \times m},    
\end{align}
and $m$ denotes the hidden dimension. The softmax is applied row-wise to normalize attention scores. The scaling factor $\frac{1}{\sqrt{d}}$ stabilizes the computation numerically. 
%but the non-linear softmax operation renders dot-product attention non-Lipschitz continuous, complicating the computation of the Lipschitz constant, $\mathrm{Lip}[\text{Attention}]$, which quantifies the layer's sensitivity to input perturbations and is critical for ensuring robustness and generalization in transformers.

\paragraph{Multi-Head Dot-Product Self-Attention.} 
In practice, transformers employ $h$ parallel self-attention heads to jointly attend to information from different representation subspaces \citep{vaswani2017attention}. Each head $i$ has its own projection matrices:
\begin{align}
W_{Q,i}, W_{K,i}, W_{V,i} \in \mathbb{R}^{d \times m_i},   
\end{align}
where $m_i = \frac{m}{h}$, $h$ denotes the number of heads, and produces an output for head $i$:
\begin{align}
\mathrm{Attention}_i(x) \in \mathbb{R}^{n \times m_i}
.
\end{align}
The outputs are concatenated:
\begin{align}
\mathrm{Attention}(x) =\bigl[
\mathrm{Attention}_1(x),\mathrm{Attention}_2(x), \cdots, \mathrm{Attention}_h(x)
\bigr]    \in \mathbb{R}^{n \times m}
,
\end{align}
produces the final output.
% and projected via an output matrix $W_O \in \mathbb{R}^{d \times d}$. 

% \textbf{Notes.} It is worth noting that the Lipschitz constants of both single-head and multi-head dot-product self-attention mechanisms are globally unbounded, implying that these mappings are not globally Lipschitz continuous. For example, \citeauthor{kim2021lipschitz} show that the $2$-norm Lipschitz for sequence length $n$, input dimension $d$, $h$ heads is scaled by at least $\sqrt{hn}\bigl[4\phi^{-1}(n-1)+1\bigr]$ where $\phi(x)=x\exp(x+1)$ is an invertible univariate function on $x>0$ \citep[Theorem~3.2]{kim2021lipschitz}. Details are discussed in Section~\ref{sec:selfattention_non_lipschitz}.


% For a single-head self-attention module, this is because that:
% \begin{align}
%     \| \mathrm{Attention}(x) \|_2 &= 
%     \Bigl\|
% \mathrm{softmax}\left( \frac{Q K^{\top}}{\sqrt{d}} \right)
% V
% \Bigr\|_2 \\
% &\leq
%     \Bigl\|
% \mathrm{softmax}\left( \frac{Q K^{\top}}{\sqrt{d}} \right)
% \Bigr\|_2 
% \;
% \|
% V
% \|_2 \\
% &\leq
% n \|\mathrm{softmax}\|_2 
% \;\max_i
% \Bigl\|\frac{QK^\top}{\sqrt{d}}\Bigr\|_2
% \|V\|_2.
% \end{align}
% Consider that $\|\mathrm{softmax}\|_2=\frac{1}{2}$ (Table~\ref{tab:lipschitz_activations}), this leads:
% \begin{align}
% \| \mathrm{Attention}(x) \|_2 &\leq 
% \frac{n}{2\sqrt{d}} \|Q\|_2\; \|K\|_2\;  \|V\|_2
% ,
% \end{align}
% which shows that dot-product self-attention is not bounded for arbitrary sequence length $n$ and the bound is scaled by at least $O(n)$. 

% \textbf{Notes.} It is worth noting that the Lipschitz constants of both single-head and multi-head dot-product self-attention mechanisms are globally unbounded, implying that these mappings are not globally Lipschitz continuous. For a single-head self-attention module, this is because that:
% \begin{align}
%     \| \mathrm{Attention}(x) \|_2 &= 
%     \Bigl\|
% \mathrm{softmax}\left( \frac{Q K^{\top}}{\sqrt{d}} \right)
% V
% \Bigr\|_2 \\
% &\leq
%     \Bigl\|
% \mathrm{softmax}\left( \frac{Q K^{\top}}{\sqrt{d}} \right)
% \Bigr\|_2 
% \;
% \|
% V
% \|_2
% \end{align}



%While multi-head dot-product self-attention improves expressivity, its Lipschitz constant depends on the largest product of spectral-norms across heads, scaled by $\sqrt{n}/\sqrt{d}$ \citep{kim2021lipschitz}, retaining the same $\sqrt{n}$ growth as the single-head case.


\subsubsection{Locally Lipschitz Continuous} 
% Standard dot-product self-attention is locally Lipschitz continuous, and several works have derived explicit upper bounds for its local Lipschitz constant. \citeauthor{hu2024specformer} show that for the self-attention layer operating on $\mathrm{vec}(X)$ within a ball $B_R(\mathrm{vec}(X))$, the following holds:
% \begin{align}
%     \mathrm{Lip}(\mathrm{Attn}; B_R(\mathrm{vec}(X))) 
%     \le n(n+1)\left( \|X\|_F + R \right)^2 \left[ \|W_V\|_2 \, \|W_Q\|_2 \, \|W_K\|_2 + \|W_V\|_2 \right],
% \end{align}
% where $n$ is the sequence length, $R$ is the ball radius, $\|\cdot\|_F$ is the Frobenius norm, and $\|\cdot\|_2$ is the spectral-norm.

Standard dot-product self-attention is locally Lipschitz continuous, and several works have derived explicit upper bounds for its local Lipschitz constant. Let $\mathcal{B}(x_0,\delta)=\{x \mid \|x-x_0\|_2 < \delta \}$ denote a ball centered $x_0$ with a radius $\delta$. \citeauthor{hu2024specformer} show that for the dot-product self-attention layer within a ball $\mathcal{B}_2(x,\delta)$ is locally Lipschitz continuous bounded by:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}; \mathcal{B}_2(x,\delta)\Bigr] 
    \leq
    n(n+1)\Bigl(\|x\|_2 + \delta\Bigr)^2
    \Bigl[
    \|W_V\|_2
    \|W_Q\|_2
    \|W_K^\top\|_2
    +
    \|W_V\|_2
    \Bigr]
    ,
\end{align}
where $x \in \mathbb{R}^{n \times d}$, $n$ is the sequence length, $d$ is the input dimension, $W_K, W_Q, W_V \in \mathbb{R}^{d \times m}$ are the \emph{key}, \emph{query} and \emph{value} parameter matrices, and $\delta$ is a $2$-norm radius \citep[Theorem~2]{hu2024specformer}. \citeauthor{castin2023smooth} provide a tighter bound by $\sqrt{n}$ up to a constant factor, showing that within a ball $\mathcal{B}_2(0, \delta)$, the Lipschitz constant of dot-product self-attention is bounded by:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}; \mathcal{B}_2(0,\delta)\Bigr] 
    \leq
    \sqrt{3} \|W_V\|_2 
    \Biggl[
    \Bigl\|\frac{W_K^\top\,W_Q}{\sqrt{d}}\Bigr\|_2^2
    \delta^4
    (4n+1)+n
    \Biggr]^{\frac{1}{2}},
\end{align}
where $A$ is the attention score matrix \citep[Theorem~3.3]{castin2023smooth}. 

Most recently, \citet{yudin2025pay} refine the bound by explicitly incorporating the Jacobian of the softmax function, given by:
\begin{align}
\mathcal{M}(P_x) := \nabla \, \mathrm{softmax}\left(x\right) = 
\mathrm{diag}(P_x) - P_x^\top P_x,
\end{align}
where:
\begin{align}
    P_x = \Biggl( \frac{\mathrm{e}^{x_i}}{\sum_j \mathrm{e}^{x_j}} \Biggr) 
    ,
\end{align}
leading that the Lipschitz constant for a single head is bounded by:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}\Bigr] 
    \leq
    \|W_V\|_2
    \Biggl(
    \|P\|_2 + 2 \|x\|_2^2 \; \|A\|_2 \; \max_i \|\mathcal{M}(P_{i, :})\|_2
    \Biggr)
\end{align}
with:
\begin{align}
    P = \mathrm{softmax}\Bigl(
    x
    A
    x^\top
    \Bigr) \in \mathbb{R}^{n \times n} \qquad \text{and} \qquad A = \frac{W_QW_K^\top}{\sqrt{d}} \in \mathbb{R}^{d \times d}
\end{align}
\citep[Theorem~3]{yudin2025pay}. 

%This refined bound isolates the contribution of the attention-score distribution to the local Lipschitz constant, enabling targeted regularization strategies such as JaSMin (Jacobian Softmax norm Minimization) to directly control this term \citep{yudin2025pay}.



\subsubsection{Globally Non-Lipschitz Continuous} 
\label{sec:selfattention_non_lipschitz}


It is worth noting that the Lipschitz constants of both single-head and multi-head dot-product self-attention are not globally bounded. This is because the Lipschitz bound for dot-product self-attention grows with the input sequence length, implying that the dot-product self-attention is not globally Lipschitz continuous \citep[Theorem~3.1]{kim2021lipschitz}. \citeauthor{kim2021lipschitz} show that, for a sequence length $n$, input dimension $d$, and $h$ heads, the $2$-norm Lipschitz bound is:
\begin{align}
\mathrm{Lip}\left[\mathrm{Attention}\right]
\leq
\frac{\sqrt{n}}{\sqrt{\sfrac{d}{h}}}
\Bigl[
4\phi^{-1}(n-1)+1
\Bigr]
\Biggl(
\sqrt{
\sum_{h_i} 
\|W_{Q,h_i}\|_2^2\;
\|W_{V,h_i}\|_2^2\;
}
\Biggr)
\|W_O\|_2
,
\end{align}
and the $\infty$-norm Lipschitz bound:
\begin{align}
\mathrm{Lip}_{\infty}\left[\mathrm{Attention}\right]
&\leq 
\Biggl[
4\phi^{-1}(n-1) + \frac{1}{\sfrac{d}{h}}
\Biggr]
\notag\\
&\qquad\qquad
\|W_O^\top\|_{\infty}
\;
\max_{h_i} 
\|W_{Q,h_i}\|_{\infty}
\|W_{Q,h_i}^\top\|_{\infty}
\;
\max_{h_j}  \|W_{V,h_j}^\top\|_{\infty}
,
\end{align}
where:
\begin{align}
\phi(x)=x\exp(x+1)    
\end{align}
is an invertible univariate function on $x>0$,
$W_{Q,h_i}$ is the \emph{query} parameter matrix for head $h_i$, $W_{V,h_i}$ is the \emph{value} parameter matrix for head $h_i$, and $W_O$ is the projection parameter matrix \citep[Theorem~3.2]{kim2021lipschitz}. They further conclude that their results can lead that the $2$-norm Lipschitz bound is at the scale:
\begin{align}
\mathrm{Lip}[\mathrm{Attention}] \sim O(\sqrt{n} \log n),    
\end{align}
and the $\infty$-norm Lipschitz bound is at the scale:
\begin{align}
\mathrm{Lip}_{\infty}[\mathrm{Attention}] \sim
O(\log n)
\end{align}
\citep[Theorem~3.2]{kim2021lipschitz}. The bounds in \citep[Theorem~3.2]{kim2021lipschitz} are complemented by concurrent work \citep{vuckovic2020mathematical} with a measure-theoretical framework. \citeauthor{vuckovic2020mathematical} show that the $1$-norm Lipschitz bound is at the scale:
\begin{align}
\mathrm{Lip}_1[\mathrm{Attention}] \sim O(\sqrt{\log{n}})
\end{align}
\citep[Theorem 29 \& Corollary 30]{vuckovic2020mathematical}.







\subsection{Lipschitz Continuity of Neural Networks}
\label{sec:network_lipschitz}

\begin{definition}[Feedforward Network]
Let $f: \mathbb{R}^m \to \mathbb{R}^n$ denote a feedforward neural network consisting of $L$ layers, defined as the composition:
\begin{align}
    f := h^{(L)} \circ \cdots \circ h^{(2)} \circ h^{(1)},
\end{align}
where each layer $h^{(\ell)}$ is composed of a linear transformation $\phi^{(\ell)}(\cdot)$ followed by a non-linear activation function $\rho^{(\ell)}(\cdot)$:
\begin{align}
    h^{(\ell)} := \rho^{(\ell)} \circ \phi^{(\ell)}.
\end{align}
\end{definition}


%Theorem 9.19, \S~9]{rudin1976principles
%~\cite{miyato2018spectral,sedghi2019singular,kim2021lipschitz,luo2025lipschitz}
\begin{proposition}[Lipschitz Constant of a Linear Layer]
\label{prop:lipschitz_constant_of_linear_unit}
Let $\phi^{(\ell)}: \mathbb{R}^{m_{\ell}} \to \mathbb{R}^{n_{\ell}}$ denote a linear transformation implemented either as a convolutional layer:
\begin{align}
    \phi^{(\ell)}(z^{(\ell-1)}) = \boldsymbol{\theta}^{(\ell)} \circledast z^{(\ell-1)} + b^{(\ell)},
\end{align}
or as a fully connected (dense) layer:
\begin{align}
    \phi^{(\ell)}(z^{(\ell-1)}) = \boldsymbol{\theta}^{(\ell)} z^{(\ell-1)} + b^{(\ell)},
\end{align}
where $\boldsymbol{\theta}^{(\ell)}$ is the weight matrix (or convolution kernel), $b^{(\ell)}$ is the bias term, $\circledast$ denotes the convolution operator, and $z^{(\ell-1)}$ is the output from the previous layer. The Lipschitz constant of $\phi^{(\ell)}$ with respect to the Euclidean norm is given by:
\begin{align}
    \mathrm{Lip}[\phi^{(\ell)}] = \| \boldsymbol{\theta}^{(\ell)} \|_2,
\end{align}
where $\| \boldsymbol{\theta}^{(\ell)} \|_2$ denotes the spectral-norm of the associated linear operator.
\end{proposition}


%~\cite{golub2013matrix,strang2009introduction,sedghi2019singular,luo2025spectralvariation}
\begin{proposition}[Spectral-Norm via Singular Value Decomposition]
% \label{prop:spectralnorm_bound_single_layer}
Let $\boldsymbol{\theta} \in \mathbb{R}^{n \times m}$ be a matrix, admitting a truncated singular value decomposition (SVD):
\begin{align}
\boldsymbol{\theta} = \sum_{i=1}^{r} \sigma_i \boldsymbol{u}_i \boldsymbol{v}_i^\top,
\quad \text{with} \quad \sigma_1 > \sigma_2 > \cdots > \sigma_r > 0,
\quad r = \operatorname{rank}(\boldsymbol{\theta}),
\end{align}
where $\sigma_i$ are the singular values, and $\boldsymbol{u}_i$, $\boldsymbol{v}_i$ are the left and right singular vectors, respectively. Then, the spectral-norm of $\boldsymbol{\theta}$ (\ie, its operator norm induced by the Euclidean norm) is given by the largest singular value:
\begin{align}
    \| \boldsymbol{\theta} \|_2 = \sigma_1
\end{align}
 \citep[Example 5.6.6, \S~5]{horn2012matrix}.
\end{proposition}

\begin{proposition}[Lipschitz Constant Upper Bound of Feedforward Neural Network]
\label{prop:survey_upper_bound_lipschitz}
Let $f: \mathbb{R}^m \to \mathbb{R}^n$ be an $L$-layer feedforward neural network composed of linear transformations $\phi^{(\ell)}$ and activation functions $\rho^{(\ell)}$. The Lipschitz constant of $f$ with respect to the Euclidean norm is defined as:
\begin{align}
\mathrm{Lip}[f] = \sup_{\forall~u \neq v} \frac{\|f(u) - f(v)\|_2}{\|u - v\|_2},
\end{align}
which immediately admits an upper bound by applying Proposition~\ref{prop:lipschitz_composition}~(\nameref{prop:lipschitz_composition}):
\begin{align}
    \mathrm{Lip}[f] 
    \leq 
    \prod_{\ell=1}^{L} \; \mathrm{Lip}[\rho^{(\ell)}] 
    \;
    \prod_{\ell=1}^{L} \; \mathrm{Lip}[\phi^{(\ell)}]
\end{align}
\citep[Proposition 8, \S~5]{luo2025lipschitz}. 
\end{proposition}

\begin{corollary}[Spectral-Norm Upper Bound of Feedforward Neural Network]
For an $\ell$-layer feedforward network $f$ with only linear or convolutional layers and $1$-Lipschitz activation functions, combining
Proposition~\ref{prop:lipschitz_constant_of_linear_unit} and Proposition~\ref{prop:survey_upper_bound_lipschitz} immediately yields a spectral-norm product bound:
\begin{align}
    \mathrm{Lip}\left[f\right] \leq \prod_{\ell=1}^{L} \| \theta^{(\ell)} \|_2
    ,
\end{align}
where $\theta^{(\ell)}$ is the $\ell$-th layer parameter matrix. 
% Under two assumptions:
% \begin{enumerate}
%     \item the singular vectors of parameter matrices between any two consecutive layers are independent,
%     \item and each layer is sufficiently wide,
% \end{enumerate}
% this spectral-norm bound can be further refined into:
% \begin{align}
% \mathrm{Lip}\left[f\right] 
% \lessapprox 
% \frac{\prod_{\ell=1}^{L} \| \theta^{(\ell)} \|_2}{\pi^{L-1}}
% \end{align}
% almost surely \citep[Lemma 2]{virmaux2018lipschitz}.
\end{corollary}



\subsubsection{Lipschitz Continuity for a Directed Acyclic Graph (DAG)}


\begin{figure}[t!]
  \centering
  \begin{tikzpicture}[
    ->, 
    %>=Stealth, 
    node distance=1.8cm and 2cm,
    every node/.style={circle, draw, minimum size=10mm},
    shorten >=1pt]

% Nodes
\node (s)  at (0, 0)       {$s$};
\node (u1) at (2, 2.5)     {$u_1$};
\node (u2) at (2, 0.8)     {$u_2$};
\node (u3) at (2, -0.8)    {$u_3$};
\node (v)  at (4, 0)       {$v$};
\node (t)  at (6, 0)       {$t$};

% s → u1, u2, u3
\draw (s) to[out=90, in=180] (u1);
\draw (s) to[out=45, in=180] (u2);
\draw (s) to[out=-45, in=180] (u3);

% u1, u2, u3 → v
\draw (u1) to[out=0, in=90] (v);
\draw (u2) to[out=0, in=130] (v);
\draw (u3) to[out=0, in=220] (v);

% v → t (straight)
\draw (v) -- (t);

% s → t (long curved arc)
\draw (s) to[out=-90, in=-90] (t);

\end{tikzpicture}

  \caption[Example of Feedforward DAG Network]{Example of Feedforward DAG Network. There are four computational paths: $s\to u_1 \to v \to t$, $s\to u_2 \to v \to t$, $s\to u_3 \to v \to t$, and $s\to t$. A node is a module in the DAG neural network $f$.}
  
  \label{fig:dag_network}
\end{figure}

To the best of our knowledge, the existing literature does not present an explicit Lipschitz bound for a general feedforward network with skip connections. Prior literature such as \citep{miyato2018spectral,virmaux2018lipschitz} focuses strictly on sequential architectures, while norm-based capacity measures such as the path norm \citep{neyshabur2015norm} implicitly involve path enumeration but are not formulated as direct Lipschitz bounds. More recent path-metric bounds \citep{gonon2024_rescaling_invariant} apply to arbitrary DAGs but are expressed in a rescaling-invariant metric form rather than the simple sum-over-paths structure we consider. 

Figure \ref{fig:dag_network} provides an illustrative example of a DAG network. To complement the survey, we derive an explicit bound in Theorem \ref{thm:path_lipschitz_general} using graph-theoretic method. To the best of our knowledge, this result has not previously appeared in the literature.

%Figure~\ref{fig:dag_network} gives an illustrative example of a DAG network. To complement the survey, we derive an explicit bound in Theorem~\ref{thm:path_lipschitz_general} using graph theory. To the best of our knowledge, this result does not appear in the literature.


\begin{theorem}[Lipschitz Bound for DAG Network]
\label{thm:path_lipschitz_general}
Let $G=(V,E)$ be a finite directed acyclic graph (DAG) representing a feedforward neural network with unique input node $s\in V$ and output node $t\in V$.  
Each node $v \in V$ is a module $h_v$ that is Lipschitz continuous with constant $\mathrm{Lip}[h_v]$.  
An edge $(u \to v) \in E$ represents the computation of $h_v$ immediately after $h_u$. Let $x_{v_i}: x \to x_{v_i}(x)$ represent the output at a node $v_i \in V$. The network is evaluated additively along incoming edges:
\begin{align}
x_s(x) &= x, \\
x_v(x) &= \sum_{(u\to v)\in E} h_v\!\big(x_u(x)\big), \quad v\neq s.
\end{align}

A \emph{computational path} $p$ from $s$ to $t$ is an ordered sequence of nodes
\begin{align}
p = (v_0=s, v_1, \dots, v_{L_p}=t),
\end{align}
where $(v_{i-1} \to v_i) \in E$ for all $i=1,\dots,L_p$.
Define for each edge $(u\to v)$ the constant
\begin{align}
C_{(u\to v)} := \mathrm{Lip}[h_v],
\end{align}
and for a path $p$ set
\begin{align}
C_p := \prod_{i=1}^{L_p} \mathrm{Lip}[h_{v_i}]
= \prod_{i=1}^{L_p} C_{(v_{i-1}\to v_i)}.
\end{align}
Let $\mathcal{P}$ be the set of all such paths from $s$ to $t$.  
Then the Lipschitz constant of the overall network $f(x):=x_t(x)$ satisfies
\begin{align}
\mathrm{Lip}[f] \;\le\; \sum_{p \in \mathcal{P}} C_p.
\end{align}
\end{theorem}





\begin{proof}
Fix any topological order of $V$. For $v\in V$, define the scalar
\begin{align}
S(v) := 
\begin{cases}
1, & v=s,\\[2pt]
\displaystyle \sum_{(u\to v)\in E} C_{(u\to v)}\, S(u), & v\neq s.
\end{cases}
\end{align}
\emph{Claim:} for all $v\in V$,
\begin{align}
\label{eq:node_lip_bound}
\mathrm{Lip}[x_v] \;\le\; S(v).
\end{align}
We prove \eqref{eq:node_lip_bound} by induction along the topological order.

\emph{Base case ($v=s$).} $x_s(x)=x$, hence $\mathrm{Lip}[x_s]=1=S(s)$.

\emph{Inductive step.} Let $v\neq s$ and assume \eqref{eq:node_lip_bound} holds for all predecessors $u$ of $v$. Applying Minkowski inequality, for any $x,y$ in the input space,
\begin{align}
\|x_v(x)-x_v(y)\|
&= \left\| \sum_{(u\to v)} h_v\big(x_u(x)\big) - \sum_{(u\to v)} h_v\big(x_u(y)\big) \right\| \\
&\le \sum_{(u\to v)} \big\| h_v\big(x_u(x)\big) - h_v\big(x_u(y)\big) \big\| \\
&\le \sum_{(u\to v)} \mathrm{Lip}[h_v] \,\big\| x_u(x) - x_u(y) \big\| \\
&\le \sum_{(u\to v)} \mathrm{Lip}[h_v] \,\mathrm{Lip}[x_u] \,\|x-y\| \\
&= \sum_{(u\to v)} C_{(u\to v)}\, \mathrm{Lip}[x_u] \,\|x-y\| \\[2pt]
&\le \left( \sum_{(u\to v)} C_{(u\to v)}\, S(u) \right) \|x-y\| = S(v)\,\|x-y\|
,
\end{align}
since inductive hypothesis:
\begin{align}
\mathrm{Lip}[x_u] \le S(u)
.
\end{align}


Thus $\mathrm{Lip}[x_v]\le S(v)$. In particular,
\begin{align}
\mathrm{Lip}[f]=\mathrm{Lip}[x_t] \;\le\; S(t).
\end{align}

It remains to show $S(t)=\sum_{p\in\mathcal P} C_p$. More generally:

\emph{Lemma (Path expansion of $S$).} For every $v\in V$,
\begin{align}
\label{eq:path-expansion}
S(v) = \sum_{p\in\mathcal P(s\to v)} \prod_{e\in p} C_e ,
\end{align}
where $\mathcal P(s\to v)$ is the set of all directed paths from $s$ to $v$.

\emph{Proof of Lemma.} Proceed again by induction in topological order. For $v=s$, $\mathcal P(s\to s)$ contains only the empty path with product $1$, so \eqref{eq:path-expansion} holds.
Assume \eqref{eq:path-expansion} holds for all predecessors $u$ of $v$. Then
\begin{align}
S(v)
&= \sum_{(u\to v)} C_{(u\to v)}\, S(u)
= \sum_{(u\to v)} C_{(u\to v)} \left( \sum_{p\in\mathcal P(s\to u)} \prod_{e\in p} C_e \right) \\[2pt]
&= \sum_{(u\to v)} \sum_{p\in\mathcal P(s\to u)} \left( \prod_{e\in p} C_e \right) C_{(u\to v)}.
\end{align}
Concatenating each $p\in\mathcal P(s\to u)$ with the edge $(u\to v)$ yields a bijection onto $\mathcal P(s\to v)$, and multiplies the edge constants accordingly; thus \eqref{eq:path-expansion} holds for $v$. \hfill$\square$

Applying the lemma at $v=t$ gives $S(t)=\sum_{p\in\mathcal P} C_p$, and hence
\begin{align}
\mathrm{Lip}[f] \;\le\; S(t) = \sum_{p\in\mathcal P} \prod_{i=1}^{L_p} \mathrm{Lip}[h_{v_i}]
.
\end{align}

\end{proof}

\begin{figure}[t!]
  \centering
  \resizebox{0.9\linewidth}{!}{
  \begin{tikzpicture}[
    ->, 
    %>=Stealth, 
    node distance=1.8cm and 2cm,
    every node/.style={circle, draw, minimum size=10mm},
    shorten >=1pt]


    \node[circle, fill=gray!20, inner sep=10pt] (S1) {$S_1$};
    
    \node[circle, inner sep=1.5pt, right = of S1, xshift=-1cm] (a1) {$a_1$};

    \node[circle, fill=gray!20, inner sep=10pt, right=of a1,xshift=-1cm] (S2) {$S_2$};

    \node[circle, inner sep=1.5pt, right = of S2,xshift=-1cm] (a2) {$a_2$};


    \node[circle, inner sep=1.5pt, right = of a2] (aLminusOne) {$a_{L-1}$};
    
    \node[circle, fill=gray!20, inner sep=10pt, right=of aLminusOne,xshift=-1cm] (SL) {$S_L$};


    \draw (S1) -- (a1);
    \draw (a1) -- (S2);
    \draw (S2) -- (a2);
    \draw[dashed] (a2) -- (aLminusOne);
    \draw (aLminusOne) -- (SL);
    
\end{tikzpicture}
}%resizebox

  \caption[Non-Biconnected DAG Network]{Topology of non-biconnected DAG network. If a DAG is separated into two sub-DAGs by the removal of a vertex $a_i$, then $a_i$ is referred to as a \emph{cut vertex} (or \emph{articulation point}), and the DAG is said to be \emph{non-biconnected}. This diagram shows the topology for a DAG that contains $L-1$ articulation points $a_1, a_2, \dots, a_{L-1}$ and $L$ corresponding sub-DAGs $S_1, S_2, \dots, S_L$.}
  
  \label{fig:nonbiconnected_dag_network}
\end{figure}

\subsubsection{Lipschitz Constant of Non-Biconnected DAG}


If a DAG is separated into two disconnected sub-DAGs by the removal of a vertex, then the removed vertex is referred to as \emph{cut vertex} or \emph{articulation point}. Modern deep learning architectures often give rise to computation DAGs that are not biconnected: the DAGs can be separated into multiple subgraphs by removing a small set of vertices. 


%\textcolor{blue}{
\begin{theorem}[Lipschitz Bound for Non-Biconnected DAG Network]
\label{thm:nonbiconnected_dag_lipschitz}
Figure~\ref{fig:nonbiconnected_dag_network} shows the typical non-biconnected DAG topology found in modern deep learning architectures. The DAG contains a set of cut vertexes $a_1,a_2, \cdots, a_{L-1}$ and biconnected DAGs $S_1,S_2,\cdots,S_L$. Suppose the DAG network $f$ in Figure~\ref{fig:nonbiconnected_dag_network} is:
\begin{align}
    f= S_L\,\circ\,a_{L-1}\,\cdots\,a_2\,\circ\,S_2\,\circ\,a_1\,\circ\,S_1
    ,
\end{align}
then it is not difficult to show that the Lipschitz constant bound of this DAG is:
\begin{align}
\label{equ:nonbiconnected_dag_lipschitz}
\mathrm{Lip}\left[ f \right] \leq 
\Biggl(
\prod_{i=1}^{L}    \mathrm{Lip}\left[ S_i \right] 
\Biggr)
\Biggl(
\prod_{j=1}^{L-1}    \mathrm{Lip}\left[ a_i \right] 
\Biggr)
,
\end{align}
where each the Lipschitz bound of sub-DAG $\mathrm{Lip}\left[ S_i \right]$ is given by Theorem~\ref{thm:path_lipschitz_general} (\nameref{thm:path_lipschitz_general}).
\end{theorem}
%}

%\textcolor{blue}{
\begin{remark}
Theorem~\ref{thm:nonbiconnected_dag_lipschitz} (\nameref{thm:nonbiconnected_dag_lipschitz}) is particularly valuable for estimating the Lipschitz bound of a deep model. In contrast to path-based bound of Theorem~\ref{thm:path_lipschitz_general} (\nameref{thm:path_lipschitz_general}), which can be quite loose due to its combinatorial dependence on the number of paths, Theorem~\ref{thm:nonbiconnected_dag_lipschitz} yields significantly tighter and more structurally informed bounds.
\end{remark}
%}



\subsubsection{Lipschitz Constant of Residual Network}
\label{sec:lipschitz_of_residual_module}

%\textcolor{blue}{
Residual networks \citep{he2016deep} address the optimization challenges of very deep neural architectures by introducing \emph{residual modules}, which is illustrated in Figure~\ref{fig:residual_module}. Each module $m_{\mathrm{res}}$ has the structure:
\begin{align}
    m_{\mathrm{res}}(x) = x + \phi(x),
\end{align}
which consists a non-identity unit $\phi$ and an identity skip connection. The resulting residual mapping $m_{\mathrm{res}}(x)$ maintains stable gradient flow, mitigates vanishing-gradient effects, and enables the training of substantially deeper networks without degradation. This simple architectural principle has proven highly effective and forms the backbone of many state-of-the-art deep learning models. Using Theorem~\ref{thm:path_lipschitz_general} (\nameref{thm:path_lipschitz_general}), it is not difficult to show that the Lipschitz constant bound of this structure is:
\begin{align}
    \mathrm{Lip}\left[m_{\mathrm{res}}\right] \leq 
    \mathrm{Lip}\left[s\right] +\mathrm{Lip}\left[\phi\right] = 
    1 + \mathrm{Lip}\left[\phi\right]
    ,
\end{align}
which recovers the same results in \citep[Lemma 2, \S~2]{Behrmann2019InvertibleResidual}, \citep[\S~3.4]{gouk2021regularisation} and Proposition~\ref{prop:lipschitz_composition}~(\nameref{prop:lipschitz_composition}) by setting $s$ to an identity map.
%}

\begin{figure}[t!]
    \centering

    \begin{tikzpicture}[>=latex, node distance=2.5cm, thick]

  % Nodes
  \node (x) {$x$};

  \node[circle, fill=black, inner sep=1.5pt, right=of x, xshift=-1.5cm] (input) {};
  
  \node[draw, rectangle, minimum width=1.5cm, minimum height=1cm, right=of input, xshift=-1.5cm] (phi) {$\phi$};
  
  \node[circle, draw, right=of phi, inner sep=1pt, minimum size=0.6cm, xshift=-1.5cm] (sum) {$+$};
  
  \node[right=of sum, xshift=-1.5cm] (z) {$z$};

  % Main path: x -> φ -> +
  \draw[->] (x) -- (phi);
  \draw[->] (phi) -- (sum);

  % Skip connection above φ with label s
  \draw[->] ($(input) + (0,0)$) |- ([yshift=0.8cm]sum.north) -- node[above, xshift=-2.cm,yshift=0.4cm] {$s$} (sum);

  % Output: + -> z
  \draw[->] (sum) -- (z);

\end{tikzpicture}


    \caption[Structure of Residual Module]{A residual module $m(x)=x + \phi(x)$ consists of a non-identity unit $\phi: x \mapsto \phi(x)$ and an identity skip connection unit $s: x \mapsto x$.}
    
    \label{fig:residual_module}
    
\end{figure}





%p48 of mohri2018foundations
%Lemma 4.2 Talagrand’s lemma
\subsection{Complexity-Theoretic Generalization Bound}
\label{sec:generalization_bounds}

%{\color{blue}

\paragraph{Notations.} Let $\mathcal{H}$ be a hypothesis family and $\mathcal{H} \ni h: X \to Y$ be a hypothesis. Let $\ell: Y \times Y \to \mathbb{R}$ be a loss function. For each $\ell(h(x), y)$, we can associate $\ell$ and $h$ with a map $G \ni g: X \times Y \to \mathbb{R}$, where $G$ is the family of loss functions associated to with hypothesis family $\mathcal{H}$.

The generalization capacity of a neural network is fundamentally governed by its Lipschitz constant \citep{mohri2018foundations}. To quantify this capacity for a hypothesis, the concept of \emph{generalization gap} is often used to measure the error between \emph{true risk} and \emph{empirical risk} (Definition~\ref{def:generalization_gap}). This gap for a model $h \in \mathcal{H}$ is proportional to its empirical Rademacher complexity of the hypothesis family $\mathcal{H}$, and the empirical Rademacher complexity is proportional to the Lipschitz constant $\mathrm{Lip}\left[\mathcal{H}\right]:=\sup_{h \in \mathcal{H}} \mathrm{Lip}\left[h\right]$ of the hypothesis family:
\begin{align}
\text{Generalization gap of $h$} \sim \text{Rademacher complexity} \sim O(\mathrm{Lip}\left[\mathcal{H}\right])
\end{align}
(\citet[\S~3]{mohri2018foundations}; \citet[Part IV]{shalev2014understanding}). A smaller Lipschitz constant enforces smoother mappings, reducing the complexity of the function class and mitigating overfitting, thereby enhancing robustness to noise and adversarial perturbations \citep{neyshabur2015norm,gouk2021regularisation,castin2023smooth}. 

%\par}

%\subsubsection{Generalization Gap}

\begin{definition}[Generalization Gap]
\label{def:generalization_gap}
Let $S:=\{(x_i,y_i)\}_{i=1}^m$ be a dataset where $(x_i,y_i)$ is sampled \emph{i.i.d.} from an unknown distribution $\mathcal{D}_X$. The true (population) risk for hypothesis $h$ is defined as:
\begin{align}
    R(h) := \mathbb{E}_{(x,y)\sim\mathcal{D}_X}[\ell(h(x),y)]
    ,
\end{align}
and the empirical risk on $S$ is defined as:
\begin{align}
   R_S(h) :=  \frac{1}{m} \sum_{i=1}^m \ell(h(x_i), y_i) 
\end{align}
(\citet[\S~3]{mohri2018foundations}; \citet[Part IV]{shalev2014understanding}). Accordingly, the generalization gap on $S$ is given by:
\begin{align}
     R(h) - R_S(h).
\end{align}

\end{definition}







\subsubsection{Rademacher Complexity and its Bounds}

%{\color{blue}

In learning theory, \emph{Rademacher complexity} quantifies the expressiveness of a hypothesis family $G:=\{g: X \to \mathbb{R}\}$ by measuring how well the $G$ can fit data associated with random labels \citep[\S~3.1]{mohri2018foundations}. Let $S = (x_1, x_2, \dots, x_m)$ be a dataset of size $m$ with each $x_i \in X$ drawn i.i.d. from an unknown distribution $\mathcal{D}_X$. Let $h : X \to \mathbb{R}$ be a hypothesis that assigns a real-valued score to each input. Let $\sigma_1, \dots, \sigma_m$ be $m$ independent \emph{Rademacher variables}, \ie, random variables uniformly distributed over $\{-1, +1\}$ \citep[\S~3.1]{mohri2018foundations}. For random labels $\sigma_1, \dots, \sigma_m$ assigned to $S$, the maximal correlation between the labels and the predictions of hypotheses in $\mathcal{H}$ is given by
\begin{align}
    \sup_{g \in G} \frac{1}{m} \sum_{i=1}^m \sigma_i g(x_i).
\end{align}
By assigning all possible random labels to the dataset $S$, we can thus define \emph{Rademacher Complexity} for hypothesis family $\mathcal{G}$, stated in Definition~\ref{def:empirical_rademacher} (\nameref{def:empirical_rademacher}).

%\par}

\begin{definition}[Rademacher Complexity {\citep[Definition 3.1, \S~3]{mohri2018foundations}}]
\label{def:empirical_rademacher}
The \emph{empirical Rademacher complexity} of $G$ with respect to $S$ is defined as
\begin{align}
\widehat{\mathfrak{R}}_S(G)
:= \mathbb{E}_{\sigma} \left[ \sup_{g \in G} \frac{1}{m} \sum_{i=1}^m \sigma_i g(x_i) \right],
\end{align}
and the (expected) \emph{Rademacher complexity} is the expectation of $\widehat{\mathfrak{R}}_S(G)$ over all dataset $S$ of size $m$:
\begin{align}
\mathfrak{R}_m(G)
:= \mathbb{E}_{S \sim \mathcal{D}_X^m} \left[ \widehat{\mathfrak{R}}_S(G) \right]
,
\end{align}
where $S \sim \mathcal{D}_X^m$ denotes $m$ samples i.i.d. drawn from $\mathcal{D}$. 
\end{definition}

%{\color{blue}
%\begin{remark}

In the paradigm of machine learning, for the case of the hypothesis family $\ell\circ \mathcal{H}$ is the composition of a model $h \in \mathcal{H}:=\{h:\mathbb{R}^n \to \mathbb{R} \}$ and loss function $\ell: \mathbb{R} \to \mathbb{R}$:
\begin{align}
    \ell\circ \mathcal{H} := \{\ell\circ h \mid h \in \mathcal{H}\},
\end{align}
by Talagrand's Contraction Lemma \citep[Lemma 4.2, \S~4]{mohri2018foundations}, the empirical Rademacher complexity of $\ell\circ \mathcal{H}$ on $S$ admits:
\begin{align}
    \widehat{\mathfrak{R}}_S(\ell\circ \mathcal{H}) \leq 
    \mathrm{Lip}\left[\ell\right] \;\widehat{\mathfrak{R}}_S(\mathcal{H}) 
    .
\end{align}

For any $\delta > 0$, with probability at least $1-\delta$, the generalization gap for $h \in \mathcal{H}$ on $S$ is bounded by empirical Rademacher complexity of $\ell\circ \mathcal{H}$:
\begin{align}
    R(h) - R_S(h) \leq 2 \;\widehat{\mathfrak{R}}_S(\ell\circ\mathcal{H}) + 
    3 \sqrt{\frac{\log{\frac{2}{\delta}}}{2m}}
    \leq
    2\; \mathrm{Lip}\left[\ell\right] \;\widehat{\mathfrak{R}}_S(\mathcal{H}) + 3 \sqrt{\frac{\log{\frac{2}{\delta}}}{2m}}
\end{align}
\citep[Theorem 3.1 \& Theorem 3.3, \S~3]{mohri2018foundations}. If $\mathcal{H}$ is a $K_{\mathcal{H}}$-Lipschitz continuous hypothesis family, that is:
\begin{align}
    \mathcal{H}:= \{ h: \mathbb{R}^n \to \mathbb{R} \mid \mathrm{Lip}\left[h\right] \leq K_{\mathcal{H}}\}
    ,
\end{align}
and let:
\begin{align}
\Phi:=\{\phi: \mathbb{R}^n \to \mathbb{R}^n \mid \phi~\text{is a coordinate-wise identity map}\}    
\end{align}
be an coordinate-wise identity hypothesis family. By using vector contraction theorem \citep[Equation 1 \& Corollary 4]{Maurer2016Contraction}, $\widehat{\mathfrak{R}}_S(\mathcal{H})$ holds an inequality:
\begin{align}
   \widehat{\mathfrak{R}}_S(\mathcal{H}) = \widehat{\mathfrak{R}}_S(\mathcal{H} \circ \Phi) \leq \sqrt{2} K_{\mathcal{H}}  \; \widehat{\mathfrak{R}}_S(\Phi)
   ,
\end{align}
where $\widehat{\mathfrak{R}}_S(\Phi)$ is bounded by the $2$-norm dataset diameter $\max_{x\in S}\|x\|_2$ of $S$:
\begin{align}
    \widehat{\mathfrak{R}}_S(\Phi) = 
    \mathbb{E}_{\sigma} \left[ \sup \frac{1}{m} \sum_{i=1}^m \sigma_i x_i \right]
    \leq \frac{\sqrt{\sup
    \sum_{i=1}^{m}\|x_i\|_2^2
    }}{m}
    = \frac{\max_{x \in S} \|x\|_2}{\sqrt{m}}
,
\end{align}
this immediately yields:
\begin{align}
    R(h) - R_S(h) \leq O(K_{\mathcal{H}})
    .
\end{align}

The literature on norm-based generalization bounds \citep{bartlett2017spectrally,golowich18acomplexity} also shows that the empirical Rademacher complexity of general neural networks with ReLU activations can be bounded by the product of the layerwise parameter $2$-norms, which in turn provides an upper bound on the Lipschitz constant of the hypothesis family. For example, \citeauthor{bartlett2017spectrally} show that the lower bound of the empirical Rademacher complexity depends on an upper bound $K_{\mathcal{H}}^{+,\ell_2}$ of Lipschitz constant $K_{\mathcal{H}}$ of an $L$-layer network:
\begin{align}
K_{\mathcal{H}} \leq  K_{\mathcal{H}}^{+,\ell_2} := O\Bigl(
\prod_{\ell=1}^{L} \|\theta^{(\ell)}\|_2
\Bigr)
,
\end{align}
where $\|\theta^{(\ell)}\|_2$ is the $2$-norm of the $\ell$-th layer parameter matrix, this leads:
\begin{align}
   \widehat{\mathfrak{R}}_S(\mathcal{H}) \geq O(K_{\mathcal{H}}^{+,\ell_2}), 
\end{align}
\citep[Theorem 3.4., \S~3.3]{bartlett2017spectrally}. The Lipschitz upper bound $K_{\mathcal{H}}^{+,\ell_2}$ is given by the product of the spectral-norms of parameter matrices (Proposition~\ref{prop:survey_upper_bound_lipschitz}). \citeauthor{golowich18acomplexity} explicitly show that, for ReLU networks, the $\widehat{\mathfrak{R}}_S(\mathcal{H})$ is bounded by:
\begin{align}
\widehat{\mathfrak{R}}_S(\mathcal{H}) \leq 
    O\Bigl(
    \frac{K_{\mathcal{H}}^{+,\ell_2}}{\sqrt{m}}
    \Bigr)
\end{align}
\citep[Theorem 2]{golowich18acomplexity}.
%\end{remark}
%\par}



% \begin{lemma}[Talagrand's Contraction Lemma {\citep[Lemma 4.2, \S~4]{mohri2018foundations}}]
% \label{lem:talagrands_contraction}
% Let $\mathcal{F}$ be a class of functions mapping from $\mathcal{X}$ to $\mathbb{R}^m$, and let $\phi:\mathbb{R}^m \to \mathbb{R}$ be $K$-Lipschitz with respect to the Euclidean norm and satisfy $\phi(0) = 0$. Then,
% \begin{align}
% \widehat{\mathfrak{R}}_n(\phi \circ \mathcal{F})
% \;\le\;
% K \; \widehat{\mathfrak{R}}_n(\mathcal{F}).
% \end{align}

% In particular, if $\mathcal{H}$ is a class of scalar-valued functions with $\mathrm{Lip}[h] \le K$ and $\|x_i\|_2 \le B$ for all sample points, then
% \begin{align}
% \widehat{\mathfrak{R}}_n(\mathcal{H}) \;\le\; \frac{K B}{\sqrt{n}}.
% \end{align}
% \end{lemma}

% \subsubsection{Empirical Risk Bound}

% \subsubsection{Empirical Risk Bound -- Binary-Class Classification}

% % section Rademacher Complexity and VC-Dimension
% %Theorem 3.3 (page 47) 
% For any $\delta > 0$, with probability at least $1-\delta$, the generalization gap for $h \in \mathcal{H}$ on $S$ is bounded by empirical Rademacher complexity of $\ell\circ \mathcal{H}$:
% \begin{align}
%     R(h) - R_S(h) \leq 2 \;\widehat{\mathfrak{R}}_S(\ell\circ\mathcal{H}) + 
%     3 \sqrt{\frac{\log{\frac{2}{\delta}}}{2m}}
%     \leq
%     2\; \mathrm{Lip}\left[\ell\right] \;\widehat{\mathfrak{R}}_S(\mathcal{H}) + 3 \sqrt{\frac{\log{\frac{2}{\delta}}}{2m}}
% \end{align}
% \citep[Theorem 3.1 \& Theorem 3.3, \S~3]{mohri2018foundations}.



% \begin{theorem}[Rademacher Complexity Bounds -- Binary Classification {\citep{mohri2018foundations}}]
% \label{thm:rademacher_generalization}
% Let $\mathcal{H}$ be a hypothesis class mapping from $\mathcal{X}$ to $[0,1]$. Then, for any $\delta \in (0,1)$, with probability at least $1-\delta$ over the choice of an i.i.d.\ sample of size $n$,
% \begin{align}
% \forall h \in \mathcal{H}, \quad
% R(h) \;\le\; \hat{R}(h) \;+\; 2 \, \widehat{\mathfrak{R}}_n(\mathcal{H}) \;+\; 3 \sqrt{\frac{\log(2/\delta)}{2n}},
% \end{align}
% where $R(h)$ is the true risk, $\hat{R}(h)$ the empirical risk, and $\widehat{\mathfrak{R}}_n(\mathcal{H})$ the empirical Rademacher complexity of $\mathcal{H}$.
% \end{theorem}

% %page 382 in Understanding Machine Learning: From Theory to Algorithms
% \begin{lemma}[Empirical Rademacher Complexity of $\ell_2$-Bounded Linear Functions {\citep{shalev2014understanding}}]
% \label{lem:linear_rc}
% Let $S=\{x_1,\dots,x_n\}\subset \mathbb{R}^m$ with $\|x_i\|_2 \le B$ for all $i$.
% For $\mathcal{F}=\{x \mapsto w^\top x : \|w\|_2 \le 1\}$,
% \begin{align}
% \widehat{\mathfrak R}_S(\mathcal{F})
% \;\le\; \frac{1}{n}\,\mathbb{E}_{\sigma}\Big\|\sum_{i=1}^n \sigma_i x_i\Big\|_2
% \;\le\; \frac{B}{\sqrt{n}}.
% \end{align}
% \end{lemma}





% \begin{corollary}[Lipschitz Continuity Bounds Empirical Risk]
% \label{corollary:lipschitz_bounds_empirical_risk}
% Combining Theorem~\ref{thm:rademacher_generalization} and Lemma~\ref{lem:talagrands_contraction} for a $K$-Lipschitz hypothesis class with $\|x\|_2 \le B$ yields:
% \begin{align}
% R(f) \;\le\; \hat{R}(f) \;+\; \frac{2 K B}{\sqrt{n}} \;+\; 3 \sqrt{\frac{\log(2/\delta)}{2n}}.
% \end{align}    
% \end{corollary}

% \begin{remark}
% Corollary~\ref{corollary:lipschitz_bounds_empirical_risk} shows that, in the binary classification setting, the empirical risk bound for a function
% \begin{align}
% f := \phi \circ \mathcal{H}, \quad
% \mathcal{H}: \mathbb{R}^n \to \mathbb{R}^m, \quad
% \phi: \mathbb{R}^m \to \mathbb{R},
% \end{align}
% is directly controlled by the Lipschitz constant $K := \mathrm{Lip}[\mathcal{H}]$ of the feature mapping $\mathcal{H}$.  
% In particular, the complexity term in the bound scales linearly with $K$, so reducing $K$ (e.g., via spectral-norm constraints or weight regularization) tightens the bound and can improve generalization.
% \end{remark}

% \subsubsection{Empirical Risk Bound -- Multi-Class Classification}


% %page 233, theorem 9.2
% \begin{theorem}[Margin Bound for Multi-Class Classification {\citep{mohri2018foundations}}]
% \label{thm:multiclass_margin_mohri}
% Let $\mathcal{Y} = \{1,\dots,k\}$ be a finite label set and let $\mathcal{H} \subset \mathbb{R}^{\mathcal{X} \times \mathcal{Y}}$ be a set of scoring functions, 
% where each $h \in \mathcal{H}$ maps $(x,y) \in \mathcal{X} \times \mathcal{Y}$ to a real-valued score $h(x,y) \in \mathbb{R}$.

% \textbf{Prediction Margin.} For a sample $S = \{(x_i, y_i)\}_{i=1}^m$ and $\rho > 0$, the \emph{margin} of $h$ at $(x,y)$ is
% \begin{align}
% \rho_h(x,y) \;:=\; h(x,y) - \max_{y' \neq y} h(x,y').
% \end{align}

% \textbf{Empirical Margin Loss.} The \emph{empirical $\rho$-margin loss} is
% \begin{align}
% \widehat{R}_{S,\rho}(h) 
% \;:=\; \frac{1}{m} \sum_{i=1}^m \Phi_\rho\!\big( \rho_h(x_i, y_i) \big),
% \end{align}
% where $\Phi_\rho$ is the \emph{margin loss function} (Definition 5.5 in \citealp{mohri2018foundations}).

% Define the projection operator $\Pi_1(\mathcal{H})$ by
% \begin{align}
% \Pi_1(\mathcal{H}) \;:=\; \{ x \mapsto h(x,y) \;:\; y \in \mathcal{Y},\ h \in \mathcal{H} \}
% .
% \end{align}

% \textbf{Claim.} Then, for any $\delta \in (0,1)$, with probability at least $1 - \delta$, the following bound holds for all $h \in \mathcal{H}$:
% \begin{align}
% R(h) \;\le\; \widehat{R}_{S,\rho}(h) \;+\; \frac{4k}{\rho}\, \mathfrak{R}_m\!\big(\Pi_1(\mathcal{H})\big)
% \;+\; \sqrt{\frac{\log(1/\delta)}{2m}},
% \end{align}
% where $\mathfrak{R}_m(\cdot)$ denotes the (expected) Rademacher complexity over samples of size $m$.
% \end{theorem}


% \begin{corollary}[Lipschitz Continuity Bounds Multi-Class Margin]
% \label{cor:multiclass_margin_lipschitz}
% Assume that for every $h\in\mathcal H$ and $y\in\mathcal Y$, the map $x\mapsto h(x,y)$ is $K$-Lipschitz and $h(0,y)=0$, and that $\|x\|_2\le B$ almost surely. Then
% \begin{align}
% \mathfrak R_m\!\big(\Pi_1(\mathcal H)\big) \;\le\; \frac{K B}{\sqrt{m}},
% \end{align}
% and, applying Theorem~\ref{thm:multiclass_margin_mohri},
% \begin{align}
% R(h) \;\le\; \widehat{R}_{S,\rho}(h) \;+\; \frac{4k\,K B}{\rho\sqrt{m}} \;+\; \sqrt{\frac{\log(1/\delta)}{2m}}
% \qquad \text{for all } h\in\mathcal H,
% \end{align}
% with probability at least $1-\delta$ over the sample $S$.
% \end{corollary}



% \begin{remark}
% Corollary~\ref{cor:multiclass_margin_lipschitz} shows that, in the multi-class setting, the generalization gap is directly controlled by the Lipschitz constant $K$ of the coordinate functions $x \mapsto h(x,y)$.  
% Specifically, when each coordinate is $K$-Lipschitz and the inputs are bounded by $B$, the complexity term in the multi-class margin bound scales as $\tfrac{4kKB}{\rho\sqrt{m}}$. Thus, reducing $K$ --- for example, via spectral-norm regularization or path-norm constraints --- tightens the bound, leading to improved generalization guarantees.
% \end{remark}



\subsection{Training Dynamics of Lipschitz Continuity}
\label{sec:optimization_induced_dynamics}



The Lipschitz continuity of a parameterized network evolves as optimization updates its parameters. Consequently, the optimization process induces the dynamics of the network's Lipschitz continuity. While existing work in deep learning theory has largely focused on bounding the Lipschitz constants of neural networks, understanding how Lipschitz continuity evolves throughout training remains an open problem. Only a few studies have begun to explore this aspect. In particular, \citet{luo2025lipschitz} introduces the concept of \emph{optimization‐induced dynamics} establishes a continuous‐time stochastic framework that explicitly links the optimization process to the time‐varying Lipschitz continuity bound of deep networks. The literature \citep{luo2025lipschitz} uses the operator-theoretical results regarding how the largest singular values of parameter matrices vary with respect to perturbations from the literature \citep{luo2025spectralvariation}, along with the theory from high-dimensional stochastic differential equations (SDEs) from stochastic analysis, for establishing a mathematical framework modeling the evolution of a spectral-norm based Lipschitz continuity upper bound. They further validate their theoretical framework with experiments across datasets and regularization scenarios.






Consider an $L$‐layer feed‐forward neural network $f: \mathbb{R}^m \to \mathbb{R}$ with 1‐Lipschitz activation functions (\eg, ReLU). Let $\boldsymbol{\theta}^{(\ell)}(t) \in \mathbb{R}^{m_\ell \times n_\ell}$ be the $\ell$-layer parameter matrix at time $t$ and $\boldsymbol{\theta}(t)$ be the collection of $\boldsymbol{\theta}^{(\ell)}(t)$ for all layers. Let $\mathcal{L}_f(\boldsymbol{\theta}^{(\ell)}(t))$ be the loss expectation for the $f$ with parameters $\boldsymbol{\theta}(t)$ at time $t$. Suppose that $\boldsymbol{\Sigma}_t^{(\ell)} \in \mathbb{R}^{(m_\ell n_\ell) \times (m_\ell n_\ell)}$ is the layer‐wise covariance matrix of stochastic gradient noise, arising from mini‐batch sampling. Let $K^{(\ell)}(t)$ be the Lipschitz constant at layer $\ell$. Let $K(t)$ be the network Lipschitz spectral-norm bound. \citet{luo2025lipschitz} show that the continuous‐time dynamics of the parameters under stochastic gradient descent (SGD) with a sufficiently small learning rate $\eta > 0$ are given by a system of SDEs \citep[Definition 10]{luo2025lipschitz}:
\begin{numcases}{}
    \dd \mathrm{vec}(\boldsymbol{\theta}^{(\ell)}(t)) = - \mathrm{vec}\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right]  \, \dd t   + \sqrt{\eta} \left[\boldsymbol{\Sigma}_t^{(\ell)} \right]^{\frac{1}{2}} \, \dd \boldsymbol{B}_t^{(\ell)} \notag\\
    K^{(\ell)}(t)=\|\boldsymbol{\theta}^{(\ell)}(t)\|_{op}  \notag\\
    Z(t)  = \sum_{l=1}^L \log K^{(\ell)}(t) \notag\\
    K(t) = \mathrm{e}^{Z(t)} \notag
\end{numcases}
where:
\begin{itemize}
    \item $\mathrm{vec}: \mathbb{R}^{m \times n} \to \mathbb{R}^{mn}$ represents major-column vectorization operator.

    \item $\|\cdot\|_{op}$ the matrix operator (spectral) norm.

    
    \item $\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))$ is the gradient of the loss with respect to the $\ell$‐th layer parameters.

    
    \item $\boldsymbol{B}_t^{(\ell)}$ is a standard $(m_\ell n_\ell)$‐dimensional Wiener process.

\end{itemize}


This stochastic dynamical system characterizes, in continuous time, the evolution of both layer‐wise and network‐level Lipschitz continuity bounds induced by the optimization process. \citet[Theorem 15]{luo2025lipschitz} show that the layer‐wise dynamics decompose into three \emph{driving forces}:
\begin{align}
\frac{\dd K^{(\ell)}(t)}{K^{(\ell)}(t)}  = \left( \mu^{(\ell)}(t) + \kappa^{(\ell)}(t) \right) \,  \dd t + \boldsymbol{\lambda}^{(\ell)}(t)^\top \, \dd \boldsymbol{B}_t^{(\ell)} 
, 
\end{align}    
where $\dd\,\boldsymbol{B}_t^{(\ell)} \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{\mathrm{I}}_{m_{\ell}n_{\ell}} \dd t)$ represents the increment of a standard Wiener process in $\mathbb{R}^{m_{\ell}n_{\ell}}$,
and the three \emph{driving forces} are:
\begin{enumerate}
    \item \textbf{Optimization‐induced drift}:
    \begin{align}
    \mu^{(\ell)}(t) 
    &= \frac{\left\langle \boldsymbol{J}_{op}^{(\ell)}(t), -\mathrm{vec}\!\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right] \right\rangle}
            {\sigma_{1}^{(\ell)}(t)},
    \end{align}
    where $\boldsymbol{J}_{op}^{(\ell)}(t)$ is the Jacobian of the operator norm with respect to $\mathrm{vec}(\boldsymbol{\theta}^{(\ell)}(t))$ and $\sigma_{1}^{(\ell)}(t)$ is its largest singular value. This term captures the deterministic component of Lipschitz evolution driven by the mean gradient flow. This shows that the alignment of the gradient $\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))$ and principal direction of the $\ell$-th layer parameter matrix $\boldsymbol{J}_{op}^{(\ell)}(t)$ at time $t$ determines the contribution of the optimization to the increment of the layer-wise Lipschitz constant.

    \item \textbf{Noise–curvature entropy production}:
    \begin{align}
    \kappa^{(\ell)}(t) 
    &= \frac{\eta}{2\,\sigma_{1}^{(\ell)}(t)}
       \left\langle \boldsymbol{H}_{op}^{(\ell)}(t), \boldsymbol{\Sigma}_t^{(\ell)} \right\rangle \ge 0,
    \end{align}
    where $\boldsymbol{H}_{op}^{(\ell)}(t)$ is the Hessian of the operator norm and $\boldsymbol{\Sigma}_t^{(\ell)}$ is the gradient‐noise covariance. This non‐negative term quantifies irreversible growth of the Lipschitz bound due to the interaction between stochastic gradient noise and curvature.

    \item \textbf{Diffusion‐modulation intensity}:
    \begin{align}
    \boldsymbol{\lambda}^{(\ell)}(t) 
    &= \frac{\sqrt{\eta}}{\sigma_{1}^{(\ell)}(t)}
       \left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{1/2\top} \boldsymbol{J}_{op}^{(\ell)}(t),
    \end{align}
    which controls the variance of Lipschitz evolution by scaling the Wiener noise term from mini‐batch sampling.
\end{enumerate}

\citet[Theorem 16]{luo2025lipschitz} show that, at the network level, these quantities aggregate as:
\begin{align}
\mu_Z(t) = \sum_{\ell=1}^L \mu^{(\ell)}(t) 
,\qquad
\kappa_Z(t) = \sum_{\ell=1}^L \kappa^{(\ell)}(t)
,  \qquad
\lambda_Z(t) = \left[\sum_{\ell=1}^L \|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2\right]^{\frac{1}{2}}
,
\end{align}
governing the deterministic trend, irreversible growth, and stochastic fluctuations of the overall Lipschitz bound $K(t)$.


Their framework is particularly useful for interpreting the behaviors of neural networks, such as the near-convergence behavior, noisy supervision and mini-batch sampling trajectories. \citet[\S~8]{luo2025lipschitz} show that:
\begin{enumerate}
    \item The Lipschitz constant bound irreversibly increase since the term \emph{noise-curvature entropy production} $\boldsymbol{\kappa}_Z(t)$ is \emph{non-negative}, which increases the system entropy \citep[\S~8.3]{luo2025lipschitz}.

    \item The magnitude of supervision noise affects the Lipschitz bound \citep[\S~8.4 \& 8.5]{luo2025lipschitz}. In particular, larger supervision noise leads to a lower Lipschitz bound for the network. This is because the supervision noise shrinks the \emph{optimization-induced drift} $\boldsymbol{\mu}_Z(t)$.

    \item Mini-batch trajectories do not affect the variance of the Lipschitz bound if batch size is sufficiently large \citep[\S~8.6]{luo2025lipschitz}.
    
\end{enumerate}

\begin{remark}
The dynamical analysis of Lipschitz continuity in deep learning models remains an open research problem. For instance, the dynamics under small-batch training remains poorly understood.
\end{remark}



\section{Estimation Methods}
\label{sec:estimating_lipschitz}


Proposition~\ref{prop:survey_upper_bound_lipschitz} gives an upper bound of the Lipschitz constant of a network \citep{miyato2018spectral,luo2025lipschitz}. However, exact computation of the Lipschitz constant
\begin{align}
K = \sup_{x \neq y} \frac{\|f(x) - f(y)\|_2}{\|x - y\|_2}
= \sup_{x} \|\nabla f(x)\|_2
\end{align}
is generally NP-hard \citep{virmaux2018lipschitz,jordan2020exactly}. This section surveys major estimation and bounding techniques, ranging from statistical sampling to certified convex relaxations.  
We group them into \emph{Power Iteration}, \emph{Extreme Value Theory}, \emph{Derivative Bound Propagation}, \emph{Spectral Alignment}, \emph{Convex Optimization Relaxations}, and \emph{Exact/Relaxed MILP formulations}. 

\subsection{Power Iteration for Single Linear Unit}
\label{sec:estimation:power_iteration}


% \citep{miyato2018spectral}

\textbf{Power Iteration \citep{mises1929praktische}} is also known as the Von Mises iteration \citep{mises1929praktische}. It is the standard way to estimate the Lipschitz constant for a linear layer --- fully-connected or convolutional, by approximating the spectral-norm of weight matrices, which bounds the layer Lipschitz constant (Proposition~\ref{prop:lipschitz_constant_of_linear_unit}) \citet{miyato2018spectral,sedghi2019singular,kim2021lipschitz,luo2025lipschitz}. Another desirable property of \emph{power iteration} in optimization is that \emph{power iteration} is differentiable. For example, \citet{miyato2018spectral} and \citet{miyato2018spectral} use \emph{power iteration} for computing the largest singular values of parameter matrices, in which the differentiability of \emph{power iteration} allows the gradient propagation for gradient based optimization.

%\citep[Example 5.6.6, \S~5]{horn2012matrix}. 

Suppose that $W \in \mathbb{R}^{m \times m}$ is the parameter matrix of a fully-connected layer or a convolutional layer, then the largest singular value $\sigma_1(W)$ is its operator norm:
\begin{align}
    \mathrm{Lip}[W] = \sigma_1(W)
    .
\end{align}
Computing the exact value of $\sigma_1(W)$ for a large $m \times m$ matrix $W$ is computationally expensive, as classical algorithms require $O(m^3)$ time. However, the largest singular value can be approximated using \emph{power iteration} by assuming the existence of a uniquely dominant singular value \citep[\S~7.3]{golub2013matrix}. Starting with random unit vectors $u_0, v_0$, one step of power iteration updates
\begin{align}
v_{k+1} \;\leftarrow\; \frac{W^\top u_k}{\|W^\top u_k\|_2},
\qquad
u_{k+1} \;\leftarrow\; \frac{W v_k}{\|W v_k\|_2}
,
\end{align}
and uses 
\begin{align}
\hat{\sigma}_1^{(k+1)} = u_{k+1}^\top W v_{k+1}    
\end{align}
as a differentiable estimate of $\sigma_1(W)$ at step $k+1$. At the iteration number $T$, the estimated Lipschitz constant of $W$ is approximated as:
\begin{align}
    \mathrm{Lip}[W] \approx 
    u_{T}^\top W v_T
    ,
\end{align}
where $T$ is the number of iterations. The estimation error is proportional to:
\begin{align}
    |\sigma_1 - \hat{\sigma}_1^{(T)} | = O\Bigl( \Bigl[ \frac{\sigma_2}{\sigma_1} \Bigr]^T \Bigr)
    ,
\end{align}
where $\sigma_1$ and $\sigma_2$ are the largest, and second largest singular values, respectively \citep[Equation 7.3.5, \S~7.3]{golub2013matrix}.

% (see Algorithm~\ref{alg:power_iteration_estimates_matrix_2_norm}) 
% \begin{center}
% \adjustbox{max width=0.85\textwidth}{%
% \begin{algorithm}[H]
% \caption{Power Iteration of Computing $\|W\|_2$}
% \label{alg:power_iteration_estimates_matrix_2_norm}
% \KwIn{Matrix $W$, number of power steps $T$}

% $u \leftarrow$ random vector of same shape as column dimension of $W$\;
% $u \leftarrow \frac{u}{\|u\|_2}$\;
% $v \leftarrow$ random vector of same shape as row dimension of $W$\;
% $v \leftarrow \frac{v}{\|v\|_2}$\;

% \For{$t \leftarrow 1$ \KwTo $T$}{
%     $v \leftarrow W^\top u$\;
%     $v \leftarrow \frac{v}{\|v\|_2}$\;
%     $u \leftarrow W v$\;
%     $u \leftarrow \frac{u}{\|u\|_2}$\;
% }


% \KwOut{$u^\top W v$}
% \end{algorithm}
% }
% \end{center}

% We compare against
% the following estimation techniques: CLEVER [14], FastLip [6], LipSDP [31], SeqLip [13] and
% our MIP formulation (LipMIP) and its LP-relaxation (LipLP). 



\subsection{Extreme Value Theory}

% Paper: EVALUATING THE ROBUSTNESS OF NEURAL NETWORKS: AN EXTREME VALUE THEORY APPROACH
% ICLR2018
\textbf{CLEVER \citep{weng2018clever}} --- \emph{Cross-Lipschitz Extreme Value for nEtwork Robustness} --- converts the problem of estimating the attack-independent robustness into the problem of estimating the \emph{local} Lipschitz constant by sampling gradient norms in a neighborhood of the input \citep{weng2018clever}. This is because the $q$-norm Lipschitz constant of a network $g: \mathbb{R}^m \to \mathbb{R}$ is determined by:
\begin{align}
    \mathrm{Lip}_q\left[g\right] = \sup_x \|\nabla\; g(x) \|_q
    ,
\end{align}
for any inputs $x$ and $y$:
\begin{align}
    |g(x) - g(y)| \leq \mathrm{Lip}_q\left[f\right] \|x-y\|_p
\end{align}
\citep[Lemma 3.1]{weng2018clever} where $1 \leq p, q \leq \infty$ satisfy the H\"older conjugacy relation \citep[\S~6]{rudin1976principles}:
\begin{align}
    \frac{1}{p} + \frac{1}{q} = 1
    .
\end{align}



\paragraph{Adversarial Perturbation Bound.} \citet{weng2018clever} further show that the local Lipschitz constant can be used for deriving the adversarial perturbation bound. Let 
\begin{align}
f: \mathbb{R}^m \to \mathbb{R}^k    
\end{align}
be a $k$-class classifier and $f_i$ be the $i$-th prediction. Let:
\begin{align}
    c(x) = \argmax_{1 \leq i \leq k} f_i(x)
\end{align}
be the prediction. Then the $p$-norm adversarial perturbation $\|\delta\|_p$ to an input $x_0$ is bounded above by:
\begin{align}
    \|\delta\|_p \leq \min_{j \neq c} \frac{f_c(x_0) - f_j(x_0)}{\mathrm{Lip}_q\left[f_j\right]}
    ,
\end{align}
where the local Lipschitz constant $\mathrm{Lip}_q\left[f_j\right]$ can be estimated through:
\begin{align}
    \mathrm{Lip}_q\left[f_j\right] = \max_{x \in B_p(x_0, \delta)} \|\nabla\; f_j(x) \|_q
\end{align}
and $B_p(x_0, \delta)$ is a $p$-norm ball centered at $x_0$ with a radius $\delta$ \citep[Theorem 3.2]{weng2018clever}.

\paragraph{Distribution of Extreme Value $\max_{x \in B_p(x_0, \delta)} \|\nabla\; f_j(x) \|_q$.} Estimating:
\begin{align}
\max_{x \in B_p(x_0, \delta)} \|\nabla_x\; f_j(x) \|_q    
\end{align}
can be through sampling $x \in B_p(x_0, \delta)$. Suppose the $n$ samples are $\{x^{(1)}, x^{(2)}, \cdots, x^{(n)} \}$. Their gradient $q$-norms are $\{\|\nabla\; f_j(x^{(1)}) \|_q, \|\nabla\; f_j(x^{(2)}) \|_q, \cdots, \|\nabla\; f_j(x^{(n)}) \|_q\}$. \citet{weng2018clever} show that the extreme value of the gradient $q$-norm:
\begin{align}
  Y := \lim_{n \to \infty} \; \max_{x^{(i)} \in B_p(x_0, \delta)} \Bigl\{\|\nabla\; f_j(x^{(1)}) \|_q, \|\nabla\; f_j(x^{(2)}) \|_q, \cdots, \|\nabla\; f_j(x^{(n)}) \|_q \Bigr\} 
\end{align}
can only be a distribution $P_Y$ of three distribution classes --- \emph{Gumbel class (Type I)}, \emph{Fr\'echet class (Type II)} and \emph{Reverse Weibull class (Type III)} --- according to Fisher-Tippett-Gnedenko Theorem \citep[Theorem 4.1]{weng2018clever}. The extreme value $\max\|\nabla\; f_j(x^{(1)}) \|_q$ is thus converted to estimating the mean of the distribution $P_Y$:
\begin{align}
     \mathrm{Lip}_q\left[f_j\right] \approx \mathbb{E}_{Y \sim P_Y}\left[ Y \right]
     .
\end{align}


% \subsection{Derivative Bound Propagation}
\subsection{Coordinate-Wise Gradient}


%Towards fast computation of certified robustness for relu networks
%ICLR
%\citep{weng2018fastlip}

\textbf{Fast-Lip \citep{weng2018fastlip}} derives a lower bound of local Lipschitz constant in the form of coordinate-wise gradients by analyzing the activation patterns of ReLU networks. Let $n_k$ denote the number of neurons at the $k$-th layer of an $m$-layer network and Let $n_0$ be the input dimension. Let $\phi_k: \mathbb{R}^{n_0} \to \mathbb{R}^{n_k}$ be the map from input to the output of $k$-th layer. Let $\sigma$ be the coordinate-wise activation function. Then the relation between the $(k-1)$-th layer and the $k$-th layer can be written as:
\begin{align}
    \phi_k(x) = \sigma\Bigl(
    W^{(k)} \phi_{k-1}(x) + b^{(k)}
    \Bigr)
    ,
\end{align}
where $W^{(k)} \in \mathbb{R}^{n_k \times n_{k-1}}$ is the $k$-th layer parameter matrix, and $b^{(k)} \in \mathbb{R}^{n_k}$ is the bias. Set $f(x) = \phi_m(x)$ and let $f_j(x)$ denote the $j$-th output of $f$. \citet{weng2018fastlip} start from analyzing the ReLU activation patterns and then deriving gradient bounds under this setting for bounding local Lipschitz constant.


\paragraph{Activation Patterns of ReLU Networks.} Let $l_r^{(k)}$ and $u_r^{(k)}$ denote the lower and upper bound for the $r$-th neuron in the $k$-th layer and let $z_r^{(k)}$ be the pre-activation at the $k$-th layer, given as:
\begin{align}
    z_r^{(k)} = W_{r,:}^{(k)} \phi_{k-1}(x) + b_r^{(k)}
    ,
\end{align}
where $W_{r,:}^{(k)}$ denotes the $r$-th row of $W^{(k)}$ \citep[\S~3.2]{weng2018fastlip}. For the neurons indexed by $[n_k]:=\{1, 2, \cdots, n_k\}$, then there are only three activation patterns:
\begin{enumerate}
    \item \textbf{Always Activated.} Neurons are always activated: $\mathcal{I}_k^+ := \{ r \in [n_k] \mid u_r^{(k)} \geq l_r^{(k)} \geq 0\}$.
    
    \item \textbf{Always Inactivated.} Neurons are always inactivated: $\mathcal{I}_k^- := \{ r \in [n_k] \mid l_r^{(k)} \leq u_r^{(k)} \leq 0\}$.
    
    \item \textbf{Either Activated or Inactivated.} Neurons are either activated or inactivated: $\mathcal{I}_k := \{ r \in [n_k] \mid l_r^{(k)} \leq 0 \leq u_r^{(k)} \}$.
\end{enumerate}


\paragraph{Gradient Analysis of ReLU Networks.} Gradient norm carries the information for local Lipschitz constant. \citet{weng2018fastlip} then analyze the coordinate-wise gradients of ReLU networks with a manner of layer-wise. Using the activation patterns of ReLU networks, the $k$-th layer output can be rewritten into:
\begin{align}
    \phi_k(x) = \Lambda^{(k)} \Bigl(
    W^{(k)}\phi_{k-1}(x) + b^{(k)}
    \Bigr)
    ,
\end{align}
where $\Lambda^{(k)}$ is the activation pattern matrix:
\begin{align}
    \Lambda^{(k)}_{r,r} = \begin{cases}
        1~\text{or}~0, &\text{if}~r \in \mathcal{I}_k \\
        1, &\text{if}~r \in \mathcal{I}_k^+ \\
        0, &\text{if}~r \in \mathcal{I}_k^-
    \end{cases}
    .
\end{align}
Let $\Lambda^{(k)}_{a}$ be the diagonal activation matrix for neurons in the $k$-th layer that are always activated and set $\Lambda^{(k)}_{u}: = \Lambda^{(k)} - \Lambda^{(k)}_{a}$. Starting by analyzing the bound of the gradient $\nabla \phi_k(x)$ coordinate-wisely in a $2$-layer ReLU network, \citet{weng2018fastlip} show that an inequality for gradient $q$-norm holds:
\begin{align}
    \max_{x \in B_p(x_0, \epsilon)}
    \;
    \Bigl| \left[ \nabla f_j(x) \right]_k \Bigr|
    \leq
    \max \Bigl( 
    C_{j,k}^{(1)} + L_{j,k}^{(1)}
    ,\;
    C_{j,k}^{(1)} + U_{j,k}^{(1)}
    \Bigr)
    ,
\end{align}
where:
\begin{align}
    C_{j,k}^{(1)} = W_{j,:}^{(2)} \Lambda^{(1)}_{a} W_{:,k}^{(1)}
    , 
\end{align}
\begin{align}
L_{j,k}^{(1)} = \sum_{i \in \mathcal{I}_1, W_{j,i}^{(2)}W_{i,k}^{(2)} < 0} W_{j,i}^{(2)}W_{i,k}^{(2)}, 
    \quad
    \text{and}
    \quad
    U_{j,k}^{(1)} = \sum_{i \in \mathcal{I}_1, W_{j,i}^{(2)}W_{i,k}^{(2)} > 0} W_{j,i}^{(2)}W_{i,k}^{(2)}
    .
\end{align}
Then the gradient $q$-norm can be bounded above by:
\begin{align}
\mathrm{Lip}_q\left[f_j; B_p(x_0, \epsilon)\right]
=
\max_{x \in B_p(x_0, \epsilon)} \| \nabla f_j(x) \|_q 
\leq
\Biggl[ 
\sum_k
\Bigl(
\max_{x \in B_p(x_0,\epsilon)}
\| \nabla f_j(x) \|_k
\Bigr)
\Biggr]^{\frac{1}{q}}
,
\end{align}
yielding a local Lipschitz constant upper bound. This method is referred to as \textbf{Fast-Lip} in \citet{weng2018fastlip}.





\subsection{Spectral Alignment}

\textbf{SeqLip \citep{virmaux2018lipschitz}} refines the upper bound of an $L$-layer sequential network $f$ with $1$-Lipschitz activation functions:
\begin{align}
    \mathrm{Lip}\left[f\right]^+ = \prod_{\ell=1}^{L} \|W^{(\ell)}||_2
    ,
\end{align}
where $W^{(\ell)} \in \mathbb{R}^{n_{\ell} \times n_{\ell+1}}$ is the $\ell$-th layer parameter matrix, and $\mathrm{Lip}\left[f\right]^+$ is referred to as \textbf{AutoLip} bound in \citet{virmaux2018lipschitz}. By taking into account the spectral alignment between the parameter matrices of two consecutive layers, the bound is then refined as:
\begin{align}
  \mathrm{Lip}\left[f\right] &\leq 
  \mathrm{Lip}\left[f\right]^+ \notag\\
  &\quad\Biggl(
  \underbrace{
  \prod_{\ell}^{L-1}
  \sqrt{
  (1 - r_{\ell} - r_{\ell+1}) 
  \quad\max_{t^{(\ell)} \in [0,1]^{n_\ell}} 
  \langle
  t^{(\ell)} \cdot 
  v_1^{(\ell+1)}
  ,\;
  u_1^{(\ell)}
  \rangle^2
  +r_{\ell} + r_{\ell+1} + r_{\ell}r_{\ell+1}
  }
  }_{\text{spectral alignment}}
  \;
  \Biggr)
  ,
\end{align}
% \begin{align}
%   \mathrm{Lip}\left[f\right] \leq 
%   \mathrm{Lip}\left[f\right]^+
%   \left\Biggl(
%   \underbrace{
%   \prod_{\ell}^{L-1}
%   \sqrt{
%   \begin{aligned}
%   &(1 - r_{\ell} - r_{\ell+1}) \notag\\
%   &\quad\max_{t^{(\ell)} \in [0,1]^{n_\ell}} 
%   \langle
%   t^{(\ell)} \cdot 
%   v_1^{(\ell+1)}
%   ,\;
%   u_1^{(\ell)}
%   \rangle^2
%   +r_{\ell} + r_{\ell+1} + r_{\ell}r_{\ell+1}
%   \end{aligned}
%   }
%   }_{\text{spectral alignment}}
%   \;
%   \right\Biggr)
%   ,
% \end{align}
where $t^{(\ell)} [0,1]^{n_\ell}$ represents the $\ell$-th layer gradient patterns from activation functions for $n_{\ell}$ neurons --- the coordinate-wise gradient of an activation function such as ReLU falls in $[0, 1]$, $u_1^{(\ell)}$ is the first left-singular vector for $W^{(\ell)}$, $v_1^{(\ell+1)}$ is the first right-singular vector for $W^{(\ell+1)}$, and $r_{\ell}=\frac{\sigma_2^{(\ell)}}{\sigma_1^{(\ell)}}$ is the ratio of the second largest singular value to the first largest singular value for $W^{(\ell+1)}$ \citep[Theorem 3]{virmaux2018lipschitz}.


\citet{virmaux2018lipschitz} also show that, if $u, v \mathbb{R}^n$ are two independent random vectors taken uniformly from $\mathbb{S}^{n-1}=\{ x \in \mathbb{R}^n \mid \|x\|_2=1\}$, the following limit:
\begin{align}
    \lim_{n \to \infty}\;
    \max_{t \in [0,1]^n} \Bigl | 
    \langle
    t \cdot u 
    \;,
    v
    \rangle
    \Bigr |
    =\frac{1}{\pi}
\end{align}
holds \emph{almost surely}. Under this independent assumption, the bound reduces to:
\begin{align}
    \mathrm{Lip}\left[f\right] \leq \frac{\mathrm{Lip}\left[f\right]^+}{\pi^{L-1}}
\end{align}
\citep[Lemma 2]{virmaux2018lipschitz}. In real setting, the singular vectors are not independent across layers. 

\subsection{Convex Optimization Relaxation}

\textbf{LipSDP \citep{fazlyab2019efficient}} interpret activation functions as gradients of convex potential functions, satisfying certain properties described by quadratic constraints. Therefore, Lipschitz constant estimation problem is treated as a semidefinite program (SDP) problem.

Let $f: \mathbb{R}^{n_0} \to \mathbb{R}^{n_L}$ be an $L$-layer feed-forward network, recursively defined as:
\begin{align}
    \begin{cases}
        x^{(0)} = x \\
        x^{(k+1)} = \phi \Bigl( W^{(k)x^{(k)}} + b^{(k)} \Bigr)
    \end{cases}
    ,
\end{align}
where $x^{(\ell)}$ is the output at the $\ell$-th layer, $W^{(\ell)} \in \mathbb{R}^{n_{\ell+1} \times n_{\ell}}$ is the parameter matrix at the $\ell$-th layer, $b^{(\ell)} \in \mathbb{R}^{n_{\ell+1}}$ is the bias at the $\ell$-th layer, and $\phi$ is the coordinate-wise activation function. For a single layer network:
\begin{align}
f(x) = W^{(1)} \phi \bigl(
W^{(0)}x + b^{(0)} + b^{(1)}
\bigr) 
,
\end{align}
\citet{fazlyab2019efficient} shows that the Lipschitz constant of $f$ is given by a SDP problem:
\begin{align}
    \mathrm{Lip}\left[f\right] \leq \sqrt{\rho}
    ,
\end{align}
defined by:
\begin{align}
    \text{minimize}    \qquad &\rho \\
    \text{subject to}  \qquad &M(\rho, T) \preceq 0 \quad T \in T_n,
\end{align}
where $\phi$ is \emph{slope-restricted} on $[\alpha, \beta]$:
\begin{align}
    \alpha \leq \frac{\phi_j(x) - \phi_j(y)}{x-y} \leq \beta \qquad \forall x,y \in \mathbb{R}
\end{align}
and:
\begin{align}
   M(\rho, T) :=
   \begin{bmatrix}
       -2\alpha\beta (W^{(0)})^\top T W^{(0)} &(\alpha + \beta)(W^{(0)})^\top \\
       (\alpha + \beta) T W^{(0)} & -2T + (W^{(1)})^\top W^{(1)}
   \end{bmatrix} 
   \preceq 0
\end{align}
holds true for $T \in T_n$ \citep[Theorem 1]{fazlyab2019efficient}. For more general $L$-layer fully-connected network, \citet{fazlyab2019efficient} show that $M(\rho, T)$ is:
\begin{align}
    M(\rho, T) = 
    \begin{bmatrix}
        A \\
        B
    \end{bmatrix}^\top
    \begin{bmatrix}
        -2\alpha\beta\,T & (\alpha + \beta)T \\
        (\alpha + \beta)T & -2T
    \end{bmatrix}
    \begin{bmatrix}
        A \\
        B
    \end{bmatrix}
    +
    \begin{bmatrix}
        -\rho I_{n_0} &0 &\cdots &0 \\
        0             &0 &\cdots &0 \\
        \vdots        &\vdots &\ddots &\vdots \\
        0             &0 &\cdots &(W^{(L)})^\top\,W^{(L)}
    \end{bmatrix}
    \preceq 0
    ,
\end{align}
where:
\begin{align}
    A=\begin{bmatrix}
        W^{(0)} &0 &\cdots &0 &0 \\
        0        &W^{(1)} &\cdots &0 &0 \\
        \vdots &\vdots &\ddots &\vdots &\vdots \\
        0 &0 &\cdots &W^{(L-1)} & 0
    \end{bmatrix}
    , \qquad
    B=\begin{bmatrix}
        0 &I_{n_1} &0 &\cdots &0 \\
        0  &0 &I_{n_2} &\cdots &0 \\
        \vdots &\vdots &\vdots &\ddots &\vdots \\
        0 &0 &0 &\cdots &I_{n_L}
    \end{bmatrix}
    ,
\end{align}
and:
\begin{align}
    C=\begin{bmatrix}
        0 &\cdots &0 &W^{(L)}
    \end{bmatrix}
    ,
    \qquad
    b=\begin{bmatrix}
        (b^{(0)})^\top \cdots (b^{(L-1)})^\top
    \end{bmatrix}^\top
\end{align}
\citep[Theorem 2]{fazlyab2019efficient}.





\subsection{Integer Programming for ReLU Networks}

It is well known that computing the Lipschitz constant of an arbitrary scalar- or vector-valued function is NP-hard \citep{virmaux2018lipschitz,jordan2020exactly}. A common approximation is to estimate the Lipschitz constant using gradient norms, where the Jacobians can be explicitly derived via the chain rule. However, nondifferentiabilities, \eg, those arising in ReLU networks, can introduce inaccuracies into these estimates. An alternative approach is to formulate the Lipschitz bounding problem as an integer programming problem, which avoids such inaccuracies by directly bounding the Jacobians.


\textbf{LipMIP \citep{jordan2020exactly}} is a method that provably exactly compute
$2$-norm and $\infty$-norm Lipschitz constants of non-smooth ReLU networks. We summarize their method by simplifying their notations. Let $f: \mathbb{R}^d \to \mathbb{R}$ be a ReLU network. Let $\sigma$ be activation function. Then, an $L$-layer ReLU network is recursively defined as:
\begin{align}
    \begin{cases}
        f(x) = \sigma(Z_L(x)) \\
        Z^{(\ell)}(x) = W^{(\ell)}\;\sigma\Bigl(Z^{(\ell-1)}(x)\Bigr) + b^{(\ell)} \\
        Z^{(0)} = x
    \end{cases}
,
\end{align}
where $W^{(\ell)} \in \mathbb{R}^{n_{\ell} \times n_{\ell-1}}$ is the $\ell$-th layer parameter matrix, and $Z^{(\ell)}(x)$ is the output of the $\ell$-th layer neurons. Let $\partial f(x)$ be the Clarke sub-differential convex hull of $f$ at point $x$ --- see Section~\ref{sec:subdifferential}~(\nameref{sec:subdifferential}). For example:
\begin{align}
 \partial \sigma(0)=[0,1]   
 .
\end{align}
Let $\partial f(X)$:
\begin{align}
    \partial f(X) = \Bigl\{
    g \mid\; g \in \partial f(x), x \in X
    \Bigr\}
\end{align}
be the set-valued Clarke sub-differentials at set $X$. Let $\nabla^{\sharp} f(\bullet)$ be the pushforward set that the sub-gradients of ReLU activation at value $0$ come from the hull set $\partial \sigma(0)$:
\begin{align}
    \nabla^{\sharp} f(\bullet) =\Bigl\{
    \nabla f(\bullet) \mid \text{the sub-differentials of activations come from the hull set}~\partial\sigma(0)
    \Bigr\}
    .
\end{align}
Thus for a ReLU network, the \emph{feasible set} for its gradients on $X$ are given as:
\begin{align}
\nabla^{\sharp} f(X) =
  \Bigl\{   
    G \in \nabla^{\sharp} f(x) \mid x \in X 
  \Bigr\}
  .
\end{align}
\cite{jordan2020exactly} show that the push forward set sub-gradient $\nabla^{\sharp} f(x)$ is the Clarke sub-gradient hull $\partial f(x)$, that is:
\begin{align}
    \nabla^{\sharp} f(x) = \partial f(x)
\end{align}
\citep[Theorem 2]{jordan2020exactly}. Then the local $p \to q$ Lipschitz constant of $f$ on $X$ is given as:
\begin{align}
    \mathrm{Lip}_{p \to q}\left[f;X\right] =\sup_{G \in \nabla^{\sharp} f(X)} \sup_{\|v\|_p \leq 1} \frac{\|G^\top\,v\|_{q}}{\|v\|_p}
    = \sup_{G \in \nabla^{\sharp} f(X)} \|G^\top \|_q
    .
\end{align}
Finding the Lipschitz constant on $X$ can be formulated as an integer programming problem on the feasible set $\nabla^{\sharp} f(X)$. Let $n=\sum_{\ell=1}^L n_{\ell}$ be the number of neurons in $f$. The set:
\begin{align}
    \Bigl\{
    \|G^\top\|_q \mid G \in \nabla^{\sharp} f(X)
    \Bigr\}
\end{align}
is then represented as a mixed-integer programming problem for maximizing $\|G^\top\|_q$ by solving the combinations of input $x \in X$ and ReLU's sub-gradient $a \in [0, 1]^n$ on a mixed-integer polytope in $X \times [0, 1]^n$, such that $\nabla^{\sharp} f(x)$ is represented with some $A$, $B$ and $c$:
\begin{align}
    \nabla^{\sharp} f(x) = Ax + Ba < c
\end{align}
by analyzing gradients with chain rules on ReLU networks \citep[Definition 6 \& Lemma 1]{jordan2020exactly}. This problem can be solved by off-the-shelf MIP solvers.



















\section{Regularization Approaches}
\label{sec:lipschitz_regularizations}


A variety of techniques have been developed to explicitly or implicitly enforce Lipschitz continuity in deep neural networks. These approaches can be categorized into:
\begin{enumerate}[label=(\roman*)]
    \item Section~\ref{sec:lipschitz_regularizations:weight}: \textbf{\nameref{sec:lipschitz_regularizations:weight}} --- constraining or regularizing weight matrices during initialization and training;
    
    \item Section~\ref{sec:lipschitz_regularizations:gradient}: \textbf{\nameref{sec:lipschitz_regularizations:gradient}} --- penalizing or normalizing gradient norms during training;

    \item Section~\ref{sec:lipschitz_regularizations:activation}: \textbf{\nameref{sec:lipschitz_regularizations:activation}} --- designing or constraining activation functions to be Lipschitz-bounded; 


    \item Section~\ref{sec:lipschitz_regularizations:class_margin}: \textbf{\nameref{sec:lipschitz_regularizations:class_margin}} --- implicitly enforcing Lipschitz constraints via maximizing class decision boundaries;


    \item Section~\ref{sec:lipschitz_regularizations:architecture}: \textbf{\nameref{sec:lipschitz_regularizations:architecture}} --- enforcing Lipschitz constraints by designing architectures, particularly for transformers.

    %\item \textbf{Data Regularization} --- implicitly controlling the Lipschitz constant through data augmentation or perturbation-based training;

\end{enumerate}


\subsection{Weight Regularization}
\label{sec:lipschitz_regularizations:weight}


This subsection reviews methods that control the Lipschitz constant by directly constraining or regularizing the network's weight parameters, either at initialization or during training.

\subsubsection{Spectral-Norm Regularization}

Spectral-norm regularization constrains the Lipschitz constant of a neural network by bounding the spectral-norm of its weight matrices, which is the largest singular value of the matrix (Proposition~\ref{prop:lipschitz_constant_of_linear_unit}). \citet{miyato2018spectral} propose normalizing the weight matrix $W$ of a linear layer by:
\begin{align}
W \leftarrow \frac{W}{\|W\|_2},
\end{align}
ensuring a Lipschitz constant of at most $1$ for the layer \citep[\S~3]{miyato2018spectral}. This method, later adopted by \citeauthor{miyato2018spectral} in generative adversarial networks (GANs) \citep{goodfellow2014generative}, for improving the generations \citep[\S~2.1]{miyato2018spectral}. 





\subsubsection{Weight Clipping}
Weight clipping is a straightforward method to enforce Lipschitz continuity by limiting the magnitude of weight matrices. This is because for a matrix $W$, the operator-norm variation $\|W\|_{op}$ in $\ell_2$ for $W$ under perturbation $\Delta\,W$ is bounded above by:
\begin{align}
    \|W\|_{op} = \sigma_1(W) = \langle u_1 v_1^\top,\; \Delta W \rangle \leq \|u_1 v_1^\top\|_2\; \|\Delta\,W\|_2
    ,
\end{align}
with Cauchy–Schwarz inequality, where $\sigma_1(W)$ is the largest singular value of $W$, $u_1, v_1$ are the left- and right-singular vectors corresponding the largest singular value \citep[Lemma 5.1]{luo2025spectralvariation}.

In the setting of GANs, \citet{arjovsky2017wasserstein} show that the discriminator $f$ of a GAN evaluates the Wasserstein distance $W\left(\mathbb{P}, \mathbb{Q}\right)$ between two distributions $\mathbb{P}$ and $\mathbb{Q}$. The Kantorovich-Rubinstein duality \citep{villani2008optimal} tells that:
\begin{align}
    W\left(\mathbb{P}, \mathbb{Q}\right) = K \; \sup_{\mathrm{Lip}\left[f\right] \leq K} \;
    \mathbb{E}_{x \sim \mathbb{P}}\bigl[f(x)\bigr] - \mathbb{E}_{y \sim \mathbb{Q}}\bigl[f(y)\bigr]
\end{align}
\citep[Equation 2]{arjovsky2017wasserstein}. Therefore reducing the Lipschitz constant $K$ can reduce the Wasserstein distance $W\left(\mathbb{P}, \mathbb{Q}\right)$. \citet{arjovsky2017wasserstein} propose clipping weights to a fixed range:
\begin{align}
W \leftarrow \text{clip}(W, -c, +c)
\end{align}
\citep[Algorithm 1]{arjovsky2017wasserstein}, where $c$ is a small positive constant (\eg, $c=0.01$). Weight clipping is computationally efficient, but can lead to exploding or vanishing gradients if $c$ is too small, reducing model capacity, as criticized in the a later literature \citep{gulrajani2017improved}. 






\subsubsection{Orthogonal Weight}

%Parseval Networks: Improving Robustness to Adversarial Examples
% 4.1. Parseval Regularization
\paragraph{Parseval Networks \citep{cisse2017parseval}.} Parseval networks enforce approximate orthonormality on weight matrices to bound their spectral-norms \citep{cisse2017parseval}. For a weight matrix $W^{(\ell)}$ in layer $\ell$, \citet{cisse2017parseval} minimize the $2$-norm of the deviation from orthonormality:
\begin{align}
\|W^{(\ell)\top} W^{(\ell)} - \mathrm{I}\|_F,
\end{align}
ensuring $\|W^{(\ell)}\|_2 \leq 1$ \citep[\S~4.2]{cisse2017parseval}. For a feedforward network with $L$ layers and 1-Lipschitz activations (\eg, ReLU), the global Lipschitz constant is bounded by:
\begin{align}
K \leq \prod_{\ell=1}^L \|W^{(\ell)}\|_2 \leq 1
\end{align} (Proposition~\ref{prop:survey_upper_bound_lipschitz}). \cite{cisse2017parseval} argue that the robustness to adversarial attacks is enhanced since the reduced sensitivity to perturbations.







\subsection{Gradient Regularization}
\label{sec:lipschitz_regularizations:gradient}

%\subsubsection{Gradient Norm Penalty}
%\paragraph{Direct Gradient Penalty.} 

Gradient-based regularization methods enforce Lipschitz continuity by constraining the gradient norm of the loss function or network output with respect to inputs, ensuring smooth decision boundaries and robustness. Note that, for a network $f$ on convex $X$, its $2$-norm Lipschitz constant on $X$ is given by:
\begin{align}
    \mathrm{Lip}\left[f\right] = \sup_{x \in X} \|\nabla\,f(x)\|_2
    ,
\end{align}
see \ref{lemma:lipschitz_bounds_gradient} (\nameref{lemma:lipschitz_bounds_gradient}). Theoretically, constraining $\|\nabla\,f(x)\|_2$ can bound Lipschitz constant of $f$. 

For example, \citet{gulrajani2017improved} argue that bounding Lipschitz constant by weight clipping can lead exploding or vanishing gradients, and reduce capacity of the critic in a GAN. They then introduce a regularization method by directly bounding the gradients of the critic network $D$ through:
\begin{align}
    \mathbb{E}_{x\,\sim\,\mathbb{P}_X}
    \Bigl[
    \bigl(
    \|\nabla\,D(x)\|_2 -1
    \bigr)^2
    \Bigr]
    ,
\end{align}
where $\mathbb{P}_X$ is the distribution of training sample set $X$ \citep[\S~4]{gulrajani2017improved}. 






\subsection{Activation Regularization}
\label{sec:lipschitz_regularizations:activation}

Activation regularization methods modulates Lipschitz continuity by constraining the properties of activation functions or their outputs. Such approaches may impose explicit norm bounds, design activations that are inherently norm-preserving, or apply penalties to activation magnitudes, thereby limiting the contribution of nonlinearities to the overall Lipschitz constant of the network.

\subsubsection{Group-Sorting Activation}

Bounding the Lipschitz constant of a network by ensuring $1$-Lipschitz for affine units through spectral-norm constraints can improve robustness \citep{miyato2018spectral}. However, this often comes at the cost of reduced expressiveness \citep{anil2019sorting}. \citet{anil2019sorting} first show that, to remain expressive in a spectral-norm constrained network, the network must preserve the gradient norms at each layer \citep{anil2019sorting}. ReLU networks can only satisfy this for positive values, this is because:
\begin{align}
    \frac{\partial\,\mathrm{ReLU}(x)}{\partial\,x} = \begin{cases}
        1, &x > 0\\
(0,1), &\text{in sub-differential sense} \\ 
        0, &x < 0
    \end{cases}
    .
\end{align}
To preserve the gradient norms at activation layer, \citet{anil2019sorting} use a general purpose $1$-Lipschitz
activation function $\textbf{GroupSort}(x)$ which is homogeneous: 
\begin{align}
\textbf{GroupSort}(\alpha\,x)=\alpha\,\textbf{GroupSort}(x)    
\end{align}
\citep{anil2019sorting}. \textbf{GroupSort} activation separates
a pre-activation $x$ into $k$ groups:
\begin{align}
    x = (
    \underbrace{
    x_1, \cdots, x_{g_1}
    }_{\text{group 1}}
    ,\, 
    \underbrace{
    x_{g_1+1}, \cdots, x_{g_2}
    }_{\text{group 2}}
    ,\cdots\,
    \underbrace{
    x_{g_{k-1}+1}, \cdots, x_{g_k}
    }_{\text{group k}}
    )
    ,
\end{align}
and sorts each group into ascending order:
\begin{align}
    \textbf{GroupSort}(x) = (
    \underbrace{
    x_{s_1}, \cdots, x_{s_{g_1}}
    }_{\text{group 1}}
    ,\, 
    \underbrace{
    x_{s_{g_1}+1}, \cdots, x_{s_{g_2}}
    }_{\text{group 2}}
    ,\cdots\,
    \underbrace{
    x_{s_{g_{k-1}}+1}, \cdots, x_{s_{g_k}}
    }_{\text{group k}}
    )
,
\end{align}
where the $i$-th sorted group satisfies:
\begin{align}
x_{s_{g_{i-1}}+1} \leq 
x_{s_{g_{k-1}}+2} \leq
\cdots \leq
x_{s_{g_{k}}}
\end{align}
\citep{anil2019sorting}. For the pre-activation in a linear unit:
\begin{align}
   Wx 
\end{align}
where $W \in \mathbb{R}^{m \times n}$ and $x \in \mathbb{R}^n$, if the linear unit is with spectral-norm constraint such that:
\begin{align}
    \|W\|_2 = 1
    ,
\end{align}
\textbf{GroupSort} activation directly gives rise an $1$-Lipschitz constant activation:
\begin{align}
    \sup_{\|x\|_2=1} \| \textbf{GroupSort}(Wx) \|_2
    = \sup_{\|x\|_2=1} \| Wx \|_2 = \|W\|_2.
\end{align}
When the group size is $2$, \citet{anil2019sorting} refers to this special case as \textbf{MaxMin}, which is equivalent to the Orthogonal Permutation Linear Unit (OPLU) \citep{chernodub2017normpreservingorthogonalpermutationlinear}; when the group size is the entire input, this is referred to as \textbf{FullSort} in the literature \citep{chernodub2017normpreservingorthogonalpermutationlinear}.

To train a network with \textbf{GroupSort} activations and guarantee that all linear units are exactly $1$-Lipschitz during optimization instead of bounded by $1$ \citep{cisse2017parseval,gulrajani2017improved}, \citet{chernodub2017normpreservingorthogonalpermutationlinear} approximate the updated parameter matrix $W_0$ with a closest orthogonal matrix through a differentiable, iterative algorithm, referred to as \emph{Bj\"orck Orthogonalization} \citep{bjorck1971}. This algorithm is defined by:
\begin{align}
    W_{k+1} = W_k \Bigl(
    I + \frac{1}{2} Q_k + \cdots + (-1)^p 
    \begin{pmatrix}
        -\frac{1}{2} \\
        p
    \end{pmatrix}
    Q_k^p
    \Bigr)
    ,
\end{align}
where $W_{k}$ is the $k$-th iterative result, $p$ is a chosen hyper-parameter and $Q_k$ is:
\begin{align}
    Q_k = I - W_k^\top W_k
\end{align}
\citep[\S~4.2.1]{chernodub2017normpreservingorthogonalpermutationlinear}. As a result, the iteration at step $T$ leads to:
\begin{align}
    W_T^\top W_T \approx I
    ,
\end{align}
which provably ensures the linear unit with parameter matrix $W$ is $1$-Lipschitz continuous:
\begin{align}
    \|W_T\|_2 \approx 1.
\end{align}


\subsubsection{Contraction Activation and Invertible Residual Map}

%Invertible DenseNets with Concatenated LipSwish
%

Flow-based models or flows learn to transform a source distribution $p_X$ to target distribution $p_Z$, consisting of invertible networks \citep{Rezende2015VariationalNormalizingFlows}. Ensuring that the transformation is invertible and its Jacobian are computable is a straightforward way for ensuring invertibility:
\begin{align}
    \log\,p_X(x) = \log\,p_Z(z) + \log\, \left| \det J_F(x) \right|
\end{align}
where $F: \mathbb{R}^m \to \mathbb{R}^m$ is an invertible map and $J_F(x)$ is the Jacobian of $F$ at $x$ \citep{berg2018sylvester,dinh2017density}. Different from explicit computation of Jacobian, \citet{Behrmann2019InvertibleResidual} propose a method for inverting residual networks \citep{he2016deep} by ensuring the Lipschitz constants be less than $1$, so that the residual networks are \emph{contraction maps} \citep{Behrmann2019InvertibleResidual,perugachi2021invertible}. 

\paragraph{Inverting Residual Layer.} Let 
\begin{align}
    F(x) = x + g(x)
\end{align}
be a residual layer where $F: \mathbb{R}^m \to \mathbb{R}^m$, $g: \mathbb{R}^m \to \mathbb{R}^m$ and $x \in \mathbb{R}^m$. Let $g$ be a contraction map:
\begin{align}
    \mathrm{Lip}\left[g\right] < 1
    .
\end{align}
Suppose that the inversion $F^{-1}$ exists and set $y =F(x)$, so that:
\begin{align}
    F^{-1}(x) = x = y - g(x).
\end{align}
Set:
\begin{align}
    T(x) = y - g(x)
,
\end{align}
note that:
\begin{align}
    \mathrm{Lip}\left[T\right] = \mathrm{Lip}\left[g\right] < 1
\end{align}
is a contraction mapping. Using \emph{Banach contraction principle} or \emph{Banach fixed-point theorem}, set $x_0=y$, the $F^{-1}(y)$ can be approximated through:
\begin{align}
    x_{k+1} = y - g(x_k)
\end{align}
iteratively. The \textbf{essential condition} for inverting $g$ is that $g$ must be a contraction map:
\begin{align}
    \mathrm{Lip}\left[g\right] < 1.
\end{align}


\paragraph{Contraction Activation.} \citet{chen2019residualflows} first introduce \textbf{LipSwish} activation function for inverting residual networks, defined as:
\begin{align}
    \textbf{LipSwish}(x) = \frac{x\sigma(\beta\,x)}{1.1}
    ,
\end{align}
where $\sigma$ is the sigmoid function, and $\beta > 0$ is a learnable negative constant, initialized with $0.5$. $\textbf{LipSwish}$ has a Lipschitz constant at most $1$. However, the negative axis of $\textbf{LipSwish}$ has zero gradients almost everywhere. In a $1$-Lipschitz continuous network, the Jacobian norm across two consecutive layers is reduced to be at most one, which limits the network's expressiveness and referred to as \emph{gradient norm attenuation} problem \citep{anil2019sorting,li2019preventinggradientattenuation}. To mitigate this problem, \citet{perugachi2021invertible} use specially designed activation function \textbf{CLipSwish} by concatenating two \textbf{LipSwish} functions. The \textbf{CLipSwish} is therefore given as:
\begin{align}
    \Phi(x)=
    \begin{bmatrix}
        \textbf{LipSwish}(x) \\
        \textbf{LipSwish}(-x)
    \end{bmatrix}
    ,
    \qquad
    \textbf{CLipSwish}(x)= \frac{\Phi(x)}{\mathrm{Lip}\left[\Phi\right]} \leq 1
    ,
\end{align}
where $\mathrm{Lip}\left[\Phi\right] \approx 1.004$ \citep[\S~3.4]{perugachi2021invertible}. This concatenation overcomes the gradient attenuation problem introduced by $\textbf{LipSwish}$ since the negative axis has zero gradients almost everywhere while ensuring the activation is a contraction map. 


\subsection{Class-Margin Regularization}
\label{sec:lipschitz_regularizations:class_margin}

%Lipschitz-Margin Training: Scalable Certification of Perturbation Invariance for Deep Neural Networks

The goal of adversarial defense in classification task is to ensure that, for a $k$-class classifier $f: \mathbb{R}^d \to \mathbb{R}^k$, and an input $x \in \mathbb{R}^d$, a bounded perturbation $\|\epsilon_x\|_2 < c$ does not alter the prediction:
\begin{align}
    \argmax\limits_{i \in [k]=\{1,2,\cdots,k\}} \;f_i(x+\epsilon_x),
\end{align}
where $f_i(x)$ denotes the output at the $i$-th coordinate. The margin $m(x)$ is defined as:
\begin{align}
    m(x) = f_i(x) - \max_{j \neq i} f_j(x)
    ,
\end{align}
where $i$ is the ground-truth \citep[\S~4.1]{tsuzuku2018lipschitz}. Then, a guaranteed $2$-norm perturbation bound does not alter the prediction, if:
\begin{align}
    \|\epsilon_x\|_2 \leq \frac{m(x)}{\sqrt{2} \;\mathrm{Lip}\left[f\right]}
\end{align}
\citep{szegedy2014intriguing,cisse2017parseval}. This implies that the class margin must be at least:
\begin{align}
    m(x) = f_i(x) - \max_{j \neq i} f_j(x) \geq \sqrt{2} \;\mathrm{Lip}\left[f\right]
\end{align}
\citep[Proposition 1 \& 2]{tsuzuku2018lipschitz}. Suppose $i$ is the ground-truth for $x$, in training stage, \citet{perugachi2021invertible} adjust each class margin $j \neq i$ by:
\begin{align}
    f_j(x) \leftarrow f_j(x) + \sqrt{2}\,c\,\mathrm{Lip}\left[f\right]
    ,
\end{align}
where $c$ is a guaranteed perturbation bound \citep[Algorithm 1]{perugachi2021invertible}. For each linear unit $\phi: \mathbb{R}^m \to \mathbb{R}^n$ in the network, and let $u \in \mathbb{R}^m$ be drawn i.i.d. from $\mathcal{N}(0,1)$. \citet{perugachi2021invertible} use a general method for estimating the Lipschitz constant of $\phi$ iteratively by:
\begin{align}
    u_{k} \leftarrow \frac{u_k}{\|u_k\|_2}, \qquad 
    v_{k} \leftarrow \phi(u_{k}), \qquad
    u_{k+1} \leftarrow \frac{1}{2}\frac{\partial\,\|v_k\|_2^2}{\partial\,u}.
\end{align}
At the end of the iteration $T$, the Lipschitz constant of $\phi$ is given by:
\begin{align}
    \mathrm{Lip}\left[\phi\right] \approx \|u_T\|_2
,
\end{align}
almost surely \citep{perugachi2021invertible}.



\subsection{Architectural Regularization}
\label{sec:lipschitz_regularizations:architecture}

Lipschitz continuity can also be constrained through architectural design choices, including activation functions, parameter structures, initialization schemes, and optimization. As a complement to regularization approaches that do not fall into one single category, we survey these approaches in this section.

\subsubsection{Orthogonalizing Convolution}

%\paragraph{Orthogonalizing Convolutional Layers}
%https://arxiv.org/pdf/2104.07167
% \paragraph{Cayley transform \citep{trockman2021orthogonalizing}}.

Parameter orthogonality in neural networks can directly yield $1$-Lipschitz continuous (Proposition~\ref{prop:column_orthogonal_matrix})~(\nameref{prop:column_orthogonal_matrix})). This is because, for a matrix $W \in \mathbb{R}^{m \times n}$, an semi-orthogonal matrix $W$ preserves the $2$-norm:
\begin{align}
    W^\top\,W = I_n
    \quad \text{or} \quad
    WW^\top = I_m
    \quad
    \Longrightarrow 
    \quad
    \mathrm{Lip}\left[ W \right]=1
    ,
\end{align}
if $m \geq n$ and $W^\top W=I_n$, $W$ is an isometric map; if $m < n$ and $WW^\top = I_m$, $W$ is a contraction map on the kernel $\ker(W)$ strictly (Proposition~\ref{prop:column_orthogonal_matrix})~(\nameref{prop:column_orthogonal_matrix})).

\paragraph{Extending Semi-Orthogonality to Convolution.} Let $W \in \mathbb{R}^{c_{out} \times c_{in} \times n \times n}$ be a convolutional filter where $c_out$ is the number of output channels, $c_in$ is the number of input channels, and $n \times n$ are the input dimensions. The action on an input $x \in \mathbb{R}^{cc_{in} \times n \times n}$ is denoted by:
\begin{align}
    W \circledast x: \mathbb{R}^{c_{in} \times n \times n} \to \mathbb{R}^{c_{out} \times n \times n}.
\end{align}
Using the norm preserving concept for $1$-Lipschitz maps on $\ell_2$, for $\forall\;x \in \mathbb{R}^{cc_{in} \times n \times n}$, if the $2$-norms are preserved:
\begin{align}
    \|W \circledast x\|_2 = \|x\|_2
    ,
\end{align}
then the convolutional filter $W$ is referred to as semi-orthogonal \citep{trockman2021orthogonalizing}. %By assuming the convolutions are circular, the 3D convolution $W \circledast x$ can be converted to a 2D convolution filter $\Tilde{W}$ acting on a 1D input vector $\Tilde{x}$.


\paragraph{Filter Orthogonalization via Cayley Transform.} However, convolutional operation is not matrix multiplication, to apply the existing results from matrix theory, \citet{trockman2021orthogonalizing} harness the \emph{Convolutional Theorem} \citep{jain1989fundamentals} for converting the convolutional operation in spatial domain to multiplication in frequency domain by:
\begin{align}
    \mathscr{F}\left[W \circledast x\right][:,i,j] =\mathscr{F}\left[W\right][:,:,i,j] \; \mathscr{F}\left[x\right][:,:,i,j] = \widehat{W}[:,i,j]\widehat{x}[:,i,j]
    ,
\end{align}
where $\mathscr{F}$ represents Fourier transform, $\widehat{W}=\mathscr{F}\left[W\right]$, $\widehat{x}=\mathscr{F}\left[x\right]$, $[:,:,i,j]$ and $[:,i,j]$ are slicing operations by fixing indices $(i,j)$) \citep[Equantion 3 \& 4, \S~4]{trockman2021orthogonalizing}. Note that $\widehat{W}[:,:,i,j]$ is not orthogonal or semi-orthogonal, \citet{trockman2021orthogonalizing} use a bijective \emph{Cayley Transform} for deriving an orthogonal matrix $Q[:,:,i,j]$ from $\widehat{W}[:,:,i,j]$ by:
\begin{align}
    Q[:,:,i,j] = (I - A[:,:,i,j])(I + A[:,:,i,j])^{-1},
\end{align}
where:
\begin{align}
    A[:,:,i,j] = \widehat{W}[:,:,i,j] - \widehat{W}[:,:,i,j]^*
    ,
\end{align}
and $A[:,:,i,j]$ is referred to as \emph{skew-symetric} matrix \citep{trockman2021orthogonalizing}. Conceptually, the convolution on frequency domain is then computed through:
\begin{align}
    \mathscr{F}\left[W \circledast x \right][:,i,j] &= Q[:,:,i,j] \; \widehat{x}[:,i,j] \\
    &=(I - A[:,:,i,j])(I + A[:,:,i,j])^{-1} \;\widehat{x}[:,i,j]
    ,
\end{align}
then $Q[:,:,i,j] \; \widehat{x}[:,i,j]$ is inverted back to spatial domain by:
\begin{align}
    \mathscr{F}^{-1}\left[ Q[:,:,i,j] \; \widehat{x}[:,i,j]\right],
\end{align}
which leads to the convolution $1$-Lipschitz continuous.


\subsubsection{Orthogonality with Lie Unitary Group}

%\paragraph{Orthogonality with Lie Group Theory \citep{lezcano2019cheap}.} 

\citet{lezcano2019cheap} introduce a method, stemming from Lie group theory, through the exponential map, for ensuring $1$-Lipschitz by construction. Orthogonal
constraints networks can improve the robustness and generalization capabilities \citep{huang2018orthogonalweight,Bansal2018orthogonality}. For a matrix $A$, if $AA^*=I$, then the matrix $A$ is referred to as an unitary matrix. Unitary matrices allow to solve the exploding or vanish gradients \citep{Arjovsky2016unitary,arjovsky2017wasserstein}. In the sense of Lie algebra, these unitary matrices form a special orthogonal group on field $\mathbb{R}$:
\begin{align}
    SO(n) = \Bigl\{ 
    A \in \mathbb{R}^{n \times n} \mid A^\top A = I
    \Bigr\}
\end{align}
and unitary group on field $\mathbb{C}$:
\begin{align}
    U(n) = \Bigl\{ 
    A \in \mathbb{C}^{n \times n} \mid A^* A = I
    \Bigr\}
\end{align}
\citep[\S~3.1]{lezcano2019cheap}. We are interested of converting a parameter matrix $W \in \mathbb{R}^{n \times n}$ to on $SO(n)$ or $U(n)$. \citet{lezcano2019cheap} harness the concept of \emph{skew-symmetric matrix} group (Definition~\ref{def:skew_hermitian}~(\nameref{def:skew_hermitian})) as a bridge:
\begin{align}
    \mathfrak{so}(n)=\{B\in\mathbb{R}^{n\times n}\;:\;B=-B^\top\}
\end{align}
and:
\begin{align}
    \mathfrak{u}(n)=\{B\in\mathbb{R}^{n\times n}\;:\;B=-B^*\}
    .
\end{align}
Taking:
\begin{align}
    B=W - W^\top
\end{align}
can easily send a parameter matrix $W$ to $\mathfrak{u}(n)$. 

\paragraph{Connecting to Lie Orthogonal Group.} Then there exist an exponential \emph{surjective} map between two groups:
\begin{align}
    \exp: \mathfrak{so}(n) \to SO(n)
\end{align}
and:
\begin{align}
    \exp: \mathfrak{u}(n) \to U(n)
,
\end{align}
which is defined as:
\begin{align}
    \exp(B) = I + B + \frac{1}{2}B^2 + \cdots
\end{align}
\citep[\S~3.2]{lezcano2019cheap}. Then a network $f(x; W)$ is parameterized on the Lie group $SN(n)$ by an algebraic mapping chain:
\begin{align}
    W \in \mathbb{R}^{n \times n} 
    \xlongrightarrow[]{B=W-W^\top}  B \in \mathfrak{so}(n) \xlongrightarrow[]{A=\exp(A)}  A \in SO(n)
    ,
\end{align}
and the optimization problem becomes:
\begin{align}
    \min_{A}~f(x; A) \Longleftrightarrow \min_{B}~f(x; \exp(B))
\end{align}
\citep[\S~3.3]{lezcano2019cheap}. 


\paragraph{Optimizing on Lie Orthogonal Group.} The Lie group $SO(n)$ forms a Riemannian manifold, to optimize a function $f$ on the Riemannian manifold $SO(n)$:
\begin{align}
    f: \mathcal{X} \times SO(n) \to \mathbb{R}
    ,
\end{align}
where $\mathcal{X}$ is input space, one may use \emph{Riemannian gradient descent} \citep{absil2009optimization}. Given a point on the manifold $A \in SO(n)$, $\mathcal{T}_A\,SO(n)$ is the tangent space at $A$ with induced metric, and a gradient $\Omega \in \mathcal{T}_A\,SO(n)$, then the geodesic update is:
\begin{align}
    A \leftarrow A \, \exp\left(-\eta\,A^* \, \Omega\right)
    ,
\end{align}
where $\eta$ is a learning rate $\eta > 0$ \citep{lezcano2019cheap}. Computing the Riemannian exponential map is expensive, \citet{lezcano2019cheap} use a first-order approximation, \ie, \emph{Cayley map}, for the update instead:
\begin{align}
    A \leftarrow A \, \phi\left(-\eta\,A^* \, \Omega\right)
    ,
\end{align}
where $\phi$ is the \emph{Cayley map}:
\begin{align}
    \phi(A) = (I+\frac{1}{2}A)(I-\frac{1}{2}A)^{-1}    
\end{align}
\citep{Wisdom2016FullCapacity,Vorontsov2017Orthogonality}. Finally, this induces an update rule on $B \in \mathfrak{so}(n)$:
\begin{align}
    \exp(B) \leftarrow \exp\Bigl(B-\eta\,\nabla\,f\left(x;\exp(B)\right)\Bigr)\,
\end{align}
where $\nabla\,f\left(x;\exp(B)\right)$ is the usual gradient with Euclidean metric. In a specially designed recurrent neural network (RNN), \citet{lezcano2019cheap} transform the matrix exponential maps skew-symmetric matrices to orthogonal matrices transforming an optimization problem with orthogonal constraints \citep{lezcano2019cheap}. Particularly, \citet{lezcano2019cheap} use Pad\'e approximants and the scale-squaring trick to compute machine-precision approximations of the matrix exponential and its gradient \citep{lezcano2019cheap}. As a result, the optimization remains in the group and the Lipschitz constants of the updated matrices remain $1$ by design.


\subsubsection{Lipschitz Continuous Transformer}

% https://arxiv.org/pdf/2304.09856
\citet{qi2023lipsformer} demonstrate that enforcing Lipschitz continuity in Transformer architecture \citep{vaswani2017attention} is more crucial for ensuring training stability in contrast to the tricks such as \emph{learning rate warmup}, \emph{layer normalization}, \emph{attention formulation}, and \emph{weight initialization} \citep{qi2023lipsformer}. Their proposed method, referred to as \textbf{LipsFormer}, replaces the Transformer parts with their Lipschitz continuous counterparts: \emph{CenterNorm} for \emph{LayerNorm}, \emph{spectral initialization} for \emph{Xavier initialization}, \emph{scaled cosine similarity attention} for \emph{dot-product attention}, and \emph{weighted residual shortcut} for \emph{residual connection} \citep{qi2023lipsformer}. These modifications result in a Transformer architecture with a provably bounded Lipschitz constant.


\paragraph{CenterNorm instead of LayerNorm.} LayerNorm \citep{ba2016layer} is widely used in Transformer, defined as:
\begin{align}
    \mathrm{LN}(x) = \gamma \, \odot \, z + \beta
    ,
\end{align}
and:
\begin{align}
    z = \frac{y}{\mathrm{std}(y)}, \qquad y = \Bigl(I_d - \frac{1}{d}\boldsymbol{1}_d\boldsymbol{1}_d^\top\Bigr)x
    ,
\end{align}
where $x \in \mathbb{R}^d$ is input, $I_d$ is an identity matrix in $\mathbb{R}^{d \times d}$, $\boldsymbol{1}_d$ is an all-ones vector in $\mathbb{R}^d$, $\mathrm{std}(y)$ is the standard deviation of $y$, $\odot$ is element-wise product, $\alpha$ and $\beta$ are learnable parameters initialized to $1$ and $0$ respectively \citep{qi2023lipsformer}. The Jacobian of $z$ with respect to $x$ is given as:
\begin{align}
    \frac{\partial\,z}{\partial\,x} = \frac{1}{\mathrm{std}(y)} 
    \Bigl(I_d - \frac{1}{d}\boldsymbol{1}_d\boldsymbol{1}_d^\top\Bigr)
    \Bigl(
    I_d - \frac{yy^\top}{\|y\|_2^2}
    \Bigr)
    ,
\end{align}
which shows that \textbf{LayerNorm} is not Lipschitz continuous when $\mathrm{std}(y) \to 0$. To address this problem, \citet{qi2023lipsformer} introduce \textbf{CenterNorm}, defined as:
\begin{align}
    \mathrm{CN}(x) = \gamma\,\odot\,\frac{d}{d-1}
    \Bigl(I_d-\frac{1}{d}\boldsymbol{1}_d\boldsymbol{1}_d^\top\Bigr)x + \beta
    ,
\end{align}
which admits a Lipschitz constant:
\begin{align}
    \mathrm{Lip}\left[\mathrm{CN}\right] = \frac{d}{d-1} \approx 1
\end{align}
for sufficient large $d$, $\alpha=1$, and $\beta=0$ \citep{qi2023lipsformer}.


\paragraph{Scaled Cosine Similarity Attention (SCSA).} \citet{kim2021lipschitz} show that standard dot-product self-attention is not globally Lipschitz continuous since the Lipschitz constant depends on sequence length which is not bounded \citep{kim2021lipschitz}, see also Section~\ref{sec:selfattention_lipschitz} (\nameref{sec:selfattention_lipschitz}). To address this problem, \citet{qi2023lipsformer} replace standard dot-product attention part with \textbf{SCSA}, defined as:
\begin{align}
    \mathrm{SCSA}(x;v,\tau)=vPV, \qquad P = \mathrm{softmax}(\tau\,QK^\top),
\end{align}
where $K,Q,V$ are row-wise normalized in $\ell_2$ \citep[\S~4.1.2]{qi2023lipsformer}. 

\begin{remark}
It is worth noting that their method reduces the Lipschitz constant of the attention module; however, the module remains not globally Lipschitz continuous since the Lipschitz constant still depends on sequence length $n$:
\begin{align}
    \mathrm{Lip}_2\left[SCSA\right] \leq O(n), \qquad \text{and} \qquad \mathrm{Lip}_{\infty}\left[SCSA\right] \leq O(n^2)
\end{align}
\citep[Theorem 1]{qi2023lipsformer}.
\end{remark}


\paragraph{Weighted Residual Shortcut.} For a residual module:
\begin{align}
    h(x) = x + g(x)
    ,
\end{align}
where $g: \mathbb{R}^d \to \mathbb{R}^d$, $h: \mathbb{R}^d \to \mathbb{R}^d$ and $x \in \mathbb{R}^d$, the Lipschitz constant of $h$ is bounded by:
\begin{align}
    \mathrm{Lip}\left[h\right] \leq  1 + \mathrm{Lip}\left[g\right]
    ,
\end{align}
see Section~\ref{sec:lipschitz_of_residual_module} (\nameref{sec:lipschitz_of_residual_module}). To further reduce the Lipschitz constant introduced by residual module, \citet{qi2023lipsformer} replaces the standard residual module with:
\begin{align}
    \mathrm{WRS}(x) = x + \alpha \, \odot\, g(x)
    ,
\end{align}
where $\alpha$ is a learnable parameter, initialized to a small value $[0.1, 0.2]$ \citep{qi2023lipsformer}. \textbf{Note that the result:
\begin{align}
\mathrm{Lip}\left[\mathrm{WRS}\right] = 1 + \max(\alpha)    
\end{align}
in the \citet[\S~4.1.3]{qi2023lipsformer} is incorrect mathematically.} The Lipschitz constant of $\mathrm{WRS}$ in residual module should be bounded by:
\begin{align}
\mathrm{Lip}\left[\mathrm{WRS}\right] \leq 1 + \max(\alpha)
.
\end{align}


\paragraph{Spectral-based Weight Initialization.} \citet{qi2023lipsformer} further normalize the parameters at initialization by spectral-norm. Let $W$ be a parameter matrix, the $W$ is normalized by:
\begin{align}
    W \leftarrow \frac{W}{\|W\|_2}
\end{align}
\citep[\S~4.1.4]{qi2023lipsformer}.



\subsubsection{Jacobian Norm Minimization}


%https://arxiv.org/pdf/2507.07814

Constraining the Lipschitz constant of Transformer architecture for stable optimization and robustness remains an open research problem. \citet{yudin2025pay} first derive an explicit tight local Lipschitz constant for self-attention module in Transformer architecture by analyzing the Jacobian of softmax \citep{yudin2025pay}. Building on top of the Jacobian analsis, they present \textbf{JaSMin} (\textbf{Ja}cobian \textbf{S}oftmax norm \textbf{Min}imization) for enhancing Transformer's robustness by constraining the local Lipschitz constant \citep{yudin2025pay}.


\paragraph{Bounding Lipschitz through Softmax Jacobian.} Consider the softmax function:
\begin{align}
    \mathrm{softmax}: \mathbb{R}^d \to \mathbb{R}^d
    ,
\end{align}
then the Jacobian of the softmax function is:
\begin{align}
\mathcal{M}(P_x) := \nabla \, \mathrm{softmax}\left(x\right) = 
\mathrm{diag}(P_x) - P_x^\top P_x,
\end{align}
where:
\begin{align}
    P_x = \Biggl( \frac{\mathrm{e}^{x_i}}{\sum_j \mathrm{e}^{x_j}} \Biggr) 
    .
\end{align}
\citet{yudin2025pay} incorporate this Jacobian expression of the softmax function into self-attention, leading a Lipschitz constant bound for a single head:
\begin{align}
    \mathrm{Lip}\Bigl[\mathrm{Attention}\Bigr] 
    \leq
    \|W_V\|_2
    \Biggl(
    \|P\|_2 + 2 \|x\|_2^2 \; \|A\|_2 \; \max_i \|\mathcal{M}(P_{i, :})\|_2
    \Biggr)
\end{align}
with:
\begin{align}
    P = \mathrm{softmax}\Bigl(
    x
    A
    x^\top
    \Bigr) \in \mathbb{R}^{n \times n} \qquad \text{and} \qquad A = \frac{W_QW_K^\top}{\sqrt{d}} \in \mathbb{R}^{d \times d}
\end{align}
\citep[Theorem~3]{yudin2025pay}. It worthy noting that the local Lipschitz constant contains a term:
\begin{align}
 \mathrm{Lip}\Bigl[\mathrm{Attention}\Bigr] \leq
 O\Bigl(
 \max_i \|\mathcal{M}(P_{i, :})\|_2
 \Bigr)
 ,
\end{align}
which shows that softmax Jacobian norm determines an upper bound of the local Lipschitz constant.

\paragraph{Jacobian Softmax Norm Minimization.} To approximate the Jacobian norm more efficiently, \citet{yudin2025pay} introduce a surrogate function $g$ that captures the partial ordering of the singular values of softmax mappings. For $x \in \mathbb{R}_{>0}^n$, let $x_{(k)}$ be the $k$-th largest component of $x$. Define:
\begin{align}
    g_k(x) := x_{(k)}(1 - x_{(k)} + x_{(k+1)})
,
\end{align}
for $k=1,2,\cdots,n-1$ \citep[Definition 1]{yudin2025pay}. Let $A = \mathrm{diag}(x) - xx^\top$, then the following inequality holds true:
\begin{align}
    x_{(1)} \geq g_1(x) \geq \sigma_1(A)
    \geq
    x_{(2)} \geq g_2(x) \geq \sigma_2(A)
    \geq
    x_{(n)} \geq g_n(x) \geq \sigma_n(A)
    \geq 0
\end{align}
\citep[Theorem 4]{yudin2025pay}.

Building on the derived bound, \citet{yudin2025pay} propose an efficient regularization loss expressed in terms of the function $g$ with two forms:
\begin{align}
    \mathcal{L}_{\mathrm{JaSMin}(k=0)}
    = \sum_{\ell=1}^{L}
    \sum_{h_i=1}^{h}
    \max_j\log
    \Bigl[
    g_1\Bigl(
    P_{j,:}^{\ell, i}
    \Bigr)
    \Bigr]
    ,
\end{align}
and:
\begin{align}
    \mathcal{L}_{\mathrm{JaSMin}(k)}
    = \sum_{\ell=1}^{L}
    \sum_{h_i=1}^{h}
    \max_j\log
    \Biggl[
    \frac{
    g_1\Bigl(
    P_{j,:}^{\ell, i}
    \Bigr)
    }{
    g_k\Bigl(
    P_{j,:}^{\ell, i}
    \Bigr)
    }
    \Biggr]
    ,
\end{align}
where $P_{j,:}^{\ell, i}$ represents the softmax map for the $\ell$-th attention module ($1\leq \ell \leq L$), $i$-th head ($1 \leq i \leq h$), and the $j$-th row of the map \citep[\S~4]{yudin2025pay}. They also show that for $\sfrac{g_1}{g_k}$ is bounded below $\gamma$:
\begin{align}
    \frac{
    g_1\Bigl(P_{j,:}^{\ell,i}\Bigr)
    }{
    g_k\Bigl(P_{j,:}^{\ell,i}\Bigr)
    } \leq \gamma
,
\end{align}
for $1 \leq \gamma \leq \frac{k}{4}$. Then the softmax Jacobian $2$-norm is bounded by:
\begin{align}
   \| \mathcal{M}(P_{j,:}^{\ell,i}) \|_2 \leq
   O\Bigl(\frac{\gamma}{k}\Bigr)
\end{align}
\citep[Proposition 1]{yudin2025pay}.




\section{Certifiable Robustness}
\label{sec:certifiable_robustness}


Certifiable robustness, a cornerstone of trustworthy deep learning, guarantees that a neural network's predictions remain consistent under adversarial perturbations within a specified norm ball. Unlike empirical defenses like adversarial training, which lack formal guarantees, Lipschitz-based certification methods leverage the Lipschitz constant to bound sensitivity to input changes, ensuring provable robustness. While some literature, such as \citep{clevert2015elu}, have been introduced previously from the perspectives --- such as \textbf{theoretical foundations}, \textbf{estimation methods} and \textbf{regularization approaches}, we may revisit some of them in this section from the perspective of \textbf{certifiable robustness}.


%%
%% paper: CLEVER paper, section before 3
%% paper: Formal Guarantees on the Robustness of a Classifier against Adversarial Manipulation
%% paper: Lipschitz-Margin Training: Scalable Certification of Perturbation Invariance for Deep Neural Networks
%%

%\subsection{Lipschitz Margin Robustness Radius}
\subsection{Formal Robustness Guarantees}

% In the setting of a $n$-class classifier $f$ with Lipschitz constant $K_f$, for adversarial defense, we are interested in what is the largest perturbation norm that does not alter the prediction. 

In the setting of an $n$-class classifier $f$ with Lipschitz constant $K$, a central question in adversarial defense is to determining the largest perturbation norm that leaves the prediction unchanged.

\begin{theorem}[Lipschitz Margin Robustness Radius in $\ell_2$-Normed Spaces]
Let $f:\mathbb{R}^d\to\mathbb{R}^n$ be a classifier. Let $f_i$ be the $i$-th output. Let $c=\arg\max_i f_i(x)$ be the predicted class for $x$. Define the (one-versus-rest) margin
\begin{align}
m(x)\;:=\;f_c(x)-\max_{j\ne c} f_j(x).
\end{align}
Assume that $f$ is $K$-Lipschitz from the input $\ell_2$ norm to the output $\ell_2$ norm, \ie,
\begin{align}
\|f(x)-f(y)\|_2 \;\le\; K\,\|x-y\|_2 \quad \text{for all } x,y.
\end{align}

Then for any perturbation $\delta$ with
\begin{align}
\|\delta\|_2 \;<\; \frac{m(x)}{\sqrt{2}\,K},
\end{align}
the prediction is unchanged: 
\begin{align}
 \arg\max_i f_i(x+\delta)=c
 .
\end{align}
\end{theorem}

\begin{remark}
This result is particularly useful for analyzing the adversarial defense problem. Similar results have been discussed in the literature~\citep{szegedy2014intriguing,hein2017formal,cisse2017parseval,tsuzuku2018lipschitz,perugachi2021invertible}.
\end{remark}

\begin{proof}
Let $e_i \in \mathbb{R}^n$ denote the $i$-th standard basis vector, \ie, $e_i$ has a $1$ in the $i$-th position and $0$ elsewhere. Then
\begin{align}
    f_i(x) = e_i^\top f(x).
\end{align}

For each $j \ne c$, define the pairwise margin function:
\begin{align}
g_j(x) := f_c(x) - f_j(x) = (e_c - e_j)^\top f(x)
.
\end{align}

By H\"older's inequality,
\begin{align}
|g_j(x) - g_j(y)| 
&= |(e_c - e_j)^\top (f(x) - f(y))| \\
&\le \|e_c - e_j\|_2 \cdot \|f(x) - f(y)\|_2 \\
&\le \sqrt{2} \cdot K \cdot \|x - y\|_2,
\end{align}
so each $g_j$ is $\sqrt{2}K$-Lipschitz:
\begin{align}
    \mathrm{Lip}[g_j] = \sqrt{2}K.
\end{align}

Note that the margin $m(x)$ can be expressed as
\begin{align}
m(x) = f_c(x) - \max_{j \ne c} f_j(x) = \min_{j \ne c} g_j(x).
\end{align}

Now let $\delta \in \mathbb{R}^d$ be a perturbation satisfying
\begin{align}
\|\delta\|_2 < \frac{m(x)}{\sqrt{2}K}.
\end{align}

Then for all $j \ne c$,
\begin{align}
g_j(x + \delta) 
&\ge g_j(x) - \mathrm{Lip}[g_j] \cdot \|\delta\|_2 \\
&> m(x) - \sqrt{2}K \cdot \frac{m(x)}{\sqrt{2}K} = 0.
\end{align}

Hence, $f_c(x + \delta) > f_j(x + \delta)$ for all $j \ne c$, which implies
\begin{align}
\arg\max_i f_i(x + \delta) = c. 
\end{align}
\end{proof}


\begin{theorem}[Lipschitz Margin Robustness Radius in Conjugate-Normed Spaces]
Let $f: \mathbb{R}^d \to \mathbb{R}^n$ be a classifier with predicted class 
$c = \arg\max_i f_i(x)$ and one-versus-rest margin
\begin{align}
m(x) := f_c(x) - \max_{j \ne c} f_j(x).
\end{align}
Assume $f$ is $K$-Lipschitz from the input $\ell_p$ norm to the output $\ell_q$ norm:
\begin{align}
\|f(x) - f(y)\|_{q} \;\le\; K \, \|x - y\|_{p}.
\end{align}
Let $p$ be the dual exponent of $q$, \ie, $\tfrac{1}{q} + \tfrac{1}{p} = 1$.  
Then the classification of $x$ is certifiably robust to any perturbation $\delta$ with
\begin{align}
\|\delta\|_{p} \;<\; r_{\mathrm{cert}}(x) 
:= \frac{m(x)}{2^{\frac{1}{p}}\,K}
,
\end{align}
where $e_i \in \mathbb{R}^n$ denotes the $i$-th standard basis vector --- \eg, one-hot vector. 
\end{theorem}

\begin{remark}
Similar results have been discussed in the literature~\citep{hein2017formal,weng2018clever}. 
\end{remark}

\begin{proof}
Let $e_i \in \mathbb{R}^n$ denote the $i$-th standard basis vector, \ie, $e_i$ has a $1$ in the $i$-th position and $0$ elsewhere. Then
\begin{align}
    f_i(x) = e_i^\top f(x).
\end{align}

For each $j \ne c$, define the pairwise margin function:
\begin{align}
g_j(x) := f_c(x) - f_j(x) = (e_c - e_j)^\top f(x)
.
\end{align}

By H\"older's inequality and the Lipschitz property of $f$,
\begin{align}
|g_j(x) - g_j(y)| 
&\le \|e_c - e_j\|_{p} \, \|f(x) - f(y)\|_{q} \\
&\le K \, \|e_c - e_j\|_{p} \, \|x - y\|_{p}.
\end{align}

Thus the Lipschitz constant of $g_j$ is: 
\begin{align}
\mathrm{Lip}[g_j] \le K \, \|e_c - e_j\|_{p} .   
\end{align}
  
If:
\begin{align}
\|x' - x\|_{p} < 
\frac{g_j(x)}{\mathrm{Lip}[g_j]}
,  
\end{align}
for all $j \ne c$, then $g_j(x') > 0$ for all $j \ne c$, preserving the predicted class.  
Taking the minimum over $j$ yields
\begin{align}
r_{\mathrm{cert}}(x) 
= \min_{j \ne c} \frac{g_j(x)}{\mathrm{Lip}[g_j]} 
\ge \frac{m(x)}{K \, \max_{j \ne c} \|e_c - e_j\|_{p}}
=
\min_{j \ne c} \frac{g_j(x)}{\mathrm{Lip}[g_j]} 
\ge \frac{m(x)}{K \, 2^{\frac{1}{p}}}
.
\end{align}

\end{proof}

\begin{remark}
Note that:
\begin{align}
    \alpha = \max_{j \ne c} \|e_c - e_j\|_{p} = 2^{\frac{1}{p}}
    ,
\end{align}
common output norm choices yield:
\begin{align}
\text{$\ell_2$ output norm:} & \quad \alpha = \sqrt{2} 
& \Rightarrow && r_{\text{cert}} \ge \frac{m(x)}{\sqrt{2} \, K}, \\
\text{$\ell_\infty$ output norm:} & \quad \alpha = 1
& \Rightarrow && r_{\text{cert}} \ge \frac{m(x)}{K}, \\
\text{$\ell_1$ output norm:} & \quad \alpha = 2 
& \Rightarrow && r_{\text{cert}} \ge \frac{m(x)}{2K}.
\end{align}
Note that the number of classes $n$ affects the certified radius only through the margin $m(x)$; it does not appear explicitly in the bound.
\end{remark}


\subsection{Certifiable Robustness via Global Lipschitz Bound}

For a network $f$ with 1-Lipschitz activations and $W^{(\ell)}$ is the $\ell$-th layer parameter matrix, the spectral-norm product bounds the Lipschitz constant of $f$ globally:
\begin{align}
\mathrm{Lip}[f] \le \prod_{\ell=1}^L \|W^{(\ell)}\|_2,
\end{align}
providing a \emph{certified global bound}. This is computationally cheap but typically loose. \textbf{SeqLip} \citep{virmaux2018lipschitz} refines this spectral product by incorporating singular-vector alignment between layers, also producing certified global bounds. \textbf{LipSDP} \citep{fazlyab2019efficient} interprets activation functions as gradients of convex potential functions, satisfying certain properties described by quadratic constraints. Therefore, Lipschitz constant estimation problem is treated as a semi-definite program (SDP) problem. 

\subsection{Certifiable Robustness via Local Lipschitz Bound}

Local Lipschitz bounds are computed over a neighborhood. \textbf{Fast-Lip} \citep{weng2018fastlip} analyze the activation patterns of ReLU networks and derive a gradient norm based local Lipschitz bound. \textbf{CLEVER} \citep{weng2018clever} estimates local constants via extreme value theory on sampled gradient norms; this improves tightness but does not yield a formal certificate. MILP-based methods \citep{jordan2020exactly} encode the exact piecewise-linear constraints of ReLU networks within the ball, yielding exact local Lipschitz constants (and thus exact certified radii), but are limited to small networks.  



\subsection{Certifiable Robustness in Language Models}

%\paragraph{Bounded Levenshtein Distance \citep{rocamora2025certified}.}  

\paragraph{Proper Distance Metrics for Text.} Language models typically operate on text sequences as inputs, for which the conventional notion of a Lipschitz constant over $\mathbb{R}$ with $\ell_p$ norm does not directly apply. The \emph{Levenshtein distance} \citep{levenshtein1966binary} measures the number of character replacements, insertions or deletions needed in order to transform a sequence $x$ to sequence $y$. It is a proper metric that satisfies all axioms of a metric space:
\begin{enumerate}
    \item \textbf{Non-Negativity.} $d_{\mathrm{lev}}(x,y) \geq 0$;
    \item \textbf{Identity.} $d_{\mathrm{lev}}(x,y) = 0 \Longleftrightarrow x =y$;
    \item \textbf{Symmetry.} $d_{\mathrm{lev}}(x,y) = d_{\mathrm{lev}}(y,x)$;
    \item \textbf{Triangle Inequality.} $d_{\mathrm{lev}}(x,z) \leq d_{\mathrm{lev}}(x,y) + d_{\mathrm{lev}}(y,z)$;
\end{enumerate}
where $d_{\mathrm{lev}}(x,y)$ denotes the Levenshtein distance between two sequence $x$ and $y$. Thereby it provides a principled foundation for discussing Lipschitz continuity in the context of language models. For tokenized text --- where each vocabulary item is represented as a one-hot vector --- a variant of the \emph{Levenshtein distance}, known as the \emph{ERP distance}, has been proposed for comparing sequences of one-hot vectors \citep{chen2004editdistance}.

% The \emph{Levenshtein distance} $d_{\mathrm{Lev}}(x, x')$ between two token sequences $x$ and $x'$ is defined as the minimum number of insertions, deletions, and substitutions required to transform $x$ into $x'$.  
% In the context of robustness certification, a model $f$ is said to be \emph{$L_f$-Lipschitz with respect to $d_{\mathrm{Lev}}$} if
% \begin{align}
%     \| f(x) - f(x') \| \le L_f \, d_{\mathrm{Lev}}(x, x'),
% \end{align}
% for all $x, x'$. Enforcing $L_f \le 1$ ensures that the model output changes by at most the number of edits applied to the input.

% When inputs or intermediate representations are sequences of real-valued vectors (\eg, word embeddings), $d_{\mathrm{Lev}}$ cannot be directly applied. In this case, the \emph{edit distance with real penalty} (ERP), $d^p_{\mathrm{ERP}}(A,B)$, which extends $d_{\mathrm{Lev}}$ to $\mathbb{R}^d$-valued sequences and recovers $d_{\mathrm{Lev}}$ when $A$ and $B$ are one-hot sequences and $p = \infty$.

\citet{rocamora2025certified} introduce \textbf{LipsLev}, a method for training convolutional text classifiers that are \emph{1-Lipschitz} in the sense of Levenshtein distance for Lipschitz constant based defense \citep{rocamora2025certified}. That is, for a classifier $f: S \to \mathbb{R}^c$, two one-hot vector-valued sequences $x \in \mathbb{R}^{n \times d} \subset S $ and $x \in \mathbb{R}^{m \times d} \subset S$ where $n,m$ are sequence lengths and $d$ is one-hot vector dimension, the classification margin must hold:
\begin{align}
    | f_i(x) - f_j(y)| \leq K_{\mathrm{lev}} \; d_{\mathrm{lev}}(x, y)
\end{align}
for a constant $K_{\mathrm{lev}} > 1$, so that the prediction does not change under perturbation radius $d_{\mathrm{lev}}(x, y) < R$ \citep[Theorem 3.3]{rocamora2025certified}. They then train a 1-Lipschitz classifier over text sequences --- in the sense of the Levenshtein distance --- by normalizing each layer's outputs through division by its corresponding Lipschitz constant \citep[\S~3.3]{rocamora2025certified}.


% \section{Large Language Models (LLMs)}
% \label{sec:llms}


% LLMs have achieved remarkable success \citep{brown2020language, chowdhery2022palm, touvron2023llama, openai2024gpt4technicalreport, deepseekai2025deepseekr1}, yet the study of Lipschitz continuity in such models remains largely open. This section identifies and analyzes the most recent research developments concerning Lipschitz continuity in LLMs.


% \paragraph{Bounding Lipschitz in LLM Optimization.} 




\section{Conclusions}

Lipschitz continuity serves as a cornerstone for enhancing the robustness, generalization, and optimization stability of deep neural networks, providing a rigorous mathematical framework to quantify and control sensitivity to input perturbations. This comprehensive survey synthesizes key insights across theoretical foundations, estimation techniques, regularization approaches, and certifiable robustness, highlighting their interconnections and practical implications. By unifying disparate research threads, we address a critical gap in the literature, offering a cohesive resource for researchers and practitioners. Challenges remain in balancing bound tightness with computational scalability, preserving model expressivity under constraints, and extending certifications to diverse norms and large-scale architectures like transformers, paving the way for future advancements in trustworthy deep learning systems.




==> main_matter/chapters/LiteratureReview/tikz/lipschitz_surveytree.tex <==
% \forestset{parent color/.style args={#1}{
%     {fill=#1},
%     for tree={fill/.wrap pgfmath arg={#1!##1}{1/level()*80},draw=#1!80!darkgray}},
%     root color/.style args={#1}{fill={{#1!60!gray!25},draw=#1!80!darkgray}}
% }
\begin{forest}
  % Define styles for each node type
  root/.style={
    fill=white,
    draw,
    rounded corners=6pt,
    drop shadow,
    %blur shadow,
    %text width=30mm,
    minimum width=28ex,
    align=center,
    inner sep=5pt,
  },
  node/.style={
    fill=lime!20,
    draw,
    rounded corners=6pt,
    drop shadow,
    %text width=30mm,
    minimum width=28ex,
    align=center,
    inner sep=5pt,
  },
  leaf/.style={
    fill=white,
    draw=white,
    %text width=25mm,
    align=left,
    inner sep=2pt,
    anchor=west,
  },
  % Base settings for all nodes
  for tree={
    grow=east,
    % minimum width=28ex, %(\textwidth-6*1.5ex)/3.5,
    minimum height=4ex,
    edge path={
      \noexpand\path[\forestoption{edge},->, >={latex}] 
      (!u.parent anchor) -- +(5mm,0) |- (.child anchor)\forestoption{edge label};
    },
    parent anchor=east,
    child anchor=west,
    l sep=10mm,
    tier/.wrap pgfmath arg={tier #1}{level()},
    %edge={-Latex},
    edge={
      ultra thick,           % This will be overridden by line width
      rounded corners=2pt,
      teal!80,              % Set arrow color to green!80
      line width=1.5pt,      % Set arrow width to 1.5pt
    },
    %text centered,
    %fill=blue!80!darkgray!25,
    %blur shadow
  },
  % Tree structure with manually specified node types
  [Lipschitz Continuity, root, 
    [Challenges, node, fill=ForestGreen!80, 
      [Generative models, node, fill=ForestGreen!40]
      [LLMs, node, fill=ForestGreen!40]
      [Optimization instability, node, fill=ForestGreen!40]
    ]
    [Applications, node, fill=yellow!80
      [Interpretability, node, fill=yellow!40]
      [Ethics, node, fill=yellow!40
        [Fairness, node, fill=yellow!20]
        [Privacy, node, fill=yellow!20]
       ]
      [Domain adaptation, node, fill=yellow!40]
      [Adversarial robustness, node, fill=yellow!40]
      [Out-of-distribution (OOD), node, fill=yellow!40]
      [Distributional robustness, node, fill=yellow!40]
      [RL, node, fill=yellow!40]
      [LLM, node, fill=yellow!40]
      [Safety, node, fill=yellow!40
        [Certificated robustness, node, fill=yellow!20]
       ]
      [Generative models, node, fill=yellow!40
         [Diffusion models, node, fill=yellow!20]
         [GAN, node, fill=yellow!20]
       ]
    ]
    [Methods, node, fill=WildStrawberry!80
      [Explicit regularization, node, fill=WildStrawberry!40
        [Sepctral normalization, leaf]
        [Gradient penalty, leaf]
       ]
      [Implicit regularization, node, fill=WildStrawberry!40
        [Dropout, leaf]
        [Adversarial training, node, fill=WildStrawberry!10]
       ]
      [Architecture, node, fill=WildStrawberry!40
        [Bounding activations, node, fill=WildStrawberry!10]
        [Bounding layers, node, fill=WildStrawberry!10]
      ]
    ]
    [Theory, node, fill=lime!80
      [Generalization, node, fill=lime!40]
      [Complexity, node, fill=lime!40]
      [Smoothness, node, fill=lime!40]
      [RL, node, fill=lime!40]
      [Dynamics, node, fill=lime!40
        [Continuous-Time Lipschitz Dynamics \citep{luo2025lipschitz}, leaf]]
      [Frequency propagation, node, fill=lime!40]
      [Optimization, node, fill=lime!40
         [Convergence, node]
         [Stability, node]
       ]
      [PAC, node, fill=lime!40]
      [Generative models, node, fill=lime!40,
         [Diffusion models, node]
         [Flow matching, node]
       ]
       [Network, node, fill=lime!40,
         [xx, leaf]
       ]
       [Activation, node, fill=lime!40,
         [xx, leaf]
       ]
    ]
  ]
\end{forest}

==> main_matter/chapters/OptimizationInducedDynamics/tables/tab_gradient_generalization.tex <==
\begin{table*}[t!]

\centering

\caption{Effect of gradient regularizations}

\label{tab:gradient_regularization}

\resizebox{1\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\textbf{Regularization} & $\nabla^{(\ell)} L_f(\boldsymbol{\theta}(t); \xi)$ & $\Sigma_t^{(\ell)}$ & $\mu_Z(t)$ & $\lambda_Z(t)$ & $\kappa_Z(t)$ & $\mathbb{E}\left[K(t)\right]$ & $\mathrm{Var}\left[K(t)\right]$ \\
\hline
\hline

\textit{bath normalization} \citep{ioffe2015batch} %method
 & $\downarrow$  %\citep{santurkar2018does}  gradient mean
 & $\downarrow$ % \citep{bjorck2018understanding} gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{scaled dropout} \citep{srivastava2014dropout} %method
 & -   %gradient mean
 & $\downarrow$ %\citep{wager2013dropout,liu2023dropout}  gradient variance 
 & -  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & -  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline
 
\textit{weight decay} \citep{krogh1991simple} %method
& $\downarrow$  %\citep{krogh1991simple} gradient mean
 & $\downarrow$ %\citep{loshchilov2017decoupled} gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{mixup} \citep{zhang2017mixup} %method
& $\downarrow$  %gradient mean
 & $\downarrow$  % gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{auto-augment} \citep{cubuk2019autoaugment} %method
& $\downarrow$  % gradient mean
 & $\downarrow$  % gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{label smoothing} \citep{szegedy2016rethinking} %method
& $\downarrow$  %gradient mean
 & $\downarrow$  % gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline


 
\end{tabular}%
}
\end{table*}

% including \textit{batch normalization} \citep{ioffe2015batch,santurkar2018does,bjorck2018understanding}, \textit{dropout} \citep{srivastava2014dropout}, \textit{weight decay} \citep{krogh1991simple}, \textit{mixup} \citep{zhang2017mixup,zhang2020does,guo2019mixup}, \textit{auto-augment} \citep{cubuk2019autoaugment}, \textit{label smoothing} \citep{szegedy2016rethinking,muller2019does} and \textit{adversarial training} \citep{madry2018towards}, dampen gradient magnitudes during training. Consequently, the Lipschitz continuity bounds will be decreased.

==> main_matter/chapters/OptimizationInducedDynamics/tables/tab_gradient_noise.tex <==
\begin{table*}[t!]

\centering

\caption{Methods for modeling SGD gradient noise}

\label{tab:sgd_noise_models}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{>{\raggedright\arraybackslash}l|l|l}

\hline
\textbf{Type} & \textbf{Graident noise $\Sigma$} & \textbf{Citations}  \\
\hline
Isotropic scalar
 & $\Sigma=\sigma^2 I$ 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{welling2011bayesian}\\
 \cite{stephan2017stochastic}
 \end{tabular}
  \\
\hline
Diagonal 
 & \(\mathrm{diag}\bigl(\sigma_1^2(\theta),\dots,\sigma_K^2(\theta)\bigr)\) 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{jastrzkebski2018relation}\\
 \cite{simsekli2020fractional}
 \end{tabular}
  \\
\hline
Full structure
 & \(\mathrm{Cov}_\xi\bigl[\nabla \ell(\theta;\xi)\bigr]\in\mathbb{R}^{K\times K}\) 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{li2017stochastic}\\
 \cite{mandt2015continuous}\\
 \cite{zhu2018anisotropic}
 \end{tabular}
  \\
\hline
Structural Approx. 
 & \(U_r \Lambda_r U_r^\top\) or Kronecker/Block‐diag 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{zhu2018anisotropic}\\
 \cite{grosse2016kronecker}\\
 \cite{malladi2022sdes}\\
 \cite{simsekli2019tail}
 \end{tabular}
  \\
\hline
\end{tabular}%
}
\end{table*}

==> main_matter/chapters/OptimizationInducedDynamics/text.tex <==
\section{Introduction}


%Introduction to robustness and Lipschitz continuity.

\lettrine[lines=3]{R}{ecent} advancements in deep learning have led to models that excel across a broad range of domains, from vision to language. Their vulnerability to input perturbations remains a significant challenge for establishing trustworthy learning systems \citep{szegedy2014intriguing,goodfellow2014explaining,madry2018towards}. Lipschitz continuity (Definition~\ref{def:lipschitz_definition}) measures the worst-case sensitivity of the output of a network to small input perturbations. Furthermore, several fundamental properties, including robustness to perturbation \citep{luo2024interpreting} and generalization capability, are closely linked to network Lipschitz continuity \citep{shalev2014understanding,bartlett2017spectrally,yin2019rademacher,zhang2021understanding}. Networks with lower Lipschitz constants tend to be more resilient to input perturbations (\eg~adversarial perturbations) and exhibit improved generalization capabilities \citep{zhang2022rethinking,fazlyab2023certified,khromov2024some}. 


\begin{definition}[Globally $K$-Lipschitz Continuous \citep{yosida2012functional}]
\label{def:lipschitz_definition}
Let $f: X \mapsto Y$ be a function, where $X \subseteq \mathbb{R}^d$ and $Y \subseteq \mathbb{R}^c$. The function $f$ is said to be \emph{globally $K$-Lipschitz continuous} if there exists a constant $K > 0$ such that:
\begin{equation}
    \|f(u) - f(v)\|_2 \leq K \|u - v\|_2, \quad \forall\, u, v \in X
\end{equation}
upper-bounds the function $f$.
\end{definition}


\begin{figure}[!t]
  
  
  \centering
  
  \input{optimization_induced_dynamics_subfig}
  
  \caption[Optimization-Induced Stochastic Dynamics of Lipschitz Continuity]{\textbf{Optimization-induced dynamics}. During the training, the network parameters, starting from $\boldsymbol{\theta}_0$, moves towards a solution $\boldsymbol{\theta}_A$ or $\boldsymbol{\theta}_B$ as shown in the loss landscape~\protect\subref{subfig:loss_landscape}, driven by optimization process. Accordingly, this dynamics, driven by the optimization, induces the evolution of the network Lipschitz continuity, starting from $K_0$ to $K_A$ or $K_B$, as shown in the Lipschitz landscape~\subref{subfig:lipschitz_landscape}. The trajectories in the loss landscape~\subref{subfig:loss_landscape} and the Lipschitz landscape~\subref{subfig:lipschitz_landscape} are visualized on the same parameter space $\alpha O \beta$. The $\alpha$ and $\beta$ are two randomly-chosen orthogonal directions in the parameter space. }

  \label{fig:lipschitz_and_loss_landscape}

\end{figure}







%relationship beween gradient-based optimization and Lipschitz continuity.
Gradient-based optimization methods, such as stochastic gradient descent (SGD) and its variants \citep{robbins1951stochastic,hinton2012neural,diederik2014adam}, are fundamental to training deep learning models by iteratively minimizing the loss function through parameter updates with gradients. The optimization dynamics in a neural network induce the corresponding dynamics of its Lipschitz continuity, which we refer to as \textbf{optimization‐induced dynamics}. As illustrated in Figure~\ref{fig:lipschitz_and_loss_landscape}, every optimization trajectory in the loss landscape induces a corresponding trajectory in the Lipschitz landscape. Although the dynamics (\ie~temporal evolution) of SGD has been extensively explored in the literature, including topics such as: (i) continuous‐time/SDE modeling \citep{li2019stochastic,malladi2022sdes,welling2011bayesian,zhu2018anisotropic}; (ii) edge-of-stability and implicit bias \citep{li2021happens,damian2022self}; (iii) convergence analysis \citep{li2017convergence}; (iv) sharp versus flat minima and generalization \citep{keskar2016large,chaudhari2019entropy,zhang2021understanding}, a comprehensive understanding of how the Lipschitz constant evolves over time during training remains lacking. 





 %original
% \begin{figure*}[!t]
%   \centering

%   \begin{minipage}[t]{1\textwidth}
%      \centering 
%      \subfloat[Numerical validation on CIFAR-10]{
%       \includegraphics[width=1\linewidth]{theoretical_versus_observed_lipschitz_cifar10.pdf}  
%       \label{fig:validation:cifar10}
%      }
%   \end{minipage}
  
%   \begin{minipage}[t]{1\textwidth}
%      \centering 
%      \subfloat[Numerical validation on CIFAR-100]{
%       \includegraphics[width=1\linewidth]{theoretical_versus_observed_lipschitz_cifar100.pdf}  
%       \label{fig:validation:cifar100}
%      }
%   \end{minipage}

%   % plot_epochs:  200
%   % plot_steps:  30000
%   \caption[Numerical Validation of Our Mathematical Framework in Characterizing Optimization-Induced Stochastic Dynamics of Lipschitz Continuity]{\textbf{Numerical validation of our mathematical framework}. The theoretical Lipschitz constants computed using our framework closely agree with empirical observations. To validate our framework, we train a five-layer ConvNet on CIFAR-10 and CIFAR-100 across multiple configurations for $30,000$ steps ($200$ epochs). We collect the instance-wise gradients over time for all layers. Using Theorem~\ref{theorem:layer_dynamics}, Theorem~\ref{theorem:network_dynamics}, Theorem~\ref{theorem:integral_form_network_dynamics} and Theorem~\ref{theorem:statistics_of_lipschitz}, we are able to theoretically compute the predicted Lipschitz continuity. The inset plots zoom in on the first $50$ steps, and demonstrate that \textbf{the trends of Lipschitz constants do not necessarily grow monotonically}. Results with more regularization configurations on CIFAR-10 are provided in Appendix~\ref{sec:full_validation_cifar10}.
%   }
  
%   \label{fig:validation}

%   %\vspace{-1em}
% \end{figure*}


%Padhraic wishes that the figure larger
\begin{sidewaysfigure}
  \centering

  \begin{minipage}[t]{1\textwidth}
     \centering 
     \subfloat[Numerical validation on CIFAR-10]{
      \includegraphics[width=1\linewidth]{theoretical_versus_observed_lipschitz_cifar10.pdf}  
      \label{fig:validation:cifar10}
     }
  \end{minipage}
  
  \begin{minipage}[t]{1\textwidth}
     \centering 
     \subfloat[Numerical validation on CIFAR-100]{
      \includegraphics[width=1\linewidth]{theoretical_versus_observed_lipschitz_cifar100.pdf}  
      \label{fig:validation:cifar100}
     }
  \end{minipage}

  % plot_epochs:  200
  % plot_steps:  30000
  \caption[Numerical Validation of Our Mathematical Framework in Characterizing Optimization-Induced Stochastic Dynamics of Lipschitz Continuity]{\textbf{Numerical validation of our mathematical framework}. The theoretical Lipschitz constants computed using our framework closely agree with empirical observations. To validate our framework, we train a five-layer ConvNet on CIFAR-10 and CIFAR-100 across multiple configurations for $30,000$ steps ($200$ epochs). We collect the instance-wise gradients over time for all layers. Using Theorem~\ref{theorem:layer_dynamics}, Theorem~\ref{theorem:network_dynamics}, Theorem~\ref{theorem:integral_form_network_dynamics} and Theorem~\ref{theorem:statistics_of_lipschitz}, we are able to theoretically compute the predicted Lipschitz continuity. The inset plots zoom in on the first $50$ steps, and demonstrate that \textbf{the trends of Lipschitz constants do not necessarily grow monotonically}. Results with more regularization configurations on CIFAR-10 are provided in Appendix~\ref{sec:full_validation_cifar10}.
  }
  
  \label{fig:validation}

  %\vspace{-1em}
\end{sidewaysfigure}

This gap motivates us to establish a rigorous theoretical framework for modeling the dynamics of Lipschitz continuity, induced by optimization dynamics. Equipped with the toolkit from stochastic differential equations (SDEs) \citep{applebaum2009levy,karatzas2012brownian,oksendal2013stochastic} and operator perturbation theory \citep{kato1995perturbation,luo2025spectralvariation}, we can rigorously analyze the evolution of the matrix operator norm (\ie~matrix Lipschitz constant), induced by the optimization process, within an SDE framework. Our framework can capture both the deterministic and stochastic forces driving the temporal evolution of Lipschitz constants. The effectiveness of our mathematical framework is empirically verified in Figure~\ref{fig:validation}, where the theoretical implications derived using our framework (Theorem~\ref{theorem:integral_form_network_dynamics} and Theorem~\ref{theorem:statistics_of_lipschitz}) are closely aligned with the observations. Furthermore, our theoretical framework sheds light on questions such as how batch size, parameter initialization, mini‐batch sampling trajectories, label noise, \etc., shape the Lipschitz continuity evolution during optimization.





\subsection{Contributions}
\label{sec:contributions}

We highlight the key contributions below:
\begin{enumerate}
    %\setlength{\itemsep}{0pt}
    %\setlength{\parskip}{6pt}
    
    \item \textbf{Theoretical Framework} (Section~\ref{sec:preliminaries}-\ref{sec:theoretical_analysis}). We present a rigorous mathematical framework that models the dynamics of Lipschitz continuity, leveraging an SDE system driven by Wiener processes. This SDE-based framework captures both deterministic and stochastic forces, providing a comprehensive understanding of the dynamics of Lipschitz continuity. To ensure practical applicability, we also develop a low-rank approximation method for modeling gradient noise in Section~\ref{sec:gradient_noise}, enabling efficient computation of these dynamics. 

    \item \textbf{Principal Driving Forces} (Section~\ref{sec:layer_dyanmics}-\ref{sec:statistics}). Our theoretical analysis (Theorem~\ref{theorem:integral_form_network_dynamics}) identifies three principal forces governing the dynamics: (i) the projection of gradient flows, induced by the optimization dynamics, onto the operator-norm Jacobian of parameter matrices; (ii) the projection of gradient noise, arising from the randomness in mini-batch sampling, onto the operator-norm Jacobian; and (iii) the projection of the gradient noise onto the operator-norm Hessian of parameter matrices. In the evolution of Lipschitz continuity, forces (i) and (iii) act as deterministic forces, while force (ii) modulates the stochasticity of the dynamics.
     

    \item \textbf{Framework Validation and Theoretical Implications} (Section~\ref{sec:validation}-\ref{sec:theoretical_implications}). Firstly, we validate our theoretical framework under multiple configurations, including \textit{batch normalization}, \textit{dropout}, \textit{weight decay}, \textit{mixup}, \textit{auto-augment}, \textit{label smoothing} and \textit{adversarial training}. Furthermore, we test the theoretical implications derived from our framework, as detailed in Section~\ref{sec:theoretical_implications}, including parameter initialization, noisy gradient regularization, uniform label corruption, batch size, and mini-batch sampling trajectories shape the evolution of Lipschitz continuity. The results show a strong agreement between the theoretical implications and observed behaviors.
    

\end{enumerate}















\section{Preliminaries}
\label{sec:preliminaries}

%Its $n$-th order derivative is denoted by $D^n f$, following the \textit{denominator layout convention} \citep{magnus2019matrix}. 
We define the notation used in our theoretical analysis. Let $f: \mathbb{R}^d \to \mathbb{R}^c$ be a function. For a time-dependent function $g$, we use $g_k$ to denote its value at discrete time step $k$, and $g(t)$ for its value at continuous time $t$. For a random variable $\xi$, \eg, representing data sampling, gradient noise, Wiener process, and filtration \citep{oksendal2013stochastic}, we consistently use subscripts, such as $\xi_k$ or $\xi_t$, for brevity. A function written as $g^{(\ell)}$ indicates that $g$ is the $\ell$-th layer of a neural network. We use $\mathrm{I}_n$ to denote an $n \times n$ identity matrix; $\mathbb{1}_n$ to denote an $n$-dimensional all-ones vector.

%ICMLR reviewer neEG suggested us to revise the notations: k->t
\medskip
\noindent
\textbf{Mini-Batch Sampling}. Let $\mathcal{D} := \{(x_i, y_i)\}_{i=1}^{N} \subseteq \mathcal{X} \times \mathcal{Y}$ denote a dataset consisting of $N$ samples, where $(x_i, y_i)$ represents the $i$-th data point and its corresponding target. Let $\xi_t := \{(x_{t_j}, y_{t_j})\}_{j=1}^{M} \subset \mathcal{X} \times \mathcal{Y}$ denote a mini-batch sampled from $\mathcal{D}$ at time point $t$, where $M$ ($M \ll N$) is the size of the mini-batch. The sequence $\{\xi_i\}_{i=0}^t$ up to time $t$ is referred to as a \textit{sampling trajectory} from $D$. The $\sigma$-algebra $\mathcal{F}_t = \sigma\bigl\{\xi_0,\xi_1,\dots,\xi_t\bigr\}$, defined on mini-batch sampling, is referred to as the \textit{filtration} generated by the sampling trajectory $\{\xi_i\}_{i=0}^t$ \citep{oksendal2013stochastic}. In stochastic analysis, $\mathcal{F}_t$ represents that the information accumulates up to time $t$ (\ie~history). Any history up to a time point $t_k$ contains the history up to a time point $t_l$ for all $t_k \geq t_l$, \ie~$\mathcal{F}_{t_l} \subseteq \mathcal{F}_{t_k}$. 



\medskip
\noindent
\textbf{Feed-Forward Network}. Let $\boldsymbol{\theta}^{(\ell)} \in \mathbb{R}^{m_{\ell} \times n_{\ell}}$ denote the parameter matrix of the $\ell$-th layer of an $L$-layer feed-forward network. Let $\boldsymbol{\theta} := \{ \boldsymbol{\theta}^{(1)}, \boldsymbol{\theta}^{(2)}, \dots, \boldsymbol{\theta}^{(L)} \} \in \Theta$ denote the collection of all $L$ parameter matrices. Let $f_{\boldsymbol{\theta}}: \mathbb{R}^d \mapsto \mathbb{R}^c$ represent a feed-forward network parameterized by $\boldsymbol{\theta}$. Let $\mathrm{vec}(\boldsymbol{\theta}^{(\ell)}) \in \mathbb{R}^{m_{\ell} n_{\ell}}$ denote the vectorized $\boldsymbol{\theta}^{(\ell)}$ with \textit{column-major convention} \citep{horn2012matrix}. 


\begin{remark}
The explicit use of the $\mathrm{vec}(\cdot)$ operator is essential for rigorous spectral analysis of parameter matrices beyond the usual context of parameter updates in SGD optimization.
\end{remark}


\medskip
\noindent
\textbf{Instance and Population Loss}. Let $\ell_f(\boldsymbol{\theta}; x, y): \Theta \times \mathcal{X} \times \mathcal{Y} \mapsto \mathbb{R}$ denote the instance loss for $f_{\boldsymbol{\theta}}$. Let $\mathcal{L}_f(\boldsymbol{\theta}; \xi)$ denote the population loss over a mini-batch $\xi$:
\begin{align}
    \mathcal{L}_f(\boldsymbol{\theta}; \xi) := \frac{1}{M} \sum_{x_{i}, y_{i} \in \xi} \ell_f(\boldsymbol{\theta}; x_{i}, y_{i}) \notag
    .
\end{align}
Let $\mathcal{L}_f(\boldsymbol{\theta})$ denote the population loss over the dataset $\mathcal{D}$:
\begin{align}
    \mathcal{L}_f(\boldsymbol{\theta}) := \mathbb{E}_{(x_i, y_i) \sim \mathcal{D}} \left[ \ell_f(\boldsymbol{\theta}; x_i, y_i) \right] \notag
    .
\end{align}    



\medskip
\noindent
\textbf{Unbiased Gradient Estimator}. For brevity, we use:
\begin{align}
\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}):=\nabla_{\boldsymbol{\theta}^{(\ell)}} \mathcal{L}_f(\boldsymbol{\theta})   , \quad \text{and} \quad 
\nabla \mathcal{L}_f(\boldsymbol{\theta}) := \nabla_{\boldsymbol{\theta}} \mathcal{L}_f(\boldsymbol{\theta}) \notag
, 
\end{align}
to denote the gradient with respect to the $\ell$-th layer parameter matrix, and the gradient with respect to the collective parameter matrices, respectively. Note that $\nabla \mathcal{L}_f(\boldsymbol{\theta}; \xi)$ is an unbiased gradient estimator for $\nabla \mathcal{L}_f(\boldsymbol{\theta})$:
\begin{align}
    \mathbb{E} \left[ \nabla L_t(\boldsymbol{\theta}; \xi) \right] = \mathbb{E} \left[ \nabla \mathcal{L}_f(\boldsymbol{\theta}) \right] = \mathbb{E} \left[ \nabla \ell_f(\boldsymbol{\theta}; x, y) \right] \notag
    .
\end{align}





\section{Vectorized SDE for Continuous-Time SGD}

SGD and its variants (\eg~Adam) \citep{robbins1951stochastic,hinton2012neural,diederik2014adam} serve as cornerstone optimization algorithms widely used for training deep neural networks. Formally, at a time point $k$, the SGD-based update regarding the parameter $\boldsymbol{\theta}_{k}^{(\ell)}$ with a mini-batch $\xi_k$ can be formulated by:
\begin{align}
    \label{equ:sgd}
    \boldsymbol{\theta}_{k+1}^{(\ell)} = \boldsymbol{\theta}_{k}^{(\ell)} - \eta \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_k; \xi_k) 
    ,
\end{align}
where $\eta$ is the learning rate. Some studies \citep{mandt2015continuous,su2016differential,stephan2017stochastic} view SGD as a deterministic process with a deterministic ordinary differential equation (ODE) as:
\begin{align}
    \frac{\dd \boldsymbol{\theta}^{(\ell)}(t)}{\dd t} = - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t)) \notag
    ,
\end{align}
where $t \approx k\eta$ and $\dd t \approx \eta \to 0$. 



However, the inherent stochasticity in the population gradients $\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_k; \xi_k)$, arising from the randomness in mini-batch sampling $\xi_k$, is not accounted for by ODE methods. The \textit{layer-wise batch gradient noise} (\ie~batch gradient fluctuations) \citep{welling2011bayesian, keskar2016large, chaudhari2019entropy,zhang2021understanding}, defined as a positive semi-definite (PSD) matrix:
\begin{align}
\label{equ:batch_gradient_noise}
 \boldsymbol{\Sigma}_k^{(\ell)} := \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_k; \xi_k) \right)\right]  = \frac{1}{M} \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y) \right)\right] 
 \in \mathbb{R}^{m_{\ell}n_{\ell} \times m_{\ell}n_{\ell}}
 ,
\end{align}
induced by mini-batch sampling, can influence the optimization trajectory. \textbf{It remains under-explored in the literature how such stochasticity affects the evolution of Lipschitz continuity of neural networks over time}.  

\begin{assumption}[Collective Gradient Noise Structure Assumption]
\label{assump:layerwise_noise}
For tractability, we assume that gradient‐noise covariances between different layers are negligible. Equivalently, $\Sigma_t$ has block‐diagonal structure:
\begin{align}
   \boldsymbol{\Sigma}_t = 
   \mathrm{diag}(\boldsymbol{\Sigma}_t^{(1)}, \boldsymbol{\Sigma}_t^{(2)}, \cdots, \boldsymbol{\Sigma}_t^{(L)})  \notag
   ,
\end{align}
so that we model batch gradient noise on a per‐layer basis only. This layer‐wise approximation is common in large‐scale SDE analyses, \eg~\citep{grosse2016kronecker,malladi2022sdes,simsekli2019tail}.
\end{assumption}

To address the limitations of ODE methods, SDE methods \citep{li2017convergence,zhu2018anisotropic,chaudhari2019entropy} extend ODE methods by accounting for gradient noise. SDE-based methods capture the stochasticity inherent in mini-batch updates and its effects on the optimization trajectory. The multivariate Central Limit Theorem (CLT) states that the population gradient estimator:
\begin{align}
 \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_k; \xi_k) = \frac{1}{M} \sum_{(x_i, y_i) \in \xi_k} \nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x_i, y_i) \notag
 ,
\end{align}
distributionally converges to a normal distribution in $\mathbb{R}^{m_{\ell}n_{\ell}}$:
\begin{align}
\mathrm{vec}\left(\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_k; \xi_k)\right)  \xrightarrow{\text{d}}  \mathcal{N}\left(\mathrm{vec}(\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_k)), \boldsymbol{\Sigma}_k^{(\ell)}\right) \notag
,
\end{align}
as $M \to \infty$, where the samples $(x_i, y_i)$ are \emph{i.i.d}. Therefore, SGD can be modeled as an It\^o process, which provides a more accurate representation of the dynamics by considering the continuous-time SDEs \citep{mandt2015continuous, stephan2017stochastic}.




\begin{definition}[Vectorized SDE for Continuous-Time SGD]
Under Assumption~\ref{assump:layerwise_noise}, and the assumption that $\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_t)$ and $\boldsymbol{\Sigma}_t^{(\ell)}$ satisfy global Lipschitz and linear‐growth conditions \citep{oksendal2013stochastic,karatzas2012brownian}, the SGD update for the parameter $\boldsymbol{\theta}_t^{(\ell)}$ with a mini-batch $\xi_t$ at time $t$ can be formulated as a matrix-valued It\^o's SDE by:
\begin{align}
\label{equ:ct_sgd}
\dd  \mathrm{vec}  \left(\boldsymbol{\theta}^{(\ell)}(t)\right) &= -\mathrm{vec} \left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right] \dd t + \sqrt{\eta}\left[\boldsymbol{\Sigma}_t^{(\ell)} \right]^{\frac{1}{2}}\dd \boldsymbol{B}_t^{(\ell)}
,
\end{align}
where the batch gradient noise $\left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\sfrac{1}{2}} \in \mathbb{R}^{m_{\ell}n_{\ell} \times m_{\ell}n_{\ell}}$ satisfies:
\begin{align}
   \left(\boldsymbol{\Sigma}_t^{(\ell)}\right)^{\frac{1}{2}}
   \left[\left(\boldsymbol{\Sigma}_t^{(\ell)}\right)^{\frac{1}{2}}\right]^\top
    = \boldsymbol{\Sigma}_t^{(\ell)},
    \quad \text{and} \quad 
    \mathbb{R}^{m_{\ell}n_{\ell}} \ni \dd \boldsymbol{B}_t^{(\ell)} \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{\mathrm{I}}_{m_{\ell}n_{\ell}} \dd t) \notag
\end{align}
represents the infinitesimal increment of a Wiener process (standard Brownian motion) adapted to the filtration $\mathcal{F}_t$ in $\mathbb{R}^{m_{\ell}n_{\ell}}$. 

\label{def:ct_sgd}
\end{definition}









 
\section{Estimating batch gradient noise}
\label{sec:gradient_noise}




The covariance of gradient noise structure reflects how neurons interact with each other. Capturing the full structure of gradient noise for numerically analyzing the spectra of network parameters \citep{StewartSun1990,horn2012matrix,kato1995perturbation} is shaped by the stochasticity arising from mini batch sampling. However, modeling the full gradient noise covariance is computationally prohibitive: accurately estimating batch gradient noise requires sampling all gradient trajectories over the entire dataset, which leads to intractable storage and computational costs \citep{mandt2015continuous,li2019stochastic}. 


SDE-based models often have strong assumptions regarding the structure of gradient noise. For example, in the literature \citep{welling2011bayesian,stephan2017stochastic}, the gradient noise is reduced into a constant scalar. Under this assumption, the SDE reduces to an Ornstein-Uhlenbeck process \citep{oksendal2013stochastic,karatzas2012brownian}. However, this simplification overlooks the covariance structures inherent in mini-batch sampling. To address this, some literature assume a diagonal structure for the gradient noise \citep{jastrzkebski2018relation,simsekli2020fractional}. While this approximation captures varying variances across parameters, it neglects potential correlations between them. 



    

In practice, \citeauthor{mandt2015continuous} compute the exact $2\times2$ covariance matrix for a low‐dimensional logistic‐regression problem;  \citeauthor{zhu2018anisotropic} estimate the full noise covariance --- solely to extract its leading eigenpairs --- in an MLP with several hundred parameters \citep{zhu2018anisotropic}. Nonetheless, these methods do not scale to modern deep networks, where the number of parameters can be on the order of millions. In the remaining part of this section, we aim to develop experiment-friendly method for tracking full structure of gradient noise.




\subsection{Unbiased batch gradient noise estimator}

To capture the complex interactions among neurons, we model the complete structure of the gradient noise. However, by Equation~\ref{equ:batch_gradient_noise}, the exact $\boldsymbol{\Sigma}_t^{(\ell)}$ is given by at time point $t$:
\begin{align}
 \boldsymbol{\Sigma}_t^{(\ell)} &:= \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}_t; \xi_t) \right)\right] \\  
 &= \frac{1}{M} \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y)\right)\right]  \\
 &= \frac{1}{M} \mathbb{E}\Biggl[
 \Bigl\{ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y)\right) - 
 \mathbb{E}\Bigl[
 \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y)\right)
 \Bigr]
 \Bigr\}
 \Biggr. \notag \\
 &\qquad\qquad \Bigl\{ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y)\right) - 
 \mathbb{E}\Bigl[
 \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y)\right)
 \Bigr]
 \Bigr\}^\top
 \Biggl.
 \Biggr]
 ,
\end{align}
which suggests that the $\boldsymbol{\Sigma}_t^{(\ell)}$ requires the evaluation of
\begin{align}
  \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y)\right) \qquad \text{and}  \qquad \mathbb{E}\Bigl[
 \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}_k; x, y)\right)
 \Bigr]
\end{align}
over the entire dataset for each time point $t$. Therefore, the computational cost of $\boldsymbol{\Sigma}_t^{(\ell)}$ poses a challenge to the applicability of our framework. This computation remains highly demanding, even when using state-of-the-art GPUs. To overcome this, we develop a low-rank approximation method. We now seek to estimate $\boldsymbol{\Sigma}_t^{(\ell)}$ without bias. 

% To capture the complex interactions among neurons, we model the complete structure of the gradient noise. However, the computational cost of $\boldsymbol{\Sigma}_t^{(\ell)}$, which requires the evaluation on the entire dataset $\mathcal{D}$ for each $t$, poses a challenge to the applicability of our framework. This computation remains highly demanding, even when using state-of-the-art GPUs. To overcome this, we develop a low-rank approximation method. We now seek to estimate $\boldsymbol{\Sigma}_t^{(\ell)}$ without bias. 

\begin{proposition}[Unbiased Batch Gradient Noise Estimator]
\label{prop:unbiased_batch_gradient_noise_estimator}
Starting from Equation~\ref{equ:batch_gradient_noise}, the batch gradient noise at time $t$ is approximately estimated from a batch $\xi_t$ by:
\begin{align}
\label{equ:unbiased_batch_gradient_noise_estimator}
\boldsymbol{\Sigma}_t^{(\ell)} 
%&=\frac{1}{M} \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x, y) \right)\right] \notag\\ 
% &=\frac{1}{M}\mathbb{E}\left[
% \left\{ \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x, y)  - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right]\right\}\right.\notag\\
% &\left.\qquad\qquad
% \left\{ \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x, y)  - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right]\right\}^\top
% \right] \notag\\
&\approx \frac{1}{M} \left[\frac{1}{M-1} 
\sum_{x_{t_i},y_{t_i} \in \xi_t}
\underbrace{
\left\{ \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x_{t_i}, y_{t_i})  - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t);\xi_t)\right]\right\}
}_{(\boldsymbol{\Omega}_{t_i}^{(\ell)})^\top}
\right.\notag\\
&\left.\qquad\qquad\qquad\qquad\qquad
\underbrace{
\left\{ \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x_{t_i}, y_{t_i})  - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t);\xi_t)\right]\right\}^\top
}_{\boldsymbol{\Omega}_{t_i}^{(\ell)}}
\right] \notag\\
&=\frac{1}{M}
\left(
\frac{1}{\sqrt{M-1}}
\begin{bmatrix}
    \boldsymbol{\Omega}_{t_1}^{(\ell)} \\
    \boldsymbol{\Omega}_{t_2}^{(\ell)} \\
    \vdots\\
    \boldsymbol{\Omega}_{t_M}^{(\ell)}
\end{bmatrix}
\right)^\top
\left(
\frac{1}{\sqrt{M-1}}
\begin{bmatrix}
    \boldsymbol{\Omega}_{t_1}^{(\ell)}\\
    \boldsymbol{\Omega}_{t_2}^{(\ell)}\\
    \vdots\\
    \boldsymbol{\Omega}_{t_M}^{(\ell)}
\end{bmatrix}
\right)=\frac{1}{M} (\boldsymbol{\Omega}_t^{(\ell)})^\top \boldsymbol{\Omega}_t^{(\ell)}
,
\end{align}
where $\boldsymbol{\Omega}_{t_i}^{(\ell)}$ is the point-wise gradient fluctuation:
\begin{align}
(\boldsymbol{\Omega}_{t_i}^{(\ell)})^\top = \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x_{t_i}, y_{t_i})  - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t);\xi_t)\right]    \in \mathbb{R}^{m_{\ell}n_{\ell}} \notag
,
\end{align}
and $\boldsymbol{\Omega}_t^{(\ell)}$ is batch-wise gradient fluctuation:
\begin{align} 
\boldsymbol{\Omega}_t^{(\ell)} &=
\frac{1}{\sqrt{M-1}}
\begin{bmatrix}
    \boldsymbol{\Omega}_{t_1}^{(\ell)}\\
    \boldsymbol{\Omega}_{t_2}^{(\ell)}\\
    \vdots\\
    \boldsymbol{\Omega}_{t_M}^{(\ell)}
\end{bmatrix}
=
\sqrt{\frac{1}{M-1}}
    \begin{pmatrix}
    \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x_{t_1}, y_{t_1}) - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t);\xi_t)\right]^\top \\
    \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x_{t_2}, y_{t_2}) - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t);\xi_t)\right]^\top \\
    \vdots \\
    \mathrm{vec}\left[\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x_{t_M}, y_{t_M}) - \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t);\xi_t)\right]^\top
    \end{pmatrix} \notag
    .
\end{align}

\end{proposition}

\subsection{Estimating variance and covariance}

To study the contributions of variances (diagonal elements) and covariances (off-diagonal elements) of gradient noise to the dynamics, we decompose the gradient noise into variance and covariance components using Proposition~\ref{prop:variance_and_covariance_of_gradient_noise}.

\begin{proposition}[Diagonal and Off-Diagonal Elements of Batch Gradient Noise]
\label{prop:variance_and_covariance_of_gradient_noise}
The diagonal variance $\boldsymbol{\Sigma}_{t}^{(\ell)}\mid_{\mathrm{var}}$ and the off-diagonal covariance $\boldsymbol{\Sigma}_{t}^{(\ell)}\mid_{\mathrm{cov}}$ are computed, respectively, by:
\begin{align}
     \boldsymbol{\Sigma}_{t}^{(\ell)}\mid_{\mathrm{var}} \approx \frac{1}{M}\left(\boldsymbol{\Omega}_t^{(\ell)} \odot \boldsymbol{\Omega}_t^{(\ell)}\right)^\top \boldsymbol{\mathbb{1}}_{M} 
     ,
     \quad 
     \text{and}
     \quad
      \boldsymbol{\Sigma}_{t}^{(\ell)}\mid_{\mathrm{cov}} \approx \boldsymbol{\Sigma}_t^{(\ell)} - \boldsymbol{\Sigma}_{t}^{(\ell)}\mid_{\mathrm{var}} \notag
      ,
\end{align}
where $\odot$ denotes Hadamard product. Note that $\boldsymbol{\Sigma}_{t}^{(\ell)}\mid_{\mathrm{cov}}$ is not necessarily a PSD matrix. 
\end{proposition}


\begin{proof}
Starting from Equation~\ref{equ:unbiased_batch_gradient_noise_estimator}, this can be obtained by:
    \begin{align}
    \left(\boldsymbol{\Sigma}_{t}^{(\ell)}\mid_{\text{var}} \right)_{i,i} &=\left(\Sigma_t^{(\ell)}\right)_{i,i} 
        \approx \frac{1}{M} \left( (\boldsymbol{\Omega}_t^{(\ell)})^\top \boldsymbol{\Omega}_t^{(\ell)} \right)_{i,i} \notag
        = \frac{1}{M}\sum_{j=1}^{M} \left((\boldsymbol{\Omega}_t^{(\ell)})^\top\right)_{i,j} \boldsymbol{\Omega}_{j,i}^{(\ell)} \notag\\
        &=  \frac{1}{M}\sum_{j=1}^{M} \boldsymbol{\Omega}_{j,i}^{(\ell)} \boldsymbol{\Omega}_{j,i}^{(\ell)} 
        = \frac{1}{M}\sum_{j=1}^{M} \left(\boldsymbol{\Omega}_t^{(\ell)} \odot \boldsymbol{\Omega}_t^{(\ell)} \right)_{j,i} 
        = \frac{1}{M}\left(\left(\boldsymbol{\Omega}_t^{(\ell)} \odot \boldsymbol{\Omega}_t^{(\ell)} \right)^\top \mathbb{1}_{M}\right)_i \notag
        .
    \end{align}
\end{proof}

\subsection{Computing square root}

Direct computation of $(\boldsymbol{\Sigma}_t^{(\ell)})^{\sfrac{1}{2}}$ by
\begin{align}
(\boldsymbol{\Sigma}_t^{(\ell)})^{\frac{1}{2}} 
\approx
\left[
    \frac{1}{M} (\boldsymbol{\Omega}_t^{(\ell)})^\top \boldsymbol{\Omega}_t^{(\ell)}
    \right]^{\frac{1}{2}}
    \in
    \mathbb{R}^{m_{\ell}n_{\ell} \times m_{\ell}n_{\ell}} \notag
\end{align}
is computationally infeasible for large parameter matrices. Note that
\begin{align}
 \frac{1}{M} \boldsymbol{\Omega}_t^{(\ell)}(\boldsymbol{\Omega}_t^{(\ell)})^\top   \in \mathbb{R}^{M \times M}
 ,
 \quad
 M \ll m_{\ell}n_{\ell} \notag
 ,
\end{align}
has low-rank structure and the same spectrum of $\boldsymbol{\Sigma}_t^{(\ell)}$. We seek an efficient method by exploiting the low-rank SVD in $\frac{1}{M}\boldsymbol{\Omega}_t^{(\ell)}(\boldsymbol{\Omega}_t^{(\ell)})^\top$. 


\begin{proposition}[Square Root Approximation of Covariance Matrix]
\label{prop:}

Suppose $\sfrac{\boldsymbol{\Omega}_t^{(\ell)}}{\sqrt{M}}$ admits SVD:
\begin{align}
\frac{\boldsymbol{\Omega}_t^{(\ell)}}{\sqrt{M}} = \boldsymbol{U}_t^{(\ell)} (\boldsymbol{\Lambda}_t^{(\ell)})^{\frac{1}{2}} (\boldsymbol{V}_t^{(\ell)})^\top \notag
, 
\end{align}
where $\boldsymbol{\Lambda}_t^{(\ell)}$ and $\boldsymbol{U}_t^{(\ell)}$ are the eigenvalues and eigenvectors of $\frac{1}{M} \boldsymbol{\Omega}_t^{(\ell)}(\boldsymbol{\Omega}_t^{(\ell)})^\top$. Then:
\begin{align}
(\boldsymbol{\Sigma}_t^{(\ell)})^{\frac{1}{2}}    
\approx
\left[
\frac{ (\boldsymbol{\Omega}_t^{(\ell)})^\top \boldsymbol{U}_t^{(\ell)}}{\sqrt{M}}
\right]
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\left[
\frac{ (\boldsymbol{\Omega}_t^{(\ell)})^\top \boldsymbol{U}_t^{(\ell)}}{\sqrt{M}}
\right]^\top \notag
.
\end{align}
\end{proposition}

\begin{proof}
Starting from Equation~\ref{equ:unbiased_batch_gradient_noise_estimator}, this can be obtained by:
\begin{align}
(\boldsymbol{\Sigma}_t^{(\ell)})^{\frac{1}{2}}
&\approx
\left[
    \frac{1}{M} (\boldsymbol{\Omega}_t^{(\ell)})^\top \boldsymbol{\Omega}_t^{(\ell)}
\right]^{\frac{1}{2}}
=
\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top}
{\sqrt{M}}
\boldsymbol{U}_t^{(\ell)} (\boldsymbol{U}_t^{(\ell)})^\top
\frac{\boldsymbol{\Omega}_t^{(\ell)}}{\sqrt{M}} 
\right]^{\frac{1}{2}}
\notag\\
&=
\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }{\sqrt{M}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}(\boldsymbol{\Lambda}_t^{(\ell)})
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\frac{(\boldsymbol{U}_t^{(\ell)})^\top\,\boldsymbol{\Omega}_t^{(\ell)}}{\sqrt{M}} 
\right]^{\frac{1}{2}} %\notag\\
\end{align}

Set:
\begin{align}
\boldsymbol{P}=\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }
{\sqrt{M}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}} \notag
, 
\end{align}
and note:
\begin{align}
\boldsymbol{P}=
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }
{\sqrt{M}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
 =  \left[
\boldsymbol{U}_t^{(\ell)} (\boldsymbol{\Lambda}_t^{(\ell)})^{\frac{1}{2}} (\boldsymbol{V}_t^{(\ell)})^\top 
 \right]^\top 
 \boldsymbol{U}_t^{(\ell)} (\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}  = \boldsymbol{V}_t^{(\ell)} \notag
\end{align}
is orthonormal.

Hence:
\begin{align}
(\boldsymbol{\Sigma}_t^{(\ell)})^{\frac{1}{2}}
&\approx
\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }{\sqrt{M}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}(\boldsymbol{\Lambda}_t^{(\ell)})
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\frac{(\boldsymbol{U}_t^{(\ell)})^\top\,\boldsymbol{\Omega}_t^{(\ell)}}{\sqrt{M}} 
\right]^{\frac{1}{2}} \notag\\
&=
\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }{\sqrt{M}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\right]
(\boldsymbol{\Lambda}_t^{(\ell)})^{\frac{1}{2}}
\left[
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\frac{(\boldsymbol{U}_t^{(\ell)})^\top\,\boldsymbol{\Omega}_t^{(\ell)}}{\sqrt{M}} 
\right]^{\frac{1}{2}} \notag\\
&=
\underbrace{
\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }
{\sqrt{M}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\right]
}_{\boldsymbol{P}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{\frac{1}{2}}
\underbrace{
\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }
{\sqrt{M}}
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\right]^\top
}_{\boldsymbol{P}^\top}
\notag\\
&=\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }
{\sqrt{M}}
\right]
(\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
\left[
\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }
{\sqrt{M}}
\right]^\top \notag
.
\end{align}

% since
% \begin{align}
% \boldsymbol{P}=\frac{(\boldsymbol{\Omega}_t^{(\ell)})^\top\,\boldsymbol{U}_t^{(\ell)} }
% {\sqrt{M}}
% (\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}
%  =  \left[
% \boldsymbol{U}_t^{(\ell)} (\boldsymbol{\Lambda}_t^{(\ell)})^{\frac{1}{2}} (\boldsymbol{V}_t^{(\ell)})^\top 
%  \right]^\top 
%  \boldsymbol{U}_t^{(\ell)} (\boldsymbol{\Lambda}_t^{(\ell)})^{-\frac{1}{2}}  = \boldsymbol{V}_t^{(\ell)} \notag
% \end{align}
% is orthonormal.


\end{proof}




\section{Temporal evolution of Lipschitz upper bound}


%We only focus on the concept of the temporal evolution of the Frobenius-norm Lipschitz continuity of networks. 

Suppose that an $L$-layer feed-forward neural network $f$ is the composition of $L$ layers, each comprising a linear unit with an activation unit, expressed as:
\begin{align}
    f := \left(\rho^{(L)} \circ~\phi^{(L)}\right) \circ \cdots \circ~\left(\rho^{(2)} \circ~\phi^{(2)} \right)\circ~\left(\rho^{(1)} \circ~\phi^{(1)}\right) \nonumber
\end{align}
where $\left(\rho^{(\ell)} \circ~\phi^{(\ell)}\right)$ represents the $\ell$-th layer consisting of the linear unit $\psi^{(\ell)}(\cdot)$ and the activation unit $\rho^{(\ell)}(\cdot)$. Let the Lipschitz constants of $\rho^{(\ell)}$ and $\phi^{(\ell)}$ be $A^{(\ell)}$ and $K^{(\ell)}$, respectively. The upper bound of the network Lipschitz constant of $f$ then is the product of $A^{(\ell)}$ and $K^{(\ell)}$ across all layers, as shown in Proposition~\ref{prop:network_lipschitz_bound} \citep{miyato2018spectral,fazlyab2019efficient,virmaux2018lipschitz,gouk2021regularisation,virmaux2018lipschitz}. 


\begin{proposition}[Lipschitz Continuity Bound in Feed-Forward Network]
\label{prop:network_lipschitz_bound}
Let $\hat{K}(t)$ be the Lipschitz constant of a feed-forward neural network $f$ without skip connections. The network Lipschitz constant $\hat{K}(t)$ is upper-bounded by:
\begin{align}
    \hat{K}(t):=\sup_{\forall~u \neq v} \frac{\|f(u) - f(v)\|_2}{\|u-v\|_2} \leq K(t):=\prod_{l=1}^{L} A^{(\ell)} \cdot \prod_{l=1}^{L} K^{(\ell)}(t) \notag
    .
\end{align} 
This upper bound is useful in robust certification and theoretical analysis of deep models with complex topologies \citep{fazlyab2019efficient, gouk2021regularisation, virmaux2018lipschitz}. We refer to $K(t)$ as Lipschitz continuity or Lipschitz constant for brevity.
\end{proposition}




Since most activation functions, such as ReLU, Leaky ReLU, Tanh, Sigmoid, \etc, have $1$-Lipschitz continuity \citep{virmaux2018lipschitz}, we set $A^{(\ell)}=1$ for brevity in theoretical analysis. Note that Proposition~\ref{prop:network_lipschitz_bound} does not take into account skip connections. %To simplify the theoretical analysis, we discuss the network Lipschitz constant defined in Lemma~\ref{lemma:network_lipschitz}.    



% \begin{lemma}[Lipschitz Constant of General Network]
% \label{lemma:path_lipschitz}
% More generally, the Lipschitz constant for a general neural network $f$ can be represented by path-based method as:
% \begin{align}
% \label{equ:path_lipschitz}
%     K_{path}(t) = \sum_{p=1}^P \left(\prod_{l=1}^{L^{(p)}} A_p^{(\ell)} \cdot \prod_{l=1}^{L^{(p)}} K_p^{(\ell)}(t) \right)
% \end{align}
% where $L^{(p)}$ represents the number of layers in the $p$-th path, $A_p^{(\ell)}$ and $K_p^{(\ell)}(t)$ represent the $\ell$-th layer Lipschitz constants of activation unit and linear unit in the $p$-th path \citep{neyshabur2015norm}.     
% \end{lemma}




\begin{proposition}[Operator Norm of Linear Unit] 
\label{prop:operator_norm_of_linear_unit}
Suppose the $\phi^{(\ell)}(t)$ is a linear unit with matrix multiplication or convolution:
\begin{align}
    \phi^{(\ell)}(t)(z) := \boldsymbol{\theta}^{(\ell)}(t)(z) + \boldsymbol{b}^{(\ell)}(t),
\end{align}
where $\boldsymbol{\theta}^{(\ell)}(t)$ and $\boldsymbol{b}^{(\ell)}(t)$ are the $\ell$-th layer parameter matrix and bias, respectively. Then, the operator norm of $\phi^{(\ell)}(t)$ (\ie~spectral norm) admits:
\begin{align}
\|\phi^{(\ell)}(t)\|_{op} = \|\boldsymbol{\theta}^{(\ell)}(t)\|_{op} = \sigma_{1}^{(\ell)}(t) \notag
,
\end{align}
where $\sigma_{1}^{(\ell)}(t)$ is the largest singular value of $\theta^{(\ell)}(t)$ \citep{miyato2018spectral,sedghi2019singular}.
\end{proposition}



\begin{definition}[Stochastic Dynamical System of Lipschitz Continuity Bound]
\label{def:lipschitz_dynamical_system}
Collect: 
\begin{enumerate}
    \item Definition~\ref{def:ct_sgd}: Vectorized SDE for Continuous-Time SGD;
    \item Proposition~\ref{prop:network_lipschitz_bound}: Lipschitz Continuity Bound in Feed-Forward Network;
    \item Proposition~\ref{prop:operator_norm_of_linear_unit}: Operator Norm of Linear Unit,
\end{enumerate}
so that the dynamics of Lipschitz continuity bound for a feed-forward neural network is characterized by a system of SDEs:
\begin{numcases}{}
%\setlength{\jot}{-1pt} 
    \dd \mathrm{vec}(\boldsymbol{\theta}^{(\ell)}(t)) = - \mathrm{vec}\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right]  \, \dd t   + \sqrt{\eta} \left[\boldsymbol{\Sigma}_t^{(\ell)} \right]^{\frac{1}{2}} \, \dd \boldsymbol{B}_t^{(\ell)} \notag\\
    K^{(\ell)}(t)=\|\boldsymbol{\theta}^{(\ell)}(t)\|_{op}  \notag\\
    Z(t)  = \sum_{l=1}^L \log K^{(\ell)}(t) \notag\\
    K(t) = \mathrm{e}^{Z(t)} \notag
\end{numcases}
adapted to the filtration $\mathcal{F}_t$, where: (i) $K^{(\ell)}(t)$ governs the $\ell$-th layer dynamics of Lipschitz continuity; (ii) $K(t)$ governs the network dynamics of Lipschitz continuity bound; and (iii) $Z(t)$ is the logarithmic Lipschitz constant to facilitate theoretical deductions. \textbf{This stochastic dynamical system characterizes the dynamics of the Lipschitz continuity bound induced by the optimization dynamics}.

\end{definition}


% %original
% \begin{figure*}[t!]
%     \centering

%  %\begin{minipage}[t]{1\textwidth}
 
%   % layer dynamics
%   \begin{minipage}[t]{1\textwidth}
%      \centering 
%      \subfloat[Layer-specific dynamics]{
%       \includegraphics[width=1\linewidth]{plots/longrange_layer_dynamics_integral.pdf}  
%       \label{fig:dynamics:layer}
%      }
%   \end{minipage}
  
%   %\vfill
%   % network dynamics
%   \begin{minipage}[t]{1\textwidth}
%       \centering
%       \subfloat[Network-specific dynamics (differential)]{
%       \includegraphics[width=1\linewidth]{plots/longrange_network_dynamics_differential_rasterized.pdf}  
%       \label{fig:dynamics:network:differential}
%      }
%   \end{minipage}
  
%   %\vfill
%   % network dynamics
%   \begin{minipage}[t]{1\textwidth}
%       \centering
%       \subfloat[Network-specific dynamics (integral)]{
%       \includegraphics[width=1\linewidth]{plots/longrange_network_dynamics_integral_rasterized.pdf}  
%       \label{fig:dynamics:network}
%      }
%   \end{minipage}

%   % \begin{minipage}[t]{0.25\textwidth}
%   %     \centering
%   %     \subfloat[Loss]{
%   %     \includegraphics[width=1\linewidth]{plots/longrange_loss.pdf}  
%   %     \label{fig:dynamics:loss}
%   %    }
%   % \end{minipage}
%   % \begin{minipage}[t]{0.25\textwidth}
%   %     \centering
%   %     \subfloat[Loss]{
%   %     \includegraphics[width=1\linewidth]{plots/longrange_accuracy.pdf}  
%   %     \label{fig:dynamics:acc}
%   %    }
%   % \end{minipage}


%    %num_epochs:  1766
%    %total_steps:  344370
%    %inset: 330000 for 100 steps.
%    %last train_loss:  0.009750319093179244
%    %last test_loss:  2.223605284324059
%    %last train_acc:  0.9999599358974359
%    %last test_acc:  0.6853966346153846
   
%   \caption[Stochastic Dynamics of Lipschitz Continuity Near Convergence]{Dynamics near convergence. We profile both layer-specific and network-specific dynamics over $344,370$ steps ($1766$ epochs) on CIFAR-10. At the end of training, the final training loss and test loss are $9.75 \times 10^{-3}$ and $2.22$, respectively; the final training accuracy and test accuracy are $0.99996$ and $0.68540$, respectively. To investigate how the variances (\ie~diagonal elements) and covariances (\ie~off‐diagonal elements) of the gradient noise affect the dynamics, the dynamics are computed with respect to variances ($\Sigma_{\mathrm{var}}$) and covariances ($\Sigma_{\mathrm{cov}}$) respectively, using Theorem~\ref{theorem:network_dynamics}. The results indicate that: (i) the optimization‐trajectory drift plays the primary role in shaping Lipschitz continuity over time; (ii) the covariances dominate the noise contributions; and (iii) the noise-curvature entropy production $\kappa_Z(t)$ remains significant near convergence, leading to a gradual and steady increase in Lipschitz continuity. The inset plot zooms in on $100$ steps at $t=330,000$. The moving averages are computed over a window of $500$ steps.}
  
%   \label{fig:longrange_dynamics}
  
% \end{figure*}


\begin{sidewaysfigure}
%\begin{figure*}[t!]
    \centering

 %\begin{minipage}[t]{1\textwidth}
 
  % layer dynamics
  \begin{minipage}[t]{0.8\textwidth}
     \centering 
     \subfloat[Layer-specific dynamics]{
      \includegraphics[width=1\linewidth]{plots/longrange_layer_dynamics_integral.pdf}  
      \label{fig:dynamics:layer}
     }
  \end{minipage}
  
  % %\vfill
  % % network dynamics
  % \begin{minipage}[t]{0.8\textwidth}
  %     \centering
  %     \subfloat[Network-specific dynamics (differential)]{
  %     \includegraphics[width=1\linewidth]{plots/longrange_network_dynamics_differential_rasterized.pdf}  
  %     \label{fig:dynamics:network:differential}
  %    }
  % \end{minipage}
  
  %\vfill
  % network dynamics
  \begin{minipage}[t]{0.8\textwidth}
      \centering
      \subfloat[Network-specific dynamics (integral)]{
      \includegraphics[width=1\linewidth]{plots/longrange_network_dynamics_integral_rasterized.pdf}  
      \label{fig:dynamics:network}
     }
  \end{minipage}

  % \begin{minipage}[t]{0.25\textwidth}
  %     \centering
  %     \subfloat[Loss]{
  %     \includegraphics[width=1\linewidth]{plots/longrange_loss.pdf}  
  %     \label{fig:dynamics:loss}
  %    }
  % \end{minipage}
  % \begin{minipage}[t]{0.25\textwidth}
  %     \centering
  %     \subfloat[Loss]{
  %     \includegraphics[width=1\linewidth]{plots/longrange_accuracy.pdf}  
  %     \label{fig:dynamics:acc}
  %    }
  % \end{minipage}


   %num_epochs:  1766
   %total_steps:  344370
   %inset: 330000 for 100 steps.
   %last train_loss:  0.009750319093179244
   %last test_loss:  2.223605284324059
   %last train_acc:  0.9999599358974359
   %last test_acc:  0.6853966346153846
   
  \caption[Stochastic Dynamics of Lipschitz Continuity Near Convergence]{Dynamics near convergence. We profile both layer-specific and network-specific dynamics over $344,370$ steps ($1766$ epochs) on CIFAR-10. At the end of training, the final training loss and test loss are $9.75 \times 10^{-3}$ and $2.22$, respectively; the final training accuracy and test accuracy are $0.99996$ and $0.68540$, respectively. To investigate how the variances (\ie~diagonal elements) and covariances (\ie~off‐diagonal elements) of the gradient noise affect the dynamics, the dynamics are computed with respect to variances ($\Sigma_{\mathrm{var}}$) and covariances ($\Sigma_{\mathrm{cov}}$) respectively, using Theorem~\ref{theorem:network_dynamics}. The results indicate that: (i) the optimization‐trajectory drift plays the primary role in shaping Lipschitz continuity over time; (ii) the covariances dominate the noise contributions; and (iii) the noise-curvature entropy production $\kappa_Z(t)$ remains significant near convergence, leading to a gradual and steady increase in Lipschitz continuity. The inset plot zooms in on $100$ steps at $t=330,000$. The moving averages are computed over a window of $500$ steps.}
  
  \label{fig:longrange_dynamics}
  
%\end{figure*}
\end{sidewaysfigure}

\section{Theoretical analysis}
\label{sec:theoretical_analysis}

Note that the equation system in Definition~\ref{def:lipschitz_dynamical_system} is driven by a Wiener process, which consists of stochastic differential equations (SDEs), and is adapted to the filtration $\mathcal{F}_t$, with time-dependent parameters $\theta^{(\ell)}(t)$. We leverage It\^o's Lemma \citep{ito1951stochastic,oksendal2013stochastic} to analyze this SDE system. We aim to analyze the dynamics of $Z(t)$ and $K(t)$. The sketch for theoretical analysis is:
\begin{enumerate} 
    %\setlength{\itemsep}{0.2em}
    %\setlength{\parskip}{0pt}
    
    \item \textbf{Layer-Specific Dynamics} (Section~\ref{sec:layer_dyanmics}). We derive the SDE for $\dd K_t^{(\ell)}$ by applying It\^o's Lemma to the process $\dd \mathrm{vec}\left[\theta^{(\ell)}(t)\right]$. This step establishes a direct connection between parameter-level updates driven by the optimization process and the layer-wise operator norm.
      
    \item \textbf{Network-Specific Dynamics} (Section~\ref{sec:network_dynamics}). Building on the layer-specific analysis, we derive the network-level SDE for $\dd Z(t)$ by applying It\^o's Lemma to the processes $\dd K^{(\ell)}(t)$ across $L$ layers. The process $Z(t)$ captures the logarithmic, network-level dynamics of Lipschitz continuity. Finally, we obtain the dynamics of $K(t)$ from $\dd Z(t)$ via It\^o calculus.
        
    \item \textbf{Statistical Characterization} (Section~\ref{sec:statistics}). We analyze the statistical properties of $Z(t)$ and $K(t)$, including their expectations and variances. These results provide insight into the asymptotic behavior of the system near convergence.
\end{enumerate}




\subsection{First- and second-order operator-norm derivatives}
\label{sec:jacobian_and_hessian}

Stochastic spectral analysis regarding the parameter matrices requires the first-order and second-order derivatives of the largest singular values with respect to parameter matrices. The first-order operator-norm derivative is well-known in the literature \citep{luo2025spectralvariation,kato1995perturbation,horn2012matrix,magnus2019matrix} (Lemma~\ref{lemma:jacobian_spectral_norm}). The second-order operator-norm derivative can be derived through perturbation theory \citep{kato1995perturbation,luo2025spectralvariation}. Lemma~\ref{lemma:hessian_spectral_norm} is proved in the literature \citep{luo2025spectralvariation} based on perturbation theory for linear operators \citep{kato1995perturbation}. Let $\boldsymbol{\theta}^{(\ell)}(t)$ admit a SVD:
\begin{align}
    \boldsymbol{\theta}_t^{(\ell)} = \sum_{i=1}^{r} 
    \sigma_{i}^{(\ell)}(t) \boldsymbol{u}_{i}^{(\ell)} (t)
    \boldsymbol{v}_{i}^{(\ell)}(t)^\top
    ,\quad
    \sigma_{1}^{(\ell)}(t) > \sigma_{2}^{(\ell)}(t) > \cdots > \sigma_{r}^{(\ell)}(t)
    ,\quad
    r = \rank(\boldsymbol{\theta}^{(\ell)}(t))
    ,\notag
\end{align}
under the Assumption~\ref{assump:differentiability}.


\begin{assumption}[\textbf{Spectral Differentiability}]
\label{assump:differentiability}
We assume the singular values of parameter matrices are \emph{simple}: $\sigma_i^{(\ell)} \neq \sigma_j^{(\ell)}$, for all $i \neq j$. This assumption guarantees $\sigma_i^{(\ell)}, \boldsymbol{u}_i^{(\ell)}, \boldsymbol{v}_i^{(\ell)} \in C^{\infty}$ (\ie~differentiable at arbitrary integer order) \citep{kato1995perturbation}.
\end{assumption}

%niall wants me to add things.
% \begin{remark}
% If Assumption~\ref{assump:differentiability} does not hold, the singular-value derivatives are not defined, and It\^o's lemma fails to be applied to derive the dynamics of Lipschitz continuity.
% \end{remark}


\begin{lemma}[Operator-Norm Jacobian]
\label{lemma:jacobian_spectral_norm}
The operator-norm Jacobian of $\|\boldsymbol{\theta}^{(\ell)}(t)\|_{op}$ with respect to $\mathrm{vec}\left[\boldsymbol{\theta}^{(\ell)}(t)\right]$ is given by:
\begin{align}
\boldsymbol{J}_{op}^{(\ell)}(t) 
=\frac{\partial \|\boldsymbol{\theta}^{(\ell)}(t)\|_{op}}{\partial \operatorname{vec}\left[\boldsymbol{\theta}^{(\ell)}(t)\right]}
=\boldsymbol{v}_{1}^{(\ell)}(t) \otimes \boldsymbol{u}_{1}^{(\ell)}(t) 
\in \mathbb{R}^{m_{\ell}n_{\ell}}
\notag
,
\end{align} 
where $\otimes$ denotes Kronecker product (\ie~tensor product) \citep{luo2025spectralvariation,kato1995perturbation,horn2012matrix,magnus2019matrix}.
\end{lemma}


\begin{lemma}[Operator-Norm Hessian \citep{luo2025spectralvariation}]
\label{lemma:hessian_spectral_norm}
The operator-norm Hessian of $\|\boldsymbol{\theta}^{(\ell)}(t)\|_{op}$ with respect to $\mathrm{vec}\left[\boldsymbol{\theta}^{(\ell)}(t)\right]$ is given by:
\begin{align}
\boldsymbol{H}_{op}^{(\ell)}(t) 
=
\frac{\partial}{\partial \operatorname{vec}\left[ \boldsymbol{\theta}^{(\ell)}(t)\|_{op} \right]}
\operatorname{vec}\left[\frac{\partial \|\boldsymbol{\theta}^{(\ell)}(t)\|_{op}}{\partial \boldsymbol{\theta}^{(\ell)}(t)}\right]
= \boldsymbol{H}_{L}^{(\ell)}(t) + \boldsymbol{H}_{R}^{(\ell)}(t) + \boldsymbol{H}_{C}^{(\ell)}(t) 
\in \mathbb{R}^{m_{\ell}n_{\ell} \times m_{\ell}n_{\ell}}
\notag
,
\end{align}
where:
\begin{gather}
\boldsymbol{e}_{i,j}^{(\ell)}(t) := \boldsymbol{v}^{(\ell)}_i(t) \otimes \boldsymbol{u}^{(\ell)}_j(t) , \notag \\
\boldsymbol{H}_{L}^{(\ell)}(t) =\sum_{i \neq 1, i \leq m_{\ell}} \frac{\sigma_1^{(\ell)}(t)}{\sigma_1^{(\ell)}(t)^2 - \sigma_i^{(\ell)}(t)^2} \boldsymbol{e}_{1,i}^{(\ell)}(t) \otimes  \boldsymbol{e}_{1,i}^{(\ell)}(t)^\top  ,\notag\\
\boldsymbol{H}_{R}^{(\ell)}(t) = \sum_{j \neq 1, j \leq n_{\ell}} \frac{\sigma_1^{(\ell)}(t)}{\sigma_1^{(\ell)}(t)^2 - \sigma_j^{(\ell)}(t)^2} \boldsymbol{e}_{j,1}^{(\ell)}(t) \otimes \boldsymbol{e}_{j,1}^{(\ell)}(t)^\top , \notag\\
\boldsymbol{H}_{C}^{(\ell)}(t) = \sum_{k \neq 1, k \leq r_{\ell}} \frac{\sigma_k^{(\ell)}(t)}{\sigma_1^{(\ell)}(t)^2 - \sigma_k^{(\ell)}(t)^2} 
\left[
\boldsymbol{e}_{1,k}^{(\ell)}(t) \otimes \boldsymbol{e}_{k,1}^{(\ell)}(t)^\top +  \boldsymbol{e}_{k,1}^{(\ell)}(t) \otimes \boldsymbol{e}_{1,k}^{(\ell)}(t)^\top \right] \notag 
,
\end{gather}
and $r_{\ell}=\rank(\boldsymbol{\theta}^{(\ell)}(t))$.

\end{lemma}

\begin{remark}
Note that the function $\sigma_1^{(\ell)}(t): \boldsymbol{\theta}^{(\ell)}(t) \mapsto \mathbb{R}$ is convex. Since the Hessian of a convex function is PSD, it follows that $\boldsymbol{H}_{\text{op}}^{(\ell)}(t)$ is PSD.
\end{remark}


\subsection{Layer-specific dynamics}
\label{sec:layer_dyanmics}



\begin{theorem}[Layer-Specific Dynamics]
\label{theorem:layer_dynamics}
The layer-specific dynamics of Lipschitz continuity is given by:
\begin{align}
\frac{\dd K^{(\ell)}(t)}{K^{(\ell)}(t)}  = \left( \mu^{(\ell)}(t) + \kappa^{(\ell)}(t) \right) \,  \dd t + \boldsymbol{\lambda}^{(\ell)}(t)^\top \, \dd \boldsymbol{B}_t^{(\ell)} 
, 
\end{align}    
where $\dd\,\boldsymbol{B}_t^{(\ell)} \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{\mathrm{I}}_{m_{\ell}n_{\ell}} \dd t)$ represents the increment of a standard Wiener process in $\mathbb{R}^{m_{\ell}n_{\ell}}$, and:
\begin{gather}
\mu^{(\ell)}(t) =  \frac{1}{\sigma_{1}^{(\ell)}(t)} \left\langle \boldsymbol{J}_{op}^{(\ell)}(t), \, -\mathrm{vec}\left[ \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t)) \right] \right\rangle ,\notag \\
\boldsymbol{\lambda}^{(\ell)}(t) = \frac{\sqrt{\eta}}{\sigma_{1}^{(\ell)}(t)}  
\left(\left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}}\right)^\top 
\boldsymbol{J}_{op}^{(\ell)}(t)
, \quad
\|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2 = \boldsymbol{\lambda}^{(\ell)}(t)^\top \boldsymbol{\lambda}^{(\ell)}(t) \geq 0,\notag \\
\kappa^{(\ell)}(t) =\frac{\eta}{2\sigma_{1}^{(\ell)}(t)} \left\langle \boldsymbol{H}_{op}^{(\ell)}(t),  \boldsymbol{\Sigma}_t^{(\ell)}\right\rangle \geq 0,\notag 
\end{gather}
where we refer to:
\begin{enumerate}
    % \setlength{\itemsep}{0.2em}
    % \setlength{\parskip}{0pt}


    \item $\mu^{(\ell)}(t)$ as \textbf{layer optimization-induced drift}, representing the contribution of the gradient flow $\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))$ --- induced by the optimization process --- to the expectation of Lipschitz continuity. This term corresponds to the projection of the negative gradient expectation onto the principal subspace (\ie~largest singular value) of the parameter matrix, and acts as a deterministic drift in the evolution of the Lipschitz constant.


    \item $\boldsymbol{\lambda}^{(\ell)}(t)$ as \textbf{layer diffusion-modulation intensity}, representing the contribution of the gradient noise $\boldsymbol{\Sigma}_t^{(\ell)}$ --- arising from the randomness in mini-batch sampling --- to the stochasticity of Lipschitz continuity. This term modulates the stochasticity of Lipschitz continuity and governs the uncertainty of temporal evolution.


    \item $\kappa^{(\ell)}(t)$ as \textbf{layer noise-curvature entropy production}, representing the non-negative, irreversible contribution of the gradient noise $\boldsymbol{\Sigma}_t^{(\ell)}$ to the deterministicity of Lipschitz continuity. Intuitively, the dynamical system baths in the stochastic gradient fluctuations captured by $\boldsymbol{\Sigma}_t^{(\ell)}$, arising from mini-batch sampling. The stochastic fluctuations ``dissipate'' into the system via the curvature of the operator-norm landscape $\boldsymbol{H}_{op}^{(\ell)}(t)$, driving an irreversible increase in the Lipschitz constant and entropy.
    
\end{enumerate}    

\end{theorem}

% \begin{remark}[System Entropy Production]
% By viewing $K^{(\ell)}(t)$ as a system state, the Fokker-Plank Equation (FPE) can give the distribution of $K^{(\ell)}(t)$ as $p(K^{(\ell)},t)$. At a $t$, the Shannon entropy of $K^{(\ell)}(t)$ is given by:
% \begin{align}
%     S(K^{(\ell)},t) := -\int p(K^{(\ell)},t) \,\log{p(K^{(\ell)},t)} \;\dd K^{(\ell)}(t),
% \end{align}
% where the $\boldsymbol{\kappa}^{(\ell)}(t)$ contributes to the non-negative, irreversible increments of the system entropy, arising from the interaction between operator-norm curvature and gradient noise arising from mini-batch sampling. 
% \end{remark}

\begin{proof}
Start with Definition~\ref{def:lipschitz_dynamical_system}:
\begin{numcases}{}
\dd  \mathrm{vec}  \left(\boldsymbol{\theta}^{(\ell)}(t)\right) = -\mathrm{vec} \left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right] \dd t + \sqrt{\eta}\left[\boldsymbol{\Sigma}_t^{(\ell)} \right]^{\frac{1}{2}}\dd \boldsymbol{B}_t^{(\ell)} \label{equ:layer_proof_ct_sgd}\\
K^{(\ell)}(t) = \|\boldsymbol{\theta}^{(\ell)}(t)\|_{op} = \sigma_1^{(\ell)}(t) \label{equ:layer_proof_operator_norm}
\end{numcases}

Using Lemma~\ref{lemma:jacobian_spectral_norm} and Lemma~\ref{lemma:hessian_spectral_norm}, we apply It\^o's Lemma on Equation~\ref{equ:layer_proof_operator_norm}:
\begin{align}
    \dd K^{(\ell)}(t) = \underbrace{
    \boldsymbol{J}_{op}^{(\ell)}(t)^\top \dd \operatorname{vec}\left(\boldsymbol{\theta}^{(\ell)}(t)\right)
    }_{A} + 
    \underbrace{
    \frac{1}{2} \left(\dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t)\right)^\top \; \boldsymbol{H}_{op}^{(\ell)}(t) \; \dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t))}_{B}.
\end{align}

\medskip
\noindent
\textbf{Compute $A$ and $B$}.
\begin{enumerate}
    \item Substitute Equation~\ref{equ:layer_proof_ct_sgd} into $A$:
\begin{align}
\label{equ:layer_proof_expanded_A}
    A &= \boldsymbol{J}_{op}^{(\ell)}(t)^\top \dd \operatorname{vec}\left(\boldsymbol{\theta}^{(\ell)}(t)\right) \notag\\
    &=\boldsymbol{J}_{op}^{(\ell)}(t)^\top \left[ - \mathrm{vec}\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right] \, \dd t   + \sqrt{\eta} \left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}} \, \dd \boldsymbol{B}_t^{(\ell)} \right] \notag\\
    &= \left\langle \boldsymbol{J}_{op}^{(\ell)}(t), - \mathrm{vec}\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right] \right\rangle \dd t + \boldsymbol{J}_{op}^{(\ell)}(t)^\top \sqrt{\eta} \left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}} \, \dd \boldsymbol{B}_t^{(\ell)}. 
\end{align}

\item Use trace identity $\tr(XYZ)=\tr(YZX)$:
\begin{align}
    B &= \frac{1}{2} \left(\dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t)\right)^\top \boldsymbol{H}_{op}^{(\ell)}(t)  \dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t)) \notag\\
    &= \frac{1}{2} \tr\left[  \boldsymbol{H}_{op}^{(\ell)}(t)  \, \dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t))  \left(\dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t)\right)^\top \right]. \notag
\end{align}

Substituting Equation~\ref{equ:layer_proof_ct_sgd} into $B$, we obtain:
\begin{align}
   B &= \frac{1}{2} \tr\left[ \boldsymbol{H}_{op}^{(\ell)}(t) \dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t)) \left(\dd \operatorname{vec}(\boldsymbol{\theta}^{(\ell)}(t)\right)^\top \right] \notag\\
   &= \frac{1}{2} \tr\left[ \boldsymbol{H}_{op}^{(\ell)}(t) \eta \left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}} \left\{\left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}}\right\}^\top \dd \boldsymbol{B}_t^{(\ell)} (\dd \boldsymbol{B}_t^{(\ell)})^\top \right]\notag \\
    &=\frac{1}{2}\eta \tr\left[ \boldsymbol{H}_{op}^{(\ell)}(t)\left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}} \left\{\left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}}\right\}^\top  \right] \dd t \notag \\
    &=\frac{1}{2} \eta \tr\left[  \boldsymbol{H}_{op}^{(\ell)}(t)   \boldsymbol{\Sigma}_t^{(\ell)} \right] \dd t 
    =
    \frac{1}{2} \eta \left\langle  \boldsymbol{H}_{op}^{(\ell)}(t),   \boldsymbol{\Sigma}_t^{(\ell)}\right\rangle \dd t,  
\end{align}
by dropping higher-order infinitesimal terms, as $ o\left((\dd t)^2\right) \to 0$ and $o\left(\dd t \dd \boldsymbol{B}_t^{(\ell)}\right) \to \boldsymbol{0}$.
 
\end{enumerate}


\medskip
\noindent
\textbf{Combine $A+B$}. Combine expanded $A$ and $B$:
\begin{align}
    \frac{\dd K^{(\ell)}(t)}{K^{(\ell)}(t)} 
    &= \left[
    \underbrace{\frac{1}{\sigma_1^{(\ell)}(t)} \left\langle \boldsymbol{J}_{op}^{(\ell)}(t), - \mathrm{vec}\left[\nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t))\right] \right\rangle
    }_{ \mu^{(\ell)}(t) }+ 
    \underbrace{
    \frac{\eta}{2\sigma_1^{(\ell)}(t)}  \left\langle  \boldsymbol{H}_{op}^{(\ell)}(t),   \boldsymbol{\Sigma}_t^{(\ell)}\right\rangle 
    }_{ \kappa^{(\ell)}(t) }
    \right]\dd t \notag \\
    & \qquad +
    \underbrace{
    \frac{\sqrt{\eta}}{\sigma_1^{(\ell)}(t)} \boldsymbol{J}_{op}^{(\ell)}(t)^\top  \left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}}
    }_{ \boldsymbol{\lambda}^{(\ell)}(t)^\top }
    \, \dd \boldsymbol{B}_t^{(\ell)}.
\end{align}

\end{proof}





%\vspace{-1em}
\subsection{Network-specific dynamics}
\label{sec:network_dynamics}

% Consider the differentials:
% \begin{align}
% \frac{\partial Z(t)}{\partial K^{(\ell)}(t)}  = \frac{1}{K^{(\ell)}(t)} ,
% \quad
% \text{and}\quad 
% \frac{\partial^2 Z(t)}{\partial K^{(\ell)}(t)^2}  = -\frac{1}{K^{(\ell)}(t)^2} .
% \end{align}
% %We apply It\^o's Lemma on $Z(t)$ with respect to all processes $\dd K^{(\ell)}(t)$ across $L$ layers to derive the logarithmic, network-specific dynamics as stated in Theorem~\ref{theorem:network_dynamics}.

\begin{theorem}[Logarithmic Network-Specific Dynamics]
\label{theorem:network_dynamics}
The logarithmic, network-specific dynamics of Lipschitz continuity is given by:
\begin{align}
\label{equ:log_dynamics}
   \dd Z(t) = \left( \mu_Z(t) + \kappa_Z(t) - \frac{1}{2}  \lambda_Z(t)^2 \right) \dd t + \lambda_Z(t) \, \dd W_t,  
\end{align}
where $\dd W_t \sim \mathcal{N}(0, \dd t)$ represents the increment of a standard Wiener process  adapted to the filtration $\mathcal{F}_t$ in $\mathbb{R}$ by:
\begin{gather}
    \dd W_t := 
    %\frac{1}{\sqrt{\sum_{\ell=1}^{L} \|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2} }
    \left[\sum_{\ell=1}^{L} \|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2\right]^{-\frac{1}{2}}
    \cdot
    \sum_{\ell=1}^{L} \boldsymbol{\lambda}^{(\ell)}(t)^\top \, \dd \boldsymbol{B}_t^{(\ell)} \quad \sim\quad \mathcal{N}(0, \dd t), \notag\\
    \mu_Z(t) = \sum_{\ell=1}^{L} \mu^{(\ell)}(t) \in \mathbb{R} , \quad
    \kappa_Z(t) = \sum_{\ell=1}^{L}   \kappa^{(\ell)}(t) \in \mathbb{R}_{+},\quad
    \lambda_Z(t) = \left[\sum_{\ell=1}^{L} \|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2\right]^{\frac{1}{2}} \in \mathbb{R}_{+}, \notag
\end{gather}   
where we refer to: (i) $\mu_Z(t)$ as \textbf{network optimization-induced drift}; (ii) $\lambda_Z(t)$ as \textbf{network diffusion-modulation intensity}; and (iii) $\kappa_Z(t)$ as \textbf{network noise-curvature entropy production}, respectively. 
\end{theorem}

\begin{proof}
Consider the differentials:
\begin{align}
\frac{\partial Z(t)}{\partial K^{(\ell)}(t)}  = \frac{1}{K^{(\ell)}(t)} ,
\quad
\text{and}\quad 
\frac{\partial^2 Z(t)}{\partial K^{(\ell)}(t)^2}  = -\frac{1}{K^{(\ell)}(t)^2} .
\end{align}


We apply It\^o's Lemma on $\dd K^{(\ell)}$ across all layers to derive the dynamics of:
\begin{align}
    Z(t)  = \sum_{l=1}^L \log K^{(\ell)}(t) \notag
    ,
\end{align}
so that:
\begin{align}
    &\dd Z(t)  = \dd \left( \sum_{l=1}^L \log K^{(\ell)}(t) \right) = \sum_{l=1}^L \left( 
    \underbrace{
    \frac{\partial Z(t)}{\partial K^{(\ell)}(t)} \dd K^{(\ell)}(t)
    }_{C} 
    + 
    \underbrace{
    \frac{1}{2} \frac{\partial^2 Z(t)}{\partial K^{(\ell)}(t)^2} \left(\dd K^{(\ell)}(t)
    \right)^2 
    }_{D}
    \right) \notag
    .
\end{align}

\textbf{Derive $C$ and $D$}.
\begin{enumerate}
    \item Derive $C$:
    \begin{align}
    C=\frac{\partial Z(t)}{\partial K^{(\ell)}(t)} \dd K^{(\ell)}(t) = \frac{\dd K^{(\ell)}(t)}{K^{(\ell)}(t)} = \left( \mu^{(\ell)}(t) + \kappa^{(\ell)}(t) \right)  \, \dd t + \boldsymbol{\lambda}^{(\ell)}(t)^\top  \dd \boldsymbol{B}_t^{(\ell)} \notag .
\end{align}

    \item Derive $D$:
\begin{align}
   D=\frac{1}{2} \frac{\partial^2 Z(t)}{\partial K^{(\ell)}(t)^2} \left(\dd K^{(\ell)}(t)
    \right)^2 = -\frac{1}{2K^{(\ell)}(t)^2} \left(\dd K^{(\ell)}(t)
    \right)^2 = -\frac{1}{2} \|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2 \dd t \notag
    ,
\end{align}
by dropping higher-order infinitesimal terms as $o((\dd t)^2) \to 0$ and $ o(\dd t \dd \boldsymbol{B}_t^{(\ell)}) \to \boldsymbol{0}$.

\end{enumerate}

\medskip
\noindent
\textbf{Combine $C+D$}. Hence:
\begin{align}
   \dd Z(t) &= \left( \sum_{l=1}^{L} \mu^{(\ell)}(t) + \kappa^{(\ell)}(t) - \frac{1}{2}\|\boldsymbol{\lambda}^{(\ell)}(t)\|_2^2 \right) \dd t +  \sum_{\ell=1}^{L} \boldsymbol{\lambda}^{(\ell)}(t)^\top \dd \boldsymbol{B}_t^{(\ell)} \nonumber \\
&= \left( \mu_Z(t) + \kappa_Z(t) - \frac{1}{2}  \lambda_Z(t)^2 \right) \dd t + \lambda_Z(t) \dd W_t \nonumber 
\label{equ:log_dynamics}
\end{align}
where $\dd W_t \sim \mathcal{N}(0, \dd t)$ represents the increment of a Wiener process in $\mathbb{R}$.

\end{proof}


\begin{theorem}[Integral-Form Dynamics of Lipschitz Continuity]
\label{theorem:integral_form_network_dynamics}
Using It\^o's calculus, the integral-form dynamics of Lipschitz continuity is stated as:
 \begin{align}
    \begin{cases}
    Z(t)  =  Z(0) + \displaystyle\int_0^t \left[ \mu_Z(s) + \kappa_Z(s) - \frac{1}{2} \lambda_Z(s)^2 \right] \, \dd s +  \displaystyle\int_0^t \lambda_Z(s) \, \dd W_s     \\
    K(t) =\exp\left\{Z(t)\right\} \nonumber
    \end{cases}
\end{align}
where $Z(0)$ is the initial value of $Z(t)$.
\end{theorem}


\subsection{Statistical characterization}
\label{sec:statistics}

\begin{theorem}[Statistics of Lipschitz Continuity]
\label{theorem:statistics_of_lipschitz}
Let $K(0)$ be the initial Lipschitz continuity bound, and hence $Z(0) = \log K(0)$. The expectation and variance of $K(t)$ are given as:
\begin{gather}
\mathbb{E}[K(t)] = \mathrm{e}^{\mathbb{E}[Z(t)] + \frac{1}{2}\mathrm{Var}\left[Z(t)\right]} 
% =\mathrm{e}^{Z(0) + \int_0^t \left[ \mu_Z(s) + \kappa_Z(s)  \right] \dd s}
= K(0)\cdot 
%\underbrace{
\mathrm{e}^{\int_0^t \mu_Z(s) \dd s}
%}_{\text{gradient expectation}}
\cdot 
%\underbrace{
\mathrm{e}^{\int_0^t  \kappa_Z(s)   \dd s}
%}_{\text{gradient noise}}
\\
\mathrm{Var}[K(t)] = \mathbb{E}[K(t)]^2 \left(\mathrm{e}^{\mathrm{Var}[Z(t)]} - 1\right)
=\mathbb{E}[K(t)]^2
\left(
\mathrm{e}^{\int_0^t  \lambda_Z(s)^2   \dd s}  - 1
\right)
,
\end{gather}
where:
\begin{gather}
    \mathbb{E}[Z(t)] = Z(0) + \int_0^t \left[ \mu_Z(s) + \kappa_Z(s) - \frac{1}{2} \lambda_Z(s)^2 \right] \dd s  
    \\
    \mathrm{Var}\left[Z(t)\right] = \int_0^t \lambda_Z(s)^2 \, \dd s .
\end{gather}
\end{theorem}



\begin{remark}
%The results reveal that the deterministic force (i) plays a dominant role in the evolution, while stochastic forces (ii) and (iii) contribute to a lesser extent. Entropy-production $\kappa$ can not be ignored.

% \medskip
% \noindent
% \textbf{Expectation}. 

The expectation of Lipschitz continuity is dominated only by three factors: 
\begin{enumerate}[label=\roman*]
    \item \textbf{Parameter initialization $K(0)$}. The parameter initialization determines the network Lipschitz continuity. We discuss the details in Section~\ref{sec:parameter_initialization}.
    
    \item \textbf{Optimization-induced drift $\mu_Z(t)$}. The projection of gradient expectations on the operator-norm Jacobian, induced by optimization process, drive the evolution of Lipschitz continuity;
    
    \item \textbf{Noise-curvature entropy production $\kappa_Z(t)$}. The gradient fluctuations, arising from mini-batch sampling, has a deterministic, non-negative and irreversible increase in the Lipschitz continuity.
\end{enumerate}



The uncertainty of Lipschitz continuity is determined by two factors:
\begin{enumerate}[label=\roman*]
    \item \textbf{Lipschitz continuity expectation $\mathbb{E}\left[K(t)\right]$}. The uncertainty is proportional to the current Lipschitz constant bound. Larger Lipschitz constant bound leads  to larger uncertainty of the evolution;
    
    \item \textbf{Diffusion-modulation intensity $\lambda_Z(t)$}. The projection of the gradient fluctuations on the operator-norm Jacobian modulates the diffusion process of Lipschitz continuity, hence dominates the uncertainty of the evolution.
    
\end{enumerate}    
\end{remark}

\begin{proof}

%Consider that $\dd W_s$ is a martingale increment with zero mean in Theorem~\ref{theorem:integral_form_network_dynamics}.

% \begin{lemma}[Moment-Generating Function (MGF) of $M(t) \sim \mathcal{N}(\mu, \sigma^2)$]
% \label{lemma:mgf_normal}
% The MGF of $M(t)$ is given as:
% \begin{align}
%        \mathbb{E}\left[e^{kM(t)}\right] =e^{k\mu + \frac{1}{2}k^2\sigma^2}. 
%     \end{align}
% \end{lemma}

\begin{lemma}[Moment-Generating Function of $Z(t)$]
\label{lemma:mgf_zt}
Consider $Z(t)$:
\begin{align}
    Z(t) \sim \mathcal{N}\left(\mathbb{E}\left[Z(t)\right], \operatorname{Var}\left[Z(t)\right]\right)
    ,
\end{align}
then the MGF of $Z(t)$ is given as:
    \begin{align}
      \mathbb{E}\left[e^{kZ(t)}\right] =e^{k \mathbb{E}\left[Z(t)\right] + \frac{1}{2}k^2\operatorname{Var}\left[Z(t)\right]}.
    \end{align}
\end{lemma}


Set $k=1$:
\begin{align}
    \mathbb{E}\left[K(t)\right]  &= \mathbb{E}\left[e^{Z(t)}\right] = e^{ \mathbb{E}\left[Z(t)\right] + \frac{1}{2}\operatorname{Var}\left[Z(t)\right]}
    = \mathrm{e}^{Z(0) + \int_0^t \left[ \mu_Z(s) + \kappa_Z(s)  \right] \dd s}
    ,
\end{align}
so that:
\begin{align}
\left(\mathbb{E}\left[K(t)\right]\right)^2  &= \left(\mathbb{E}\left[e^{Z(t)}\right]\right)^2 = e^{ 2\mathbb{E}\left[Z(t)\right] + \operatorname{Var}\left[Z(t)\right]}
=\mathrm{e}^{2Z(0) + \int_0^t \left[ 2\mu_Z(s) + 2\kappa_Z(s)  \right] \dd s}
.
\end{align}

Set $k=2$:
\begin{align}
    \mathbb{E}\left[ K(t)^2 \right]  &= \mathbb{E}\left[e^{2Z(t)}\right] = e^{ 2\mathbb{E}\left[Z(t)\right] + 2\operatorname{Var}\left[Z(t)\right]}.
\end{align}

Hence:
\begin{align}
\operatorname{Var}\left[K(t)\right] &= \mathbb{E}\left[ K(t)^2 \right] - \left(\mathbb{E}\left[K(t)\right]\right)^2 
=\mathbb{E}\left[K(t)\right]^2\left( e^{\operatorname{Var}\left[Z(t)\right]} - 1\right).
\end{align}



\end{proof}






\section{Framework validation}
\label{sec:validation}




%Although we have developed an efficient gradient noise estimator, the experiments still require approximately $570+$ hours (\ie~$24+$ days) on a single NVIDIA RTX\textsuperscript{TM} 6000 Ada Generation, owing to the substantial computational demands. 
\textbf{Experimental Settings}. We conduct numerical experiments to validate our framework, using a five-layer ConvNet (details in Table~\ref{tab:network_config_cnn} in the Appendix), optimized with SGD (without momentum). Experimental details are as follows:
\begin{enumerate}
    % \setlength{\itemsep}{0.2em}
    % \setlength{\parskip}{0pt}

    \item \textbf{Datasets}. To validate the effectiveness of our framework across various datasets, the ConvNet is trained on CIFAR-10 and CIFAR-100 respectively, for $39,000$ steps ($200$ epochs) with a learning rate of $10^{-3}$ and a batch size of $256$. 

    \item \textbf{Regularizers}. To validate the effectiveness of our framework under various regularization configurations (see Table~\ref{tab:regularization_config} in Appendix), the ConvNet is trained with multiple regularizers, including \textit{batch normalization}, \textit{mixup}, and \textit{label smoothing}. Additional results with \textit{dropout}, \textit{weight decay}, \textit{auto-augment}, and \textit{adversarial training} are presented in the Appendix.
       
\end{enumerate}



    
\medskip
\noindent
\textbf{Experimental Results}. Figure~\ref{fig:validation:cifar10} presents the results on CIFAR-10, and Figure~\ref{fig:validation:cifar100} shows the corresponding results on CIFAR-100. These experiments demonstrate that our mathematical framework closely captures the dynamics of Lipschitz continuity across a range of regularizers.





\section{Theoretical implications}
\label{sec:theoretical_implications}

Our theoretical framework provides a unified perspective for analyzing and interpreting the evolution of Lipschitz continuity in neural networks. Specifically, it enables us to answer the following questions:
\begin{enumerate}

    \item Section~\ref{sec:key_factors}: \textbf{Key factors}. What are the key factors governing the temporal evolution of Lipschitz continuity during training?

    \item Section~\ref{sec:parameter_initialization}: \textbf{Parameter initialization}. How does parameter initialization affect the temporal evolution of Lipschitz continuity?

    
    \item Section~\ref{sec:near_convergence}: \textbf{Unbounded growth near convergence}. What dynamics emerge as the network approaches convergence, particularly in the regime where the training loss approaches zero?

    %\item Section~\ref{sec:adversarial_training}: \textbf{Dampening effect of adversarial training}. What mechanism explains how adversarial training attenuates the temporal evolution of Lipschitz continuity?
    
    \item Section~\ref{sec:noisy_gradient}: \textbf{Noisy gradient regularization}. How does gradient noise regulate the temporal evolution of Lipschitz continuity?
    
    %What mechanism does the regularity of noisy gradients affect the temporal evolution of Lipschitz continuity?
  
    \item Section~\ref{sec:uniform_label_noise}: \textbf{Uniform label corruption}. How does uniform label corruption implicitly regularize the dynamics of Lipschitz continuity?

    \item  Section~\ref{sec:effect_batch_size}: \textbf{Batch size}. What role does batch size play in shaping the temporal evolution of Lipschitz continuity?
      
    \item Section~\ref{sec:sampling_trajectory}: \textbf{Mini-batch sampling trajectory}. What impact does mini-batch sampling have on the temporal evolution of Lipschitz continuity?

    % \item \textbf{Effect of correlation in neurons}. How do correlations between neurons affect Lipschitz continuity?

\end{enumerate}





\begin{figure}[t]
    \centering

  %
  \begin{minipage}[t]{0.48\textwidth}
    \begin{figure}[H]
      \centering
      \includegraphics[width=\linewidth]{effect_dataseed.pdf}
      \caption[Predicted Effect of Trajectory in Mini-Batch Sampling on Lipschitz Continuity]{Predicted effect of the trajectory in mini-batch sampling on Lipschitz continuity. The inset plot zooms in on $50$ steps at $t=23000$.} %where the Lipschitz constant variance among all trajectories $\abs{\Delta K} \leq 1.4\times 10^{-2}$.
      \label{fig:effect_trajectories}
    \end{figure}
  \end{minipage}
  \hfill
  %
  \begin{minipage}[t]{0.48\textwidth}
    \begin{figure}[H]
      \centering
      \includegraphics[width=\linewidth]{effect_batchsize.pdf}
      \caption[Predicted Effect of Batch Size on Variance of Lipschitz Continuity]{Predicted effect of batch size on the variance of Lipschitz continuity.}
      \label{fig:effect_batchsize}
    \end{figure}
  \end{minipage}

  %
  \begin{minipage}[t]{0.48\textwidth}
    \begin{figure}[H]
      \centering
      \includegraphics[width=\linewidth]{effect_gradscale.pdf}
      \caption[Predicted Effect of Gradient Magnitude and Perturbation]{Predicted effect of gradient magnitude and perturbation.}
      \label{fig:effect_gradmagnitude}
    \end{figure}
  \end{minipage}
  \hfill
  %
  \begin{minipage}[t]{0.48\textwidth}
    \begin{figure}[H]
      \centering
      \includegraphics[width=\linewidth]{effect_labelnoise.pdf}
      \caption[Predicted Effect of Uniform Label Corruption]{Predicted effect of uniform label corruption.}
      \label{fig:effect_labelnoise}
    \end{figure}
  \end{minipage}
  
\end{figure}




\subsection{Key factors driving dynamics}
\label{sec:key_factors}


\textbf{Principal driving factors}. Theorem~\ref{theorem:layer_dynamics} and Theorem~\ref{theorem:network_dynamics} identify four principal factors driving the evolution of Lipschitz continuity at both the layer and network levels: 
\begin{enumerate}[label=(\roman*)]
 
    \item \textbf{Gradient-principal-direction alignment}. The alignment between the gradient expectations and the principal directions of parameter matrices determines \textit{optimization-induced drift} the $\mu_Z(t)$. As shown in Figure~\ref{fig:longrange_dynamics}, this force dominates the drift of the Lipschitz continuity (see Theorem~\ref{theorem:layer_dynamics} and Theorem~\ref{theorem:network_dynamics}).

    \item \textbf{Directional gradient noise}. The directional projection of gradient fluctuations, arising from mini-batch sampling, on the principal directions of parameter matrices determines the \textit{diffusion-modulation intensity} $\lambda_Z(t)$ arises from. As shown in Figure~\ref{fig:longrange_dynamics}, this factor modulates the diffusion of the Lipschitz continuity.
    
    \item \textbf{Deterministic effect of gradient noise}. The interaction between the gradient fluctuations, arising from mini-batch sampling, and the operator-norm curvatures determines the \textit{noise-curvature entropy production} $\kappa_Z(t)$. Our theoretical framework suggests that this term gives a deterministic, non-negative, and irreversible increase contributing to the drift of the dynamics.

    \item \textbf{Gradient noise amplification effect}. Lemma~\ref{lemma:hessian_spectral_norm} and Theorem~\ref{theorem:layer_dynamics} suggest that the inverted principal spectral gaps in parameter matrices, defined as $\left[\sigma_1^{(\ell)}(t)^2 - \sigma_j^{(\ell)}(t)^2\right]^{-1}$, for all $j \neq 1$, can amplify the gradient noise. Thus smaller spectral gaps amplifies gradient noise, contributing to larger \textit{noise-curvature entropy production} $\kappa_Z(t)$.

\end{enumerate}




    




\subsection{Parameter initialization}
\label{sec:parameter_initialization}

%\textbf{Dense initialization}. 

According to Theorem~\ref{theorem:statistics_of_lipschitz}, the network initialization $K(0)$ affects both the expectation and uncertainty of Lipschitz continuity in the evolution. Suppose that the entries of a parameter $\theta^{(\ell)} \in \mathbb{R}^{m_{\ell} \times n_{\ell}}$ are sampled from $\mathcal{N}(0, s_{\ell}^2)$. According to the Tracy-Widom limiting distribution \citep{tracy1994level,tao2012topics}, the largest singular value limit is $\sigma_1^{\ell} \to (\sqrt{m_\ell} + \sqrt{n_\ell}) \cdot s_{\ell}$, if $m_\ell \cdot n_\ell$ is sufficiently large. For a network with $L$ layers, 
\begin{align}
K(0) \to \prod_{\ell=1}^{L}\left(\sqrt{m_{\ell}} + \sqrt{n_{\ell}}\right)  \cdot s_{\ell} \notag
     ,
\end{align}
hence a larger network has a larger Lipschitz continuity. For the case of Kaiming initialization, $s_{\ell} = \sqrt{\sfrac{2}{n_{\ell}}}$ \citep{he2015delving}. 


% \medskip
% \noindent
% \textbf{Sparse initialization}. Sparse initialization refers to initializing a subset of weights to near zeros, aiming to reduce initial complexity of models \citep{glorot2010understanding,gale2019state}. For example, the $K$-sparse Erd\"os-R\'enyi sparse initialization scheme \citep{mocanu2018scalable}...



    
\subsection{Unbounded growth near-convergence}
\label{sec:near_convergence}

 

Suppose a negative‐log‐likelihood loss:
\begin{align}
    \ell_f(\boldsymbol{\theta}(t); x, y) = -\log p_{\boldsymbol{\theta}(t)} (y\mid x) \notag
\end{align}
near convergence:
\begin{align}
   \ell_f(\boldsymbol{\theta}(t); x, y) \to 0 \notag
   . 
\end{align}

Under Assumption~\ref{assump:layerwise_noise}, 
the Fisher information matrix (FIM) of $p_{\boldsymbol{\theta}(t)} (y\mid x)$ with respect to parameters $\boldsymbol{\theta}^{(\ell)}(t)$ \citep{martens2020new} is defined as
\begin{align}
\label{equ:fim_approx_sigma}
    \boldsymbol{F}^{(\ell)}(t) &:= \mathbb{E} \left[
    \operatorname{vec}\left[
    \nabla^{(\ell)} p_{\boldsymbol{\theta}(t)} (y\mid x)\right] 
    \operatorname{vec}\left[
    \nabla^{(\ell)} p_{\boldsymbol{\theta}(t)} (y\mid x)\right]^\top
    \right] \approx M \cdot \boldsymbol{\Sigma}_t^{(\ell)}  \notag
    ,
\end{align}
as $\ell_f(\theta; x, y) \to 0$, where $M$ is the batch size \citep{stephan2017stochastic,li2021happens,martens2020new}. This will serve as a foundation for our later theoretical analysis of the near‐convergence dynamics.

\begin{proposition}[Unbounded Growth Near-Convergence]
Consider the terms in the dynamics (Theorem~\ref{theorem:layer_dynamics}):
\begin{gather}
\mu^{(\ell)}(t) =  \frac{1}{\sigma_{1}^{(\ell)}(t)} \left\langle \boldsymbol{J}_{op}^{(\ell)}(t), \, -\mathrm{vec}\left[ \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta}(t)) \right] \right\rangle 
\approx 0 , \notag\\
\boldsymbol{\lambda}^{(\ell)}(t) = \frac{\sqrt{\eta}}{\sigma_{1}^{(\ell)}(t)}  
\left(\left[\boldsymbol{\Sigma}_t^{(\ell)}\right]^{\frac{1}{2}}\right)^\top 
\boldsymbol{J}_{op}^{(\ell)}(t)
 \approx 
 \frac{\sqrt{\eta}}{\sigma_{1}^{(\ell)}(t)}  
\left(\left[\frac{1}{M}\boldsymbol{F}^{(\ell)}(t)\right]^{\frac{1}{2}}\right)^\top 
\boldsymbol{J}_{op}^{(\ell)}(t) 
\to \boldsymbol{0}, \notag\\
\kappa^{(\ell)}(t) =\frac{\eta}{2\sigma_{1}^{(\ell)}(t)} \left\langle \boldsymbol{H}_{op}^{(\ell)}(t),  \boldsymbol{\Sigma}_t^{(\ell)}\right\rangle
\approx
\frac{\eta}{2\sigma_{1}^{(\ell)}(t)} \frac{1}{M}\left\langle \boldsymbol{H}_{op}^{(\ell)}(t),  \boldsymbol{F}^{(\ell)}(t)\right\rangle > 0
\notag
,
\end{gather}
so that Lipschitz continuity is not bounded in expectation:
\begin{align}
\lim_{t \to \infty}
\mathbb{E}\left[K(t)\right]  
    = \lim_{t \to \infty}\mathrm{e}^{Z(0) + \int_0^t \left[ \mu_Z(s) + \kappa_Z(s)  \right] \dd s}
    = 
    \lim_{t \to \infty}
    \mathrm{e}^{Z(0) + \int_0^t \kappa_Z(s)  
    \dd s} \to \infty \notag
    ,
\end{align}
and uncertainty:
\begin{align}
\lim_{t \to \infty}
\operatorname{Var}\left[K(t)\right] 
=
\lim_{t \to \infty}
\mathbb{E}\left[K(t)\right]^2\left( e^{\operatorname{Var}\left[Z(t)\right]} - 1\right) \to \infty \notag
,
\end{align}
as $t \to \infty$. This result demonstrates that the Lipschitz continuity bound monotonically increases as optimization progresses. This phenomenon has been noted in literature \citep{miyato2018spectral,bartlett2017spectrally,sedghi2019singular,gamba2023lipschitz}.

\end{proposition}

%num_epochs:  1766
   %total_steps:  344370
   %inset: 330000 for 100 steps.
   %last train_loss:  0.009750319093179244
   %last test_loss:  2.223605284324059
   %last train_acc:  0.9999599358974359
   %last test_acc:  0.6853966346153846
   
\medskip
\noindent
\textbf{Experimental Results}. We extend the training of the five-layer ConvNet on
CIFAR-10 without regularization to
$344,370$ steps ($1766$ epochs) for observing the long range dynamics near convergence. Figure~\ref{fig:dynamics:layer} shows the layer-specific dynamics; Figure~\ref{fig:dynamics:network} shows the network-specific dynamics. The observations are as follows:
\begin{enumerate}[label=(\roman*)]

    \item \textbf{Unbounded growth}. We train the network for up to $344,370$ steps, near convergence. The gradual increase driven by $\kappa_Z(t)$ persists throughout the training, with no observable indication of stopping, suggesting that the dynamics do not admit a finite-time steady state.

    \item \textbf{Non-negligible contribution of gradient noise}. Although the magnitude of $\kappa_Z(t)$ is typically one order smaller than that of $\mu_Z(t)$ in our experiments, its cumulative effect on the growth of Lipschitz continuity near-convergence is non-negligible and persists throughout training.

    \item \textbf{Four Phases}. We observe that $\kappa_Z(t)$ exhibits four distinct phases: (i) phase 1 --- a rapid initial increase at the beginning of training, (ii) phase 2 --- large fluctuations prior to overfitting, (iii) phase 3 --- a steady decline, and (iv) phase 4 --- convergence to a non-negative constant.
    
\end{enumerate}




\subsection{Noisy gradient regularization}
\label{sec:noisy_gradient}




Prior work shows that injecting noise into gradients during training can improve robustness \citep{welling2011bayesian} and help escape local minima \citep{neelakantan2015adding}. Our theoretical framework elucidates the mechanism by which gradient noise serves as a regularizer for Lipschitz continuity. Consider a loss $\ell_*$ with noisy supervision consists of a signal loss $\ell_f$ and a noisy loss $\ell_n$:
\begin{align}
\label{equ:noisy_loss}
    \ell_*(\boldsymbol{\theta};x,y) = \sqrt{\rho} \cdot  \ell_f(\boldsymbol{\theta};x,y) + 
    \sqrt{1-\rho} \cdot \ell_n(\boldsymbol{\theta};x,y) ,
\end{align}
where $\rho \in [0, 1]$. The corresponding batch loss is:
\begin{align}
    \label{equ:noisy_loss_nabla}
    \nabla^{(\ell)} \mathcal{L}_*(\boldsymbol{\theta};\xi) = \sqrt{\rho} 
    \cdot \nabla^{(\ell)} \mathcal{L}_f(\boldsymbol{\theta};\xi) + 
    \sqrt{1-\rho} \cdot \nabla^{(\ell)} \mathcal{L}_n(\boldsymbol{\theta};\xi), %\notag
\end{align}
and the gradient noise covariance is:
\begin{align}
    \label{equ:noisy_loss_sigma}
    \Sigma^{(\ell),*} = \rho \cdot \Sigma^{(\ell),f} + (1-\rho) \cdot \Sigma^{(\ell),n} %\notag
    .
\end{align}
If the noise is sampled from $\mathcal{N}(0, \sigma^2)$, $\Sigma^{(\ell),n} = \sigma^2\;\mathrm{I}$, the dynamics has the changes:
\begin{gather}
\mu_*^{(\ell)}(t) =  \sqrt{\rho} \mu^{(\ell)}(t)  \notag
, 
\end{gather}
and
\begin{align}
\kappa_*^{(\ell)}(t) &= \rho \cdot \kappa^{(\ell)}(t) + 
(1 -\rho) \cdot \frac{\eta}{2\sigma_{1}^{(\ell)}(t)} 
\underbrace{
\left\langle \boldsymbol{H}_{op}^{(\ell)}(t),  \sigma^2\; \mathrm{I} \right\rangle 
}_{\text{variance is negligible}}
\approx \rho \cdot \kappa^{(\ell)}(t) \notag
.
\end{align}
The variance contribution from $\boldsymbol{H}_{op}^{(\ell)}(t)$ is neglected, as experimental results indicate it is negligible (see Figure~\ref{fig:longrange_dynamics}). According to Theorem~\ref{theorem:statistics_of_lipschitz}, by ignoring $\lambda_Z(t)$, we have:
\begin{align}
\label{equ:gradient_magnitude}
\mathbb{E}\left[K(t)\right]  
    \approx \mathrm{e}^{Z(0) + \int_0^t  \sqrt{\rho} \cdot \mu_Z(s)  \dd s + \int_0^t  \rho \cdot \kappa_Z(s)  \dd s}
    = 
    K(0)\left[ \mathrm{e}^{\int_0^t  \mu_Z(s)  \dd s} \right]^{\sqrt{\rho}} \left[ \mathrm{e}^{\int_0^t  \kappa_Z(s)  \dd s} \right]^{\rho}
    .
\end{align}


Although the integrals $\int_0^t \mu_{Z}(s) \dd s$ and $\int_0^t \kappa_{Z}(s) \dd s$ are unlikely to be computed --- without the structural information of the noisy supervision regarding Equation (\ref{equ:noisy_loss}), (\ref{equ:noisy_loss_nabla}) and (\ref{equ:noisy_loss_sigma}), it provides insight how gradient magnitude affects the evolution of Lipschitz continuity bound. This result shows higher gradient magnitude leads larger Lipschitz continuity bound. This framework can be used to analyze the uniform label corruption (see Section~\ref{sec:uniform_label_noise}).



\medskip
\noindent
\textbf{Experimental Results}. We train a MLP (see Table~\ref{tab:network_config_mlp}) on the MNIST with a batch size of $128$ and a learning rate of $0.01$, using SGD without momentum. During training, the gradients are scaled by $\sqrt{\rho}$, and additive noise is injected sampled from: (i) a Gaussian distribution $\mathcal{N}(0, 1)$; (ii) a uniform distribution $U[-0.5, 0.5]$; and (iii) zero noise, scaled by $\sqrt{1 - \rho}$. As shown in Figure~\ref{fig:effect_gradmagnitude}, the Lipschitz constant decreases monotonically as $\rho$ decreases.


\subsection{Uniform label corruption}
\label{sec:uniform_label_noise}
Suppose a classifier is trained with a negative-log-likelihood loss function $\ell_f(\theta;x,y):= -\log p_{\theta}(y|x)$. Further suppose that the label corruption probability is $\epsilon \in [0, 1]$ with a uniform distribution $U(\mathcal{Y})$, while the label remains intact with a probability $1-\epsilon$. Therefore the gradient with label corruption can be expressed as \citep{natarajan2013learning,patrini2017making,ghosh2017robust}:
\begin{align}
 \mathbb{E}\left[
 \nabla^{(\ell)} 
 \ell_f(\theta;x,y)
 \right]
 &:= 
 (1-\epsilon)\cdot 
 \mathbb{E}_{x,y}\left[\nabla^{(\ell)} 
 \left[-\log p_{\theta}(y|x)\right] 
 \right]
 \notag\\
 &\qquad\qquad
 +\epsilon \cdot 
 \mathbb{E}_x\left[
 \nabla^{(\ell)}
 \frac{1}{|\mathcal{Y}|}\sum_{ \Tilde{y} \sim U(\mathcal{Y}) }
 \left[-\log p_{\theta}(\Tilde{y}|x)\right]
 \right]
 ,
 \notag
\end{align}
where $\Tilde{y} \sim U(\mathcal{Y}) $. The literature on this topic \citep{natarajan2013learning,ghosh2017robust} assumes that the loss component with label noise contributes only a constant, hence zero gradient:
\begin{align}
\langle 
\boldsymbol{J}_{op}^{(\ell)}(t), \operatorname{vec}\left[ -\nabla^{(\ell)} \mathbb{E}_{x,\Tilde{y}}\left[ -\log p_{\theta}(\Tilde{y}|x) \right]\right]
\rangle
\to 0. \notag
\end{align}

According to Equation~\ref{equ:noisy_loss}, we can treat the label noise as $\ell_n$. By using Equation~\ref{equ:gradient_magnitude}, note $\rho = (1-\epsilon)^2$, then we have:
\begin{align}
\mathbb{E}\left[ K'(t)\right] \approx K(0) \cdot \left[ \mathrm{e}^{\int_0^t \mu_Z(s) \dd s} \right]^{1-\epsilon} 
\cdot \left[ \mathrm{e}^{\int_0^t \kappa_Z(s) \dd s} \right]^{(1-\epsilon)^2}
\notag
.
\end{align}

%We can conclude that larger noise levels lead smaller Lipschitz bounds.

\medskip
\noindent
\textbf{Experimental Results}. We train a MLP (see Table~\ref{tab:network_config_mlp}) on the MNIST with a batch size of $128$ and a learning rate of $0.01$, using SGD without momentum. We inject uniform label noise into the dataset with a level from $0$ to $1$. As shown in Figure~\ref{fig:effect_labelnoise}, the Lipschitz constant decreases monotonically as label noise level increases.

\subsection{Batch size}
\label{sec:effect_batch_size}

Suppose that the batch size $M$ in mini-batch sampling affects only the gradient noise $\Sigma(t)$, and does not affect the expectations of gradients $\nabla \mathcal{L}_f(\theta)$. Therefore, the batch size $M$ affects only the diffusion term (Theorem~\ref{theorem:statistics_of_lipschitz}). We analyze the effect of mini-batch size.

\begin{proposition}[Uncertainty Under Large Batch]
\label{proposition:effect_batch_size}
Let the batch size be $M$ and sufficiently large, then:
\begin{align}
\mathrm{Var}\left[ K(t) \right] 
&\approx \mathbb{E}\left[K(t)\right]^2 \frac{C}{M} ,\notag
\end{align}
where $C$ is a constant given as:
\begin{align}
C=
\displaystyle\int_0^t \sum_{l=1}^{L}  \frac{\eta}{\sigma_1^{(\ell)} (t)^2} \boldsymbol{J}_{op}^{(\ell)}(t)  \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x, y) \right)\right]\boldsymbol{J}_{op}^{(\ell)}(t)^\top \, \dd s     \notag
\end{align}
\end{proposition}
\begin{proof}
    
Substitute Equation~\ref{equ:batch_gradient_noise} into Theorem~\ref{theorem:statistics_of_lipschitz}:
\begin{align}
    \mathrm{Var}\left[ Z(t) \right] &= \displaystyle\int_0^t \lambda_Z(s)^2 \, \dd s = \displaystyle\int_0^t \sum_{\ell=1}^{L} \|\boldsymbol{\lambda}^{(\ell)}(s)\|_2^2 \, \dd s = \displaystyle\int_0^t \sum_{l=1}^{L}  \frac{\eta}{\sigma_1^{(\ell)}(t)^2} \boldsymbol{J}_{op}^{(\ell)}(t) \boldsymbol{\Sigma}^{(\ell)}(t) \boldsymbol{J}_{op}^{(\ell)}(t)^\top \, \dd s \notag \\
    &= \displaystyle\int_0^t \sum_{l=1}^{L}  \frac{\eta}{\sigma_1^{(\ell)}(t)^2} \boldsymbol{J}_{op}^{(\ell)}(t)  
    \frac{1}{M} \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x, y) \right)\right]
    \boldsymbol{J}_{op}^{(\ell)}(t)^\top \, \dd s \notag\\
    &= \frac{1}{M} 
    \underbrace{
    \displaystyle\int_0^t \sum_{l=1}^{L}  \frac{\eta}{\sigma_1^{(\ell)} (t)^2} \boldsymbol{J}_{op}^{(\ell)}(t)  \mathrm{Var}\left[ \mathrm{vec}\left(\nabla^{(\ell)} \ell_f(\boldsymbol{\theta}(t); x, y) \right)\right]\boldsymbol{J}_{op}^{(\ell)}(t)^\top \, \dd s 
    }_{\text{a constant}}
     =  \frac{1}{M} C . \notag
\end{align}

Hence:
\begin{align}
\mathrm{Var}\left[ K(t) \right] &= \mathbb{E}\left[K(t)\right]^2\left(\mathrm{e}^{\mathrm{Var}\left[ Z(t) \right]} - 1\right) =\mathbb{E}\left[K(t)\right]^2\left(\mathrm{e}^{\frac{C}{M}} - 1\right) \notag
.
\end{align}

Suppose $M \to \infty$:
\begin{align}
\mathrm{Var}\left[ K(t) \right] &=\mathbb{E}\left[K(t)\right]^2\left(\mathrm{e}^{\frac{C}{M}} - 1\right) \approx \mathbb{E}\left[K(t)\right]^2 \left(1 + \frac{C}{M} - 1\right)  =\mathbb{E}\left[K(t)\right]^2 \frac{C}{M} 
\approxprop \frac{1}{M} \notag
.
\end{align}

\end{proof}
%

\medskip
\noindent
\textbf{Experimental Results}. We train the five-layer ConvNet (Table~\ref{tab:network_config_cnn} in the Appendix), optimized with SGD without momentum. The batch size is varied from $32$ to $384$ in increments of $32$, and each configuration is trained for $39{,}000$ steps. During training, we profile and collect the dynamics to compute the uncertainty of Lipschitz continuity $\mathrm{Var}\left[K(t)\right]$. As shown in Figure~\ref{fig:effect_batchsize}, the observed effect of batch size aligns closely with the theoretical prediction in Proposition~\ref{proposition:effect_batch_size}.

\subsection{Mini-batch sampling trajectory}
\label{sec:sampling_trajectory}

According to Proposition~\ref{proposition:effect_batch_size}, if the batch size is sufficiently large, the effect from various mini-batch sampling trajectories can be neglected since:
\begin{align}
\mathrm{Var}\left[ K(t) \right] \approx \mathbb{E}\left[K(t)\right]^2 \frac{C}{M} 
 \to 0 \notag
,
\end{align}
as batch size $M$ is sufficiently large.


\medskip
\noindent
\textbf{Experimental Results}. We train the five-layer ConvNet (Table~\ref{tab:network_config_cnn} in the Appendix), optimized with SGD without momentum. The parameter initialization random seed is fixed to $1$, while the random seed for mini-batch sampling is varied from $1$ to $5$. As shown in Figure~\ref{fig:effect_trajectories}, the sampling trajectories have a negligible effect on the evolution of Lipschitz continuity.





\section{Limitations and future work}


While our mathematical framework shows strong agreement with empirical results, it has several limitations:
\begin{enumerate}
    \item \textbf{Layer-wise noise assumption}. The simplification in Assumption~\ref{assump:layerwise_noise} neglects inter-layer interactions among neurons; this may pose as a challenging for studying large models.
    
    \item \textbf{Distributional assumption}. We assume that the gradient noise follows a time-state-dependent normal distribution varying smoothly. However, this assumption may not hold for small batch sizes, where the noise distribution can deviate significantly from Gaussian.
    
    \item \textbf{Continuous–discrete error}. Our framework models gradient dynamics in continuous time, whereas SGD operates in discrete steps. This discrepancy may introduce non-negligible errors, particularly when modeling long-range dynamics.
\end{enumerate}


\section{Conclusions}

We present a mathematical framework that models the dynamics of Lipschitz continuity in neural networks through a system of SDEs. This theoretical framework not only identifies the key factors governing the evolution of Lipschitz continuity, but also provides insight into how it is implicitly regularized during training. Beyond its analytical value, the framework offers a foundation for future research and development. Our experiments further validate the effectiveness of the proposed framework and the predicted effects of the theoretical implications.



% \section*{Impact Statement}

% We believe that this work represents a significant advancement in the field of robustness research. To the best of our knowledge, it introduces the first mathematical framework that rigorously models the temporal evolution of Lipschitz continuity in neural networks. This framework establishes foundations for future research in trustworthy machine learning. Furthermore, its profound connection to principles of physics implies the manifestation of natural laws, opening new avenues for exploration.





==> main_matter/chapters/OptimizationInducedDynamics/tikz/optimization_induced_dynamics_subfig.tex <==

\begin{minipage}[t]{0.4\linewidth}
    \subfloat[Optimization trajectories in loss landscape]{
      \begin{tikzpicture}
        \pgfmathsetmacro{\trajectoryscalefactor}{1.5}
        
        \node[inner sep=0pt, opacity=0.7] (loss) at (0, 0) {
          \includegraphics[trim={0.4cm 0.5cm 0.3cm 0.25cm},clip,width=1\linewidth]
            {plots/loss_landscape_network_cnn_epoch_0.pdf}
        };

        % trajectory A
        % \coordinate (start) at (0.28, 0.15); 
        % \coordinate (A1) at (0.6, 0.3);  
        % \coordinate (A2) at (0.9, 0.6);   
        % \coordinate (A3) at (0.8, 0.9);  
        % \coordinate (A4) at (0.7, 1.0);  
        % \coordinate (A5) at (0.6, 1.2);  

        \coordinate (start) at ($(\trajectoryscalefactor*0.28,\trajectoryscalefactor*0.15)$);
        \coordinate (A1)    at ($(\trajectoryscalefactor*0.6, \trajectoryscalefactor*0.3)$);
        \coordinate (A2)    at ($(\trajectoryscalefactor*0.9, \trajectoryscalefactor*0.6)$);
        \coordinate (A3)    at ($(\trajectoryscalefactor*0.8, \trajectoryscalefactor*0.9)$);
        \coordinate (A4)    at ($(\trajectoryscalefactor*0.7, \trajectoryscalefactor*1.0)$);
        \coordinate (A5)    at ($(\trajectoryscalefactor*0.6, \trajectoryscalefactor*1.2)$);


        \draw[lime, dashed, thick, -latex] 
          (start) -- (A1) -- (A2) -- (A3) -- (A4) -- (A5);


        % trajectory B
        % \coordinate (startB) at (0.28, 0.15); 
        % \coordinate (B1) at (-0.1, 0.6);  
        % \coordinate (B2) at (-0.3, 0.5);  
        % \coordinate (B3) at (-0.4, 0.3); 
        % \coordinate (B4) at (-0.5, 0.1); 
        % \coordinate (B5) at (-0.8, 0); 
        % \coordinate (B6) at (-1.0, 0); 

       % trajectory B (with dynamic scaling)
        \coordinate (startB) at ($(\trajectoryscalefactor*0.28,\trajectoryscalefactor*0.15)$);
        \coordinate (B1)     at ($(\trajectoryscalefactor*-0.1, \trajectoryscalefactor*0.6)$);
        \coordinate (B2)     at ($(\trajectoryscalefactor*-0.3, \trajectoryscalefactor*0.5)$);
        \coordinate (B3)     at ($(\trajectoryscalefactor*-0.4, \trajectoryscalefactor*0.3)$);
        \coordinate (B4)     at ($(\trajectoryscalefactor*-0.5, \trajectoryscalefactor*0.1)$);
        \coordinate (B5)     at ($(\trajectoryscalefactor*-0.8, \trajectoryscalefactor*0.0)$);
        \coordinate (B6)     at ($(\trajectoryscalefactor*-1.0, \trajectoryscalefactor*0.0)$);
         
        \draw[lime, dashed, thick, -latex] 
          (startB) -- (B1) -- (B2) -- (B3) -- (B4) -- (B5) -- (B6);

        \node[scale=0.8, color=lime] at (0.5, 0) {$\theta_0$};
        
        \node[scale=0.8, color=lime] at ($(\trajectoryscalefactor*0.6, \trajectoryscalefactor*1.4)$) {$\theta_A$};

        \node[scale=0.8, color=lime] at ($(\trajectoryscalefactor*-1.2, \trajectoryscalefactor*0)$) {$\theta_B$};
        
      \end{tikzpicture}\label{subfig:loss_landscape}
    }
  \end{minipage}
  \hspace{0.03\linewidth}
  \begin{minipage}[t]{0.4\linewidth}
    \subfloat[Induced trajectories in Lipschitz landscape]{
      \begin{tikzpicture}
        \pgfmathsetmacro{\trajectoryscalefactor}{1.5}
        
        \node[inner sep=0pt, opacity=0.7] (lipschitz) at (0, 0) {
          \includegraphics[trim={0.4cm 0.5cm 0.3cm 0.25cm},clip,width=1\linewidth]
            {plots/lipschitz_landscape_network_cnn_epoch_0.pdf}
        };

        % trajectory A
        \coordinate (start) at ($(\trajectoryscalefactor*0.28,\trajectoryscalefactor*0.15)$);
        \coordinate (A1)    at ($(\trajectoryscalefactor*0.6, \trajectoryscalefactor*0.3)$);
        \coordinate (A2)    at ($(\trajectoryscalefactor*0.9, \trajectoryscalefactor*0.6)$);
        \coordinate (A3)    at ($(\trajectoryscalefactor*0.8, \trajectoryscalefactor*0.9)$);
        \coordinate (A4)    at ($(\trajectoryscalefactor*0.7, \trajectoryscalefactor*1.0)$);
        \coordinate (A5)    at ($(\trajectoryscalefactor*0.6, \trajectoryscalefactor*1.2)$);


        \draw[lime, dashed, thick, -latex] 
          (start) -- (A1) -- (A2) -- (A3) -- (A4) -- (A5);

        %\node[scale=0.5, color=lime] at ($(\trajectoryscalefactor*0.6, \trajectoryscalefactor*1.3)$) {A};

        % trajectory B
        \coordinate (startB) at ($(\trajectoryscalefactor*0.28,\trajectoryscalefactor*0.15)$);
        \coordinate (B1)     at ($(\trajectoryscalefactor*-0.1, \trajectoryscalefactor*0.6)$);
        \coordinate (B2)     at ($(\trajectoryscalefactor*-0.3, \trajectoryscalefactor*0.5)$);
        \coordinate (B3)     at ($(\trajectoryscalefactor*-0.4, \trajectoryscalefactor*0.3)$);
        \coordinate (B4)     at ($(\trajectoryscalefactor*-0.5, \trajectoryscalefactor*0.1)$);
        \coordinate (B5)     at ($(\trajectoryscalefactor*-0.8, \trajectoryscalefactor*0.0)$);
        \coordinate (B6)     at ($(\trajectoryscalefactor*-1.0, \trajectoryscalefactor*0.0)$);
         
        \draw[lime, dashed, thick, -latex] 
          (startB) -- (B1) -- (B2) -- (B3) -- (B4) -- (B5) -- (B6);

        %\node[scale=0.5, color=lime] at ($(\trajectoryscalefactor*-1.1, \trajectoryscalefactor*0)$) {B};

        \node[scale=0.8, color=lime] at (0.5, 0) {$K_0$};
        
        \node[scale=0.8, color=lime] at ($(\trajectoryscalefactor*0.6, \trajectoryscalefactor*1.4)$) {$K_A$};

        \node[scale=0.8, color=lime] at ($(\trajectoryscalefactor*-1.2, \trajectoryscalefactor*0)$) {$K_B$};
      \end{tikzpicture}\label{subfig:lipschitz_landscape}
    }
  \end{minipage}


==> main_matter/chapters/PerturbationAnalysis/text.tex <==
\section{Introduction}


\lettrine[lines=3]{S}{ingular} values lie at the core of modern matrix analysis, encapsulating key spectral information such as \emph{operator norm}, \emph{conditioning}, \emph{effective rank}, and underpinning applications across numerical linear algebra, data science, control theory, and mathematical physics \citep{edelman2005random,yosida2012functional,horn2012matrix,tao2012topics}. In random matrix theory, singular values govern limiting laws such as Marchenko--Pastur distributions \citep{MarcenkoPastur1967}, edge fluctuations described by Tracy--Widom laws \citep{tracy1994level}, and fine-scale local statistics such as local eigenvalue spacings \citep{edelman2005random}. In physics and deep learning, higher-order derivatives of singular values are indispensable for rigorous analysis in stochastic dynamical settings, where systems are subject to noise and random perturbations \citep{oksendal2013stochastic}. 

For example, let $\boldsymbol{\theta}_t \in \mathbb{R}^{m \times n}$ be a continuous matrix with $r$ non-zero singular values $\sigma_1,\sigma_2,\ldots,\sigma_r$ with respect to time $t$. Assume that its dynamics are characterized by an adapted It\^o process \citep{ito1951stochastic}
\begin{align}
    \dd \mathrm{vec}(\boldsymbol{\theta}_t) 
    = G_t \dd t 
      + D_t \dd W_t,
\end{align}
where $\mathrm{vec}(\cdot)$ denotes the vectorization operator, $G_t \in \mathbb{R}^{mn}$ is the \emph{drift term}, $D_t \in \mathbb{R}^{mn \times mn}$ is the \emph{diffusion coefficient}, and $\dd W_t$ is a high-dimensional Wiener process in $\mathbb{R}^{mn}$. Let
\begin{align}
\phi_t = \phi(\sigma_1,\sigma_2,\ldots,\sigma_r)(t)    
\end{align}
denote a spectral functional of the singular values of $\boldsymbol{\theta}_t$, then applying It\^o's lemma shows that the rigorous analysis of the spectral dynamics of $\dd \phi_t$ requires the second-order derivatives of singular values \citep{oksendal2013stochastic}. Such induced dynamics arise naturally in both physics and deep learning. In physics, the \emph{von Neumann entropy} --- a measure of the statistical uncertainty within a quantum system --- is a spectral functional of singular values \citep{fano1957description}, and widely used in the study of quantum entanglement \citep{nielsen2010quantum}. In deep learning, the Lipschitz continuity of neural networks is a spectral functional of the largest singular value \citep{luo2025lipschitz}. For more general non-Gaussian drivers in stochastic dynamics, such as L\'evy processes, higher-order derivatives of singular values are indispensable for rigorous analysis and for deriving sharp bounds \citep{applebaum2009levy}.


%challenges
Although first-order derivatives of singular values are well known in the literature \citep{StewartSun1990}, explicit closed-form expressions for second- and higher-order derivatives are largely absent from the literature. A unified, highly procedural, and systematic framework for their derivation has been lacking, since direct approaches via matrix analysis are challenging due to the intricate interplay among local spectral structures (\eg, spectral gaps), left and right singular subspaces, and the associated null spaces.



To bridge this gap, we present an operator-theoretic framework for deriving arbitrary higher-order derivatives of singular values in a highly procedural approach. Our approach treats matrices as bounded linear operators on Hilbert spaces and extends Kato's analytic perturbation theory \citep{kato1995perturbation} beyond the self-adjoint setting. The key step is to embed a non-self-adjoint real rectangular matrix into a self-adjoint operator via the Jordan–Wielandt embedding (\ie, Hermitian dilation trick) \citep{StewartSun1990,shalit2021dilation}. We then analyze the asymptotic expansions of the resulting eigenvalues by extending Kato's results in eigenvalue expansions, relate these eigenvalue expansions to Fr\'echet derivatives of singular values, and express the Fr\'echet derivative tensors with Kronecker-product representation.


\subsection{Perturbation Theory}

Classical perturbation theory has developed along several independent traditions. For example, \textbf{analytic operator-theoretic perturbation theory} \citep{rellich1969perturbation,kato1995perturbation} treats holomorphic families of operators on Banach or Hilbert spaces, using resolvents, Riesz projectors, and contour integrals to prove the existence of analytic eigenvalue and eigenspace branches and to derive expansion formulas, including trace identities for eigenvalue clusters. \textbf{Matrix perturbation theory} \citep{StewartSun1990,horn2012matrix} focuses on the finite-dimensional case and derives explicit perturbation formulas via algebraic tools such as characteristic polynomials, Schur forms, and Sylvester equations, typically without explicitly invoking the operator-theoretic machinery. \textbf{Rayleigh--Schr\"odinger perturbation theory} \citep{rayleigh1896theory,schrodinger1926quantisierung,sakurai2020modern} in quantum mechanics provides basis-dependent expansions in terms of matrix elements and energy gaps; these coincide with the analytic expansions under discreteness and gap assumptions, but are often presented in physics as formal series rather than within Kato’s framework. Despite their differences in tool and emphasis, these frameworks are mathematically consistent and recover the same perturbative corrections in overlapping regimes.



\begin{figure}[t!]
    \centering
    
    \resizebox{0.75\linewidth}{!}{
      \input{spectral_analysis_framework}
    }
    
    %\setlength{\abovecaptionskip}{2.5ex}  
    %\setlength{\belowcaptionskip}{2ex}

    \caption[Theoretical Framework for Infinitesimal Spectral Variations]{\textbf{Theoretical Framework for Infinitesimal Spectral Variations}. We employ Kato's analytic perturbation theory for self-adjoint operators \citep{kato1995perturbation}. For a rectangular matrix $A$, we construct its Jordan--Wielandt embedding (Theorem~\ref{theorem:Jordan_Wielandt_relation}), a block self-adjoint operator that encodes perturbations across all subspaces (\ie, left-singular, right-singular, left-null, and right-null). Applying Kato's asymptotic eigenvalue expansions to this embedding, together with the residue theorem to simplify, yields an $n$-th order expansion of the singular values of $A$. This expansion is then related to Fr\'echet derivatives. Finally, by specializing and mapping into explicit matrix-layout conventions, we obtain a systematic procedure for deriving arbitrary-order singular-value derivatives of rectangular matrices.}
    
    \label{fig:framework_of_spectral_analysis}

\end{figure}

\subsection{Schematic Overview}
\label{sec:schematic_overview}



A schematic overview of the framework is illustrated in Figure~\ref{fig:framework_of_spectral_analysis}. To apply Kato's framework for self-adjoint operators, we first embed a non-self-adjoint $A \in \mathbb{R}^{m \times n}$ (since $A \neq A^\top$) into a self-adjoint operator $\mathcal{T}$ using the Jordan–Wielandt embedding (\ie, Hermitian dilation) \citep{StewartSun1990,edelman2005random,li2005note,horn2012matrix,shalit2021dilation}, taking:
\begin{align}
\mathcal{T} :=
\begin{bmatrix}
        O & A \\
        A^\top & O
\end{bmatrix}
\in \mathbb{R}^{(m+n)\times(m+n)}.
\end{align}
It is immediate that $\mathcal{T}$ is self-adjoint, since:
\begin{align}
    \mathcal{T}^\top
    =
    \begin{bmatrix}
        O & A \\
        A^\top & O
    \end{bmatrix}^\top
    =
    \begin{bmatrix}
        O & A \\
        A^\top & O
    \end{bmatrix}
    = \mathcal{T}.
\end{align}

This embedding preserves the complete information regarding the spectrum of $A$. The spectrum of $A$ is stated in Theorem~\ref{theorem:full_svd}~(\nameref{theorem:full_svd}), and the spectrum of $\mathcal{T}$ relates to the spectral structure of $A$ as stated in Theorem~\ref{theorem:Jordan_Wielandt_relation}~(\nameref{theorem:Jordan_Wielandt_relation}).


\begin{theorem}[Matrix Singular Value Decomposition (Full Form)]
\label{theorem:full_svd}
Let $A \in \mathbb{R}^{m \times n}$ be a real rectangular matrix. Then $A$ admits a full singular value decomposition (SVD) \citep{horn2012matrix,StewartSun1990} by:
\begin{align}
    A &= U \Sigma V^\top, \\[4pt]
    U &= \bigl[\, U_r \;\; U_0 \,\bigr] \in \mathbb{R}^{m \times m}, 
    \qquad 
    V = \bigl[\, V_r \;\; V_0 \,\bigr] \in \mathbb{R}^{n \times n}, \\[4pt]
\Sigma &=
\left[
\begin{array}{c:c}
\begin{array}{cccc}
\sigma_1 &        &        &        \\
         & \sigma_2 &      &        \\
         &        & \ddots &        \\
         &        &        & \sigma_r
\end{array}
& 
\begin{array}{c}
\; \vcenter{\hbox{$O_{\,r\times (n-r)}$}} \;
\end{array}
\\ \hdashline
\begin{array}{c}
\; \vcenter{\hbox{$O_{\, (m-r)\times r}$}} \;
\end{array}
&
\begin{array}{c}
\; \vcenter{\hbox{$O_{\, (m-r)\times (n-r)}$}} \;
\end{array}
\end{array}
\right],
\end{align}
where $\sigma_1 \geq \sigma_2 \geq \cdots \geq \sigma_r > 0$ are the non-zero singular values,
$U_r \in \mathbb{R}^{m \times r}$ and $V_r \in \mathbb{R}^{n \times r}$ contain the corresponding left and right singular vectors, and 
$U_0$ and $V_0$ span the left and right null spaces of $A$, respectively.     
\end{theorem}

%calkin2022fractal
\begin{theorem}[Spectrum of Jordan–Wielandt Embedding]
\label{theorem:Jordan_Wielandt_relation}
The singular values of $A \in \mathbb{R}^{m \times n}$ and the spectrum (\ie, eigenvalues) $\sigma(\mathcal{T})$ of its Jordan–Wielandt embedding %\citep{StewartSun1990,li2005note,bai2010spectral,horn2012matrix,shalit2021dilation}
:
\begin{align}
\mathcal{T} :=
\begin{bmatrix}
        O & A \\
        A^\top & O
\end{bmatrix}
\in \mathbb{R}^{(m+n)\times(m+n)}
\end{align}
are directly related. If $A$ admits a SVD as stated in Theorem~\ref{theorem:full_svd}, the singular values of $A$ relates to the eigenvalues of $T$ by:
\begin{align}
    \mathcal{T} \left(\frac{1}{\sqrt{2}}
    \begin{bmatrix} u_i \\ v_i \end{bmatrix}
    \right)= \sigma_i \left(\frac{1}{\sqrt{2}}
    \begin{bmatrix} u_i \\ v_i \end{bmatrix}\right),
\end{align}
and:
\begin{align}
\mathcal{T} 
    \left(\frac{1}{\sqrt{2}}
    \begin{bmatrix} u_i \\ -v_i \end{bmatrix}
    \right)
    = -\sigma_i 
    \left(\frac{1}{\sqrt{2}}
    \begin{bmatrix} u_i \\ -v_i \end{bmatrix}
    \right)
    ,
\end{align}
respectively, where the factor $\tfrac{1}{\sqrt{2}}$ ensures normalization and hence orthonormality of the eigenvectors. Thus, each singular value $\sigma_i$ of $A$ corresponds to a pair of eigenvalues:
\begin{align}
    \lambda_i^{(+)} = \sigma_i, \qquad \lambda_i^{(-)} = -\sigma_i,
\end{align}
with eigenvectors constructed directly from the singular vector pair $(u_i,v_i)$. The null spaces are also preserved in this embedding:
\begin{align}
\ker(\mathcal{T})
= \left\{
\begin{bmatrix} u_j \\ 0 \end{bmatrix} 
: u_j \in \ker(A^\top)\right\}
  \oplus
  \left\{
  \begin{bmatrix} 0 \\ v_k \end{bmatrix} 
  : v_k \in \ker(A)\right\}
  .
\end{align}
\end{theorem}

%calkin2022fractal,StewartSun1990,edelman2005random,li2005note,bai2010spectral,Horn2012
\begin{remark}
The use of the Jordan–Wielandt embedding to transfer results on Hermitian eigenvalues to singular values of rectangular matrices is well-known in the literature \citep{StewartSun1990,li2005note,calkin2022fractal}. 
%For instance, \citeauthor{StewartSun1990} employ the construction in their analysis of singular-value perturbations, using it to extend Weyl–type inequalities \citep{weyl1912asymptotische,franklin2000matrix} and sensitivity bounds from Hermitian eigenvalues to singular values \citep{StewartSun1990}. \citeauthor{li2005note} also use the embedding to transfer perturbation bounds for Hermitian eigenvalues to singular values of rectangular matrices \citep{li2005note}. Similarly, \citeauthor{horn2012matrix} present the Hermitian dilation as a standard device in matrix analysis for proving variational characterizations and interlacing properties of singular values \citep{horn2012matrix}. Unlike these works, which use the Hermitian dilation mainly as a device to transfer known eigenvalue results, our framework exploits it to develop explicit operator-theoretic expansions that yield closed-form higher-order Fr\'echet derivatives of singular values.      
\end{remark}




Next, starting from the eigenvalue expansion of reduced resolvent of operator $\mathcal{T}$ and applying the residue theorem to simplify, we derive the asymptotic eigenvalue expansion of $\mathcal{T}$ up to $n$-th order under holomorphic perturbations (Theorem~\ref{thm:expansions_of_eigenvalues}). By relating the $n$-th order term of this expansion with the corresponding $n$-th order Fr\'echet derivative, we obtain explicit expressions for higher-order derivatives of singular values. Finally, we deploy the $n$-th order Fr\'echet derivative with matrix layout conventions. In particular, the first-order case ($n=1$) recovers the well-known Jacobian of singular values; while the second-order case ($n=2$) yields the singular-value Hessian with Kronecker-product representation, which has not appeared previously in the literature. By bridging the abstract operator-theoretic expansions with matrices, our framework provides a toolkit for arbitrary-order singular-value analysis.



\subsection{Contributions}

This paper makes the following contributions:
\begin{enumerate}


    \item \textbf{Spectral Variations in Rectangular Matrices}. We present an operator-theoretic framework for analyzing $n$-th order spectral variations in real rectangular matrices (see Figure~\ref{fig:framework_of_spectral_analysis}). This framework provides a \textbf{systematic procedure} for deriving higher-order derivatives of singular values in real rectangular matrices.
    

    \item \textbf{Singular-Value Hessian}. Specializing to $n=2$ yields the second-order derivative (Hessian) of singular values, expressed in a Kronecker-product representation that, to the best of our knowledge, has not appeared previously in the literature. This result is particularly essential for analysis of \textbf{induced spectral stochastic dynamics}, where second-order derivatives arise naturally in It\^o calculus for stochastic differential equations (SDEs) driven by Wiener processes.
    
\end{enumerate}



\section{Fr\'echet Derivative and Layout Convention}
\label{sec:layout_convention}

Deploying results from abstract operator theory in matrix settings requires explicit layout conventions, particularly for the representation of derivatives. Before commencing the theoretical analysis, this section introduces the conventions fundamental to our framework. Section~\ref{sec:matrix_and_svd} introduces matrix layout and the differentiability condition; Section~\ref{sec:matrix_frechet_derivative} presents general Fr\'echet derivatives for matrix-to-matrix maps together with their tensor representations; and Section~\ref{sec:matrix_functional} specializes to Fr\'echet derivatives of matrix-to-scalar functionals and their vectorized Kronecker-product representation \citep{kolda2009tensor}.


\subsection{Matrix and Spectral Decomposition}
\label{sec:matrix_and_svd}

Let
\begin{align}
    A = \begin{bmatrix}
            A_{1,1} & A_{1,2} & \cdots & A_{1,n} \\
            A_{2,1} & A_{2,2} & \cdots & A_{2,n} \\
            \vdots  & \vdots  & \ddots & \vdots  \\
            A_{m,1} & A_{m,2} & \cdots & A_{m,n}
        \end{bmatrix}
        \in \mathbb{R}^{m \times n}
\end{align}
be a real rectangular matrix of rank $r=\mathrm{rank}(A)$, where $A_{i,j}$ denotes its $(i,j)$-th entry. $A$ admits a \emph{full} SVD as stated in Theorem~\ref{theorem:full_svd}. Specially, the \emph{reduced} or \emph{truncated} SVD of $A$ is given as:
\begin{align}
    A =\sum_{k=1}^{r} \sigma_k u_k v_k^\top,
\end{align}
where $r=\rank(A)$, and $u_k$ and $v_k$ are the left and right singular vectors associated with singular value $\sigma_k > 0$. 

\begin{lemma}[Essential Matrix Identities]
\label{lemma:essential_matrix_identities}
Let $x \in \mathbb{R}$ be a scalar, and real matrices $A$, $B$, $C$ and $V$ be of such sizes that one can form their products. Then the following identities hold \citep{franklin2000matrix,horn2012matrix}:
\begin{enumerate}
    \item $\operatorname{vec}(x) = x$,
    \item $\tr(x) = x$,
    \item $\operatorname{vec}(B V A^\top) = (A \otimes B)\operatorname{vec}(V)$,
    \item $(A \otimes B)^\top = A^\top \otimes B^\top$,
    \item $\tr(ABC) = \tr(CAB) = \tr(BCA)$
    .
\end{enumerate}
\end{lemma}

\subsection{Differentiability Condition}


To ensure the existence of higher-order differentiability of non-zero singular values and associated singular vectors, we further assume that the non-zero singular values of $A \in \mathbb{R}^{m \times n}$ are simple (\ie, each non-zero singular value has multiplicity one), as stated in Assumption~\ref{assump:simple_singular_values}~(\nameref{assump:simple_singular_values}). This \emph{simplicity} assumption is essential for ensuring that non-zero singular value $\sigma_i > 0$ of $A$ and associated singular vectors $u_i$ and $v_i$ depend smoothly on the entries of $A$, in fact yielding $u_i, v_i, \sigma_i \in C^{\infty}$ (\ie~maps are infinitely continuously differentiable). Under this assumption, non-zero singular values and their associated singular vectors vary smoothly with perturbations of $A$. 


\begin{assumption}[Simplicity Assumption of Non-Zero Singular Values]
\label{assump:simple_singular_values}
We assume that the non-zero singular values of $A$ are \emph{simple}, \ie,
\begin{align}
    \sigma_i\neq\sigma_j \quad \text{for all} \quad i\neq j
    .
\end{align}
%\citep{kato1995perturbation,horn2012matrix}.
\end{assumption}

If this assumption fails, a non-zero singular value may have multiplicity greater than one; singular values then remain continuous but may fail to be differentiable at points of multiplicity, and the associated singular subspaces are well defined whereas individual singular vectors are not unique. In such settings, higher-order derivatives generally do not exist in the classical context, and analysis must instead be carried out in terms of spectral projectors or within the framework of subdifferential calculus \citep{clarke1990optimization,lewis2005nonsmooth}.




\subsection{Matrix Fr\'echet Derivative as Multilinear Operator}
\label{sec:matrix_frechet_derivative}

We regard matrix Fr\'echet derivatives as multilinear operators \citep{yosida2012functional}. A definition for general Fr\'echet differentiable real matrix-to-matrix maps and their tensor representation are in Definition~\ref{def:frechet_derivative}~(\nameref{def:frechet_derivative}). The existence and uniqueness of the Fr\'echet derivative are stated in Theorem~\ref{thm:unique-frechet}~(\nameref{thm:unique-frechet}).


\begin{definition}[$\alpha$-Times Continuously Fr\'echet Differentiable Matrix Map]
\label{def:frechet_derivative}
Let
\begin{align}
  F:\,\mathbb{R}^{m\times n}\to\mathbb{R}^{s\times t}
\end{align}
be $\alpha$-times continuously Fr\'echet differentiable (\ie, $F\in C^\alpha$) \citep{yosida2012functional,spivak2018calculus,horn2012matrix}. The $\alpha$-th Fr\'echet derivative of $F$ is a multilinear map:
\begin{align}
D^\alpha F:\;(\mathbb{R}^{m\times n})^\alpha \to \mathbb{R}^{s\times t}.
\end{align}

Writing $F_{i,j}$ for the $(i,j)$-th component of $F$ and $A_{p,q}$ for the $(p,q)$-th entry of $A$, with:
\begin{align}
1\leq i \leq s,\qquad 1\leq j \leq t,\qquad 1\leq p \leq m,\qquad 1\leq q \leq n,
\end{align}
then the $\alpha$-th derivative $D^\alpha F$ at matrix $A$ is a tensor, defined by:
\begin{align}
\bigl[D^\alpha F(A)\bigr]_{i,j\,;\,p_1 q_1\,\dots\,p_\alpha q_\alpha}
 \;=\;
 \frac{\partial^\alpha F_{i,j}(A)}{\partial A_{p_1 q_1}\cdots \partial A_{p_\alpha q_\alpha}}
 \;\in\; \mathbb{R}.
\end{align}

The action of tensor $D^\alpha F(A)$ on directions $H_1,\dots,H_\alpha \in \mathbb{R}^{m\times n}$ is obtained \emph{component-wise} by contracting tensor $D^\alpha F(A)$ with the indices on $H_1,\dots,H_\alpha$:
\begin{align}
\bigl[D^\alpha F(A)[H_1,\dots,H_\alpha]\bigr]_{i,j}
 \;=\;
 \frac{\partial^\alpha F_{i,j}(A)}{\partial A_{p_1 q_1}\cdots \partial A_{p_\alpha q_\alpha}}
 \,
 (H_1)_{p_1 q_1}\cdots (H_\alpha)_{p_\alpha q_\alpha}.
\end{align}

Moreover, for $H\in\mathbb{R}^{m\times n}$, the $F$ at $A$ admits a multivariate Taylor expansion:
\begin{align}
F(A+H)
  = \sum_{\beta=0}^{\alpha} \frac{1}{\beta!}\, D^\beta F(A)[\underbrace{H,\dots,H}_{\beta\ \text{times}}]
    + o\bigl(\|H\|^\alpha\bigr),\qquad (\|H\|\to 0),
\end{align}
where $\|\cdot\|$ is any norm on $\mathbb{R}^{m\times n}$ (\eg, the Frobenius norm).
\end{definition}


\begin{theorem}[Uniqueness of $\alpha$-Times Fr\'echet Derivative \citep{yosida2012functional,spivak2018calculus}]
\label{thm:unique-frechet}
Suppose $F \in C^{\alpha}$ is differentiable up to order $\alpha$. Then $D^{\alpha} F$ exists, is a symmetric $\alpha$-linear map, and is \emph{unique}.  That is, there is no other $\alpha $-linear operator satisfying the defining Taylor‐remainder condition. This theorem ensures the uniqueness of the derivatives of singular values under the differentiability condition, as stated in Assumption~\ref{assump:simple_singular_values}~(\nameref{assump:simple_singular_values}).
\end{theorem}





\subsection{Representation Convention for Matrix-Valued Functionals}
\label{sec:matrix_functional}


We focus on the derivatives of singular values, which are matrix-valued functionals. To obtain matrix representations to facilitate concrete applications, we specialize the general matrix-to-matrix maps of Definition~\ref{def:frechet_derivative} to matrix-valued functionals. In general, the $\alpha$-th Fr\'echet derivative is a higher-order tensor. To express such tensors in matrix form, we employ vectorization (with a \textbf{column-major convention}) together with the Kronecker-product representation \citep{kolda2009tensor,magnus2019matrix}, as established in Corollary~\ref{corollary:vectorized_kronecker_product_representation}~(\nameref{corollary:vectorized_kronecker_product_representation}). As complementary conventions, we also introduce explicit matrix layouts for the Jacobian in Section~\ref{sec:jacobian_layout}~(\nameref{sec:jacobian_layout}) and for the Hessian in Section~\ref{sec:hessian_layout}~(\nameref{sec:hessian_layout}).

\begin{corollary}[Vectorized Kronecker-Product Representation of Fr\'echet Derivative]
\label{corollary:vectorized_kronecker_product_representation}
Let
\begin{align}
    f: \mathbb{R}^{m \times n} \to \mathbb{R}
\end{align}
be $\alpha$-times continuously Fr\'echet differentiable (\ie, $f\in C^\alpha$). For directions $H_1,\dots,H_\alpha\in\mathbb{R}^{m\times n}$, the multilinear action $D^{\alpha} f$ at $A \in \mathbb{R}^{m \times n}$ is given by the Frobenius tensor inner product \citep{kolda2009tensor,magnus2019matrix}:
\begin{align}
D^\alpha f(A)[H_1,\dots,H_\alpha]
  &=
  \bigl\langle D^\alpha f(A), H_1\otimes\cdots\otimes H_\alpha \bigr\rangle \\
  &=\bigl\langle 
  \operatorname{vec}\left(D^\alpha f(A)\right),
  \operatorname{vec}\left(
  H_1\otimes\cdots\otimes H_\alpha \right)\bigr\rangle\\
  &=\operatorname{vec}\left(D^\alpha f(A)\right)^\top \operatorname{vec}\left(
  H_1\otimes\cdots\otimes H_\alpha 
  \right)
  ,
\end{align}
where $\otimes$ represents Kronecker product (\ie, tensor product) and:
\begin{align}
 \mathrm{vec}: \mathbb{R}^{m \times n} \mapsto \mathbb{R}^{mn}   
\end{align}
represents the vectorization operator with the \textbf{column-major convention} \citep{kolda2009tensor}. 
\end{corollary}

%\begin{remark}
This vectorization is particularly useful for representing arbitrary-order derivatives of matrix-valued functionals in matrix form.
%\end{remark}

\subsubsection{Representation Convention for Jacobian of Matrix-Valued Functional}
\label{sec:jacobian_layout}

Representing the Jacobian of matrix-valued functionals in matrix form is standard in the literature \citep{horn2012matrix}. For clarity, we introduce a matrix layout as a complementary representation for the Jacobian of matrix-valued functionals. Let
\begin{align}
f: \mathbb{R}^{m \times n} \mapsto \mathbb{R}  
\end{align}
be a first-order Fr\'echet differentiable functional. Then the differential of $f$ admits:
\begin{align}
    \dd f = D f(A)[\dd A]
  =\langle Df(A),\, \dd A\rangle  
  = \Bigl( \frac{\partial f}{\partial A} \Bigr)^\top \dd A
  =\tr\left[\left(\frac{\partial f}{\partial A}\right)^\top \dd A \right]
  ,
\end{align}
where $\frac{\partial f}{\partial A}$ and infinitesimal variation $\dd A \in \mathbb{R}^{m \times n}$ are piece-wisely defined as:
\begin{align}
    \frac{\partial f}{\partial A} = 
    \begin{bmatrix}
            \frac{\partial f}{\partial A_{1,1}} & \frac{\partial f}{\partial A_{1,2}} & \cdots & \frac{\partial f}{\partial A_{1,n}} \\
            \frac{\partial f}{\partial A_{2,1}} & \frac{\partial f}{\partial A_{2,2}} & \cdots & \frac{\partial f}{\partial A_{2,n}} \\
            \vdots & \vdots & \ddots & \vdots \\
            \frac{\partial f}{\partial A_{m,1}} & \frac{\partial f}{\partial A_{m,2}} & \cdots & \frac{\partial f}{\partial A_{m,n}}
        \end{bmatrix}
\end{align}
with \textbf{denominator layout convention}, and:
\begin{align}
    \dd A =\begin{bmatrix}
        \dd A_{1,1} & \dd A_{1,2} & \cdots & \dd A_{1,n} \\
        \dd A_{2,1} & \dd A_{2,2} & \cdots & \dd A_{2,n} \\
            \vdots & \vdots & \ddots & \vdots \\
        \dd A_{m,1} & \dd A_{m,2} & \cdots & \dd A_{m,n}
        \end{bmatrix}
        .
\end{align}


\subsubsection{Representation Convention for Hessian of Matrix-Valued Functional}
\label{sec:hessian_layout}

The Hessian of a matrix-valued functional is naturally a higher-order tensor; 
for instance, it is a fourth-order tensor for matrix-valued functionals \citep{kolda2009tensor}. Let
\begin{align}
    f: \mathbb{R}^{m \times n} \to \mathbb{R}
\end{align}
be a twice Fr\'echet differentiable functional. Since
\begin{align}
    D^2 f = D(Df),
\end{align}
to obtain a matrix representation of $D^2 f$, we first consider the representation layout of the first-order derivative for a matrix-to-matrix map $F: \mathbb{R}^{m \times n} \to \mathbb{R}^{s \times t}$. We then apply vectorization together with this layout to express the second-order derivatives of matrix-valued functionals in matrix form.

Let
\begin{align}
F: \mathbb{R}^{m \times n} \mapsto \mathbb{R}^{s \times t}    
\end{align}
be a first-order Fr\'echet differentiable matrix-to-matrix map. Then there exists:
\begin{align}
\frac{\partial \operatorname{vec}(F)}{\partial \operatorname{vec}(A)} \in \mathbb{R}^{p \times q}  \quad p=mn \quad \text{and} \quad q=st ,
\end{align}
piece-wisely defined as:
\begin{align}
    \frac{\partial \operatorname{vec}(F)}{\partial \operatorname{vec}(A)} &=
    \begin{pmatrix}
            \frac{\partial \operatorname{vec}(F)_{1}}{\partial \operatorname{vec}(A)_{1}} & \frac{\partial \operatorname{vec}(F)_{2}}{\partial \operatorname{vec}(A)_{1}} & \cdots & \frac{\partial \operatorname{vec}(F)_{q}}{\partial \operatorname{vec}(A)_{1}} \\
            \frac{\partial \operatorname{vec}(F)_{1}}{\partial \operatorname{vec}(A)_{2}} & \frac{\partial \operatorname{vec}(F)_{2}}{\partial \operatorname{vec}(A)_{2}} & \cdots & \frac{\partial \operatorname{vec}(F)_{q}}{\partial \operatorname{vec}(A)_{2}} \\
            \vdots & \vdots & \ddots & \vdots \\
            \frac{\partial \operatorname{vec}(F)_{1}}{\partial \operatorname{vec}(A)_{p}} & \frac{\partial \operatorname{vec}(F)_{2}}{\partial \operatorname{vec}(A)_{p}} & \cdots & \frac{\partial \operatorname{vec}(F)_{q}}{\partial \operatorname{vec}(A)_{p}}
        \end{pmatrix}
    \end{align}
by using \textbf{denominator layout convention} on $\operatorname{vec}(F)$ and $\operatorname{vec}(A)$ \citep{horn2012matrix}. Then the Hessian of the matrix-valued functional $f$ can be defined as:
\begin{align}
    \frac{\partial}{\partial \mathrm{vec}(A)} \mathrm{vec}\left( \frac{\partial f}{\partial A}\right)
\end{align}
with vectorized representation. 


\bigskip
\noindent
\textbf{Relating Vectorized Representation to $D^2 f$.}
We now relate this vectorized representation to $D^2 f$. By Corollary~\ref{corollary:vectorized_kronecker_product_representation}~(\nameref{corollary:vectorized_kronecker_product_representation}), consider:
\begin{align}
D^2 f[\dd A, \dd A] 
    &= \langle D^2 f, \dd A \otimes \dd A \rangle
    ,
\end{align}
and use the following identities from Lemma~\ref{lemma:essential_matrix_identities}~(\nameref{lemma:essential_matrix_identities}):
\begin{enumerate}
    \item $\operatorname{vec}(x) = x$,
    \item $\operatorname{vec}(B V A^\top) = (A \otimes B)\operatorname{vec}(V)$,
\end{enumerate}
then it yields:
\begin{align}
D^2 f[\dd A, \dd A] 
&= \langle D^2 f, \dd A \otimes \dd A \rangle \\
&=   
\mathrm{vec}(D^2 f)^\top \mathrm{vec}(\dd A \otimes \dd A) \\
&= \mathrm{vec}(\dd A)^\top (D^2 f)^\top \mathrm{vec}(\dd A). 
\end{align}

\noindent
Relating 
\begin{align}
    \frac{\partial}{\partial \mathrm{vec}(A)} \mathrm{vec}\left( \frac{\partial f}{\partial A}\right)
\end{align}
with $D^2 f$ yields:
\begin{align}
    D^2f = \left[\frac{\partial}{\partial \mathrm{vec}(A)} \mathrm{vec}\left( \frac{\partial f}{\partial A}\right)\right]^\top
    ,
\end{align}
such that:
\begin{align}
    D^2 f[\dd A, \dd A] = \mathrm{vec}(\dd A)^\top 
    \left[
    \frac{\partial}{\partial \mathrm{vec}(A)} \mathrm{vec}\left( \frac{\partial f}{\partial A}\right)
    \right]
    \mathrm{vec}(\dd A).
\end{align}


\section{Refined Asymptotic Eigenvalue Expansion}
\label{sec:eigenvalue_expansion}


Kato's monograph \citep{kato1995perturbation} establishes the existence of asymptotic eigenvalue expansions and, in particular, provides a closed-form expression for the \emph{weighted mean} of eigenvalue coefficients, as stated in Theorem~\ref{thm:kato_weighted_mean}~(\nameref{thm:kato_weighted_mean}). Nevertheless, Kato's formulation is expressed with an infinite summation of contour integrals involving the perturbed resolvent and does not yield explicit, constructive formulas for the individual coefficients, which limits its direct applicability in our setting. Building on the analytic foundations laid by Kato, and by employing explicit Neumann expansions of resolvents together with the residue theorem, we refine this framework to derive an \emph{explicit, closed-form formula for arbitrary-order eigenvalue coefficients} of holomorphic families of bounded self-adjoint operators. Our main result, Theorem~\ref{thm:expansions_of_eigenvalues}~(\nameref{thm:expansions_of_eigenvalues}), goes beyond Kato's weighted mean by furnishing a fully constructive representation of each eigenvalue coefficient. The overall scheme is illustrated in Figure~\ref{fig:framework_of_spectral_analysis}.

\begin{definition}[Space of Bounded Linear Operators]
\label{def:bounded_linear_operators}
Let 
\begin{align}
 \mathcal L(X) = \{\,T : X \mapsto X \mid X \text{is a Banach space and}~T \text{ is a bounded linear operator}\}   
\end{align}
be the Banach space of bounded linear operators.     
\end{definition}


%page 77
\begin{theorem}[Kato's Weighted Mean of Eigenvalue Expansions {\citep[Ch.~II, {\S}2.2]{kato1995perturbation}}]
\label{thm:kato_weighted_mean}
Let 
\begin{align}
\mathcal{T}(x) = \mathcal{T}^{(0)} + \sum_{j=1}^\infty x^j \mathcal{T}^{(j)} \;\in\; \mathcal{L}(X)
\end{align}
be a holomorphic family of bounded operators on a Banach space $X$ \citep[Ch.~II, {\S}2.1, Eq~(2.1)]{kato1995perturbation}. Suppose $\lambda^{(0)}$ is an isolated eigenvalue of $\mathcal{T}^{(0)}$ of algebraic multiplicity $m$.


\medskip
\noindent
Let
\begin{align}
R(z) = (\mathcal{T}(x) - zI)^{-1}
\end{align}
be the perturbed resolvent, let
\begin{align}
  P(x) = -\frac{1}{2\pi i} \oint_{\Gamma} R(z) dz
  ,
\end{align}
be Riesz projector, and define
\begin{align}
\widehat{\mathcal{T}}^{(n)}
= \sum_{p=1}^\infty (-1)^{p-1}
\sum_{\substack{i_1 + \cdots + i_p = n \\ i_j \ge 1}}
\frac{1}{2\pi i}\oint_\Gamma
R(z)\,\mathcal{T}^{(i_1)}\,R(z)\cdots 
R(z)\,\mathcal{T}^{(i_p)}\,R(z)\,(z-\lambda^{(0)})\,dz
,
\end{align}
where $\Gamma$ is a small contour enclosing only $\lambda^{(0)}$ and no other spectrum \citep[Ch.~II, {\S}2.1, Eq~(2.18)]{kato1995perturbation}. Then the weighted mean of the perturbed eigenvalues is:
\begin{align}
\hat{\lambda}(x) := \frac{1}{m}\,\operatorname{tr}\!\bigl(\mathcal{T}(x) P(x)\bigr),
\end{align}
admits the expansion
\begin{align}
\hat{\lambda}(x) 
= \lambda^{(0)} + \sum_{n=1}^\infty x^n \hat{\lambda}^{(n)}
\end{align}
\citep[Ch.~II, {\S}2.1, Eq~(2.21)]{kato1995perturbation}, and:
\begin{align}
\hat{\lambda}^{(n)} = \tfrac{1}{m}\,\operatorname{tr}\bigl(\widehat{\mathcal{T}}^{(n)}\bigr)  
\end{align}
\citep[Ch.~II, {\S}2.1, Eq~(2.22)]{kato1995perturbation}.

\end{theorem}


\paragraph{\textbf{Sketch to Refine Kato's Result}.} 
Following Kato's analytic framework, we also begin with the perturbation series $\mathcal{T}(x)$ of a self-adjoint operator $\mathcal{T}$. Kato's monograph establishes eigenvalue expansions via contour integrals of the resolvent and provides a closed-form expression for the \emph{weighted mean} of eigenvalues, but it does not supply explicit constructive formulas for the individual coefficients. Our approach departs at this point: we expand the resolvent explicitly through its Neumann series, apply the residue theorem on the contour integrals, and simplify the resulting expressions. This yields a closed-form asymptotic eigenvalue expansion for $\mathcal{T}$ with computable coefficients. Unlike Kato's result, our expansion is formulated in terms of the finite summation of the series of unperturbed resolvent, which enables systematic computation and, in particular, facilitates the subsequent derivation of singular-value Fr\'echet derivatives. As a special case, it also recovers the classical Rayleigh--Schr\"odinger corrections of quantum mechanics \citep{rayleigh1896theory,schrodinger1926quantisierung,sakurai2020modern}.

\begin{theorem}[Refined Closed-Form Asymptotic Expansion of Simple Isolated Eigenvalue in Self-Adjoint Operator]
\label{thm:expansions_of_eigenvalues}
Let
\begin{align}
\mathcal{T}(x) &= \mathcal{T}^{(0)} + \sum_{j=1}^{\infty} x^j\,\mathcal{T}^{(j)} \;\in\; \mathcal{L}(X)
\end{align}
be a holomorphic family of bounded operators on a Banach space $X$, where $\mathcal{T}^{(0)}$ denotes the unperturbed operator and $x \in \mathbb{C}$ is the perturbation parameter.

\medskip
\noindent
\textbf{Unperturbed Reduced Resolvent.}
Define the unperturbed reduced resolvent \citep{kato1995perturbation,yosida2012functional} of $\mathcal{T}^{(0)}$:
\begin{align}
S^{(0)} &= \bigl(\mathcal{T}^{(0)} - \lambda^{(0)} I\bigr)^{-1}\,(I - w^{(0)}(w^{(0)})^*)
,
\end{align}
where $\lambda^{(0)}$ is a simple eigenvalue of $\mathcal{T}^{(0)}$ and $w^{(0)}$ is the associated normalized eigenvector (\ie, $\|w^{(0)}\|_2=1$). 

\medskip
\noindent
\textbf{Theorem Claim.}
Then there exists a unique holomorphic branch $\lambda(x)$ of eigenvalues of $\mathcal{T}(x)$. It admits the power series:
\begin{align}
\lambda(x) &= \sum_{n=0}^{\infty} x^n\,\lambda^{(n)}, 
\end{align}
and for each integer $n\ge1$,
\begin{align}
\lambda^{(n)}
&=
\sum_{p=1}^n(-1)^{\,p-1}
\sum_{\substack{i_1+\cdots+i_p=n\\i_j\ge1}}
\bigl\langle w^{(0)},\,
  \mathcal{T}^{(i_1)}\,S^{(0)}\,\mathcal{T}^{(i_2)}\,S^{(0)}\cdots S^{(0)}\,\mathcal{T}^{(i_p)}\,w^{(0)}
\bigr\rangle.
\end{align}
\end{theorem}

\begin{mynewproof}

We begin by presenting a compact and explicit proof of Theorem~\ref{thm:kato_weighted_mean}~(\nameref{thm:kato_weighted_mean}) in the case of a simple eigenvalue of a self-adjoint operator, which does not exist in Kato's monograph. Since $\lambda^{(0)}$ is a simple eigenvalue of $\mathcal{T}^{(0)}$, analytic‐perturbation theory ensures there exists a unique eigenvalue branch $\lambda(x)$. Let
\begin{align}
    R(z) = (\mathcal{T}(x) - zI)^{-1}
\end{align}
be the \emph{resolvent} of operator $\mathcal{T}(x)$, which encapsulates the full spectral information of $\mathcal{T}(x)$, and let
\begin{align}
    S(z) = R(z)(I - P(x))
\end{align}
be the associated reduced resolvent $S(z)$ (\ie, the regular part of the resolvent), where $P(x)$ is the Riesz--Dunford contour integral \citep{dunford1988linear,kato1995perturbation} is:
\begin{align}
P(x) =
 -\frac{1}{2\pi i}\oint_{\Gamma} R(z) \,dz
=
 -\frac{1}{2\pi i}\oint_{\Gamma} \bigl(\mathcal{T}(x) - zI\bigr)^{-1}\,dz \label{equ:dunford_riesz_contour_integral}
 , 
\end{align}
where $\Gamma$ is a small contour enclosing only $\lambda^{(0)}$ and no other spectrum. Hence the projection:
\begin{align}
\mathcal{T}(x)\,P(x)
=-\frac{1}{2\pi i}\oint_{\Gamma} \bigl[I + zR(z) \bigr] dz
=\frac{1}{2\pi i}\oint_{\Gamma} -zR(z)  dz
=
\lambda(x)\,P(x) \label{equ:identity_Riesz_projector}
,
\end{align}
holds true since the resolvent $R(z)$ for a simple eigenvalue admits the Laurent expansion \citep[Ch.~I, {\S}5.3, Eq~(5.18)]{kato1995perturbation}
\begin{align}
R(z) = \frac{P(x)}{\lambda(x)-z} + S(z) + \hat{R}(z) 
, \quad
\hat{R}(z) = \sum_{n=1}^{\infty} \big(z - \lambda(x)\big)^{n} \big(S(z)\big)^{n+1}
\label{equ:laurent_expansion_resolvent}
,    
\end{align}
where $\hat{R}(z)$ is the analytic regular remainder of $z$, and the residue of $-zR(z)$ at $z=\lambda(x)$ is
\begin{align}
\mathrm{Res}_{z=\lambda(x)}(-zR(z))= [z - \lambda(x)] [-zR(z)]\mid_{z=\lambda(x)}=
 \lambda(x) P(x)
.
\end{align}
 



\bigskip
\noindent
\textbf{Contour Integral of Perturbed Eigenvalue Series $\lambda(x)$.} 
Starting from the identity in Equation~(\ref{equ:identity_Riesz_projector}),
\begin{align}
\mathcal{T}(x)P(x) &= \lambda(x)P(x) \\
\Longrightarrow 
\tr\bigl(\mathcal{T}(x)P(x)\bigr) &= \tr\bigl(\lambda(x)P(x)\bigr) \\
&= \tr\bigl(\lambda(x)\bigr)\, \tr\bigl(P(x)\bigr) \\
&= \lambda(x)\\
\Longrightarrow 
   \lambda(x) - \lambda^{(0)} &=  \tr\bigl(\mathcal{T}(x)P(x)\bigr) - \lambda^{(0)} \\
   &= \tr\bigl(\mathcal{T}(x)P(x)\bigr) - \tr\bigl(\lambda^{(0)} P(x) \bigr) \\
   &=\tr\Bigl(\bigl(\mathcal{T}(x) -\lambda^{(0)}I\bigr) P(x)\Bigr) 
   ,
\end{align}
then substituting $P(x)$ from Equation~(\ref{equ:identity_Riesz_projector}) yields:
\begin{align}
\lambda(x) - \lambda^{(0)} &=    \tr\Bigl(\bigl(\mathcal{T}(x) -\lambda^{(0)}I\bigr) \bigl( -\frac{1}{2\pi i}\oint_{\Gamma} R(z) \,dz \bigr) \Bigr) \\
&=-\frac{1}{2\pi i}\oint_\Gamma
\operatorname{tr}\!\big((T(x)-\lambda^{(0)}I)R(z)\big)\,dz 
.
\end{align}
Considering the resolvent identity:
\begin{align}
    (\mathcal T(x)-zI)R(z) = I
\end{align}
and:
\begin{align}
\bigl(\mathcal T(x)-\lambda^{(0)} I\bigr)R(z) 
&=\Bigl(\mathcal T(x)-zI + zI-\lambda^{(0)}I\Bigr)R(z) \\
&= \Bigl(\mathcal T(x)-zI + (z-\lambda^{(0)})I\Bigr)R(z) \\
&=(\mathcal T(x)-zI)R(z) + (z-\lambda^{(0)})R(z) \\
&=I + (z-\lambda^{(0)})R(z)
,
\end{align}
it yields:
\begin{align}
\lambda(x) - \lambda^{(0)} 
&=
-\frac{1}{2\pi i}\oint_\Gamma
\operatorname{tr}\!\big((T(x)-\lambda^{(0)}I)R(z)\big)\,dz \\
&=-\frac{1}{2\pi i}\oint_\Gamma
\operatorname{tr}\!\big(
I + (z-\lambda^{(0)})R(z)
\big)\,dz \\
&=-\frac{1}{2\pi i}\oint_\Gamma
\operatorname{tr}\!\big((z-\lambda^{(0)})R(z)
\big)\,dz \\
&=-\frac{1}{2\pi i}\oint_\Gamma
 \operatorname{tr}\!\big(
 (z-\lambda^{(0)}) R(z)
 \big) \operatorname{tr}\!\big(1\big)\,dz \\
&=-\frac{1}{2\pi i}\oint_\Gamma
 \operatorname{tr}\!\big(
 (z-\lambda^{(0)})R(z)
 \big) \operatorname{tr}\!\big(P^{(0)}\big)\,dz \\
&=-\frac{1}{2\pi i}\oint_\Gamma
 \operatorname{tr}\!\big(
 (z-\lambda^{(0)}) R(z) P^{(0)}
 \big) \,dz 
\label{equ:contour_integral_lambdax_lambda0}
.
\end{align}







\bigskip
\noindent
\textbf{Resolvent Expansion.}
To expand the resolvent $R(z)$, define the unperturbed resolvent $R^{(0)}(z)$: 
\begin{align}
R^{(0)}(z) = \bigl(\mathcal{T}^{(0)} - zI\bigr)^{-1}
,
\end{align}
then this identity holds:
\begin{align}
 (\mathcal{T}^{(0)} - zI) R^{(0)}(z) = I .   
\end{align}

\noindent
Note that:
\begin{align}
\mathcal{T}(x) - zI
&= \mathcal{T}^{(0)} - zI + \sum_{j=1}^\infty x^j \mathcal{T}^{(j)} \\
&=\mathcal{T}^{(0)} - zI + I\sum_{j=1}^\infty x^j \mathcal{T}^{(j)} \\
&=\mathcal{T}^{(0)} - zI + (\mathcal{T}^{(0)} - zI) R^{(0)}(z)\sum_{j=1}^\infty x^j \mathcal{T}^{(j)} \\
&= (\mathcal{T}^{(0)} - zI)\Bigl(I + R^{(0)}(z)\,\sum_{j=1}^\infty x^j \mathcal{T}^{(j)}\Bigr)
,
\end{align}
so that the operator Neumann series of $R(z)$ expands as:
\begin{align}
R(z)&=\bigl(\mathcal{T}(x)-zI\bigr)^{-1} \\
&= \left[ (\mathcal{T}^{(0)} - zI)\Bigl(I + R^{(0)}(z)\,\sum_{j=1}^\infty x^j \mathcal{T}^{(j)}\Bigr) \right]^{-1}\\
&= \Bigl(I + R^{(0)}(z)\,\sum_{j=1}^\infty x^j \mathcal{T}^{(j)}\Bigr)^{-1} \Bigl(\mathcal{T}^{(0)} - zI\Bigr)^{-1}\\
&= \Bigl(I + R^{(0)}(z)\,\sum_{j=1}^\infty x^j \mathcal{T}^{(j)}\Bigr)^{-1} R^{(0)}(z)\\
&= \underbrace{
\Bigl(I - \bigl(-R^{(0)}(z)\,\sum_{j=1}^\infty x^j \mathcal{T}^{(j)}\bigr) \Bigr)^{-1}
}_{\text{Neumann series}} R^{(0)}(z) \\
&=\sum_{k=0}^\infty 
(-1)^k \Bigl(R^{(0)}(z)\,\sum_{j=1}^\infty x^j\mathcal{T}^{(j)}\Bigr)^k R^{(0)}(z)
\label{equ:Tx_minus_zI_2}
.
\end{align}


\bigskip
\noindent
\textbf{Asymptotic Eigenvalue Expansion.}
Expanding the term in Equation~(\ref{equ:Tx_minus_zI_2}):
\begin{align}
\Bigl(R^{(0)}(z)\,\sum_{j=1}^\infty x^j\mathcal{T}^{(j)}\Bigr)^k 
\end{align}
yields:
\begin{align}
\Bigl(R^{(0)}(z)\,\sum_{j=1}^\infty x^j\mathcal{T}^{(j)}\Bigr)^k &=   \sum_{i_1,\dots,i_k\ge1}
x^{\,i_1+\cdots+i_k}\,
R^{(0)}(z)\,\mathcal{T}^{(i_1)}\,R^{(0)}(z)\cdots R^{(0)}(z)\,\mathcal{T}^{(i_k)}    \\
&=\sum_{i_1,\dots,i_k\ge1}
x^{\,i_1+\cdots+i_k}\, R^{(0)}(z)\, R_{i_k}(z) \label{equ:Tx_minus_zI_3}
,
\end{align}
where $R_{i_k}(z)$ represents an operator composition series:
\begin{align}
    R_{i_k}(z)= \mathcal{T}^{(i_1)}\,R^{(0)}(z)\cdots R^{(0)}(z)\,\mathcal{T}^{(i_k)}
    .
\end{align}
Substituting Equation~(\ref{equ:Tx_minus_zI_3})
into Equation~(\ref{equ:Tx_minus_zI_2}) yields:
\begin{align}
R(z)
&= \sum_{k=0}^\infty(-1)^k
\sum_{i_1,\dots,i_k\ge1}
x^{\,i_1+\cdots+i_k}\,
R^{(0)}(z)R_{i_k}(z)R^{(0)}(z)  \\
&= \sum_{k=0}^\infty(-1)^k
\sum_{i_1,\dots,i_k\ge1}
x^{\,i_1+\cdots+i_k}\,
R^{(0)}(z)R_{i_k}(z)R^{(0)}(z)
\label{equ:expansion_Tx_minus_zI} 
.
\end{align}
Substituting Equation~(\ref{equ:expansion_Tx_minus_zI}) into the contour integral for $\lambda(x)-\lambda^{(0)}$ in Equation~(\ref{equ:contour_integral_lambdax_lambda0}):
\begin{align}
\lambda(x)-\lambda^{(0)} =  -\frac{1}{2\pi i}\oint_\Gamma
 \operatorname{tr}\!\big((z-\lambda^{(0)}) R(z) P^{(0)}
 \big) \,dz 
  ,
\end{align}
yields:
\begin{align}
\lambda^{(n)}
&=\sum_{k=0}^\infty(-1)^k
\!\!\!\sum_{\substack{i_1+\cdots+i_k=n\\i_j\ge1}}
-\frac{1}{2\pi i}
\oint_\Gamma
\tr\Bigl( 
(z-\lambda^{(0)}) R^{(0)}(z) R_{i_k}(z)R^{(0)}(z) P^{(0)}
\Bigr)
dz \\
&=\sum_{k=0}^{\infty} (-1)^{k-1}
\!\!\!\sum_{\substack{i_1+\cdots+i_k=n\\i_j\ge1}}
\frac{1}{2\pi i}
\oint_\Gamma
\tr\Bigl( 
(z-\lambda^{(0)}) R^{(0)}(z) R_{i_k}(z) R^{(0)}(z) P^{(0)}
\Bigr)
dz 
,
\end{align}
which recovers Theorem~\ref{thm:kato_weighted_mean}~(\nameref{thm:kato_weighted_mean}).


\bigskip
\noindent
\textbf{Contracting and Relabeling Indices.} We refine Theorem~\ref{thm:kato_weighted_mean}~(\nameref{thm:kato_weighted_mean}) further, with the aim of obtaining a constructive, computable and basis-dependent formulation. Note that only the multi-indices satisfying:
\begin{align}
    i_1 + \cdots + i_k = n    
\end{align}
contribute to the coefficient of $x^n$, and since the terms with:
\begin{align}
    k = 0 \quad \text{or} \quad k > n
\end{align}
for $n \geq 1$ vanish, we contract the summation to the admissible subset of indices. For clarity, we denote this contracted index set by $p \subseteq k$:
\begin{align}
\lambda^{(n)}
    &=\sum_{p=1}^{n} (-1)^{p-1}
\!\!\!\sum_{\substack{i_1+\cdots+i_p=n\\i_j\ge1}}
\frac{1}{2\pi i}
\oint_\Gamma
\tr\Bigl(
(z-\lambda^{(0)}) R^{(0)}(z) R_{i_p}(z)R^{(0)}(z)\,P^{(0)}
\Bigr)
dz  
\label{equ:pre_residue_eigenvalue_expansion}
.
\end{align}


\bigskip
\noindent
\textbf{Applying Cauchy's Residue Theorem}
Applying Cauchy's residue theorem via Riesz--Dunford functional calculus \citep{dunford1988linear} for Equation~(\ref{equ:pre_residue_eigenvalue_expansion}) yields:
\begin{align}
\lambda^{(n)}
&=\sum_{p=1}^n(-1)^{p-1}
\sum_{\substack{i_1+\cdots+i_p=n\\i_j\ge1}}
\operatorname{Res}_{z=\lambda^{(0)}} \Bigl[
\tr\Bigl(
(z-\lambda^{(0)}) 
R^{(0)}(z) R_{i_p}(z) R^{(0)}(z) P^{(0)} 
\Bigr)
\Bigr]
\label{equ:expansion_lambda_n}
.
\end{align}




\bigskip
\noindent
\textbf{Simplifying Residue.} We now aim to compute the residue:
\begin{align}
\operatorname{Res}_{z=\lambda^{(0)}} \Bigl[
\tr \Bigl(
(z - \lambda^{(0)}) R^{(0)}(z) R_{i_p}(z) R^{(0)}(z) P^{(0)} 
\Bigr)
\Bigr]
.
\end{align}
Note that near $z=\lambda^{(0)}$, the Laurent expansion of the unperturbed resolvent $R^{(0)}(z)$ for a simple eigenvalue $\lambda^{(0)}$ admits \citep[Ch.~I, {\S}5.3, Eq~(5.18)]{kato1995perturbation}:
\begin{align}
R^{(0)}(z) 
=\frac{P^{(0)}}{\lambda^{(0)}-z} 
+ S^{(0)} + \hat{R}^{(0)}(z),
\qquad
\hat{R}^{(0)}(z) = \sum_{n=1}^{\infty} \big(z - \lambda^{(0)}\big)^{n} \big(S^{(0)}\big)^{n+1}
,
\end{align}
where $P^{(0)} = w^{(0)}(w^{(0)})^*$, $S^{(0)}=R^{(0)}(z)(I-P^{(0)})$ is the unperturbed reduced resolvent of $R^{(0)}(z)$, and $\hat{R}^{(0)}(z)$ is the analytic regular remainder of $z$. Substitute $R^{(0)}(z)$ into the trace product:
\begin{align}
\tr\Bigl(
(z - \lambda^{(0)}) R^{(0)}(z) R_{i_p}(z) R^{(0)}(z) P^{(0)}
\Bigr)
,    
\end{align}
and consider that in the expanded trace product:
\begin{enumerate}
    \item the terms $P^{(0)}S^{(0)}=S^{(0)}P^{(0)}=0$ vanish,

    \item the terms with higher-order poles vanish, since the denominators are constant operators.
    
\end{enumerate}
Then only the term with simple pole survives:\\
\pgfmathsetmacro{\linewidthfactor}{0.78}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
\operatorname{Res}_{z=\lambda^{(0)}} \Bigl[
\tr\Bigl(
(z - \lambda^{(0)}) R^{(0)}(z) R_{i_p}(z) R^{(0)}(z) P^{(0)}
\Bigr)
\Bigr]
&=
\operatorname{Res}_{z=\lambda^{(0)}} \Bigl[
\tr\Bigl(
(z - \lambda^{(0)})
\frac{P^{(0)}\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)}P^{(0)}}{(\lambda^{(0)}-z)^2} P^{(0)}
\Bigr)
\Bigr] \\
&=\operatorname{Res}_{z=\lambda^{(0)}} \Bigl[
\tr\Bigl(
\frac{P^{(0)}\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)}P^{(0)}}{z-\lambda^{(0)}}  P^{(0)}
\Bigr)
\Bigr] \\
&=(z-\lambda^{(0)}) 
\tr\Bigl(
\frac{P^{(0)}\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)}P^{(0)}}{z-\lambda^{(0)}} P^{(0)} 
\Bigr)
\mid_{z \to \lambda^{(0)}} 
\\
&=
\tr\Bigl(
P^{(0)}\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)}P^{(0)}  P^{(0)}
\Bigr) \\
&=
\tr\Bigl(
\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)}P^{(0)}  P^{(0)} P^{(0)}
\Bigr) \\
&=
\tr\Bigl(
\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)} P^{(0)}  
\Bigr)
\label{equ:residue_of_inner_product}
,
\end{align}
\end{minipage}
}\\
since $P^{(0)}P^{(0)}=P^{(0)}$.


\bigskip
\noindent
\textbf{Producing Theorem Claim.}
Substituting the residue from Equation~(\ref{equ:residue_of_inner_product}) into Equation~(\ref{equ:expansion_lambda_n}) yields:
\begin{align}
\lambda^{(n)} &= 
\sum_{p=1}^n (-1)^{p-1} \sum_{\substack{i_1 + \cdots + i_p = n \\ i_j \geq 1}} 
\tr\Bigl(
\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)} P^{(0)}  
\Bigr) \\
&= 
\sum_{p=1}^n (-1)^{p-1} \sum_{\substack{i_1 + \cdots + i_p = n \\ i_j \geq 1}} 
\tr\Bigl(
\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)} w^{(0)} (w^{(0)})^*  
\Bigr) \\
&= 
\sum_{p=1}^n (-1)^{p-1} \sum_{\substack{i_1 + \cdots + i_p = n \\ i_j \geq 1}} 
\tr\Bigl(
\bigl(w^{(0)}\bigr)^*  
\mathcal T^{(i_1)}S^{(0)}\cdots S^{(0)}\mathcal T^{(i_p)} w^{(0)} 
\Bigr) \\
&=\sum_{p=1}^n (-1)^{p-1} \sum_{\substack{i_1 + \cdots + i_p = n \\ i_j \geq 1}} 
\Bigl\langle w^{(0)}, \mathcal{T}^{(i_1)} S^{(0)} \mathcal{T}^{(i_2)} S^{(0)} \cdots S^{(0)} \mathcal{T}^{(i_p)} w^{(0)} \Bigr\rangle 
,
\end{align}
which is basis-dependent and expressed in terms of unperturbed reduced resolvent.

{\hfill$\qed$\par}
\end{mynewproof}


% \paragraph{\textbf{Spectral Representation of the Expansion.}} 
% To rewrite the coefficients in Theorem~\ref{thm:expansions_of_eigenvalues}, 
% we use the spectral theorem for the unperturbed operator $\mathcal{T}^{(0)}$. 
% Let $\sigma(\mathcal{T}^{(0)})$ denote its spectrum, and let 
% $E_{\mathcal{T}^{(0)}}(\cdot)$ be the associated spectral measure. 
% Define the orthogonal projection
% \begin{align}
% Q := I - P^{(0)}, \qquad P^{(0)} = w^{(0)}(w^{(0)})^*,
% \end{align}
% which projects onto the orthogonal complement of the eigenspace of $\lambda^{(0)}$. 
% Then the reduced resolvent $S^{(0)}$ admits the spectral representation
% \begin{align}
% S^{(0)} 
% = Q\,(\mathcal{T}^{(0)} - \lambda^{(0)} I)^{-1} Q
% = \int_{\sigma(\mathcal{T}^{(0)}) \setminus \{\lambda^{(0)}\}}
% \frac{1}{s-\lambda^{(0)}} \, Q\, dE_{\mathcal{T}^{(0)}}(s)\, Q.
% \end{align}

% Substituting this into the expansion of Theorem~\ref{thm:expansions_of_eigenvalues},
% \begin{align}
% \lambda^{(n)}
% =\sum_{p=1}^n(-1)^{p-1}
% \!\!\!\sum_{\substack{i_1+\cdots+i_p=n\\ i_j\ge1}}
% \bigl\langle w^{(0)},\,
% \mathcal{T}^{(i_1)}S^{(0)}\mathcal{T}^{(i_2)}S^{(0)}\cdots 
% S^{(0)}\mathcal{T}^{(i_p)}w^{(0)}
% \bigr\rangle,
% \end{align}
% we obtain the multi–spectral–integral form
% \begin{align}
% \lambda^{(n)}
% &=\sum_{p=1}^n(-1)^{p-1}
% \!\!\!\sum_{\substack{i_1+\cdots+i_p=n\\ i_j\ge1}}
% \int\!\cdots\!\int
% \Biggl(\prod_{\ell=1}^{p-1}\frac{ds_\ell}{s_\ell-\lambda^{(0)}}\Biggr)\,
% \rho_{i_1,\dots,i_p}(s_1,\dots,s_{p-1}),
% \end{align}
% where
% \begin{align}
% \rho_{i_1,\dots,i_p}(s_1,\dots,s_{p-1})
% :=\bigl\langle w^{(0)},\,\mathcal T^{(i_1)}\,Q\,dE_{\mathcal{T}^{(0)}}(s_1)\,Q\,
% \mathcal T^{(i_2)}\,Q\,dE_{\mathcal{T}^{(0)}}(s_2)\,Q\,\cdots\,
% Q\,dE_{\mathcal{T}^{(0)}}(s_{p-1})\,Q\,\mathcal T^{(i_p)}\,w^{(0)}\bigr\rangle.
% \end{align}

% \medskip
% If $\mathcal{T}^{(0)}$ has a purely discrete spectrum with orthonormal eigenbasis 
% $\{w^{(m)}\}_{m\ge0}$ and eigenvalues $\{\lambda^{(m)}\}$ (with $m=0$ the reference state), 
% the integrals collapse to sums, yielding the familiar Rayleigh--Schr\"odinger–type denominators:
% \begin{align}
% \lambda^{(n)}
% &=\sum_{p=1}^n(-1)^{p-1}
% \!\!\!\sum_{\substack{i_1+\cdots+i_p=n\\ i_j\ge1}}
% \sum_{m_1,\dots,m_{p-1}\ne 0}
% \frac{
% \langle w^{(0)},\mathcal T^{(i_1)}w^{(m_1)}\rangle
% \langle w^{(m_1)},\mathcal T^{(i_2)}w^{(m_2)}\rangle \cdots
% \langle w^{(m_{p-1})},\mathcal T^{(i_p)}w^{(0)}\rangle}
% {(\lambda^{(m_1)}-\lambda^{(0)})\cdots(\lambda^{(m_{p-1})}-\lambda^{(0)})}.
% \end{align}



\begin{remark}
By refining Theorem~\ref{thm:kato_weighted_mean}~(\nameref{thm:kato_weighted_mean}), Theorem~\ref{thm:expansions_of_eigenvalues}~(\nameref{thm:expansions_of_eigenvalues}) provides an \emph{explicit, closed-form representation} of the coefficients $\lambda^{(n)}$ in the eigenvalue perturbation series. Classical analytic perturbation theory \citep{kato1995perturbation} guarantees the existence of such expansions and gives recursive characterizations of the coefficients, but does not furnish constructive closed forms. In contrast, our formulation expresses each $\lambda^{(n)}$ in terms of finitely many operator products involving the perturbation operators $\mathcal{T}^{(j)}$ and the unperturbed reduced resolvent $S^{(0)}$, making the coefficients directly computable. As a validation, for $n=1,2,\dots$, the expansion specializes to the familiar Rayleigh--Schr\"odinger corrections of quantum mechanics \citep{rayleigh1896theory,schrodinger1926quantisierung,sakurai2020modern}.
\end{remark}


% \paragraph{\textbf{Recovering Rayleigh--Schr\"odinger Perturbation from the General Schr\"odinger Equation.}}  
% In quantum mechanics, the dynamics of a particle or system are governed by the time-dependent Schr\"odinger equation  
% \begin{align}
% i\hbar \,\frac{\partial}{\partial t}\psi(t) \;=\; H(x)\,\psi(t),
% \end{align}
% where $H(x)$ is the Hamiltonian operator acting on the Hilbert space $L^2(\mathbb{R}^d)$ (or more generally, on a separable Hilbert space). Stationary solutions $\psi(t,x)=e^{-iEt/\hbar}w(x)$ reduce this to the time-independent Schr\"odinger equation
% \begin{align}
% H(x) w(x) \;=\; \lambda(x) w(x),
% \end{align}
% where $\lambda(x)$ represents the energy levels of the system.  

% We now suppose the Hamiltonian can be written as a perturbation series
% \begin{align}
% H(x) \;=\; H^{(0)} + x H^{(1)} + x^2 H^{(2)} + \cdots,
% \end{align}
% where $H^{(0)}$ is the unperturbed Hamiltonian, and $H^{(j)}$ encode perturbing interactions (e.g., external potentials, couplings). Assume $\lambda^{(0)}$ is a simple eigenvalue of $H^{(0)}$ with normalized eigenfunction $w^{(0)}$.  

% Then Theorem~\ref{thm:expansions_of_eigenvalues} guarantees that the perturbed eigenvalue branch admits an expansion
% \begin{align}
% \lambda(x) = \lambda^{(0)} + x \lambda^{(1)} + x^2 \lambda^{(2)} + \cdots,
% \end{align}
% with coefficients given explicitly by operator products of $H^{(j)}$ and the reduced resolvent 
% \begin{align}
% S^{(0)} = (H^{(0)}-\lambda^{(0)}I)^{-1}(I-w^{(0)}(w^{(0)})^*).
% \end{align}

% In particular, if $H(x) = H^{(0)} + xV$ with a single perturbation $V$, then the first few Rayleigh--Schr\"odinger corrections are
% \begin{align}
% \lambda^{(1)} &= \langle w^{(0)}, V w^{(0)} \rangle, \\[0.5em]
% \lambda^{(2)} &= -\langle w^{(0)}, V S^{(0)} V w^{(0)} \rangle
% = \sum_{m\neq 0} \frac{|\langle w^{(m)}, V w^{(0)} \rangle|^2}{\lambda^{(0)} - \lambda^{(m)}}, \\[0.5em]
% \lambda^{(3)} &= \langle w^{(0)}, V S^{(0)} V S^{(0)} V w^{(0)} \rangle
%  - \langle w^{(0)}, V w^{(0)} \rangle \,\langle w^{(0)}, V (S^{(0)})^2 V w^{(0)} \rangle.
% \end{align}

\section{Infinitesimal Higher-Order Spectral Variations}
\label{sec:spectral_variation}


Guided by the scheme in Figure~\ref{fig:framework_of_spectral_analysis}, and under Assumption~\ref{assump:simple_singular_values}~(\nameref{assump:simple_singular_values}), we exploit the spectral correspondence between a rectangular matrix $A \in \mathbb{R}^{m \times n}$ and its Jordan--Wielandt embedding $\mathcal{T}$ as established in Theorem~\ref{theorem:Jordan_Wielandt_relation}~(\nameref{theorem:Jordan_Wielandt_relation}). This allows us to derive arbitrary--order Fr\'echet derivatives of the singular values of $A$ from the asymptotic eigenvalue expansions of $\mathcal{T}$. The argument proceeds by first establishing the correspondence between the perturbation series and Fr\'echet derivatives as stated in Theorem~\ref{thm:frechet_taylor_operator}~(\nameref{thm:frechet_taylor_operator}), and then applying this relation to obtain higher--order derivatives of singular values as stated in Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}).

%A holomorphic family of type (A) admits a power series expansion in x with coefficients given by the Fréchet derivatives.
\begin{theorem}[Analytic Perturbation for Holomorphic Operators]
\label{thm:frechet_taylor_operator}
Let $X$ be a Banach space and let $\mathcal{T}(x):U\subset\mathbb{C}\to\mathcal{L}(X)$ be a holomorphic family --- \ie, type (A) in the sense of Kato's framework \citep{kato1995perturbation}, defined in a neighborhood of $0$ in the operator norm. Then $\mathcal{T}$ is $C^\infty$ in the Fr\'echet sense at $0$ and admits the convergent operator--norm expansion:
\begin{align}
\mathcal{T}(x) \;=\; \sum_{n=0}^{\infty}\frac{x^{n}}{n!}\,D^{n}\mathcal{T}(0),
\qquad |x|<\rho,
\end{align}
where $\rho$ is the distance from $0$ to the boundary of $U$. In particular, if one writes the perturbation series as:
\begin{align}
\mathcal{T}(x) = \mathcal{T}^{(0)}+\sum_{n=1}^{\infty}x^{n}\,\mathcal{T}^{(n)},
\end{align}
then the coefficients agree with the Fr\'echet derivatives, namely:
\begin{align}
\mathcal{T}^{(n)} = \tfrac{1}{n!}\,D^{n}\mathcal{T}(0), \qquad n\ge1.
\end{align}


\end{theorem}



\begin{theorem}[Higher-Order Infinitesimal Spectral Variation]
\label{thm:nth_order_singular_value}

Let 
\begin{align}
A \in \mathbb{R}^{m \times n}    
\end{align}
be a real rectangular matrix under Assumption~\ref{assump:simple_singular_values}~(\nameref{assump:simple_singular_values}). 


\bigskip
\noindent
\textbf{Matrix Perturbation Series.} 
Let 
\begin{align}
A(x)=\sum_{k=0}^\infty x^k\,A^{(k)}\in\mathbb{R}^{m\times n} 
\end{align}
be holomorphic perturbed operator near $x=0$ with unperturbed matrix $A^{(0)} = A$. 

The unperturbed matrix $A^{(0)}$ admits a full SVD:
\begin{align}
A^{(0)} = U^{(0)} \Sigma^{(0)} (V^{(0)})^T,    
\end{align}
as defined in Theorem~\ref{theorem:full_svd}~(\nameref{theorem:full_svd}), where ordered $r=\rank(A)$ non-zero singular values are given, under Assumption~\ref{assump:simple_singular_values}~(\nameref{assump:simple_singular_values}), as:
\begin{align}
\sigma_1^{(0)} > \sigma_2^{(0)} > \ldots > \sigma_r^{(0)} > 0
,
\end{align}
$u_k^{(0)}$ and $v_k^{(0)}$ are singular vectors associated with singular value $\sigma_k^{(0)}$, and:
\begin{align}
   U^{(0)} \in \mathbb{R}^{m \times m} , \quad  V^{(0)} \in \mathbb{R}^{n \times n}
\end{align}
are orthogonal matrices. For brevity, we also use $\sigma_i = \sigma_i^{(0)}$, $u_i=u_i^{(0)}$, and $v_i=v_i^{(0)}$.


\bigskip
\noindent
\textbf{Jordan--Wielandt Perturbation Series Embedding.} 
Using Theorem~\ref{theorem:Jordan_Wielandt_relation}~(\nameref{theorem:Jordan_Wielandt_relation}), we embed the perturbation series $A(x)$ into $\mathcal{T}(x)$ to construct a Jordan--Wielandt embedding:
\begin{align}
\mathcal{T}(x) = \begin{bmatrix}
0 & A(x) \\
A(x)^\top & 0
\end{bmatrix}
.
\end{align}
This embedding admits a perturbation series:
\begin{align}
\mathcal{T}(x) = \sum_{j=0}^\infty x^j \mathcal{T}^{(j)}
\end{align}
at $x$ near zero, with the unperturbed operator:
\begin{align}
\mathcal{T}^{(0)} = 
\begin{bmatrix} 
0 & A^{(0)} \\ 
(A^{(0)})^\top & 0 
\end{bmatrix},    
\end{align}
and the perturbations:
\begin{align}
\mathcal{T}^{(j)} = \begin{bmatrix} 0 & A^{(j)} \\ (A^{(j)})^\top & 0 \end{bmatrix}, \quad j \geq 1.    
\end{align}

The non-zero eigenvalues $\lambda_i^{(\pm 0)}$ of $\mathcal{T}^{(0)}$ are therefore:
\begin{align}
 \lambda_i^{(+0)} = + \sigma_i^{(0)},
 \quad 
 \lambda_i^{(-0)} = - \sigma_i^{(0)},
 \quad \text{for}~i = 1, \ldots, r,   
\end{align}
associated with eigenvectors:
\begin{align}
w_i^{(+0)} = \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_i^{(0)} \\ 
v_i^{(0)} 
\end{bmatrix}
, 
\quad w_i^{(-0)} = \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_i^{(0)} \\ 
-v_i^{(0)} 
\end{bmatrix}
,    
\end{align}
and null eigenvectors, 
\begin{align}
a_j^{(0)} = 
\begin{bmatrix} 
u_j^{(0)} \\ 
0 
\end{bmatrix}  
, \quad (\text{for}~ j=r+1,\cdots,m)    ,
\end{align}
and:
\begin{align}
b_k^{(0)}=
\begin{bmatrix} 
0 
\\ 
v_k^{(0)} 
\end{bmatrix}
, \quad (\text{for}~ j=r+1,\cdots, n) .   
\end{align}


Since $w_k^{(+0)}$ and $w_k^{(-0)}$ are eigenvalues of $T^{(0)}$, hence the identities hold:
\begin{align}
\mathcal{T}^{(0)} w_k^{(+0)} = \lambda_k^{(+0)} w_k^{(+0)}
\Longrightarrow
\mathcal{T}^{(0)} w_k^{(+0)} = \sigma_k^{(0)} w_k^{(+0)}, 
\end{align}
and:
\begin{align}
\mathcal{T}^{(0)} w_k^{(-0)} =   \lambda_k^{(-0)} w_k^{(-0)}
\Longrightarrow
\mathcal{T}^{(0)} w_k^{(-0)} =   -\sigma_k^{(0)} w_k^{(-0)}.  
\end{align}


\bigskip
\noindent
\textbf{Unperturbed Reduced Resolvent in Embedding.} 
By definition, the spectral expansion of the reduced resolvent operator associated with the eigenvalue $\lambda_k^{(+0)}=\sigma_k^{(0)}$ and associated eigenvector $w_k^{(+0)}$ of $\mathcal{T}(x)$ is given as:
\begin{align}
S_k^{(0)} = \left( \mathcal{T} - \sigma_k^{(0)} I \right)^{-1} \left( I - P_k^{(0)} \right), \quad P_k^{(0)} = w_k^{(+0)} (w_k^{(+0)})^\top
,
\end{align}
which admits the spectral expansion:\\
\pgfmathsetmacro{\linewidthfactor}{0.9}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
S_k^{(0)} = 
\sum_{i=1, ~i \neq k}^{r} \frac{w_i^{(+0)} (w_i^{(+0)})^\top}{\sigma_i^{(0)} - \sigma_k^{(0)}} + 
\sum_{i=1,i \neq k}^r \frac{w_i^{(-0)} (w_i^{(-0)})^\top}{-\sigma_i^{(0)} - \sigma_k^{(0)}} - 
\sum_{j=r+1}^m \frac{a_j^{(0)} (a_j^{(0)})^\top}{\sigma_k^{(0)}} - \sum_{j=r+1}^n \frac{b_j^{(0)} (b_j^{(0)})^\top}{\sigma_k^{(0)}}.
\end{align}
\end{minipage}
}

\bigskip
\noindent
\textbf{Theorem Claim.} 
For each integer $n \ge 1$,
\begin{align}
\sigma_k^{(n)} = \sum_{p=1}^n (-1)^{p-1} \sum_{\substack{i_1 + \cdots + i_p = n \\ i_j \geq 1}} \langle w_k^{(+0)}, \mathcal{T}^{(i_1)} S_k^{(0)} \mathcal{T}^{(i_2)} \cdots S_k^{(0)} \mathcal{T}^{(i_p)} w_k^{(+0)} \rangle.
\end{align}

By Theorem~\ref{thm:frechet_taylor_operator}~(\nameref{thm:frechet_taylor_operator}), the Fr\'echet derivative of the singular value is unique and given by:
\begin{align}
D^n \sigma_k [\dd A, \cdots, \dd A] = n! \lim_{x \to 0} \left(x^n \; \sigma_k^{(n)}\right)
,
\end{align}
where:
\begin{align}
\dd A = \lim_{x \to 0} x A^{(1)}  .
\end{align}

\end{theorem}

\begin{mynewproof}

By Theorem~\ref{thm:expansions_of_eigenvalues}~(\nameref{thm:expansions_of_eigenvalues}), one eigenvalue $\lambda_k(x)$ of $\mathcal{T}(x)$ admits an asymptotic expansion:
\begin{align}
\lambda_k(x) = \sum_{n=0}^\infty x^n \lambda_k^{(n)}    
.
\end{align}


By Theorem~\ref{theorem:Jordan_Wielandt_relation}~(\nameref{theorem:Jordan_Wielandt_relation}), for $n \geq 1$, choosing a positive eigenvalue branch $\sigma_k^{(0)}$ yields the asymptotic singular-value expansion of $A(x)$:
\begin{align}
\sigma_k^{(n)} = \sum_{p=1}^n (-1)^{p-1} \sum_{\substack{i_1 + \cdots + i_p = n \\ i_j \geq 1}} \langle w_k^{(+0)}, \mathcal{T}^{(i_1)} S_k^{(0)} \mathcal{T}^{(i_2)} \cdots S_k^{(0)} \mathcal{T}^{(i_p)} w_k^{(+0)} \rangle.    
\end{align}

By Theorem~\ref{thm:frechet_taylor_operator}~(\nameref{thm:frechet_taylor_operator}), $D^n \sigma_k$ admits:
\begin{align}
D^n \sigma_k = n! \sigma_k^{(n)}
,
\end{align}
and its action is given by:
\begin{align}
D^n \sigma_k[\dd A, \cdots, \dd A]   = n! \lim_{x \to 0} x^n \sigma_k^{(n)}
,
\end{align}
where
\begin{align}
    \dd A = \lim_{x \to 0} x A^{(1)}
    .
\end{align}




{\hfill$\qed$\par}
\end{mynewproof}


\begin{remark}
\textbf{Thanks to Kato's perturbation theory for linear operators, our framework for deriving singular-value derivatives rests on a rigorous analytic foundation and provides a procedural and systematic methodology, resting on a rigorous foundation, and going beyond the \emph{ad hoc} approaches commonly found in classical matrix analysis.} In the latter, derivatives are typically obtained through differential identities or perturbation arguments without a fully rigorous treatment of differentiability. 
For instance, \citet{horn2012matrix} present differential identities for spectral functions, but these do not constitute a unified framework for higher-order derivatives.
\end{remark}



\section{Special Case ($n=1$): Closed-Form Singular-Value Jacobian}
\label{sec:special_case_jacobian}

We now show that Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}) can recover the well-known singular-value Jacobian, stated in Lemma~\ref{lemma:jacobian_of_singular_value} \citep{StewartSun1990,magnus2019matrix}.




\begin{lemma}[Closed-Form Singular-Value Jacobian]
\label{lemma:jacobian_of_singular_value}
The Jacobian of a singular value is well‐known in the literature \citep{StewartSun1990,magnus2019matrix} in the form:
\begin{align}
\frac{\partial \sigma_k}{\partial A}
= u_k \, v_k^\top
,
\end{align}
which immediately admits an equivalent result with Kronecker-product presentation:
\begin{align}
D\sigma_k[\dd A] =
(v_k \otimes u_k)^\top \mathrm{vec}(\dd A).
\end{align}
\end{lemma}

\begin{mynewproof}
        
We specialize $n=1$ in Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}) to recover this result. 

\bigskip
\noindent
\textbf{Constructing $\dd A$.}
We construct a perturbation series on $A$:
\begin{align}
    A(x) = A + xA^{(1)}, \quad  A^{(0)}=A
    ,
\end{align}
so it yields:
\begin{align}
\dd A = \lim_{x \to 0 }xA^{(1)} 
.    
\end{align}

\bigskip
\noindent
\textbf{Specializing $n=1$.}
Specializing $n=1$ in Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}) yields:
\begin{align}
\sigma_k^{(1)} = \langle w_k^{(+0)}, \mathcal{T}^{(1)} w_k^{(0)} \rangle.
\end{align}

\bigskip
\noindent
\textbf{Simplifying First-Order Term.}
Consider:
\begin{align}
&\mathcal{T}^{(1)} w_k^{(+0)} = 
\begin{bmatrix} 
0 & A^{(1)} \\ (A^{(1)})^\top & 0 
\end{bmatrix} 
\cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_k \\ 
v_k \end{bmatrix} =
\frac{1}{\sqrt{2}} \begin{bmatrix} A^{(1)} v_k \\ (A^{(1)})^\top u_k \end{bmatrix} \\
&\xLongrightarrow[]{}
\langle w_k^{(+0)}, \mathcal{T}^{(1)} w_k^{(+0)} \rangle = 
\left( \frac{1}{\sqrt{2}} 
\begin{bmatrix} u_k \\ v_k \end{bmatrix} \right)^\top \cdot \frac{1}{\sqrt{2}} \begin{bmatrix} A^{(1)} v_k \\ (A^{(1)})^\top u_k \end{bmatrix} \\
&\xLongrightarrow[]{}
\langle w_k^{(+0)}, \mathcal{T}^{(1)} w_k^{(+0)} \rangle = 
\frac{1}{2} \left[ u_k^\top A^{(1)} v_k + v_k^\top (A^{(1)})^\top u_k \right] \\
&\xLongrightarrow[]{}
\langle w_k^{(+0)}, \mathcal{T}^{(1)} w_k^{(+0)} \rangle = u_k^\top A^{(1)} v_k \\
&\xLongrightarrow[]{}
\sigma_k^{(1)} = u_k^\top A^{(1)} v_k .
\end{align}


\bigskip
\noindent
\textbf{Adjusting Layout Representation.}
By Theorem~\ref{thm:frechet_taylor_operator}~(\nameref{thm:frechet_taylor_operator}), we have:
\begin{align}
   D \sigma_k [\dd A] 
   &= \sigma_k^{(1)}[\dd A] \\
   &= \lim_{x \to 0} \sigma_k^{(1)} x A^{(1)} \\
   &= \lim_{x \to 0} u_k^T xA^{(1)} v_k \\
   &=u_k^{\top} \dd A v_k  \in \mathbb{R}.
\end{align}


Using following identities from Lemma~\ref{lemma:essential_matrix_identities}~(\nameref{lemma:essential_matrix_identities}):
\begin{enumerate}
    \item $\tr(x)=x$,
    
    \item $\operatorname{vec}(B V A^\top) = (A \otimes B)\operatorname{vec}(V)$,

    \item $(A \otimes B)^\top = A^\top \otimes B^\top$,
    
    \item $\tr(ABC) = \tr(CAB) = \tr(BCA)$,
\end{enumerate}
yields:
\begin{align}
D \sigma_k [\dd A] 
   &= \tr(u_k^{\top} \dd A v_k) \\
   &= \tr(v_k u_k^{\top} \dd A ) \\
   &= (v_k \otimes u_k)^\top \mathrm{vec}(\dd A)
   ,
\end{align}
and:
\begin{align}
\frac{\partial \sigma_k}{\partial A}
    =(D\sigma_k)^\top = u_kv_k^\top.
\end{align}


{\hfill$\qed$\par}
\end{mynewproof}




\section{Special Case ($n=2$): Closed-Form Singular-Value Hessian}
\label{sec:special_case_hessian}

Explicit closed-form expressions for the singular-value Hessian of rectangular matrices are, to the best of our knowledge, not available in the literature. Such a result is essential for applications in stochastic analysis, for example when applying It\^o's lemma to stochastic differential equations (SDEs) or stochastic partial differential equations (SPDEs) driven by Wiener processes \citep{oksendal2013stochastic}. We now derive the singular-value Hessian for general real rectangular matrices, under Assumption~\ref{assump:simple_singular_values}~(\nameref{assump:simple_singular_values}), as stated in Lemma~\ref{lemma:hessian_of_singular_value}~(\nameref{lemma:hessian_of_singular_value}), represented in the layout:
\begin{align}
\operatorname{vec}(\dd A)^\top
\left(
\frac{\partial}{\partial \operatorname{vec}(A)} 
\operatorname{vec}\!\left( \frac{\partial \sigma_k}{\partial A}\right)
\right)
\operatorname{vec}(\dd A),
\end{align}
by specializing Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}) to the case $n=2$.



\begin{lemma}[Closed-Form Singular-Value Hessian]
\label{lemma:hessian_of_singular_value}
%Define scale factor and its inverse
The Hessian of a singular value is given as:\\
\pgfmathsetmacro{\linewidthfactor}{0.9}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
\frac{\partial}{\partial \operatorname{vec}(A)} \operatorname{vec}\left(
   \frac{\partial \sigma_k}{\partial A}
   \right) 
&=\underbrace{\sum_{i \neq k, i \leq m} \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2}\left(v_k \otimes u_i\right)\left(v_k \otimes u_i\right)^\top}_{\text{left}} +\\
    &\qquad \underbrace{\sum_{j \neq k, j \leq n} \frac{\sigma_k}{\sigma_k^2 - \sigma_j^2} \left(v_j \otimes u_k\right)\left(v_j \otimes u_k\right)^\top}_{\text{right}} + \\
    &\qquad \underbrace{\sum_{l \neq k, l \leq r} \frac{\sigma_l}{\sigma_k^2 - \sigma_l^2}\left[ \left(v_k \otimes u_l\right)\left(v_l \otimes u_k\right)^\top + \left(v_l \otimes u_k\right)\left(v_k \otimes u_l\right)^\top \right]}_{\text{left-right interaction}} 
\end{align}
\end{minipage}%
}\\
with Kronecker-product representation.
\end{lemma}

\begin{mynewproof}
We specialize $n=2$ in Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}) to derive this result. 

\bigskip
\noindent
\textbf{Constructing $\dd A$.}
We construct a perturbation series on $A$:
\begin{align}
    A(x) = A + xA^{(1)}, \quad  A^{(0)}=A
    ,
\end{align}
so it yields:
\begin{align}
\dd A = \lim_{x \to 0 }xA^{(1)} 
.    
\end{align}


\bigskip
\noindent
\textbf{Specializing $n=2$.}
Specializing $n=2$ in Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}) yields:
\begin{align}
\sigma_k^{(2)} &= \sum_{p=1}^2 (-1)^{p-1} \sum_{\substack{i_1 + \cdots + i_p = 2 \\ i_j \geq 1}} \langle w_k^{(+0)}, \mathcal{T}^{(i_1)} S_k^{(0)} \mathcal{T}^{(i_2)} \cdots S_k^{(0)} \mathcal{T}^{(i_p)} w_k^{(+0)} \rangle  \\
&=\sigma_k^{(2,p=1)} + \sigma_k^{(2,p=2)}
\end{align}
where
\begin{align}
    \sigma_k^{(2,p=1)} := \langle w_k^{(+0)}, \mathcal{T}^{(2)} w_k^{(+0)} \rangle,
\end{align}
and
\begin{align}
\sigma_k^{(2, p=2)} := - \langle w_k^{(+0)}, \mathcal{T}^{(1)} S_k^{(0)} \mathcal{T}^{(1)} w_k^{(+0)} \rangle .
\end{align}


\bigskip
\noindent
\textbf{Computing Term $\sigma_k^{(2,p=1)}$.} We first compute the term with $p=1$ ($\sigma_k^{(2,p=1)}$). By Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}), we substitute:
\begin{align}
\mathcal{T}^{(2)}=    
\begin{bmatrix} 
0 & A^{(2)} \\ 
(A^{(2)})^\top & 0 
\end{bmatrix}
\quad
\text{and} \quad
w_k^{(+0)} = \frac{1}{\sqrt{2}}
\begin{bmatrix} 
u_k \\ 
v_k 
\end{bmatrix}
\end{align}
into:
\begin{align}
\mathcal{T}^{(2)} w_k^{(+0)},
\end{align}
it yields:
\begin{align}
&\mathcal{T}^{(2)} w_k^{(+0)} = 
\begin{bmatrix} 
0 & A^{(2)} \\ 
(A^{(2)})^\top & 0 
\end{bmatrix} 
\cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_k \\ 
v_k 
\end{bmatrix} = \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(2)} v_k \\ 
(A^{(2)})^\top u_k 
\end{bmatrix} 
.
\end{align}

Substituting 
\begin{align}
\mathcal{T}^{(2)} w_k^{(+0)} = \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(2)} v_k \\ 
(A^{(2)})^\top u_k 
\end{bmatrix} 
\end{align}
into:
\begin{align}
\sigma_k^{(2,p=1)} = \langle w_k^{(+0)}, \mathcal{T}^{(2)} w_k^{(+0)} \rangle
\end{align}
yields:
\begin{align}
\sigma_k^{(2,p=1)} &= \langle w_k^{(+0)}, \mathcal{T}^{(2)} w_k^{(+0)} \rangle \\
&= \frac{1}{2} \left[ u_k^\top A^{(2)} v_k + (v_k)^\top (A^{(2)})^\top u_k \right] \\
&= u_k^\top A^{(2)} v_k 
\end{align}

In the construction of $\dd A$, there is:
\begin{align}
    A^{(2)} = O,
\end{align}
so that:
\begin{align}
\sigma_k^{(2, p=1)} = u_k^\top A^{(2)} v_k = 0.   
\end{align}


\bigskip
\noindent
\textbf{Sketch of Computing Term $\sigma_k^{(2,p=2)}$.} We compute the term with $p=2$:
\begin{align}
\sigma_k^{(2, p=2)} = - \langle w_k^{(+0)}, \mathcal{T}^{(1)} S_k^{(0)} \mathcal{T}^{(1)} w_k^{(+0)} \rangle \label{equ:hessian_term_p_2}
.
\end{align}
To simplify, we first compute:
\begin{align}
S_k^{(0)} \mathcal{T}^{(1)} w_k^{(+0)} \label{equ:hessian_STw}
,
\end{align}
then substitute this result into Equation~(\ref{equ:hessian_term_p_2}) to produce complete $\sigma_k^{(2, p=2)}$.


\bigskip
\noindent
\textbf{Computing Contributions in $S_k^{(0)} \mathcal{T}^{(1)} w_k^{(+0)} $ in $\sigma_k^{(2,p=2)}$.} 
By Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}), the unperturbed reduced resolvent is defined as:\\
\pgfmathsetmacro{\linewidthfactor}{0.9}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
S_k^{(0)} &= 
\sum_{i=1,i \neq k}^{r} \frac{w_i^{(+0)} (w_i^{(+0)})^\top}{\sigma_i^{(0)} - \sigma_k^{(0)}} + 
\sum_{i=1,i \neq k}^{r} \frac{w_i^{(-0)} (w_i^{(-0)})^\top}{-\sigma_i^{(0)} - \sigma_k^{(0)}} - 
\sum_{j=r+1}^m \frac{a_j^{(0)} (a_j^{(0)})^\top}{\sigma_k^{(0)}} 
- 
\sum_{j=r+1}^n \frac{b_j^{(0)} (b_j^{(0)})^\top}{\sigma_k^{(0)}} 
.
\end{align}
\end{minipage}%
}

By Theorem~\ref{thm:nth_order_singular_value}~(\nameref{thm:nth_order_singular_value}), substituting non-null eigenvectors of the unperturbed embedding $\mathcal{T}^{(0)}$:
\begin{align}
w_i^{(+0)} = \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_i \\ 
v_i 
\end{bmatrix}
, 
\quad w_i^{(-0)} = \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_i \\ 
-v_i 
\end{bmatrix}
,    
\end{align}
and null eigenvectors of the unperturbed embedding $\mathcal{T}^{(0)}$: 
\begin{align}
a_j^{(0)} = 
\begin{bmatrix} 
u_j \\ 
0 
\end{bmatrix}  
, \quad
b_j^{(0)}=
\begin{bmatrix} 
0 
\\ 
v_j 
\end{bmatrix}
, 
\end{align}
into $S_k^{(0)}$ yields:\\
\pgfmathsetmacro{\linewidthfactor}{0.9}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
S_k^{(0)} =
\underbrace{
\sum_{i=1, i \neq k}^{r} \frac{1}{2}\frac{
\begin{bmatrix}
    u_i \\
    v_i
\end{bmatrix}
\begin{bmatrix}
u_i^\top \; v_i^\top
\end{bmatrix}
}{\sigma_i - \sigma_k}
}_{\text{positive eigenspaces}}
+
\underbrace{
\sum_{i=1, i \neq k}^{r} \frac{1}{2}\frac{
\begin{bmatrix}
    u_i \\
    -v_i
\end{bmatrix}
\begin{bmatrix}
u_i^\top \; -v_i^\top
\end{bmatrix}
}{-\sigma_i - \sigma_k}
}_{\text{negative eigenspaces}}
-
\underbrace{
\sum_{j=r+1}^m \frac{
\begin{bmatrix}
    u_j \\
    0
\end{bmatrix}
\begin{bmatrix}
u_j^\top \; 0
\end{bmatrix}
}{\sigma_k^{(0)}} 
}_{\text{left-null eigenspaces}}
-
\underbrace{
\sum_{j=r+1}^n \frac{
\begin{bmatrix}
    0 \\
    v_j
\end{bmatrix}
\begin{bmatrix}
0 \; v_j^\top
\end{bmatrix}
}{\sigma_k^{(0)}}
}_{\text{right-null eigenspaces}}
,
\end{align}
\end{minipage}
}\\
where:
\begin{enumerate}
    \item \textbf{contributions in positive eigenspaces} ($S_k^{(+0)}$) represents the contribution in the subspaces associated with $w_{i}^{(+0)}$;

    \item \textbf{contributions in negative eigenspaces} ($S_k^{(-0)}$) represents the contribution in the subspaces associated with $w_{i}^{(-0)}$;

    \item \textbf{contributions in left-null eigenspaces} ($S_k^{(0,a)}$) represents the contribution in the subspaces associated with $a_j^{(0)}$;

    \item \textbf{contributions in right-null eigenspaces} ($S_k^{(0,b)}$) represents the contribution in the subspaces associated with $b_j^{(0)}$.
\end{enumerate}

Substituting $w_k^{(+0)}$ into:
\begin{align}
S_k^{(0)}\mathcal{T}^{(1)} w_k^{(+0)}   
\end{align}
yields:
\begin{align}
S_k^{(0)}\mathcal{T}^{(1)} w_k^{(+0)} = S_k^{(0)}\mathcal{T}^{(1)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_i \\ 
v_i 
\end{bmatrix} 
= S_k^{(0)}\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} 
,
\end{align}
then apply the explicit $S_k^{(0)}$ on this result:
\begin{align}
S_k^{(0)}\mathcal{T}^{(1)} w_k^{(+0)} = S_k^{(0)}\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} 
=(S_k^{(+0)} + S_k^{(-0)} + S_k^{(0,a)}+S_k^{(0,b)})\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} 
,
\end{align}
and discuss the contributions in terms of subspaces:
\begin{enumerate}[leftmargin=*]

\item \textbf{Contributions in Positive Eigenspaces}. 
To compute
\begin{align}
S_k^{(+0)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= \sum_{i=1,i\neq k}^r 
\frac{w_i^{(+0)} (w_i^{(+0)})^\top}{\sigma_i - \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} 
,
\end{align}
consider:
\begin{align}
(w_i^{(+0)})^\top \cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} &= 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_i^\top & v_i^\top 
\end{bmatrix} 
\cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} \notag \\
&= \frac{1}{2} \left[ u_i^\top A^{(1)} v_k + v_i^\top (A^{(1)})^\top u_k \right] .
\end{align}

Note the identity:
\begin{align}
v_i^\top (A^{(1)})^\top u_k = u_k^\top A^{(1)} v_i    \in \mathbb{R}
,
\end{align}
so that:
\begin{align}
&
(w_i^{(+)})^\top \cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} 
=
\frac{1}{2} \left[ u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i \right].
\end{align}

Therefore the contributions in positive eigenspaces are given as:
\begin{align}
S_k^{(+0)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= \sum_{i=1,i\neq k}^r 
\frac{w_i^{(+0)} (w_i^{(+0)})^\top}{\sigma_i - \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} \\
&= \sum_{i=1,i\neq k}^r  
\frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i}{2 (\sigma_i - \sigma_k)} \begin{bmatrix} u_i \\ v_i \end{bmatrix}.    
\end{align}


\item \textbf{Contributions in Negative Eigenspaces}.

To compute:
\begin{align}
S_k^{(-0)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= \sum_{i=1,i\neq k}^r 
\frac{w_i^{(-0)} (w_i^{(-0)})^\top}{-\sigma_i - \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} 
,
\end{align}
consider:
\begin{align}
(w_i^{(-0)})^\top \cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} 
&= 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_i^\top & -v_i^\top 
\end{bmatrix} 
\cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} \notag \\
&=\frac{1}{2} \left[ u_i^\top A^{(1)} v_k - v_i^\top (A^{(1)})^\top u_k \right].
\end{align}

Note the identity:
\begin{align}
v_i^\top (A^{(1)})^\top u_k = u_k^\top A^{(1)} v_i    \in \mathbb{R}
\end{align}
so that:
\begin{align}
(w_i^{(+0)})^\top \cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} 
&=
\frac{1}{2} \left[ u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i \right] \\
&= 
\frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i}{2 (-\sigma_i - \sigma_k)} 
\begin{bmatrix} 
u_i \\ 
-v_i \end{bmatrix}.   
\end{align}

Therefore the contributions in negative eigenspaces are given as:
\begin{align}
S_k^{(-0)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= \sum_{i=1,i\neq k}^r 
\frac{w_i^{(-0)} (w_i^{(-0)})^\top}{-\sigma_i - \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} \\
&=\sum_{i=1,i\neq k}^r 
\frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i}{2 (-\sigma_i - \sigma_k)} 
\begin{bmatrix} 
u_i \\ 
-v_i \end{bmatrix}.
\end{align}

\item \textbf{Contributions in Left-Null Eigenspaces}.

To compute:
\begin{align}
S_k^{(0,a)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= -\sum_{j=r+1}^{m} 
\frac{a_j^{(0)} (a_j^{(0)})^\top}{ \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} 
,
\end{align}
consider:
\begin{align}
(a_j^{(0)})^\top \cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} 
&= 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
u_j^\top & 0 
\end{bmatrix} 
\cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} \notag \\
&=\frac{1}{2} u_j^\top A^{(1)} v_k .
\end{align}

Therefore the contributions in left-null eigenspaces are given as:
\begin{align}
S_k^{(0,a)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= -\sum_{j=r+1}^{m} 
\frac{a_j^{(0)} (a_j^{(0)})^\top}{ \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} \\
&=-\sum_{j=r+1}^{m} 
\frac{1}{\sqrt{2}} \cdot \frac{u_j^\top A^{(1)} v_k}{\sigma_k} \begin{bmatrix} 
u_j \\ 
0 
\end{bmatrix}.
\end{align}


\item \textbf{Contributions in Right-Null Eigenspaces}.

To compute:
\begin{align}
S_k^{(0,b)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= -\sum_{j=r+1}^{n} 
\frac{b_j^{(0)} (b_j^{(0)})^\top}{ \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} 
,
\end{align}
consider:
\begin{align}
(b_j^{(0)})^\top \cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} 
&= 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
0 & v_j^\top 
\end{bmatrix} 
\cdot \frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k 
\end{bmatrix} \notag \\
&=\frac{1}{2} v_j^\top (A^{(1)})^\top u_k \\
&= \frac{1}{2} u_k^\top A^{(1)} v_j.
\end{align}

Therefore the contributions in right-null eigenspaces are given as:
\begin{align}
 S_k^{(0,b)}
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix}
&= -\sum_{j=r+1}^{n} 
\frac{b_j^{(0)} (b_j^{(0)})^\top}{ \sigma_k} 
\frac{1}{\sqrt{2}} 
\begin{bmatrix} 
A^{(1)} v_k \\ 
(A^{(1)})^\top u_k
\end{bmatrix} \\
&=-\sum_{j=r+1}^{n} 
\frac{1}{\sqrt{2}} \cdot \frac{u_k^\top A^{(1)} v_j}{\sigma_k} \begin{bmatrix} 
0 \\ 
v_j 
\end{bmatrix}.
\end{align}

\end{enumerate}


\bigskip
\noindent
\textbf{Computing Inner-Product Contributions in $\langle w_k, \mathcal{T}^{(1)} S_k \mathcal{T}^{(1)} w_k \rangle$.} 
We compute the inner-product contributions in in $\langle w_k, \mathcal{T}^{(1)} S_k \mathcal{T}^{(1)} w_k \rangle$:
\begin{enumerate}[leftmargin=*]

\item \textbf{Inner-Product Contributions in Positive Eigenspaces}. 
% \pgfmathsetmacro{\linewidthfactor}{0.75}
% \pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
% \scalebox{\linewidthfactor}{% scale
% \begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
Consider:
\begin{align}
    Z^{(+0)} &:= \mathcal{T}^{(1)} S_k^{(+0)} \mathcal{T}^{(1)} w_k^{(+0)} \\
    &= \mathcal{T}^{(1)}  
    \sum_{i=1,i\neq k}^r 
\frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i}{2 (\sigma_i - \sigma_k)} \begin{bmatrix} u_i \\ v_i \end{bmatrix} \\
&=\sum_{i=1,i\neq k}^r \frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i}{2 (\sigma_i - \sigma_k)} \begin{bmatrix} 
A^{(1)} v_i \\ 
(A^{(1)})^\top u_i 
\end{bmatrix}
,
\end{align}
so that:\\
\pgfmathsetmacro{\linewidthfactor}{0.9}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
\langle 
w_k, Z^{(+0)}
\rangle
&=
\sum_{i\neq k}
\left(
\frac{1}{\sqrt{2}}
\begin{bmatrix}
    u_k \\
    v_k
\end{bmatrix}
\right)^\top
\frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i}{2 (\sigma_i - \sigma_k)} \begin{bmatrix} 
A^{(1)} v_i \\ 
(A^{(1)})^\top u_i 
\end{bmatrix} \\
&=\sum_{i=1,i\neq k}^r
\left(\frac{1}{\sqrt{2}}\right)^2 \cdot \frac{u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i}{2 (\sigma_i - \sigma_k)} \cdot  \left[ u_k^\top A^{(1)} v_i + v_k^\top (A^{(1)})^\top u_i \right] \\
&= \sum_{i=1,i\neq k}^r
\frac{1}{4 (\sigma_i - \sigma_k)} \left[ u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i \right] \left[ u_k^\top A^{(1)} v_i + u_i^\top A^{(1)} v_k \right] \\
&= \sum_{i=1,i\neq k}^r
\frac{1}{4 (\sigma_i - \sigma_k)} \left[ u_i^\top A^{(1)} v_k + u_k^\top A^{(1)} v_i \right]^2  \\
&=
\sum_{i=1,i\neq k}^r
\frac{1}{4 (\sigma_i - \sigma_k)} 
\left[ \left[ u_i^\top A^{(1)} v_k \right]^2 + 2 u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i + \left[ u_k^\top A^{(1)} v_i \right]^2 \right] 
.
\end{align}
\end{minipage}
}\\

    
\item \textbf{Inner-Product Contributions in Negative Eigenspaces}. Consider:
\begin{align}
    Z^{(-0)} &:= \mathcal{T}^{(1)} S_k^{(-0)} \mathcal{T}^{(1)} w_k^{(+0)} \\
    &=\mathcal{T}^{(1)}  \sum_{i=1,i\neq k}^r  \frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i}{2 (-\sigma_i - \sigma_k)} 
\begin{bmatrix} 
u_i \\ 
-v_i 
\end{bmatrix} \\
&=\sum_{i=1,i\neq k}^r
\frac{1}{\sqrt{2}} \cdot \frac{u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i}{2 (-\sigma_i - \sigma_k)} \begin{bmatrix} A^{(1)} (-v_i) \\ (A^{(1)})^\top u_i \end{bmatrix}
,
\end{align}
so that:\\
\pgfmathsetmacro{\linewidthfactor}{0.9}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
\langle w_k, Z^{(-0)} \rangle &= \sum_{i=1,i\neq k}^r \frac{1}{2} \cdot \frac{u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i}{2 (-\sigma_i - \sigma_k)} \left[ u_k^\top A^{(1)} (-v_i) + v_k^\top (A^{(1)})^\top u_i \right] \\
&=\sum_{i=1,i\neq k}^r 
\frac{1}{4 (-\sigma_i - \sigma_k)} \left[ u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i \right] \left[ -(u_k)^\top A^{(1)} v_i + u_i^\top A^{(1)} v_k \right] \\
&=\sum_{i=1,i\neq k}^r
\frac{1}{4 (-\sigma_i - \sigma_k)} 
\left[ u_i^\top A^{(1)} v_k - u_k^\top A^{(1)} v_i \right]^2 \\
&=\sum_{i=1,i\neq k}^r
\frac{1}{4 (-\sigma_i - \sigma_k)} 
\left[ \left[ u_i^\top A^{(1)} v_k \right]^2 - 2 u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i + \left[ u_k^\top A^{(1)} v_i \right]^2 \right] %\\
% &\xLongrightarrow[]{\text{sum over}~i \neq k}
% \sum_{i=1}^r \frac{1}{4 (-\sigma_i -\sigma_k)} 
% \left[ \left[ u_i^\top A^{(1)} v_k \right]^2 - 2 u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i + \left[ u_k^\top A^{(1)} v_i \right]^2 \right]
.
\end{align}
\end{minipage}
}


\item \textbf{Inner-Product Contributions in Left-Null Eigenspaces}. Consider:
\begin{align}
    Z^{(0,a)} &:= \mathcal{T}^{(1)} S_k^{(0,a)} \mathcal{T}^{(1)} w_k^{(+0)} \\
    &= \mathcal{T}^{(1)} \sum_{j=r+1}^m
    \left( -\frac{1}{\sqrt{2}} \cdot \frac{u_j^\top A^{(1)} v_k}{\sigma_k} \begin{bmatrix} 
u_j \\ 
0 
\end{bmatrix} \right) \\
&= \sum_{j=r+1}^m 
-\frac{1}{\sqrt{2}} \cdot \frac{u_j^\top A^{(1)} v_k}{\sigma_k} \begin{bmatrix} 
0 \\ 
(A^{(1)})^\top u_j 
\end{bmatrix}
,
\end{align}
so that:
\begin{align}
\langle w_k, Z^{(0,a)} \rangle 
&= \sum_{j=r+1}^m -\frac{1}{2} \cdot \frac{u_j^\top A^{(1)} v_k}{\sigma_k} \left[ u_k^\top \cdot 0 + v_k^\top (A^{(1)})^\top u_j \right]  \\
&=\sum_{j=r+1}^m
-\frac{1}{2} \cdot \frac{u_j^\top A^{(1)} v_k u_j^\top A^{(1)} v_k}{\sigma_k} 
.    
\end{align}



\item \textbf{Inner-Product Contributions in Right-Null Eigenspaces}. Consider:
\begin{align}
    Z^{(0,b)} &:= \mathcal{T}^{(1)} S_k^{(0,b)} \mathcal{T}^{(1)} w_k^{(+0)} \\
    &= \mathcal{T}^{(1)} 
    \sum_{j=r+1}^n
    \left( -\frac{1}{\sqrt{2}} \cdot \frac{u_k^\top A^{(1)} v_j}{\sigma_k} \begin{bmatrix} 0 \\ v_j \end{bmatrix} \right) \\
    &= \sum_{j=r+1}^n -\frac{1}{\sqrt{2}} \cdot \frac{u_k^\top A^{(1)} v_j}{\sigma_k} \begin{bmatrix} A^{(1)} v_j \\ 0 \end{bmatrix} 
    ,
\end{align}
so that:
\begin{align}
\langle w_k, Z^{(0,b)} \rangle &= 
\sum_{j=r+1}^n-\frac{1}{2} \cdot \frac{u_k^\top A^{(1)} v_j}{\sigma_k} \left[ u_k^\top A^{(1)} v_j + v_k^\top \cdot 0 \right]\\
&=\sum_{j=r+1}^n 
-\frac{1}{2} \cdot \frac{\left[ u_k^\top A^{(1)} v_j \right]^2}{\sigma_k} 
.    
\end{align}



\end{enumerate}



\bigskip
\noindent
\textbf{Combining Terms.} 
Since
\begin{align}
\sigma_k^{(2, p=1)} = 0,    
\end{align}
thus,
\begin{align}
\sigma_k^{(2)} &=\sigma_k^{(2, p=2)}\\
&= 
-\left[ 
\sum_{i=1,i \neq k}^r \frac{1}{4 (\sigma_i - \sigma_k)} 
\left[ \left[ u_i^\top A^{(1)} v_k \right]^2 + 2 u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i + \left[ u_k^\top A^{(1)} v_i \right]^2 \right] \right. \\
&\qquad\left.+
\sum_{i=1,i \neq k}^r \frac{1}{4 (-\sigma_i - \sigma_k)} 
\left[ \left[ u_i^\top A^{(1)} v_k \right]^2 - 2 u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i + \left[ u_k^\top A^{(1)} v_i \right]^2 \right] \right.\\
&\qquad\left.-\sum_{j=r+1}^m \frac{1}{2 \sigma_k} \left[ u_j^\top A^{(1)} v_k \right]^2
-\sum_{j=r+1}^n \frac{1}{2 \sigma_k} \left[ u_k^\top A^{(1)} v_j \right]^2
\right] \\
&= 
-\left[ 
\sum_{i=1,i \neq k}^r \frac{(\sigma_i + \sigma_k)  -(\sigma_i - \sigma_k)}{4 (\sigma_i^2 - \sigma_k^2)} 
\left[ \left[ u_i^\top A^{(1)} v_k \right]^2  + \left[ u_k^\top A^{(1)} v_i \right]^2 \right] \right. \\
&\qquad\left.
+\frac{1}{2}\sum_{i=1,i \neq k}^r \frac{(\sigma_i + \sigma_k) + (\sigma_i - \sigma_k)}{\sigma_i^2 - \sigma_k^2} u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i
\right.\\
&\qquad\left.
-\sum_{j=r+1}^m \frac{1}{2 \sigma_k} \left[ u_j^\top A^{(1)} v_k \right]^2
-\sum_{j=r+1}^n \frac{1}{2 \sigma_k} \left[ u_k^\top A^{(1)} v_j \right]^2
\right] \\
&=\frac{1}{2} \sum_{i=1,i \neq k}^r \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2} \left[ u_i^\top A^{(1)} v_k \right]^2 +
\frac{1}{2} \sum_{i \neq k}^r \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2} \left[ u_k^\top A^{(1)} v_i \right]^2  \\
&\qquad+\frac{1}{2}\sum_{i=1,i \neq k}^r \frac{\sigma_i}{\sigma_k^2 - \sigma_i^2} u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i +\frac{1}{2}\sum_{i=1}^r \frac{\sigma_i}{\sigma_k^2 - \sigma_i^2} u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i\\
&\qquad 
+\frac{1}{2}\sum_{j=r+1}^m \frac{\sigma_k}{ \sigma_k^2-\sigma_j^2} \left[ u_j^\top A^{(1)} v_k \right]^2
+\frac{1}{2}\sum_{j=r+1}^n \frac{\sigma_k}{ \sigma_k^2-\sigma_j^2} \left[ u_k^\top A^{(1)} v_j \right]^2\\
&\xlongequal[]{\text{combine indices}}
\frac{1}{2} \sum_{i \neq k} \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2} \left[ u_i^\top A^{(1)} v_k \right]^2 \\
&\qquad\qquad\qquad\qquad\qquad+
\frac{1}{2} \sum_{i \neq k} \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2} \left[ u_k^\top A^{(1)} v_i \right]^2  \\
&\qquad\qquad\qquad\qquad\qquad +\frac{1}{2}\sum_{i=1}^r \frac{\sigma_i}{\sigma_i^2 - \sigma_k^2} u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i \\
&\qquad\qquad\qquad\qquad\qquad +\frac{1}{2}\sum_{i=1}^r \frac{\sigma_i}{\sigma_i^2 - \sigma_k^2} u_k^\top A^{(1)} v_i u_i^\top A^{(1)} v_k  .
\end{align}



\bigskip
\noindent
\textbf{Obtaining Kronecker-Product Representation.} Use following identity from Lemma~\ref{lemma:essential_matrix_identities}~(\nameref{lemma:essential_matrix_identities}):
\begin{enumerate}
    \item $\operatorname{vec}(B V A^\top) = (A \otimes B)\operatorname{vec}(V)$,
\end{enumerate}
consider:
\begin{align}
\lim_{x \to 0} x^2\left[u_i^\top A^{(1)}v_k \right]^2 &=   \lim_{x \to 0} u_i^\top xA^{(1)}v_k u_i^\top xA^{(1)}v_k \\
 &= \left[u_i^\top \dd A v_k\right] \left[u_i^\top \dd A v_k\right] \\
 &=\left[v_k^\top \dd A u_i\right] 
 \left[u_i^\top \dd A v_k\right] \\
 &=\operatorname{vec}\left[v_k^\top \dd A u_i\right]
 \operatorname{vec}\left[u_i^\top \dd A v_k\right] \\
 &=\left(u_i^\top \otimes v_k^\top\right) \operatorname{vec}(\dd A)
 \left(v_k^\top \otimes u_i^\top\right)
 \operatorname{vec}(\dd A) \\
 &=\left[\left(u_i^\top \otimes v_k^\top\right) \operatorname{vec}(\dd A)\right]^\top
 \left[\left(v_k^\top \otimes u_i^\top\right)
 \operatorname{vec}(\dd A)\right] \\
 &=\operatorname{vec}(\dd A^\top)\left(v_k \otimes u_i\right)\left(v_k \otimes u_i\right)^\top\operatorname{vec}(\dd A).
\end{align}

Similarly,
\begin{align}
\lim_{x \to 0} x^2\left[u_k^\top A^{(1)}v_i \right]^2 =    \operatorname{vec}(\dd A^\top)\left(v_i \otimes u_k\right)\left(v_i \otimes u_k\right)^\top\operatorname{vec}(\dd A),
\end{align}
\begin{align}
\lim_{x \to 0} x^2   u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i  &= \lim_{x \to 0} u_i^\top xA^{(1)} v_k u_k^\top xA^{(1)} v_i \\
&=\lim_{x \to 0} u_i^\top \dd A v_k u_k^\top \dd A v_i \\
&=\operatorname{vec}(\dd A^\top)\left(v_k \otimes u_i\right)\left(v_i \otimes u_k\right)^\top\operatorname{vec}(\dd A),
\end{align}
and:
\begin{align}
\lim_{x \to 0} x^2   u_k^\top A^{(1)} v_i u_i^\top A^{(1)} v_k  &= \lim_{x \to 0} u_k^\top xA^{(1)} v_i u_i^\top xA^{(1)} v_k \\
&=\lim_{x \to 0} u_k^\top \dd A v_i u_i^\top \dd A v_k \\
&=\operatorname{vec}(\dd A^\top)\left(v_i\otimes u_k\right)\left(v_k \otimes u_i\right)^\top\operatorname{vec}(\dd A)
.
\end{align}

\bigskip
\noindent
\textbf{Producing Lemma Claim.} Hence,
\begin{align}
D^2\sigma_k[\dd A, \dd A]
&=
\operatorname{vec}(\dd A)^\top\frac{\partial}{\partial \operatorname{vec}(A)} \operatorname{vec}\left( \frac{\partial \sigma_k}{\partial A}\right) \operatorname{vec}(\dd A) \\
&=2 \lim_{x \to 0}x^2 \sigma_k^{(2)} \\
&= \sum_{i \neq k} \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2} \lim_{x \to 0} x^2\left[u_i^\top A^{(1)}v_k \right]^2 \\
&\qquad
+ \sum_{i \neq k} \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2} \lim_{x \to 0} x^2\left[u_k^\top A^{(1)}v_i \right]^2 \\
&\qquad
+\sum_{i=1}^r \frac{\sigma_i}{\sigma_i^2 - \sigma_k^2} \lim_{x \to 0} x^2   u_i^\top A^{(1)} v_k u_k^\top A^{(1)} v_i \\
&\qquad
+\sum_{i=1}^r \frac{\sigma_i}{\sigma_i^2 - \sigma_k^2} \lim_{x \to 0} x^2   u_k^\top A^{(1)} v_i u_i^\top A^{(1)} v_k 
.
\end{align}

Re-labeling indices yields the claim:\\
\pgfmathsetmacro{\linewidthfactor}{0.85}
\pgfmathsetmacro{\inverselinewidthfactor}{1/\linewidthfactor}
\scalebox{\linewidthfactor}{% scale
\begin{minipage}{\inverselinewidthfactor\linewidth} % 1/scale
\begin{align}
D^2\sigma_k[\dd A, \dd A] &=
\operatorname{vec}(\dd A)^\top
\left[
\underbrace{\sum_{i \neq k, i \leq r} \frac{\sigma_k}{\sigma_k^2 - \sigma_i^2}\left(v_k \otimes u_i\right)\left(v_k \otimes u_i\right)^\top}_{\text{left}} \right.\\
&\left.\qquad\qquad\qquad
+\underbrace{\sum_{j \neq k, j \leq n} \frac{\sigma_k}{\sigma_k^2 - \sigma_j^2} \left(v_j \otimes u_k\right)\left(v_j \otimes u_k\right)^\top}_{\text{right}}  \right.\\
    &\left.\qquad\qquad \qquad+\underbrace{\sum_{l \neq k, l \leq r} \frac{\sigma_l}{\sigma_k^2 - \sigma_l^2}\left[ \left(v_k \otimes u_l\right)\left(v_l \otimes u_k\right)^\top + \left(v_l \otimes u_k\right)\left(v_k \otimes u_l\right)^\top \right]}_{\text{left-right interaction}} \right]
    \operatorname{vec}(\dd A)  
    .
\end{align}
\end{minipage}
}\\

%\end{proofpart}

{\hfill$\qed$\par}
\end{mynewproof}




\begin{figure}[t!]
  \centering

  \begin{minipage}[t]{1\textwidth}
     \centering 
     \subfloat[{Matrix entries i.i.d. from $\mathcal{N}(0, 1)$.}]{%
    \centering
    \includegraphics[width=1\linewidth]{jacobian_normal.pdf}%
    %\caption{The matrix is sampled from $\mathcal{N}(0, 1)$.}
    \label{fig:hessian:normal}
  }
  \end{minipage}
  
  \vspace{1em}
  
  \begin{minipage}[t]{1\textwidth}
     \centering 
   \subfloat[{Matrix entries i.i.d. from $U[0,1]$.}]{%
    \centering
    \includegraphics[width=1\linewidth]{jacobian_uniform.pdf}%
    %\caption{The matrix is sampled from $U[0, 1]$.}
    \label{fig:jacobian:uniform}
  }
  \end{minipage}
  
  \caption[Numerical Experiments for Singular-Value Jacobian]{\textbf{Numerical Experiments for Singular-Value Jacobian.} This experiment compares the singular-value Jacobian derived from our framework with that obtained via PyTorch's auto--differentiation. The error $\epsilon$ is measured as the $\ell_2$-norm between the theoretical and ground-truth results. The error is measured to be zero in these experiments, indicating no difference between the theoretical and ground-truth results.}
  
  \label{fig:jacobian:all}
  
\end{figure}

\section{Numerical Experiments}
\label{sec:numerical_experiments}

\begin{figure}[t!]
  \centering

    \begin{minipage}[t]{1\textwidth}
     \centering 
     \subfloat[{Matrix entries i.i.d. from $\mathcal{N}(0,1)$.}]{%
    \centering
    \includegraphics[width=1\linewidth]{hessian_normal.pdf}
    %\caption{The matrix is sampled from $\mathcal{N}(0, 1)$.}
    \label{fig:hessian:normal}
  }
  \end{minipage}
  
  %\vspace{1em}
  
\begin{minipage}[t]{1\textwidth}
     \centering 
     \subfloat[{Matrix entries i.i.d. from $U[0, 1]$.}]{%
    \centering
    \includegraphics[width=1\linewidth]{hessian_uniform.pdf}
    %\caption{The matrix is sampled from $U[0, 1]$.}
    \label{fig:hessian:uniform}
  }
  \end{minipage}

  
  \caption[Numerical Experiments for Singular-Value Hessian]{\textbf{Numerical Experiments for Singular-Value Hessian.} This experiment compares the singular-value Hessian derived from our framework with that obtained via PyTorch's auto--differentiation. The error $\epsilon$ is measured as the $\ell_2$-norm between the theoretical and ground-truth results. The maximum error is measured to be less than $1.3\times 10^{-14}$ in these experiments, indicating the difference between the theoretical and ground-truth results is negligible.}
  
  \label{fig:hessian:all}
\end{figure}


\begin{figure}[t!]
  \centering

    \begin{minipage}[t]{0.48\textwidth}
     \centering 
     \subfloat[{Matrix entries i.i.d. from $\mathcal{N}(0,1)$.}]{%
    \centering
    \includegraphics[width=0.9\linewidth]{hessian_error_density_normal.pdf}
    \label{fig:hessian:errors:normal}
  }
  \end{minipage}
\begin{minipage}[t]{0.48\textwidth}
     \centering 
     \subfloat[{Matrix entries i.i.d. from $U[0, 1]$.}]{%
    \centering
    \includegraphics[width=0.9\linewidth]{hessian_error_density_uniform.pdf}
    \label{fig:hessian:errors:uniform}
  }
  \end{minipage}

  
  \caption[Errors for Singular-Value Hessian]{\textbf{Errors for Singular-Value Hessian.} Random matrix entries are sampled i.i.d.\ from $\mathcal{N}(0,1)$ and $U[0,1]$, respectively. For each singular-value index $k=1,2,\dots,r$, the error $\epsilon$ is computed over $500$ trials and visualized using an unnormalized histogram density. All reported errors are below $6\times 10^{-14}$ in these experiments.}
  
  \label{fig:hessian:errors}
\end{figure}

We conduct numerical experiments to validate the correctness of the derived special cases $n=1$ and $n=2$. Matrix entries are sampled from $\mathcal{N}(0,1)$ and $U(0,1)$, respectively, for both $n=1$ and $n=2$. Ground truth is obtained numerically via PyTorch's auto--differentiation framework \citep{paszke2019pytorch}. The error $\epsilon$ is computed by the $\ell_2$-norm
\begin{align}
    \epsilon = \| R_{\text{ours}} - R_{\text{gt}} \|_2,
\end{align}
where $R_{\text{ours}}$ denotes the result from our theoretical computation and $R_{\text{gt}}$ the ground truth from auto--differentiation. Singular values are indexed by $k=1,2,\dots,r$ in the reported results. To facilitate the visualization and computation, we choose the dimensions $6 \times 10$ in all experiments. 

\bigskip
\noindent
\textbf{Reproducibility.} The random seed is fixed to $1$ for reproducibility. All experimental code is available at \url{https://github.com/roisincrtai/highorder_spectral_variation_analysis}.



\bigskip
\noindent
\textbf{Results of Singular-Value Jacobian.} Figure~\ref{fig:jacobian:all} reports the results for the singular-value Jacobian. Matrix entries are sampled i.i.d. from $\mathcal{N}(0,1)$ and $U(0,1)$, respectively. The derivative matrices are visualized using the \emph{viridis} color map. For each singular-value index $k$, results are shown in pairs: the left panel gives the theoretical computation from Lemma~\ref{lemma:jacobian_of_singular_value}, while the right panel shows the numerical ground truth obtained from PyTorch's auto--differentiation framework. The reported errors are zero across all experiments.


\bigskip
\noindent
\textbf{Results of Singular-Value Hessian.} 
Figure~\ref{fig:hessian:all} reports the results for the singular-value Hessian. Matrix entries are sampled i.i.d. from $\mathcal{N}(0,1)$ and $U(0,1)$, respectively. The derivative matrices are visualized using the \emph{viridis} color map. For each singular-value index $k$, results are shown in pairs: the left panel gives the theoretical computation from Lemma~\ref{lemma:hessian_of_singular_value}, while the right panel shows the numerical ground truth obtained from PyTorch's auto--differentiation framework. The observed errors between theoretical results and numerical ground-truth are on the order of $10^{-14}$, confirming that they are numerically negligible.






\section{Conclusion}

By viewing matrices as compact linear operators and extending Kato's perturbation theory for self-adjoint operators, we present a unified operator-theoretic framework for obtaining closed-form, arbitrary-order derivatives of singular values in real rectangular matrices. In contrast to the \emph{ad hoc} methods of classical matrix analysis, our approach is systematic and procedural, allowing the derivation of singular-value derivatives of any order. The key step is the Jordan–Wielandt embedding, which maps a real rectangular matrix, usually non-self-adjoint, to a self-adjoint operator, thereby encapsulating its complete spectral information. Based on Kato's framework, we establish a general framework for deriving higher-order singular-value derivatives. Specializing to first order ($n=1$) recovers the classical singular-value Jacobian, while specializing to second order ($n=2$) yields a Kronecker-product representation of the singular-value Hessian that, to the best of our knowledge, has not previously appeared in the literature. Beyond these cases, the framework extends to arbitrary order. Higher-order singular-value derivatives are indispensable for analyzing induced spectral dynamics in statistical physics and deep learning. 




==> main_matter/chapters/PerturbationAnalysis/tikz/spectral_analysis_framework.tex <==
\begin{tikzpicture}[node distance=10mm and 15mm, >=Stealth,
  kato/.style={  rectangle, 
                draw, 
                rounded corners, 
                fill=cyan!30, 
                align=center, 
                text width=6cm, 
                inner sep=0.2cm, 
                minimum height=3cm, 
          },
  complex/.style={  rectangle, 
                draw, 
                rounded corners, 
                fill=green!30, 
                align=center, 
                text width=6cm, 
                inner sep=0.2cm, 
                minimum height=3cm, 
          }, 
  ours/.style={
                rectangle, 
                draw, 
                rounded corners, 
                fill=orange!30, 
                align=center, 
                text width=6cm,
                inner sep=0.2cm, 
                minimum height=3cm, 
            },
  app/.style={
                rectangle, 
                draw, 
                rounded corners, 
                fill=purple!15, 
                align=center, 
                text width=6cm,
                inner sep=0.2cm, 
                minimum height=3cm, 
            }, 
  legendbox/.style={
    rectangle,
    draw,
    rounded corners,
    minimum width=8mm,
    minimum height=10mm,
    inner sep=0pt,
  },
  legend label/.style={
    anchor=west,
    font=\footnotesize,
  }
]

  %add legend
  \node[legendbox, fill=cyan!30] (legC) {};
  \node[legend label, right=1mm of legC] (labC) {Kato's framework \citep{kato1995perturbation}};

  \node[legendbox, fill=orange!30, right=5cm of legC] (legO) {};
  \node[legend label, right=1mm of legO] (labO) {Our framework};

  \node[legendbox, fill=green!50, right=3cm of legO] (legG) {};
  \node[legend label, right=1mm of legG] (labG) {Functional and complex analysis};

 \begin{scope}[yshift=-30mm]
  \node[kato] (PerturbationSeries) {
    Perturbation Series 
    $$\mathcal{T}(x)=...$$
    (see Section~\ref{sec:eigenvalue_expansion})
  };


  \node[kato, right=of PerturbationSeries] (Resolvent) {
    Resolvent Operator
    $$ R(z) = (\mathcal{T}(x) - zI)^{-1} $$
    (see Section~\ref{sec:eigenvalue_expansion})
  };


  \node[kato, right=of Resolvent] (RieszProjection) {
    Riesz Projector
    $$
    P(x) = -\frac{1}{2\pi\,i}\oint_{\Gamma} R(z) dz
    $$
    where $\Gamma$ is a small contour enclosing only an isolated eigenvalue $\lambda^{(0)}$. \\
    (see Section~\ref{sec:eigenvalue_expansion})
  };
  
  \node[kato, below=of RieszProjection, xshift=0cm] (PerturbationProjection) {
    Perturbation Projection
    \begin{align}
    &\mathcal{T}(x)P(x) = \lambda(x)P(x) \notag \\
    &\Longrightarrow \lambda(x) = ...  \notag\\
    &\Longrightarrow \text{equating coefficient of}~x^n~...\notag
    \end{align}
    (see Section~\ref{sec:eigenvalue_expansion})
  };

  
  \node[ours, below=of PerturbationProjection] (EigenvalueExpansion) {
    Theorem~\ref{thm:expansions_of_eigenvalues} (Refined Asymptotic Eigenvalue Expansion): Expanding $\lambda(x)$ and applying residue theorem to further simplify yield
    $$\lambda^{(n)}= \cdots$$
    (see Section~\ref{sec:eigenvalue_expansion})
  };

  \node[complex, left=of EigenvalueExpansion, ] (NeumannSeries) {
    Operator Neumann series of $R(z)$\\
    Residue Theorem\\
    $\cdots$\\
    (see Section~\ref{sec:eigenvalue_expansion})
  };






  \node[ours, minimum height=5cm, below=of EigenvalueExpansion] (ApplyEigenvalueExpansion) {
  Theorem~\ref{thm:nth_order_singular_value} (Infinitesimal Spectral Variation): 
    Applying Theorem~\ref{theorem:Jordan_Wielandt_relation} (Jordan--Wielandt Embedding), Theorem~\ref{thm:expansions_of_eigenvalues} (Asymptotic Eigenvalue Expansion), and Theorem~(\ref{thm:frechet_taylor_operator}) (Analytic Perturbation for Holomorphic Operators) on $\mathcal{T}(x)$ produces the higher-order eigenvalue expansion
    $$
    \sigma_k^{(n)}=\cdots %, \quad D^n \sigma_k = n! \sigma_k^{(n)}
    $$
    (see Section~\ref{sec:spectral_variation})
  };



\node[ours, minimum height=4cm, left=of ApplyEigenvalueExpansion] (ConstructTx) {
    % \node[ours, minimum height=4cm, below=of DefineAx] (ConstructTx) {
    Theorem~\ref{theorem:Jordan_Wielandt_relation} (Jordan--Wielandt Embedding): Embed $A$ into Jordan–Wielandt Embedding
    $$
    \mathcal{T}=\begin{bmatrix}
       O & A \\
       A^\top & O
    \end{bmatrix}
    $$
    for capturing perturbations from all subspaces in a rectangular matrix $A$ (see Section~\ref{sec:schematic_overview}).
  }; 


    \node[ours, minimum height=3cm, left=of ConstructTx] (DefineAx) {
  % \node[ours, minimum height=3cm, below=of PerturbationSeries] (DefineAx) {
    A rectangular matrix $A$ is a non-self-adjoint linear operator.\\
    (see Section~\ref{sec:schematic_overview}).
  };
  

  \node[ours, below=of ApplyEigenvalueExpansion] (MapToFrechetDerivative) {
    Map the perturbed eigenvalue expansion to Fr\'echet derivative by
    $$
    D^n\sigma_k[\dd A, \cdots] = n!\lim_{x \to 0}x^n\sigma_k^{(n)}
    $$
    (see Section~\ref{sec:spectral_variation})
  };

  \node[ours, left=of MapToFrechetDerivative] (MapToMatrixLayout) {
    Specialize $n$ (\eg~$n=1,2,\cdots$) and map the Fr\'echet derivative
    $$
    D^n\sigma_k[\dd A, \cdots]
    $$
    to matrix layout convention.\\
    (see Section~\ref{sec:special_case_jacobian} and Section~\ref{sec:special_case_hessian})
  };

   \node[ours, left=of MapToMatrixLayout] (LayoutConvention) {
    Fr\'echet Derivative and Layout Convention\\
    (see Section~\ref{sec:layout_convention}).
  };

  
   \draw[->,thick] (PerturbationSeries) -- (Resolvent);
   \draw[->,thick] (Resolvent)  -- (RieszProjection);
   \draw[->,thick] (Resolvent)  -- (NeumannSeries);
   %\draw[->,thick] (Resolvent)  |- (ReducedResolvent);
   \draw[->,thick] (RieszProjection)  -- (PerturbationProjection);
   \draw[->,thick] (NeumannSeries)  -- (EigenvalueExpansion);
   %\draw[->] (ResidueTheorem)  -- (EigenvalueExpansion);
   \draw[->,thick] (PerturbationProjection) -- (EigenvalueExpansion);
   \draw[->,thick,dotted] (PerturbationSeries) -- (DefineAx);
   \draw[->,thick] (DefineAx) -- (ConstructTx);
   % \draw[->,thick] (ConstructTx) |- (ApplyEigenvalueExpansion);
   \draw[->,thick] (ConstructTx) -- (ApplyEigenvalueExpansion);
   \draw[->,thick] (EigenvalueExpansion) -- (ApplyEigenvalueExpansion);
   \draw[->,thick] (ApplyEigenvalueExpansion) -- (MapToFrechetDerivative);
   %\draw[->,thick] (SimplifyEigenvalueExpansion) -- (MapToFrechetDerivative);
   \draw[->,thick] (MapToFrechetDerivative) -- (MapToMatrixLayout);
   \draw[->,thick] (LayoutConvention) -- (MapToMatrixLayout);
 \end{scope}

\end{tikzpicture}
